On the Precise Asymptotics of Universal Inference

In statistical inference, confidence set procedures are typically evaluated based on their validity and width properties. Even when procedures achieve rate-optimal widths, confidence sets can still be excessively wide in practice due to elusive constants, leading to extreme conservativeness, where the empirical coverage probability of nominal $1-\alpha$ level confidence sets approaches one. This manuscript studies this gap between validity and conservativeness, using universal inference (Wasserman et al., 2020) with a regular parametric model under model misspecification as a running example. We identify the source of asymptotic conservativeness and propose a general remedy based on studentization and bias correction. The resulting method attains exact asymptotic coverage at the nominal $1-\alpha$ level, even under model misspecification, provided that the product of the estimation errors of two unknowns is negligible, exhibiting an intriguing resemblance to double robustness in semiparametric theory.

==> main/application.tex <==
\section{Statistical Applications}\label{sec:application}
In this section, we present statistical applications of the proposed method and provide sufficient conditions for validity, along with the convergence rates of the corresponding confidence sets. For simplicity, we focus on the upper confidence bound $U_{n,\alpha_2}(\theta(P), \widehat{\theta}_1; D_2) = 0$ with $\alpha_2 = 0$. As discussed in Remark~\ref{remark:the-role-U}, this choice does not affect the validity of the confidence sets. The width analysis provided here demonstrates that the simple choice of $U_{n,\alpha_2}(\theta(P), \widehat{\theta}_1; D_2) = 0$ is sufficient for rate-optimality, while alternative choices for $U_{n,\alpha_2}(\theta(P), \widehat{\theta}_1; D_2) < 0$ will only improve upon the constant factor. For each application, we specify the choice of the loss function $m_\theta$. Once such $m_\theta$ is defined, the confidence set derived from the following expression will be referred to as the
\textit{empirical Bernstein-based confidence set}:
	\begin{align}\label{eq:ci1-application}
    &\widehat{\mathrm{CI}}^{\mathrm{E.B.}}_{n,\alpha}  := \left\{\theta \in \Theta \, : \, \mathbb{P}_n(m_{\theta}-m_{\widehat \theta_1})\le \sqrt{\frac{2\widehat \sigma^2_{\theta, \widehat\theta_1} \log(2/\alpha)}{n}} + \frac{7B_0\log(2/\alpha)}{3(n-1)}\right\}
\end{align}
where $B_0$ and $\widehat \sigma^2_{\theta, \widehat\theta_1}$ are defined in Example~\ref{prop:bernstein}. We similarly define the following set as the \textit{CLT-based confidence set}:
\begin{equation}\label{eq:ci2-application}
\widehat{\mathrm{CI}}^{\mathrm{CLT}}_{n,\alpha} := \left\{\theta \in \Theta \, : \, \mathbb{P}_n(m_{\theta}-m_{\widehat \theta_1})\le n^{-1/2}z_{\alpha} \widehat\sigma_{\theta, \widehat\theta_1}\right\}.
\end{equation}
Throughout this section, the $N$ observations are split into two sets $D_1$ and $D_2$ such that there exist $c$ and $C$ with $0 < c < |D_1|/|D_2| \le C < \infty$. All relevant proofs are provided in Section~\ref{sec:proof-applications} of the supplement.

% \begin{corollary}
%     Assume that the IID real-valued mean-zero random variable $Z$ satisfies that 
%     \begin{align}\label{eq:1}
%         \sup_{P\in\mathcal{P}}\,\sup_{\|t\|=1}\, \E_P\left[\frac{\langle t, Z\rangle^2}{B^2}\mathbf{1}\{|\langle t, Z\rangle|^2 > \varepsilon nB^2\}\right] \longrightarrow 0 \quad \text{for all $\varepsilon > 0$}.
%     \end{align}
%     Then, the uniform Lindeberg condition is satisfied. Furthermore, assume that there exists a constant $L$ such that
%     \begin{align}\label{eq:2}
%         \sup_{P\in\mathcal{P}}\,\sup_{\|t\|=1}\, \frac{\big(\mathbb{E}_P[\langle t, Z\rangle^{2+\delta}]\big)^{1/(2+\delta)}}{\big( \mathbb{E}_P[\langle t, Z\rangle^2] \big)^{1/2}} \le L \quad \text{for some $\delta \in (0,1]$}.
%     \end{align}
%     Then, up to a universal constant, it implies 
%     \begin{align*}
%         \sup_{P\in\mathcal{P}}\, \sup_{\|t\|=1}\, \left ( \E_P\left[\frac{\langle t, Z \rangle^2}{B^2} \left\{1 \wedge n^{-1/2}\frac{|\langle t, Z \rangle|}{B}\right\}\right] \right) \lesssim L^{\delta+2}n^{-\delta/2} \longrightarrow 0.
%     \end{align*}
% \end{corollary}
% Without considering the supremum, the equations \eqref{eq:1} and \eqref{eq:2} 
%  are widely known as the Lindeberg and the Lyapunov conditions respectively. 
% We provide two sufficient conditions under which the right-hand side of \eqref{eq:bentkus-result} is vanishing in our contexts. For this, we introduce the following regularity conditions:
%  \begin{enumerate}[label=\textbf{(A\arabic*)},leftmargin=2cm]
%   \setcounter{enumi}{2}
%     \item \label{as:qmd+lindeberg}
%     Additionally, the function $\dot m_{\theta(P)}$ satisfies one of the followings:
%     \begin{enumerate}[label=\textbf{(A3-\arabic*)}]
%     \item \label{as:cond1}For any $\varepsilon > 0$ and $t \in \Theta$ such that $\|t\|=1$, 
%      \begin{equation}
%         \lim_{n\longrightarrow\infty}\sup_{P\in \mathcal{P}}\, \sup_{\|t\|=1}\, \frac{P[\langle t, \dot m_{\theta(P)}\rangle^2 1\{\langle t, \dot m_{\theta(P)}\rangle^2 > n \varepsilon P\langle t, \dot m_{\theta(P)}\rangle^2\}]}{P\langle t, \dot m_{\theta(P)}\rangle^2} = 0.
%     \end{equation}
%     \item \label{as:cond2} There exists a constant $L < \infty$ and $\delta \in (0,1]$ such that 
%      \begin{equation}
%         \sup_{P\in\mathcal{P}}\, \sup_{\|t\|=1}\, \frac{(P \langle t, \dot m_{\theta(P)}\rangle^{2+\delta})^{1/(2+\delta)}}{(P \langle t, \dot m_{\theta(P)}\rangle^{2})^{1/2}} \le L.
%     \end{equation}
%     \end{enumerate}
%   \end{enumerate}
%   The first statement of \ref{as:qmd+lindeberg}, on the existence of $\dot m_{\theta(P)}$, roughly pertains to the differentiability of $m_{\theta}$ under integration. The function $\dot m_{\theta(P)}$ certainly exists when $m_{\theta}$ is continuously differentiable at $\theta(P)$; however, it allows for broader settings, including the case when $m_{\theta}$ is not differentiable at $\theta(P)$. \ref{as:cond1} is so-called Lindeberg's condition, acting on the random variable $\langle t, \dot m_{\theta(P)}\rangle$.   \ref{as:cond2} is also known as $L_{2+\delta}$-$L_2$ norm equivalence \citep{mendelson2020robust}. 
 
%  This further implies that for any $\varepsilon > 0$
% 	\begin{align}
% 		\Delta_{n,P} \le C \left ( \varepsilon + \E[W_1^2 1\{W_1^2 > n\varepsilon^2S^2\}] S^{-2} \right).
% 	\end{align}
% 	Alternatively, we also obtain for any $\delta \in (0,1]$, 
% 	\begin{align}
% 		\Delta_{n,P} \le C n^{-\delta/2}\left(\frac{(\E |W_1|^{2+\delta})^{1/(2+\delta)}}{(\E |W_1|^{2})^{1/2}}\right)^{2+\delta}
% 	\end{align}
% Under these regularity conditions, we provide the asymptotic validity statement for the confidence set based on the Gaussian approximation:


\subsection{High-dimensional mean estimation}\label{sec:mean}
Consider an IID observation $X_1, \ldots, X_N \in \mathbb{R}^d$ generated from $P \in \mathcal{P}$. The dimension $d$ is allowed to grow with $N$. In this problem, the inference of interest is the expectation of $X$ under $P$, which can be also written as
\begin{align*}
    \theta(P) := \argmin_{\theta \in \mathbb{R}^d}\, \E_P\|X-\theta\|_2^2.
\end{align*}
The covariance matrix of $X$ is denoted by $\Sigma := \E_P(X-\E_P[X])(X-\E_P[X])^\top$. Although this problem may seem trivial, mean estimation and inference in growing dimensions under weak distributional assumptions remains an active area of research \citep{lugosi2019mean}. We provide results under assumptions, requiring only the existence of the covariance matrix and the uniform Lindeberg condition \eqref{eq:validity-condition-clt}. Below, we denote by $\widehat{\mathrm{CI}}_{n,\alpha}^{\mathrm{mean}}$ the CLT-based confidence set \eqref{eq:ci2-application} with $m_{\theta}(x) = \|x-\theta\|_2^2$. We now provide the validity statement for this confidence set.
% First, we observe that 
% \begin{align*}
%     P(m_{\theta(P)}-m_{\widehat\theta_1}) = -\|\theta(P)-\widehat\theta_1\|_2^2
% \end{align*}
% and hence we can take 
% \begin{align*}
%     U_{n,\alpha_2}(\theta, \widehat\theta_1; D_2) = -\|\theta-\widehat\theta_1\|_2^2 \quad \mbox{and} \quad \eqref{eq:upper-bound} \mbox{ satisfies with } \alpha_2=0.
% \end{align*}
% The following proposition simplifies the expression for the corresponding confidence set:
% \begin{proposition}\label{prop:mean-ci}
% 	When $m_\theta(Z) := \|Z-\theta\|_2^2$, the confidence set based on \eqref{eq:general-set-gaussian} is equivalent to 
% 	\begin{align}\label{eq:confidence-set-mean}
% \widehat{\mathrm{CI}}_{n,\alpha}^{\mathrm{mean}} := \left\{\theta \in \mathbb{R}^d \, : \, \langle \overline Z_n-\theta, \widehat\theta_1 - \theta\rangle \le n^{-1/2}z_{1-\alpha} \|\widehat \theta_1 - \theta\|_{\widehat \Sigma}\right\}
% 	\end{align}	
% 	where $\widehat \Sigma := n^{-1}\sum_{i=1}^n(Z_i-\overline Z_n)(Z_i-\overline Z_n)^\top$ and $\|x\|^2_A := x^\top A x$.
% \end{proposition}
% First, we provide the validity statement.
\begin{theorem}\label{thm:mean-ci-validity}
For any $n\ge 1$, it holds
\begin{align*}
    \inf_{P\in\mathcal{P}}\, \mathbb{P}_P(\theta(P) \in \widehat{\mathrm{CI}}_{n,\alpha}^{\mathrm{mean}}) \ge 1 - \alpha -\sup_{P\in\mathcal{P}}\Delta_{n,P}
\end{align*}
where it holds for some universal constant $C_0$,
\begin{align*}
    \sup_{P\in\mathcal{P}}\Delta_{n,P} \le \min \left\{1,  C_0\sup_{P\in\mathcal{P}}\,\sup_{t\in\mathbb{S}^{d-1}}\,\E_P\left[\frac{\langle t, X-\theta(P)\rangle^2}{\|\langle t, X-\theta(P)\rangle\|_{2}^2} \min \left\{1, \frac{|\langle t, X-\theta(P)\rangle|}{n^{1/2}\|\langle t, X-\theta(P)\rangle\|_{2}}\right\}\right]\right\}.
\end{align*}
Furthermore, assume that $X-\theta(P)$ satisfies the uniform Lindeberg condition \eqref{eq:validity-condition-clt}, then 
\begin{align*}
    \liminf_{n\longrightarrow \infty}\, \inf_{P\in\mathcal{P}}\, \mathbb{P}_P(\theta(P) \in \widehat{\mathrm{CI}}_{n,\alpha}^{\mathrm{mean}}) \ge 1 - \alpha.
\end{align*}
\end{theorem}
Next, we demonstrate the convergence rate of the confidence set in $L_2$-norm.\begin{theorem}\label{thm:mean-ci-width}
Let $s_n$ be the random variable defined as \ref{as:rate-initial-estimator}. For any $\varepsilon > 0$ and $\mathrm{tr}(\Sigma) \le n$, it follows 
\begin{align*}
\mathbb{P}_P\left(\mathrm{Diam}_{\|\cdot\|_2}\big(\widehat{\mathrm{CI}}_{n,\alpha}^{\mathrm{mean}}\big)\le \mathfrak{C}\left\{\left(\frac{\mathrm{tr}(\Sigma)}{n}\right)^{1/2} + s_n^{1/2}\right\}\right) \ge 1-\varepsilon
\end{align*}	
 where $\mathfrak{C}$ only depends on $\varepsilon$ and $\alpha$. Furthermore, assume that the initial estimator satisfies
\begin{align}\label{eq:mean-init-requirement}
        \mathbb{P}_P\left(\|\widehat\theta_1 - \theta(P)\|_2^2 \le \frac{C_\varepsilon \mathrm{tr}(\Sigma)}{n} \right) \ge 1-\varepsilon
    \end{align}
    for any $\varepsilon > 0$ with a constant $C_\varepsilon$ depending on $\varepsilon$. It  then implies 
\begin{align*}
\mathbb{P}_P\left(\mathrm{Diam}_{\|\cdot\|_2}\big(\widehat{\mathrm{CI}}_{n,\alpha}^{\mathrm{mean}}\big)\le \mathfrak{C}\left(\frac{\mathrm{tr}(\Sigma)}{n}\right)^{1/2}\right) \ge 1-\varepsilon
\end{align*}	
for all $n \ge N_\varepsilon$ with $N_\varepsilon$ depending on $\varepsilon$ and $\mathfrak{C}$ depending on $\varepsilon$ and $\alpha$.
\end{theorem}
The requirement \eqref{eq:mean-init-requirement} is satisfied when $\widehat{\theta}_1$ is the sample mean. We emphasize that Theorem~\ref{thm:mean-ci-width} imposes no restrictions on the dimension $d$---hence it is typically called dimension agnostic. The dependency on $\sqrt{\mathrm{tr}(\Sigma)/n}$ is, in fact, not improvable since this is the exact risk of the mean estimation under a multivariate Gaussian distribution; see the formal minimax argument in Section 5 of \citet{lee2022optimal}. 

% We check the sufficient conditions for this set to be asymptotically valid according to Theorem~\ref{thm:validity-BE}. The sufficient regularity conditions for the validity in the mean estimation are as follows:
% \begin{enumerate}[label=\textbf{(A4-\arabic*)},leftmargin=2cm]
%     \item \label{as:mean-est1}For any $\varepsilon > 0$ and $t \in \Theta$ such that $\|t\|=1$, 
%      \begin{equation}
%         \lim_{n\longrightarrow \infty}\, \sup_{P\in\mathcal{P}}\, \sup_{\|t\|=1}\, \frac{\E_P[\langle t,Z-\theta(P)\rangle^2 1\{\langle t,Z-\theta(P)\rangle^2 > n \varepsilon \E_P\langle t, Z-\theta(P)\rangle^2\}]}{\E_P\langle t, Z-\theta(P)\rangle^2}= 0.
%     \end{equation}
%     \item \label{as:mean-est2} There exists a constant $L \in [0, \infty)$ and $\delta \in (0,1]$ such that 
%      \begin{equation}
%         \sup_{P\in\mathcal{P}}\,\sup_{\|t\|=1}\, \frac{(\E_P \langle t, Z-\theta(P)\rangle^{2+\delta})^{1/(2+\delta)}}{(\E_P \langle t, Z-\theta(P)\rangle^{2})^{1/2}} \le L.
%     \end{equation}
%     \end{enumerate}
    
% \begin{proposition}\label{prop:mean-validity}
% 	Under \ref{as:mean-est1} or \ref{as:mean-est2}, and assume $\widehat\theta_1$ satisfies \eqref{eq:uniform-convergence}.
%  Then, the confidence set given by \eqref{eq:confidence-set-mean} satisfies
%  \begin{equation}
% \lim_{n\longrightarrow \infty}\, \inf_{P\in\mathcal{P}}\, \mathbb{P}_P(\theta(P)\in \widehat{\mathrm{CI}}_{n,\alpha}^{\mathrm{mean}})  \ge 1-\alpha + o_{\mathcal{P}}(1)
% \end{equation} 
% where $o_{\mathcal{P}}(1)$ denotes the convergence in probability uniformly in $\mathcal{P}$.
% \end{proposition}
% Below, we provide the analogous width analysis to Theorem~\ref{thm:concentration-width} tailored to this context:
% \begin{proposition}\label{prop:width-mean}
% 	The confidence set $\widehat{\mathrm{CI}}_{n,\alpha}$ is contained in $B(\widehat \theta_1, \gamma_n)$ where 
% 	\begin{align}
% 		\gamma_n &:= 2n^{-1/2}z_{1-\alpha}\left\{\left(\sum_{j=1}^d(\widehat \Sigma_{jj}^{1/2}-\Sigma_{jj}^{1/2})^2\right)^{1/2}+\left(\sum_{j=1}^d \Sigma_{jj}\right)^{1/2}\right\}+\|\widehat \theta_1 - \overline Z_n\|_2 \\
% 		&\le 2n^{-1/2}z_{1-\alpha}\left\{\left(\sum_{j=1}^d(\widehat \Sigma_{jj}^{1/2}-\Sigma_{jj}^{1/2})^2\right)^{1/2}+d^{1/2}\sigma_{\mathrm{max}}\right\}+\|\widehat \theta_1 - \theta(P)\|_2 + \|\theta(P)- \overline Z_n\|_2
% 	\end{align}
% 	where $\Sigma := \E(Z-\E[Z])(Z-\E[Z])^\top$ and $\sigma^2_{\mathrm{max}} := \max_{1\le j \le d} \Sigma_{jj}$. 
% \end{proposition}
% Proposition~\ref{prop:width-mean} provides a deterministic result while Theorem~\ref{thm:concentration-width} holds only in high probability. Notice, however, that the $\|\cdot\|$-ball is now centered at $\widehat \theta_1$.
% As long as $\sigma_{\max} < \infty$ and 
% \[(n/d)^{1/2}\sup_{P\in \mathcal{P}}\, \|\widehat\theta_1 - \theta(P)\|_2 = O_{\mathcal{P}}(1)\] 
% we have $\gamma_n^2 = O_{\mathcal{P}}\left(d/n\right)$. 

\subsection{Misspecified linear regression}\label{sec:ols} 
Consider an IID observation $(Y_1, X_1^\top)^\top, \ldots, (Y_N, X_N^\top)^\top \in \mathbb{R}\times\mathbb{R}^d$ generated from the following model:
\begin{align*}
    Y_i = \theta_P^\top X_i + \xi_i \quad\text{where}\quad \mathbb{E}_P[\xi_i X_i] = 0 \quad\text{and}\quad\mathbb{E}_P[\xi_i^2 | X_i] = \sigma_i^2.
\end{align*}
We assume that the gram matrix $\Gamma_P := \E_P[XX^\top]$ is invertible such that $\theta_P \in \mathbb{R}^d$ exists even when the regression function $\E_P[Y_i| X_i]$ is not linear. In this problem, the inference of interest is $\theta_P$, which can be also written as
\begin{equation*}
    \theta_P := \argmin_{\theta \in \mathbb{R}^d}\, \E_P[Y-\theta^\top X]^2,
\end{equation*}
without making the linearity assumption for $\E_P[Y_i| X_i]$. Below, we denote by $\widehat{\mathrm{CI}}_{n,\alpha}^{\mathrm{LR}}$ the CLT-based confidence set \eqref{eq:ci2-application} with $m_{\theta}(y,x) = (y-\theta^\top x)^2$. We introduce the following assumptions for the validity statement:
\begin{enumerate}[label=\textbf{(B\arabic*)},leftmargin=2cm]
% \setcounter{enumi}{2}
\item \label{as:linreg-moment-covariate} 
There exist constants $q_x \ge 4$ and $L \ge 1$ such that 
\begin{align*}
   \|t^\top X_i\|_{q_x}\le L \|t^\top X_i\|_2 \quad \mbox{for all} \quad t \in \mathbb{S}^{d-1}.
\end{align*}
\item \label{as:eigen_value} 
There exist positive constants $\underbar{$\sigma$}, \overline{\sigma}$ such that $\underbar{$\sigma$} < \sigma_i < \overline{\sigma}$ for all $1 \le i \le n$.
\end{enumerate}
\ref{as:linreg-moment-covariate} requires the $L_{q_x}$-$L_2$ norm equivalence on $X$---see Remark~\ref{remark:norm-equiv}. \ref{as:eigen_value} ensures that the error variables $\xi$ do not become degenerate or possess infinite variance.  

The following result is obtained:
\begin{theorem}\label{thm:LR-valid}
Assume \ref{as:linreg-moment-covariate} and \ref{as:eigen_value}. Then for any $n\ge1$ and $\varepsilon > 0$, it holds 
\begin{align*}
    \inf_{P\in\mathcal{P}}\, \mathbb{P}_P(\theta_P \in \widehat{\mathrm{CI}}_{n,\alpha}^{\mathrm{LR}}) \ge 1 - \alpha - \sup_{P\in\mathcal{P}}\Delta_{n,P}
\end{align*}
where it holds for some universal constant $C_0$,
\begin{align*}
     \sup_{P\in\mathcal{P}}\Delta_{n,P}&\le \min \left\{1, C_0\sup_{P\in\mathcal{P}}\bigg[\inf_{\varepsilon > 0}\left\{\{1 \wedge \underbar{$\sigma$}^{-1}L^2 \lambda^{1/2}_{\max}(\Gamma_P)\varepsilon\} +  \mathbb{P}_P(\|\widehat\theta_1 - \theta_P\| > \varepsilon) \right\}\right.\\
    &\left.\qquad + \sup_{\|t\|=1}\,\E_P\left[\frac{\langle  t, X\xi \rangle^2}{\|\langle  t, X\xi \rangle\|^2_{2}} \min\left\{1, \frac{|\langle  t, X\xi \rangle|}{n^{1/2}\|\langle  t, X\xi \rangle\|_{ 2}}\right\}\right]\bigg]\right\}
\end{align*}
and $\lambda_{\max}(\Gamma_P)$ denotes the largest eigenvalue of the gram matrix, which depends on $P$. Furthermore, assume the existence of a positive constant  $\overline{\lambda} < \infty$ such that $\sup_{P\in\mathcal{P}}\lambda_{\max}(\Gamma_P) \le \overline{\lambda}$,  the uniform Lindeberg condition \eqref{eq:validity-condition-clt} on  the mean-zero random variable $\xi_i X_i$, and the uniform consistency of the initial estimator such that
\begin{align*}
\lim_{n\longrightarrow \infty}\, \sup_{P\in\mathcal{P}}\,\mathbb{P}_P(\|\widehat\theta_1 - \theta_P\| > \varepsilon) = 0.
\end{align*}
Then, we obtain 
\begin{align*}
    \liminf_{n\longrightarrow \infty}\,\inf_{P\in\mathcal{P}}\, \mathbb{P}_P(\theta_P \in \widehat{\mathrm{CI}}_{n,\alpha}^{\mathrm{LR}}) \ge 1 - \alpha.
\end{align*}
\end{theorem}

Next, we provide the width of the confidence set in terms of the $L_2$-norm:
\begin{theorem}\label{thm:LR-ci-width}
Let $s_n$ be the random variable defined as \ref{as:rate-initial-estimator}. Assume \ref{as:linreg-moment-covariate} and \ref{as:eigen_value}. For any $n \ge \{\left(L^2\lambda_{\max}(\Gamma_P) \lambda_{\min}^{-1}(\Gamma_P)d^{2/q_x}\log(d)\right)^{q_x/(q_x-2)} \vee d\}$, it follows 
% \begin{align*}
% \mathbb{P}_P\left(\mathrm{Diam}_{\|\cdot\|}\big(\widehat{\mathrm{CI}}_{n,\alpha}^{\mathrm{LR}}\big)\le \mathfrak{C}\left\{\left(\frac{\E_P \|\xi X\|^2 \vee (K_qd)^{4/q}}{n}\right)^{1/2} + s_n^{1/2}\right\}\right) \ge 1-\varepsilon
% \end{align*}	
% \kt{Check with Arun if $\E_P[\xi_i^2| X_i] \le \sigma^2$ is reasonable}
\begin{align*}
\mathbb{P}_P\left(\mathrm{Diam}_{\|\cdot\|_2}\big(\widehat{\mathrm{CI}}_{n,\alpha}^{\mathrm{LR}}\big)\le \mathfrak{C}\left\{\left(\frac{\overline{\sigma}^2 \mathrm{tr}(\Gamma_P)}{n\lambda^2_{\min}(\Gamma_P)}\right)^{1/2} + \left(\frac{s_n}{\lambda_{\min}(\Gamma_P)}\right)^{1/2}\right\}\right) \ge 1-\varepsilon
\end{align*}	
 where $\mathfrak{C}$ depends on $\varepsilon$ and $\alpha$. Furthermore, assume that the initial estimator satisfies
\begin{align}\label{eq:requirement-ols}
        \mathbb{P}_P\left(\|\widehat\theta_1 - \theta(P)\|_2^2 \le \frac{C_\varepsilon\overline{\sigma}^2\mathrm{tr}(\Gamma_P)}{n\lambda^2_{\min}(\Gamma_P)} \right) \ge 1-\varepsilon
    \end{align}
    for any $\varepsilon > 0$ with a constant $C_\varepsilon$ depending on $\varepsilon$. It then implies 
\begin{align*}
\mathbb{P}_P\left(\mathrm{Diam}_{\|\cdot\|_2}\big(\widehat{\mathrm{CI}}_{n,\alpha}^{\mathrm{LR}}\big)\le \mathfrak{C}\left(\frac{L^2\lambda_{\max}(\Gamma_P)\overline{\sigma}^2\mathrm{tr}(\Gamma_P)}{n\lambda^3_{\min}(\Gamma_P)}\right)^{1/2}\right) \ge 1-\varepsilon
\end{align*}	
where $\mathfrak{C}$ depends on $\varepsilon$ and $\alpha$.
\end{theorem}
The requirement \eqref{eq:requirement-ols} is satisfied when $\widehat{\theta}_1$ is the ordinary least squares (OLS). The dependency on $\overline{\sigma}^2 d/n$ in the rate is minimax optimal as shown by Theorem 1 of \citet{mourtada2022exact}. Recently, \citet{chang2024confidence} provided confidence sets for high-dimensional OLS under similar conditions as above. Their proposal is based on the formulation of the OLS as the root of an estimating equation, or $Z$-estimation. Theorem 10 of \citet{chang2024confidence} establishes that their proposed confidence set converges at the optimal rate of $\sqrt{d/n}$; however, they require $d = o(n^{1/2})$ under the equivalent condition as \ref{as:linreg-moment-covariate}. \citet{chang2023inference} provides a method based on one-step bias-correction, which requires $d = o(n^{2/3})$. On the other hand, Theorem~\ref{thm:LR-ci-width} holds as long as $C d(\log d)^{2} \le n$ (when $q_x = 4$) for some constant $C$ depending on $P$ but not on $n$ or $d$.
% Suppose an IID observation $(X_1^\top,Y_1), \ldots, (X_n^\top,Y_n) \in \mathcal{X} \times \mathcal{Y} \subseteq \mathbb{R}^d \times \mathbb{R}$ from $P$. We consider the following best linear projection: 
% \begin{equation}
%     \theta_P := \argmin_{\theta \in \mathbb{R}^d} \, \E_P (Y-\theta^\top X)^2.
% \end{equation}

% Similar to the mean estimation, the dimension $d$ is allowed to grow with $n$. In this example, we take $m_\theta(Y,X) := (Y-\theta^\top X)^2$. We do not assume that parametric assumption on the underlying statistical model such that $\E_P[Y \mid X=x] = \theta_P^{\top} x$. We denote by $\overline \theta_n$ the ordinary least squares based on $(X_1^\top,Y_1), \ldots, (X_n^\top,Y_n) \in D_2$ such that 
% \begin{align}\label{eq:ols-definition-d2}
% 	\overline \theta_n := \left(\frac{1}{n}\sum_{i=1}^n X_i X_i^{\top}\right)^{-1} \left(\frac{1}{n}\sum_{i=1}^n X_i Y_i\right).
% \end{align}
% First, we observe that 
% \begin{align}
% 	P(m_{\theta_P} - m_{\widehat \theta_1}) = -\E_P \{X^\top(\theta_P - \widehat \theta_1)\}^2.
% \end{align}
% For our preliminary analysis in this section, we propose the upper confidence bound as 
% \begin{align}
% 	U_{n,\alpha}(\theta, \widehat \theta_1; D_2) = -\frac{1}{n}\sum_{i=1}^n \{X_i^\top(\theta - \widehat \theta_1)\}^2,
% \end{align}
% which corresponds to taking $\alpha_2 = o_P(1)$ assuming $U_{n,\alpha}(\theta, \widehat \theta_1; D_2)$ converges in probability to its population counterpart under $P$ \kt{I cannot prove this statement. I can prove it if we take
% \begin{align}
%     U_{n,\alpha}(\theta, \widehat \theta_1; D_2) = -\frac{1}{n}\sum_{i=1}^n \{X_i^\top(\theta - \widehat \theta_1)\}^2 + \varepsilon
% \end{align} 
% for any $\varepsilon > 0$. Probably, we need $\varepsilon = o(d/n)$. We need to overestimate the upper bound slightly. 
% }. We then construct a confidence set for $\theta_P$ based on the Gaussian approximation, given by \eqref{eq:general-set-gaussian}. The following proposition simplifies the expression for the resulting confidence set:
% \begin{proposition}\label{prop:ols-ci-def}
% 	When $m_\theta(Y,X) := \|Y-\theta^\top X\|_2^2$, the confidence set based on \eqref{eq:general-set-gaussian} is equivalent to 
% 	\begin{align}\label{eq:confidence-set-ols}
% 	\widehat{\mathrm{CI}}_{n,\alpha}^{\mathrm{OLS}} := \left\{\theta \in \mathbb{R}^d \, : \, 2(\overline\theta_n-\theta)^\top \widehat\Sigma (\widehat\theta_1-\theta)\le n^{-1/2}z_{1-\alpha} \widehat\sigma_{\widehat\theta_1, \theta}\right\}
% 	\end{align}	
% 	where $\widehat \Sigma := n^{-1}\sum_{i=1}^n X_i X_i^\top$ and $\sigma_{\widehat\theta_1, \theta}^2 := \mathbb{P}_n \big(m_{\theta} - m_{\widehat\theta_1}-\mathbb{P}_n(m_{\theta} - m_{\widehat\theta_1})\big)^2$.
% %	Hence the confidence set is given by 
% %\begin{align}
% %	\mathrm{CI}_{\widehat\theta, \alpha} := \left\{\theta:\mathbb{R}^d \, :\, -2\mathbb{P}_n(\bar\theta^\top X-\theta^\top X)(\theta^\top X-\widehat\theta^\top X)\le n^{-1/2}z_{1-\alpha} \widehat\sigma_{\theta, \widehat \theta}\right\}
% %\end{align}
% %where $\widehat \Sigma := n^{-1}\sum_{i=1}^n(Z_i-\overline Z_n)(Z_i-\overline Z_n)^\top$ and $\|x\|^2_A := x^\top A x$.
% \end{proposition}
% We check the sufficient conditions for this set to be asymptotically valid. 
% We first define the ``error variable" as $\xi_{P,i} := Y_i - \theta_P^\top X_i$. This random variable is well-defined without assuming that $\E_P[Y \mid X=x] = \theta_P^\top x$. The sufficient regularity conditions for the validity corresponds to the following in the linear regression:
% \begin{enumerate}[label=\textbf{(A5-\arabic*)},leftmargin=2cm]
%     \item \label{as:ols-est1}For any $\varepsilon > 0$ and $t \in \Theta$ such that $\|t\|=1$, 
%      \begin{equation}
%         \lim_{n\longrightarrow \infty}\, \sup_{P\in\mathcal{P}}\,\sup_{\|t\|=1}\, \frac{\E_P[\langle t,X\xi_P \rangle^2 1\{\langle t,X\xi_P \rangle^2 > n \varepsilon \E_P\langle t, X\xi_P \rangle^2\}]}{\E_P\langle t, X\xi_P \rangle^2} = 0.
%     \end{equation}
%     \item \label{as:ols-est2} There exists a constant $L \in [0, \infty)$ and $\delta \in (0,1]$ such that 
%      \begin{equation}
%         \sup_{P\in\mathcal{P}}\,\sup_{\|t\|=1}\, \frac{(\E_P \langle t, X\xi_P \rangle^{2+\delta})^{1/(2+\delta)}}{(\E_P \langle t, X\xi_P \rangle^{2})^{1/2}} \le L.
%     \end{equation}
%     \end{enumerate}
    
% \begin{proposition}\label{prop:ols-validity}
% Under \ref{as:ols-est1} or \ref{as:ols-est2}, and assume $\widehat\theta_1$ satisfies \eqref{eq:uniform-convergence}. Additionally, assume
% \begin{align*}
%      \sup_{P\in\mathcal{P}}\, \sup_{\|t\|=1}\, \E_P \langle t, X\rangle^4 < \infty.
% \end{align*}
%  Then, the confidence set given by \eqref{eq:confidence-set-ols} satisfies
%  \begin{equation}
% \lim_{n\longrightarrow \infty}\, \inf_{P\in\mathcal{P}}\, \mathbb{P}_P(\theta(P)\in \widehat{\mathrm{CI}}_{n,\alpha}^{\mathrm{OLS}})  \ge 1-\alpha + o_{\mathcal{P}}(1).
% \end{equation} 
% \kt{I think we need to add small constant $\varepsilon$ to the $U_{n,\alpha_2}(\theta, \widehat \theta_1; D_2)$ in order to prove this.}
% \end{proposition}
% \begin{proposition}\label{prop:ols-width}
% 	The confidence set $\widehat{\mathrm{CI}}_{n,\alpha}$ is contained in $B(\widehat \theta_1, \gamma_n)$ whose radius is given by 
% 	\begin{align}
% 		\gamma_n &:= \frac{2 \left[(1+n^{-1/2}z_{1-\alpha})\|\overline{\theta}_n-\widehat\theta_1\|_{\widehat \Sigma} + n^{-1/2}z_{1-\alpha} \left(\frac{1}{n}\sum_{i=1}^n \overline\xi_i^2 \| \widehat{\Sigma}^{-1/2}X_i\|^2 \right)^{1/2} \right]}{\left[2-3n^{-1/2}z_{1-\alpha}\left(\frac{1}{n}\sum_{i=1}^n  \| \widehat{\Sigma}^{-1/2}X_i\|^4 \right)^{1/2}\right]_+\lambda^{1/2}_{\min}(\widehat \Sigma)}
% 	\end{align}
% 	where $\overline{\xi}_i:=Y_i-\overline{\theta}_n^\top X_i$, $[t]_+ = \max(t, 0)$ and $\lambda_{\min}(A)$ denotes the smallest eigenvalue of a square matrix $A$. 
% \end{proposition}
\subsection{Manski's discrete choice model}\label{sec:manski}
Consider an IID observation $(Y_1, X_1^\top)^\top, \ldots (Y_N, X_N^\top)^\top \in \{-1,1\} \times \mathbb{R}^d$ generated from the following binary response model:
\begin{align}
    Y_i := \mathrm{sgn}(\theta_P^\top X_i + \varepsilon_i) \quad \text{where} \quad \mathrm{sgn}(t) = 2\mathbf{1}\{t \ge 0\}-1.
\end{align}
Here, the error variable $\varepsilon_i$ has zero conditional median given covariates, i.e., $\mathrm{med}(\varepsilon_i | X_i)=0$, but otherwise allowed to depend on $X_i$. In this problem, the inference of interest is $\theta_P$, which can be also written as
\begin{align*}
    \theta_P := \argmin_{\theta \in \mathbb{S}^{d-1}}\, \E_P [Y\, \mathrm{sgn}(\theta^\top X)].
\end{align*}
A popular estimator for $\theta_P$ is defined as the following maximum score estimator, proposed by \citet{manski1975maximum}, which solves
\begin{align}\label{eq:maximum-score-estimator}
    \widehat\theta_1 := \argmax_{\theta \in \mathbb{S}^{d-1}}\, \sum_{i\in\mathcal{D}_1} Y_i\, \mathrm{sgn}(\theta^\top X_i).
\end{align}
The asymptotic behavior of $\widehat \theta_n$ exhibits a non-standard limit, studied by \cite{manski1985semiparametric, kim1990cube}. The inference for this problem is known to be challenging, and \cite{cattaneo2020bootstrap} proposes a bootstrap-based approach. By the fact that $Y_i\, \mathrm{sgn}(\theta^\top _i X_i)$ is uniformly bounded by one, we can use the confidence set based on the concentration inequality with $B_0 = 2$. Below, we denote by $\widehat{\mathrm{CI}}^{\mathrm{Manski}}_{n,\alpha}$ the empirical-Bernstein-based confidence set \eqref{eq:ci1-application} with $m_{\theta}(x,y) = -y\cdot\mathrm{sgn}(\theta^\top x)$. We now provide the validity statement for this confidence set.
\begin{theorem}\label{thm:manski-validity}
    For any fixed $n\ge 1$,
    \begin{align*}
\inf_{P\in\mathcal{P}}\, \mathbb{P}_P(\theta_P \in \widehat{\mathrm{CI}}^{\mathrm{Manski}}_{n,\alpha}) \ge 1-\alpha. 
\end{align*}
\end{theorem}
\begin{proof}[\bfseries{Proof of Theorem~\ref{thm:manski-validity}}]    
The validity follows immediately in view of Theorem~\ref{thm:validity-concentration}. 
\end{proof}
Next, we demonstrate the width of the confidence set in $L_2$-norm. Below, we introduce additional assumptions on the joint distribution on $X$ and $\varepsilon$. Both assumptions are standard in the literature.
\begin{enumerate}[label=\textbf{(B\arabic*)},leftmargin=2cm]
\setcounter{enumi}{2}
\item \label{as:tsybakov} Let $P \in \mathcal{P}$ be the joint distribution on $X, \varepsilon$ and $\eta_P(x) := \mathbb{P}_P(Y=1 \mid X=x)$. There exist constants $C_0$ and $0 < t^* < 1/2$ with $C_0t^* > 1$, and $\beta < \infty$, such that 
\begin{align*}
    \mathbb{P}_P\left(\left|\eta_P(X)- \frac{1}{2}\right| < t\right) \le C_0t^{1/\beta} \quad \text{for all} \quad 0 < t < t^*.
\end{align*}
\item \label{as:covariate-manski}
There exists a constant $c_1$, not depending on $n$ or $d$, such that 
\begin{align*}
    c_1\|\theta-\theta_P\|_2 \le \mathbb{P}_X\left(\mathrm{sgn}(\theta^\top  X) \neq \mathrm{sgn}(\theta_P^\top  X)\right)
\end{align*}
for all $\theta \in \mathbb{S}^{d-1}$ where $\mathbb{P}_X$ denotes the probability measure under the marginal distribution of $X$.
\end{enumerate}
Both assumptions are identical to those considered in \citet{mukherjee2019nonstandard, mukherjee2021optimal}. \ref{as:tsybakov} is often called the \textit{low noise (the margin) assumption} in the classification literature \citep{mammen1999smooth, tsybakov2004optimal}. This condition quantifies the deviation of the conditional class probability from $1/2$ near the decision boundary of the Bayes' classifier, i.e., $\mathbb{P}_P(Y=1|X)\ge 1/2$. As $\beta \longrightarrow 0$, the decision boundary becomes bounded away from $1/2$, representing the most favorable situation for the classification. \ref{as:covariate-manski} was introduced to relate the distribution of covariates $X$ to the underlying geometry in the parameter space $\mathbb{S}^{d-1}$. See \cite{mukherjee2021optimal} for further discussion. 

We provide the width of the confidence set in terms of the $L_2$-norm:
\begin{theorem}\label{thm:manski-width}
Let $s_n$ be the random variable defines as \ref{as:rate-initial-estimator}. Assume \ref{as:tsybakov} and \ref{as:covariate-manski}. Then for any $d \le n$, it follows
\begin{align*}
\mathbb{P}_P\left(\mathrm{Diam}_{\|\cdot\|_2}\big(\widehat{\mathrm{CI}}^{\mathrm{Manski}}_{n,\alpha}\big)\le \mathfrak{C}\left\{\left(\frac{d\log(n/d)}{n}\right)^{1/(1+2\beta)}  + s_n^{1/(1+\beta)}\right\}\right) \ge 1-\varepsilon
\end{align*}	
 where $\mathfrak{C}$ depends on $\alpha, \varepsilon, c_1,\beta,t^*$ and $C_0$. Furthermore, assume that the initial estimator satisfies
 \begin{align}\label{eq:manski-requirement}
     \mathbb{P}_P\left(\|\widehat\theta_1-\theta(P)\|_2 \le C_\varepsilon\left(\frac{d\log(n/d)}{n}\right)^{1/(1+2\beta)}\right) \ge 1-\varepsilon
 \end{align}
for any $\varepsilon > 0$ with a constant $C_\varepsilon$ depending on $\varepsilon$. It then implies 
\begin{align*}
\mathbb{P}_P\left(\mathrm{Diam}_{\|\cdot\|_2}\big(\widehat{\mathrm{CI}}^{\mathrm{Manski}}_{n,\alpha}\big)\le \mathfrak{C}\left(\frac{d\log(n/d)}{n}\right)^{1/(1+2\beta)}\right) \ge 1-\varepsilon
\end{align*}
for all $n \ge N_\varepsilon$ with $N_\varepsilon$ depending on $\varepsilon$ and $\mathfrak{C}$  depending on $\varepsilon$ and $\alpha$.
\end{theorem}
Theorem 3.2 of \citet{mukherjee2019nonstandard} shows that the rate requirement \eqref{eq:manski-requirement} is satisfied by the standard maximum score estimator defined as \eqref{eq:maximum-score-estimator}. The rate of convergence matches that of the minimax lower bound up to the logarithmic factor (See Theorem 3.4 of \citet{mukherjee2019nonstandard}). 
% \subsection{Nonparametric classification}
% Suppose an IID observation $(Y_1, X_1^\top)^\top, \ldots (Y_n, X_n^\top)^\top \in \{0,1\} \times \mathcal{X}$ where $\mathcal{X} \subseteq \mathbb{R}^d$. Let $\Theta$ be a collection of measurable functions $\theta: \mathcal{X}\mapsto \{0,1\}$. We consider the construction of the ``decision rule", which minimizes the following risk:
% \begin{align}\label{eq:classification}
%     \theta_P := \argmin_{\theta\in\Theta}\, \mathbb{E}_P[\mathbf{1}\{Y \neq \theta(X)\}] = \argmin_{\theta\in\Theta}\,\mathbb{P}_P(Y \neq \theta(X))
% \end{align}
% where the expectation is taken under the joint distribution between $X$ and $Y$. The validity of the confidence set based on the concentration inequality holds immediately since $m_{\theta} := \mathbf{1}\{Y\neq\theta(X)\}$, which is uniformly bounded by 1. 
% \begin{theorem}\label{thm:classification-validity}
%     For any fixed $n\ge 1$,
%     \begin{align*}
% \inf_{P\in\mathcal{P}}\, \mathbb{P}_P(\theta_P \in \widehat{\mathrm{CI}}^{\mathrm{Class.}}_{n,\alpha}) \ge 1-\alpha. 
% \end{align*}
% \end{theorem}
% \begin{proof}[\bfseries{Proof of Theorem~\ref{thm:classification-validity}}]    
% The validity follows immediately in view of Theorem~\ref{thm:validity-concentration}. 
% \end{proof}

% We now provide the width analysis. Following \citet{audibert2007fast}, we consider the family of plug-in classifiers, $\theta(x) := \mathbf{1}\{\eta(x) \ge 1/2\}$, where $\eta$ belongs to a large (nonparametric) class of functions. We can assert that the minimizer \eqref{eq:classification} corresponds to the Bayes classifier such that 
% \begin{align*}
%     \theta_P(x) := \mathbf{1}\{\eta_P(x) \ge 1/2\} \quad \text{where} \quad \eta_P(x) := \mathbb{P}_P(Y=1 \mid X=x).
% \end{align*}
% Let $\mathcal{H}$ be a set of functions that contains $\eta_P$. For any $\eta \in \mathcal{H}$, we construct a classifier by the plug-in rule $\theta_{\eta}(x) := \mathbf{1}\{\eta(x) \ge 1/2\}$. We provide the result when $\mathcal{X}=[0,1]^d$ and $\mathcal{H}$ is a set of $\gamma$-H\"{o}lder continuous functions defined as follows. For any $k=(k_1, k_2, \dots, k_d)$ of a $d$-dimensional index set where each $k_i$ is a non-negative integer and $|k|=\sum_{i=1}^d k_i$, we define the operator $D^k$ as
%     $$D^k \eta := \frac{\partial^{|k|} \eta(x)}{\partial^{k_1} x_1\dots \partial^{k_d} x_d}\quad \text{and}\quad D^0\eta := \eta.$$
% The H\"{o}lder class on $[0,1]^d$ consists of functions that satisfy the following condition:

% \begin{align*}
%     &\mathcal{H} \equiv \mathcal{H}_d(\gamma):= \left\{\eta: \sum_{0 \le |m| \le \lfloor \gamma\rfloor}\|D^m \eta\|_\infty +\sum_{|k| = \lfloor \gamma\rfloor}\sup_{x\neq y,\, x,y\in \Omega}\frac{|D^{k} \eta(y)-D^{k} \eta(x)|}{\|x-y\|^{ \gamma-|k|}}\le 1\right\}.
% \end{align*} 
% Following Section 3.4.11 of \cite{van1996weak}, one metric between two classifiers is the ``disagreement" probability:
% \begin{align}\label{eq:metric-classifier}
%     \|\theta_1-\theta_2\| = \mathbb{P}_P(\theta_1(X)\neq \theta_2(X)) = \frac{1}{2}\|\theta_1-\theta_2\|_{L_1(P)}.
% \end{align}
% The following theorem provides the convergence rate of the width of the confidence set when the metric is given by \eqref{eq:metric-classifier}.
% \begin{theorem}\label{thm:classificaiton-width}
%     Assume \ref{as:tsybakov} and $\mathcal{H}$ is a set of $\gamma$-H\"{o}lder continuous functions such that $d\beta < \gamma$. Then for any $n\ge 1$
% \begin{align*}
% \mathbb{P}_P\left(\mathrm{Diam}_{\|\cdot\|}\big(\widehat{\mathrm{CI}}^{\mathrm{Class.}}_{n,\alpha}\big)\le \mathfrak{C}\left\{n^{-\gamma/((1+\beta)\gamma+d\beta)} + s_n^{1/(1+\beta)}\right\}\right) \ge 1-\varepsilon
% \end{align*}	
%  where $\mathfrak{C}$ depends on $\alpha, \varepsilon$ and $\gamma$.
% \end{theorem}


\subsection{Quantile estimation without positive densities}\label{sec:quantile}
Consider an IID observation $X_1, \ldots, X_N \in \mathbb{R}$ generated from $P \in \mathcal{P}$ where the inference of interest is the $\gamma$-quantile defined as
\begin{align*}
\theta(P) := \inf \left\{t \, : F_P(t) \ge \gamma \right\} \quad \text{for} \quad \gamma \in (0,1)
\end{align*}
and $F_P(t) := \mathbb{P}_P(X\le t)$. It is well-known that $\theta(P)$ minimizes the following ``quantile" loss:
\begin{align*}
    \theta(P) := \argmin_{\theta \in \mathbb{R}}\, \E_P[\gamma(X-\theta)_+ + (1-\gamma)(\theta-X)_+]
\end{align*}
where $(t)_+ = \max(t, 0)$. The sample quantile converges to a Gaussian distribution at the $n^{1/2}$ rate when the distribution of $X$ has a strictly positive density at $\theta(P)$. When the density at $\theta(P)$ is zero, however, the sample quantile converges at a rate depending on the H\"{o}lder smoothness of the $F_P(t)$ in the neighborhood of $\theta(P)$. In this case, the limiting distribution is no longer Gaussian and also depends on the H\"{o}lder smoothness of the $F_P(t)$ in the neighborhood of $\theta(P)$ \citep{smirnov1952limit}. Below, we construct the CLT-based confidence set \eqref{eq:ci2-application} with $m_{\theta}(x) = \gamma(x-\theta)_+ + (1-\gamma)(\theta-x)_+$, and denote the corresponding set by $\widehat{\mathrm{CI}}_{n,\alpha}^{\gamma}$. We quantity the smoothness of the $F_P(t)$ near $\theta(P)$ as follows:
\begin{enumerate}[label=\textbf{(B\arabic*)},leftmargin=2cm]
\setcounter{enumi}{4}
\item \label{as:cdf-Holder} 
There exist $\delta >0$, $M_0,M_1 \in (0,\infty)$ and $M_0 >M_1$ such that 
\begin{align*}
    |F(\theta) - F(\theta(P)) - M_0|\theta - \theta(P)|^{\beta} \mathrm{sgn}(\theta-\theta(P))| \le M_1|\theta-\theta(P)|^\beta
\end{align*}
for all $\theta$ such that $|\theta-\theta(P)| \le \delta$.
\end{enumerate}
The H\"{o}lder smoothness as described in \ref{as:cdf-Holder} should be compared to \citet[Equation (6)]{knight1998limiting}. When $\beta=1$, this assumption becomes equivalent to requiring that the density at the true $\gamma$-quantile is bounded away from zero. We now proceed to the validity statement. 
\begin{theorem}\label{thm:quantile-validity}
Let $\{q_n\}$ be a deterministic and non-decreasing sequence such that $q_n \ge 1$ for all $n$, and
\begin{align*}
    \lim_{n\to \infty}\,\sup_{P \in \mathcal{P}}\mathbb{P}_P(q_n|\widehat \theta_1 - \theta(P)| > \delta) = 0
\end{align*}
where $\delta$ corresponds the one defined in \ref{as:cdf-Holder}. Then assuming $\{n\gamma(1-\gamma)\}^{-1} = o(1)$ and  $\{q_n^\beta\gamma(1-\gamma)\}^{-1}= O(1)$, it follows that 
\begin{align*}
    \liminf_{n\longrightarrow \infty}\,\inf_{P\in\mathcal{P}}\, \mathbb{P}_P(\theta(P) \in \widehat{\mathrm{CI}}_{n,\alpha}^{\gamma}) \ge 1 - \alpha.
\end{align*}
\end{theorem}
The result of Theorem~\ref{thm:quantile-validity} allows for $\gamma \equiv \gamma_n$ to depend on the sample size $n$. When there exist constants $c$ and $C$ such that $0 < c \le \gamma_n \le C < 1$ for all $n$, the validity holds under the consistency of the initial estimator. When $\gamma_n \longrightarrow 0$ or $\gamma_n \longrightarrow 1$, then there is a restriction on how quickly $\gamma_n$ can tend to these extreme values depending on $\beta$ and the convergence rate of $\widehat{\theta}_1$. This requirement may be relaxed under the alternative, but possibly stronger, assumptions on $P$---see Remark~\ref{remark:consistency}.
Finally, the width of the confidence set is obtained as follows:
\begin{theorem}\label{thm:quantile-ci-width}
Let $s_n$ be the random variable defined as \ref{as:rate-initial-estimator}. Then for all  $n \ge C_1 \delta^{-2\beta}$ with $\delta$ corresponding to the one in \ref{as:cdf-Holder}, it holds that 
\begin{align*}
\mathbb{P}_P\left(\mathrm{Diam}_{|\cdot|}\big(\widehat{\mathrm{CI}}_{n,\alpha}^{\gamma}\big)\le \mathfrak{C}\tau_n\right) \ge 1-\varepsilon
\end{align*}	
where
\begin{align*}
    \tau_n &:= \left(\frac{1}{n^{1/2\beta}} + s_n^{1/(1+\beta)}\right)\mathbb{P}_P(|\widehat\theta_1-\theta_0|<C_2\delta^{1+\beta}) + \delta^{-\beta}\E_P[|\widehat\theta_1 - \theta_0|\mathbf{1}\{|\widehat\theta_1-\theta_0|\ge C_2\delta^{1+\beta}\}]
\end{align*}
and $\mathfrak{C}$, $C_1$, and $C_2$ depend on $\varepsilon$, $M_0$, $M_1$, $\beta$ and $\alpha$. Furthermore, assume that the initial estimator satisfies
\begin{align}\label{eq:quantile-initial}
        \mathbb{P}_P\left(|\widehat\theta_1 - \theta(P)|^2 \le C_\varepsilon n^{-1/\beta}\right) \ge 1-\varepsilon
    \end{align}
    for any $\varepsilon > 0$ with a constant $C_\varepsilon$ depending on $\varepsilon$. It then implies for all $n \ge N_{\varepsilon,\delta}$ with $N_{\varepsilon,\delta}$ depending on $\varepsilon$, $M_0$, $M_1$, $\beta$, $\alpha$ and $\delta$, 
\begin{align*}
\mathbb{P}_P\left(\mathrm{Diam}_{|\cdot|}\big(\widehat{\mathrm{CI}}_{n,\alpha}^{\gamma}\big)\le \mathfrak{C}n^{-1/(2\beta)}\right) \ge 1-\varepsilon
\end{align*}	
where $\mathfrak{C}$ only depends on $\varepsilon$, $\alpha$, $\beta$ $M_0$ and $M_1$.
\end{theorem}
The requirement in \eqref{eq:quantile-initial} is satisfied when $\widehat{\theta}_1$ is the sample quantile. The convergence rate of the confidence set indicated by Theorem~\ref{thm:quantile-ci-width} matches that of the sample quantile under \ref{as:cdf-Holder} as given by Example 1 of \cite{knight1998limiting}. In fact, \citet{knight1998limiting} provides the limiting distribution of the sample quantile under \ref{as:cdf-Holder}; however, the traditional approach requires prior knowledge of $\beta$ to perform asymptotic inference. The proposed confidence set of this manuscript, in contrast, converges at the rate $n^{-1/(2\beta)}$ automatically without the knowledge of $\beta$. In the special case of $\beta=1$, i.e., the density is bounded away from zero at the $\gamma$-quantile, and the confidence shrinks at the parametric rate of $n^{-1/2}$. 

\begin{remark}[The proof of Theorem~\ref{thm:quantile-ci-width}]
The width analyses in this section are mostly performed as the direct applications of Theorem~\ref{thm:concentration-width} or Theorem~\ref{thm:concentration-width-unbounded}. The proof of Theorem~\ref{thm:quantile-ci-width}, however, differs significantly since the curvature assumption \ref{as:margin} only holds locally for $\theta$ such that $\|\theta-\theta(P)\| < \delta$. As a result, Theorem~\ref{thm:concentration-width-unbounded} cannot be applied for the parameter outside of this neighborhood. While the proof of Theorem~\ref{thm:quantile-ci-width} crucially relies on the convexity and Lipschitzness of the quantile loss, a general result in the spirit of Theorem~\ref{thm:concentration-width-unbounded} may be useful under the local analog to \ref{as:margin}. Towards this task, one may need to extend the ratio-type empirical process to the unbounded function spaces \citep{gine2006concentration}. We are currently investigating this direction. 
\end{remark}

==> main/clt.tex <==
\subsection{Confidence sets based on the Berry-Esseen Bound }
In this section, we propose an alternative approach to construct the lower bound satisfying \eqref{eq:lower-bound} based on the Berry-Esseen bounds. The Berry-Esseen bound for T-statistics \citep{bentkus1996berryiid} provides the following non-asymptotic statement that there exists $\delta_n>0$:
\begin{align}\label{eq:be-approximation}
	\sup_{t\in\mathbb{R}} \left|\mathbb{P}\left(n^{1/2}\left(\frac{\widehat H_n(\theta)-\widehat H(\theta)}{\widehat\sigma(\theta)}\right) \le t \mid D_1 \right )-\Phi(t)\right| \le \delta_n
\end{align}
where 
\begin{align}
	\widehat \sigma^2(\theta) = \frac{1}{|I_2|}\sum_{i \in |I_2|}\left\{ \widehat\eta_\theta(Z_i)-\widehat H_n(\theta)\right\}^2
\end{align}
and $\Phi(t)$ is a cumulative distribution function (CDF) of the standard Gaussian random variable. This approximation result can be used for constructing the high-probability lower bound \eqref{eq:lower-bound} using the symmetry of the Gaussian random variable,  

\begin{align}
	&\mathbb{P}\left(n^{1/2}\left(\frac{\widehat H(\theta)-\widehat H_n(\theta)}{\widehat\sigma(\theta)}\right) \le q_{\alpha} \mid D_1 \right )\\
	&\qquad \Longleftrightarrow \mathbb{P}\left(\widehat H(\theta)\le \widehat H_n(\theta) + n^{-1/2}q_{\alpha}\widehat\sigma(\theta) \mid D_1 \right ) \le \Phi(q_\alpha) + \delta_n = \alpha+ \delta_n.
\end{align}

Therefore, the estimator $\widehat L(\theta) := \widehat H_n(\theta) + n^{-1/2}q_{\alpha}\widehat\sigma(\theta)$ satisfies \eqref{eq:lower-bound} with probability at least $1-\alpha-\delta_n$. This yields the confidence set 
\begin{equation}
    \widehat{C}_n := \left\{\theta \in \Theta \, : \, \widehat H_n(\theta)\le n^{-1/2}q_{1-\alpha}\widehat \sigma(\theta)\right\}.
\end{equation}

Alternatively, one can shrink the confidence set without compensating the validity by finding a mapping $\theta \mapsto U(\theta, \widehat \theta)$ such that $\widehat H(\theta_0)\le U(\theta_0, \widehat \theta) \le 0$. The corresponding confidence set is
\begin{equation}
    \widehat{C}^*_n := \left\{\theta \in \Theta \, : \, \widehat H_n(\theta)\le n^{-1/2}q_{1-\alpha}\widehat \sigma(\theta)+\big(0 \wedge U(\theta, \widehat \theta)\big)\right\}.
\end{equation}

	Now the confidence set is given by 
	\begin{align}
		&\left\{\theta \in \Theta : P_0 (m_\theta-m_{\theta_0})+P_0(m_{\theta_0}-m_{\widehat \theta}) \le -(\mathbb{P}_n-P_0) (m_\theta-m_{\theta_0}+m_{\theta_0}-m_{\widehat \theta}) +q_{1-\alpha}n^{-1/2}\widehat \sigma_{\theta, \widehat\theta} \right\}\\
		& \subseteq \left\{\theta \in \Theta : P_0 (m_\theta-m_{\theta_0})\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0}) +   q_{1-\alpha}n^{-1/2}\widehat \sigma_{\theta, \theta_0}  + \Gamma_n(\widehat\theta, \theta_0)\right\}\\
		& \subseteq \left\{\theta \in \Theta : \|\theta-\theta_0\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0}) +   q_{1-\alpha}n^{-1/2}\widehat \sigma_{\theta, \theta_0} +\Gamma_n(\widehat\theta, \theta_0)\right\}
	\end{align}
	where 
	\[\Gamma_n(\widehat\theta, \theta_0) := \mathbb{P}_n(m_{\widehat \theta}-m_{\theta_0}) + q_{1-\alpha}n^{-1/2}\widehat \sigma_{\theta_0, \widehat\theta}. \]


\kt{We truncate the empirical process at level $B$ such that 
\begin{align*}
    \mathbb{G}_n(m_\theta-m_{\theta_0}) 
    &=\mathbb{G}_n\left\{(m_\theta-m_{\theta_0})1\left\{|m_\theta-m_{\theta_0}|\le B\right\}+(m_\theta-m_{\theta_0})1\left\{|m_\theta-m_{\theta_0}|> B\right\}\right\}
\end{align*}}

The assumption of IID distribution is unnecessary as the Berry-Esseen bound for T-statistics holds under sequence of non-identical distributions. See \citet{bentkus1996berry} for details.

\begin{theorem}\label{thm:validity-BE}
    Assuming \eqref{eq:be-approximation}, $\widehat C_n$ is a finite-sample valid $(1-\alpha-\delta_n)$-level confidence set for $\theta_0$ such that $\mathbb{P}(\theta_0 \in \widehat C_n \mid D_1) \ge 1-\alpha-\delta_n$ for any $n\ge2$. Analogous results hold for $\widehat{C}^*_n$.
\end{theorem}
The proof of this result is identical to Theorem~\ref{thm:validity}.
\begin{definition}[The $L_p$-$L_2$ norm equivalence]\label{def:lp-l2}
	A random vector $Z$ with mean $\theta_0$ satisfies the $L_p$-$L_2$ norm equivalence with a constant $L \ge 1$ if for every $t \in \mathbb{R}^d$,
	\begin{align}
		(\E |t^\top (Z-\theta_0)|^p)^{1/p}\le L(\E |t^\top (Z-\theta_0)|^2)^{1/2}
	\end{align}
\end{definition}
\begin{example}[High-dimensional mean estimation]
Suppose we observe $Z_1, \ldots, Z_n \in \mathcal{Z}$ from the distribution with the mean $\theta_0$ and the corresponding M-estimation problem is given by 
\begin{align}
	\theta_0 := \argmin_{\theta \in \mathcal{Z}} \int \|z-\theta\|_2^2 \,dP_0(z).
\end{align}
Let $m_\theta(z) = \|z-\theta\|_2^2$ and any pilot estimator of the mean $\widehat \theta$.
Then we have
    \begin{align*}
        \widehat{\eta}_\theta(z) &= \|z-\theta\|_2^2 - \|z-\widehat\theta\|_2^2.    \end{align*}
    Furthermore, we have 
    \begin{align*}
        \widehat H(\theta) &=  \E[\|Z-\theta\|_2^2- \|Z-\widehat\theta\|_2^2]\\
        &= -2(\widehat \theta-\theta_0)^\top (\widehat \theta-\theta)+\|\widehat\theta-\theta\|_2^2
    \end{align*}
    and therefore $\widehat H(\theta_0) = -\|\widehat \theta - \theta_0\|_2^2$
    \begin{align}
    \widehat{C}_n^* &:= \left\{\theta \in \Theta \, : \, \widehat H_n(\theta)\le n^{-1/2}q_{1-\alpha}\widehat \sigma(\theta) -\|\theta - \widehat \theta\|_2^2\right\}\\
    &=\left\{\theta \in \Theta \, : \, (\theta-\bar Z)^\top (\theta - \widehat \theta)\le n^{-1/2}q_{1-\alpha} \|\widehat \theta - \theta\|_{\widehat \Sigma}\right\}.
\end{align}
\begin{theorem}[Validity of the confidence set]\label{thm:mean-valid}
For any $N\ge 2$, the confidence is valid such that there exists an absolute constant $c > 0$
\begin{align}
	\mathbb{P}_0(\theta \in \widehat{C}_n^*) \ge 1-\alpha-cN^{-1/2}\frac{\E|(Z_1-\theta_0)^\top(\widehat \theta - \theta)  |^3 }{\left\{\E|(Z_1-\theta_0)^\top(\widehat \theta - \theta)  |^2\right\}^{3/2}}
\end{align}
Under the $L_3$-$L_2$ norm equivalence defined as \ref{def:lp-l2} with $p=3$, the confidence set is valid such that $\mathbb{P}_0(\theta_0 \in \widehat{C}_n^*) \ge 1-\alpha-cL^3N^{-1/2}$ for any $N \ge 2$.
\end{theorem}

Though Theorem~\ref{thm:mean-valid} uses the well-known form of the Berry-Esseen bound based on finite third moment of $Z_1$, this result can be extended to the case with finite $2+\delta$-moment of $Z_1$ using Theorem 1.2 of \citet{bentkus1996berry}.
\begin{corollary}[Validity under $2+\delta$-moment]\label{cor:mean-valid-delta}
When the random variable $Z_1$ has finite $2+\delta$ moment with $0 \le \delta < 1$, then for any $N\ge 2$, there exists an absolute constant $c > 0$
\begin{align}
	\mathbb{P}_0(\theta \in \widehat{C}_n^*) \ge 1-\alpha-cN^{-\delta/2}\frac{\E|(Z_1-\theta_0)^\top(\widehat \theta - \theta)  |^{2+\delta} }{\left\{\E|(Z_1-\theta_0)^\top(\widehat \theta - \theta)  |^2\right\}^{(2+\delta)/2}}
\end{align}
Under the $L_{2+\delta}$-$L_2$ norm equivalence defined as \ref{def:lp-l2} with $p=2+\delta$, the confidence set is valid such that $\mathbb{P}_0(\theta_0 \in \widehat{C}_n^*) \ge 1-\alpha-cL^{2+\delta}N^{-\delta/2}$ for any $N \ge 2$.
\end{corollary}


\end{example}

%Consider a fairly prevalent scenario of  M-estimation, which involves finding $\theta_0$ and $\widehat\theta_n$ as follows:
%\begin{align*}
%    \theta_0 := \argmin_{\theta \in \Theta} P_0 m_\theta \quad \text{and}\quad
%    \widehat\theta_n := \argmin_{\theta \in \Theta} \mathbb{P}_n m_\theta.
%\end{align*}
%Let $\eta_\theta := z \mapsto (m_\theta - m_{\widehat \theta})(z)$ and $\sigma_\theta^2 := P_0\eta_\theta^2-(P_0 \eta_\theta)^2$. We choose $U_n(\theta) := n^{-1/2}q_{1-\alpha}\sigma_\theta + P_\theta \eta_\theta$. Given $\mathcal{D}_1$, the estimator $\widehat \theta$ becomes deterministic, and thus $\eta_\theta$ is a fixed function of $Z$ indexed by $\theta$. Consequently, for any $\theta \in \Theta$, we have:
%\begin{align*}
%P_\theta \left(\mathbb{P}_n (m_\theta - m_{\widehat \theta}) \le U_n(\theta) \mid \mathcal{D}1\right) &= P_\theta \left(\mathbb{P}_n \eta_\theta \le n^{-1/2}q_{1-\alpha}\sigma_\theta + P_\theta \eta_\theta\mid \mathcal{D}_1\right)\\
%&= P_\theta \left(\mathbb{G}_n \frac{\eta_\theta}{\sigma_\theta} \le q_{1-\alpha} \mid \mathcal{D}1\right),
%\end{align*}
%where $\mathbb{G}_n$ denotes the empirical process $n^{1/2}(\mathbb{P}_n - P_0)$. By invoking the central limit theorem, the last expression converges to:
%\begin{align*}
%P_\theta \left(\mathbb{G}_n \frac{\eta_\theta}{\sigma_\theta} \le q_{1-\alpha} \right) \longrightarrow P \left(G \le q_{1-\alpha} \right) = 1-\alpha,
%\end{align*}
%where $G$ follows a standard normal distribution.
%
%\paragraph{Finite-sample coverage}
%
%The Berry-Esseen bound states that there exists a constant $C$ such that:
%\begin{equation}
%    \sup_t \left|P_\theta \left(\mathbb{G}_n \frac{\eta_\theta}{\sigma_\theta} \le  t\right)  - P\left(G \le  t\right)
%    \right|\leq C\frac{P_0 |\eta_\theta-P_0\eta_\theta|^3}{\sqrt{n}\sigma^3_\theta}.
%\end{equation}
%{\color{red}\bf First, try to verify if $P_0|\eta_{\theta}|^3/(P_0|\eta_{\theta}|^2)^{3/2}$ is bounded, then the Berry--Esseen bound is also bounded; I am not sure if this is true but I hope this is true. Also, before proceeding to the smooth objective function case, I would suggest considering the case of mean estimation. Take $m_{\theta}(z) = \|z - \theta\|_2^2$ and see how the Berry--Esseen bound behaves and analyze $\eta_{\theta}$ as well as the upper bound on the BE bound.}
%We assume that the objective function $m_\theta$ is sufficiently smooth, allowing for the following Taylor expansion about the true minimizer $\theta_0$:
%\begin{align}\label{eq:taylor_expansion}
%    \eta_{\theta_0} = m_{\theta_0} - m_{\widehat \theta} = \dot m_{\theta_0}(\theta_0 - \widehat \theta) + \frac{1}{2}\ddot{m}_{\theta_*}(\theta_0 - \widehat \theta)^2.
%\end{align}
%Here, $\dot m_{\theta_0}$ and $\ddot m_{\theta_0}$ correspond to the first and the second derivatives of the objective function with respect to $\theta$ at $\theta=\theta_0$. Additionally, the parameter $\theta_*$ is defined as $\theta_* \in [\theta_0, \widehat \theta]$. Moreover, assuming that $m_{\theta}$ is a convex function of $\theta$ and $\theta_0$ is an interior point of $\Theta$, it follows that $\dot m_{\theta_0}=0$ {\color{red}\bf $P_0\dot m_{\theta_0} = 0$ not $\dot m_{\theta_0}$}. Using these results, we can obtain
%\begin{align*}
%    \sigma_{\theta_0}^3 = \frac{1}{8}(\theta_0 - \widehat \theta)^6 \left(P_0\ddot{m}^2_{\theta_*}\right)^{3/2}\quad \text{and}\quad
%    P_0 |\eta_\theta|^3 = P_0 \left|\frac{1}{2}\ddot{m}_{\theta_*}(\theta_0 - \widehat \theta)^2\right|^3 = \frac{1}{8} (\theta_0 - \widehat \theta)^6 P_0 |\ddot{m}_{\theta_*}|^3.
%\end{align*}
%Provided $\theta_0 \neq \widehat \theta$, we have 
%\begin{align*}
%    C\frac{P_0 |\eta_\theta|^3}{\sqrt{n}\sigma^3_\theta} = \frac{C}{\sqrt{n}}\frac{P_0 |\ddot{m}_{\theta_*}|^3}{\left(P_0\ddot{m}^2_{\theta_*}\right)^{3/2}} \le \frac{C}{\sqrt{n}}\sup_{\theta \in B(\theta_0, \|\theta_0-\widehat \theta\|)}\frac{P_0 |\ddot{m}_{\theta}|^3}{\left(P_0\ddot{m}^2_{\theta}\right)^{3/2}}.
%\end{align*}
%The remainder term in the Berry-Esseen bound relies on the estimation rate of $\widehat \theta$ as indicated by the supremum of $P_0 |\ddot{m}{\theta}|^3/\left(P_0\ddot{m}^2_{\theta}\right)^{3/2}$ near $\theta_0$. Let us assume that we can control the convergence rate of $\widehat \theta$ using a suitable metric $\|\cdot\|$, such as $\|\cdot\|_{L_2(P_0)}$. Consequently, we obtain the following bound:
%\begin{align*}
%P\left(\left|C\frac{P_0 |\eta_\theta|^3}{\sqrt{n_2}\sigma^3_\theta}\right| \le \delta \right) &\le    P\left(\left|C\frac{P_0 |\eta_\theta|^3}{\sqrt{n_2}\sigma^3_\theta}\right| \le \delta , \, \|\widehat \theta-\theta\| < r_{n_1}\right) + P(\|\widehat \theta-\theta\|\ge r_{n_1})\\
%&\le P\left(Cn_2^{-1/2}\sup_{\theta \in B(\theta_0, r_{n_1})}\left|\frac{P_0 |\ddot{m}_{\theta}|^3}{\left(P_0\ddot{m}^2_{\theta}\right)^{3/2}}\right| \le \delta \right) + P(\|\widehat \theta-\theta\|\ge r_{n_1})
%\end{align*}
%This inequality characterizes the finite-sample coverage error in terms of $n_1$ and $n_2$. The first term is proportional to $n_2^{-1/2}$ and depends on the constant related to the local behavior of $\theta \mapsto \ddot{m}_{\theta}$ near $\theta_0$. On the other hand, the second term relies on the convergence rate of the estimator. Assuming, for instance, that 
%\begin{align*}
%    \sup_{\theta \in \Theta}\left|\frac{P_0 |\ddot{m}_{\theta}|^3}{\left(P_0\ddot{m}^2_{\theta}\right)^{3/2}}\right| \le K
%\end{align*}
%for some $K <\infty$ and if $n_2$ is sufficiently large, we can choose $r_n$ to be arbitrarily large as well. Therefore, the slow convergence rate of $\widehat \theta_n$ does not compromise the ``finite-sample" coverage of the proposed method.
%
%\paragraph{Confidence width}
%The width of the confidence interval is proportional to $n_2^{-1/2}\sigma_{\theta}$. Based on the previous derivation, we can write:
%\begin{align*}
%    P\left(|n_2^{-1/2}\sigma_{\theta}| \le u\right) &\le P\left(|n_2^{-1/2}\sigma_{\theta}| \le u, \, \|\widehat \theta-\theta\| < r_{n_1}\right) + P(\|\widehat \theta-\theta\|\ge r_{n_1}) \\
%    &\le P\left(1/2 n_2^{-1/2} r_{n_1}^2 \sup_{\theta \in B(\theta_0, r_{n_1})}P_0 |\ddot{m}^2_{\theta}|^{1/2} \le u\right) + P(\|\widehat \theta-\theta\|\ge r_{n_1}) 
%\end{align*}
%where the first term is now a product of $n_2^{-1/2}$ and $r^2_{n_1}$. 


% If the objective $\theta \mapsto m_\theta$ is not smooth, such that the Taylor expansion given by \eqref{eq:taylor_expansion} does not hold, then the upper bound $U_n(\theta)$ is simply the $1-\alpha$th quantile of the random variable $m_\theta(Z) - m_{\widehat \theta}(Z)$, which if a functional of $P_\theta$. Formally, we have
% \begin{align*}
%     \psi_\theta := \inf \{t \in \mathbb{R} \,: \, 1-\alpha \le F_\theta(t)\}
% \end{align*}
% where $F_\theta(t)$ is the CDF of $\eta_\theta = m_{\theta}-m_{\widehat \theta}$. By definition, we have
% \begin{equation}
%    P\big(\mathbb{P}_n \eta_\theta \leq \psi_{\theta}\mid \mathcal{D}_1\big) = 1-\alpha
% \end{equation}
% and thus the inequality~\eqref{eq:upper-bound} is satisfied. The influence function of $\psi_\theta$ relative to $P_\theta$ is well-known and given by
% \begin{align*}
%     D^*_{\theta} := z \mapsto \frac{\alpha + I(\psi_\theta \ge z)-1}{f_\theta(\psi_\theta)}
% \end{align*}
% where $f_\theta(t) := \tfrac{d}{dt} F_\theta(t)$, or the density of $\eta_\theta$ at $\psi_\theta$.

	Now the confidence set is given by 
	\begin{align}
		&\left\{\theta \in \Theta : P_0 (m_\theta-m_{\theta_0})+P_0(m_{\theta_0}-m_{\widehat \theta}) \right.\\
		&\qquad\left.\le -(\mathbb{P}_n-P_0) (m_\theta-m_{\theta_0}+m_{\theta_0}-m_{\widehat \theta}) +\sqrt{\frac{2\widehat \sigma^2_{\theta, \widehat\theta} \log(2/\alpha)}{n}} + \frac{6B_{\theta, \widehat \theta}\log(2/\alpha)}{n}\right\}\\
		& \subseteq \left\{\theta \in \Theta : P_0 (m_\theta-m_{\theta_0})\right.\\
		&\qquad\left.\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0}) +   \sqrt{\frac{2\widehat \sigma^2_{\theta, \theta_0} \log(2/\alpha)}{n}} + \frac{6B_{\theta,  \theta_0}\log(2/\alpha)}{n} + \Gamma_n(\widehat\theta, \theta_0)\right\}\\
		& \subseteq \left\{\theta \in \Theta : \|\theta-\theta_0\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0}) +   \sqrt{\frac{2\widehat \sigma^2_{\theta, \theta_0} \log(2/\alpha)}{n}} + \frac{6B_{\theta,  \theta_0}\log(2/\alpha)}{n} + \Gamma_n(\widehat\theta, \theta_0)\right\}
	\end{align}
	where 
	\[\Gamma_n(\widehat\theta, \theta_0) := \mathbb{P}_n(m_{\widehat \theta}-m_{\theta_0}) +\sqrt{\frac{2\widehat \sigma^2_{\widehat\theta, \theta_0} \log(2/\alpha)}{n}} + \frac{6B_{\widehat\theta,  \theta_0}\log(2/\alpha)}{n}. \]

==> main/concentration.tex <==
\section{Construction of the Confidence Sets}
In Section~\ref{sec:method}, we introduce a general approach for constructing a confidence set for M-estimation problems provided with estimator $\widehat L(\theta, \widehat\theta)$, satisfying the property \eqref{eq:lower-bound}. In this section, we propose several approaches for constructing the corresponding estimator with particular emphasis on non-asymptotic results. In other words, we focus on estimators that satisfy \eqref{eq:lower-bound} for finite $n$, which in turns implies the finite-sample validity of the resulting confidence sets. Throughout, we introduce additional structure to the M-estimation shared by many problems such that $\M(\theta, P_0)$ corresponds to the expectation of some loss function. Formally, we define a measurable function $m_\theta : \mathcal{Z} \mapsto \mathbb{R}$ indexed by $\theta \in \Theta$, and consider the minimization of $m_\theta$ under the expectation of $P_0$ given IID observations such that 
\begin{align*}
    \theta_0 := \argmin_{\theta\in\Theta}\, \int m_\theta(z)\, dP_0(z).
\end{align*}
One way to construct an estimator is to minimize the empirical analogue defined as 
\begin{align*}
    \widehat \theta := \argmin_{\theta\in\Theta}\, \frac{1}{|I_1|}\sum_{i\in I_1} m_\theta(Z_i).
\end{align*}
Although this is a popular choice for an estimator, our framework does not require a particular choice of an initial estimator of $\theta_0$. Given an initial estimator $\widehat\theta$, we denote by $\widehat \eta_\theta(z) := m_{\theta}(z) - m_{\widehat \theta}(z)$ and also define 
\begin{align*}
    \widehat H(\theta) = \int \widehat \eta_\theta(z)\, dP_0(z) \quad \text{ and }\quad  \widehat H_n(\theta) = \frac{1}{|I_2|}\sum_{i \in I_2} \widehat\eta_{\theta}(Z_i).
\end{align*}

\subsection{Confidence sets based on concentration inequalities}
We first propose an estimator of the lower bound based on concentration inequalities. For a random variable $\widehat \eta_\theta$, we assume that the following one-sided concentration inequality can be obtained:
\begin{align*}
    &\mathbb{P}(\widehat H_n(\theta)-\widehat H(\theta) > \varepsilon_{\alpha, \theta} \mid D_1) \le \alpha.
\end{align*}
When such an inequality holds, we can define the lower bound estimator as $\widehat L(\theta; D_2):= \widehat H_n(\theta)-\varepsilon_{\alpha, \theta}$. This estimator satisfies the property \eqref{eq:lower-bound} since 
\begin{align*}
    \mathbb{P}(\widehat H_n(\theta)-\widehat H(\theta) > \varepsilon_{\alpha, \theta} \mid D_1) \le \alpha   & \Longleftrightarrow \mathbb{P}(\widehat H_n(\theta)-\widehat H(\theta) \le \varepsilon_{\alpha, \theta}\mid D_1) \ge 1-\alpha \\
    & \Longleftrightarrow \mathbb{P}(\widehat H(\theta) \ge \widehat H_n(\theta)- \varepsilon_{\alpha, \theta}\mid D_1) \ge 1-\alpha \\
    & \Longleftrightarrow \mathbb{P}(\widehat H(\theta) \ge \widehat L(\theta; D_2)\mid D_1) \ge 1-\alpha 
\end{align*}
Therefore, the corresponding confidence set is given by 
\begin{equation}\label{eq:concentration-ci}
    \widehat{C}_n := \left\{\theta \in \Theta \, : \, \widehat H_n(\theta)\le \varepsilon_{\alpha, \theta}\right\}.
\end{equation}
Alternatively, if one can construct a upper bound $\theta \mapsto U(\theta, \widehat \theta)$ such that $U(\theta_0, \widehat \theta) <0$ then we can shrink the confidence set without compensating for the validity as 
\begin{equation}
    \widehat{C}_n^* := \left\{\theta \in \Theta \, : \, \widehat H_n(\theta)\le \varepsilon_{\alpha, \theta}+\big(0 \wedge U(\theta, \widehat \theta)\big)\right\}.
\end{equation}
\begin{example}[Hoeffding's inequality]
We assume that the loss function is uniformly bounded such that $\|m_\theta\|_\infty \le M$ for all $\theta \in \Theta$. This situation arises for classification problems or regression problems with bounded observations. Since $\widehat H_n(\theta)$ is a sample mean of the bounded random variables $\|\widehat \eta_\theta\|_\infty \le 2M$, it implies by Hoeffding's inequality that 
\begin{align}
	\mathbb{P}(\widehat H_n(\theta)-\widehat H(\theta) > t \mid D_1) \le \exp\left(-\frac{2nt^2}{4M^2}\right)
\end{align}
Solving for $\exp\left(-(2nt^2)/(4M^2)\right)=\alpha$, we obtain the corresponding confidence set as 
\begin{equation}
    \widehat{C}_n := \left\{\theta \in \Theta \, : \, \widehat H_n(\theta)\le M\big(2n^{-1}\ln(1/\alpha)\big)^{1/2}\right\}.
\end{equation}
	
\end{example}


Another approach is to use a Chernoff bound. Suppose there exits a moment-generating function $M(t)$ of a random variable $\widehat H_n(\theta)-\widehat H(\theta)$ in the neighborhood of zero $|t| \le \delta$. A Chernoff bound provide the following one-sided concentration inequality:
\begin{align}
	\mathbb{P}(\widehat H_n(\theta)-\widehat H(\theta) > t \mid D_1) \le \inf_{\lambda \in [0, \delta]} \exp(-\lambda t)M(\lambda),
\end{align}
which we can invert to construct a confidence set.



From the construction \eqref{eq:concentration-ci}, the resulting confidence sets seem similar to the universal inference~\citep{wasserman2020universal}. In what follows, we discuss the similarities and differences between our framework and the universal inference~\citep{wasserman2020universal}.
\begin{example}[Universal inference]
Suppose an observation $Z_1, \ldots, Z_n$ is independent and identically distributed from a density $p_{\theta_0}$ with respect to some base measure $\mu$. Consider the minimization problem 
\begin{align*}
    \theta_0 = \argmin_{\theta \in \Theta} \int m_{\theta}(z) \, dP(z) 
\end{align*}
where $m_{\theta}(z) = -\log p_{\theta}(z)$. Let $\widehat \theta$ be an arbitrary estimator of $\theta_0$ constructed from an independent data set. Then, the universal inference proposes a $(1-\alpha)$-level confidence set of $\theta_0$ defined as 
\begin{align}
	\widehat C_n^{UI} := \left\{\theta : \Theta : \widehat H_n(\theta) \le \log(1/\alpha) \right\}
\end{align}
This seems to coincide with the confidence set in our framework if one can show that
\begin{align}
	\mathbb{P}(\widehat H_n(\theta) - \widehat H(\theta) > \log(1/\alpha) \mid D_1) \le \alpha.
\end{align}
The inequality above is stronger than what \citet{wasserman2020universal} claim since $\widehat H(\theta) < 0$ for any $\theta \in \Theta$, 
\begin{align*}
    \mathbb{P}(\widehat H_n(\theta) > \log(1/\alpha) \mid D_1) \le \mathbb{P}(\widehat H_n(\theta)-\widehat H(\theta) > \log(1/\alpha) \mid D_1).
\end{align*}
\citet{wasserman2020universal} proves 
\begin{align}
	\mathbb{P}(\widehat H_n(\theta) > \log(1/\alpha) \mid D_1) \le \alpha.
\end{align}
The difference in two methods are \citet{wasserman2020universal} provides the lower bound for the empirical mean $\widehat H_n(\theta_0)$, such that 
\begin{equation}
    \mathbb{P}\left( \widehat H_n(\theta_0) \geq \widehat L(\theta_0; D_2) \mid D_1\right) \ge 1-\alpha
\end{equation}
while our framework constructs a lower bound of the population mean $\widehat H(\theta_0)$, such that 
\begin{equation}
    \mathbb{P}\left( \widehat H(\theta_0) \geq \widehat L(\theta_0; D_2) \mid D_1\right) \ge 1-\alpha.
\end{equation}
Hence the universal inference does not immediately imply the validity concerning the minimizer of the population mean, which is the general framework we consider. 
\end{example}


==> main/conclusion.tex <==
\section{Concluding Remarks}\label{sec:conclusions}
This manuscript introduces a general approach to constructing confidence sets for M-estimation, addressing longstanding challenges in statistical inference due to inherent irregularities in these tasks. The proposed method employs sample splitting, facilitating validity across regular and irregular settings. In particular, the method offers a dimension-agnostic solution that is particularly valuable for high-dimensional problems where inferential tools are currently limited or unavailable. The general framework is illustrated through two approaches: one based on concentration inequalities and the other on the central limit theorem (CLT). The manuscript provides foundational theorems for each case that guarantee validity and characterize their convergence rates. 

The theoretical properties of the proposed methods are demonstrated through statistical applications where inference is challenging. The first application considers mean estimation and misspecified linear regression in growing dimensions. The proposed methods remain valid even when the dimension $d$ exceeds $n^{1/2}$, a regime where many existing inferential tools fail. The convergence rates of the proposed method are also dimension-agnostic and match those of the known minimax lower bounds---these properties have been previously established in estimation but have been less known for inference. The second application extends the proposed methods to irregular settings, such as cube-root asymptotic, whose convergence rates are shown to adapt to the underlying geometry of the optimization problem at hand. 

The authors are currently exploring several directions for extending the proposed method. One key area is the constrained optimization problems, where similar irregularities emerge when the solution lies on the boundary of the constrained set. This issue includes problems involving shape constraints and sparsity. In particular, there is a lack of inferential tools for LASSO and Dantzig selectors \citep{candes2007dantzig} despite their widespread use, making the investigation in this area of significant interest. 

Several open problems remain where the proposed methods may be extended. First, inference for generalized linear models in growing dimensions, including logistic regression and Poisson regression, remains underdeveloped. Second, the extension to the Cox proportional hazard model may be interesting. This problem involves nuisance parameters, requiring the optimization in the form of $\M(\theta, \eta, P)$ for some unknown $\eta \in \mathcal{H}$, where $\mathcal{H}$ can be a nonparametric class of functions. Achieving efficiency in estimating $\M(\theta, \eta, P)$ will likely require the first-order bias correction from the estimation error of $\eta$, which is an interesting area to investigate. Third, the manuscript did not focus on optimization problems involving U-statistics or U-quantiles. Given that the CLT for U-statistics is well-established, we anticipate the general framework to be applicable to these problems as well. Finally, this manuscript considered scenarios where the sample size $n$ is fixed and not data-dependent. We envision extending this framework to data-dependent stopping rules, or \emph{anytime-valid} inference, can be achieved when the loss function is equipped with certain concentration properties, such as sub-Gaussian tails \citep{schreuder2020nonasymptotic}. For instance, our framework can be extended to anytime-valid inference for Manski's maximum score estimator where the loss function is bounded. Pursuing these extensions will require considerable additional effort and represent substantial methodological advances.

==> main/intro.tex <==
\section{Introduction}\label{sec:introduction}
% \kt{Come back to this at the end}
% TODO: Mention the following literature
%\begin{itemize}
%    \item M-estimation
%    \item Dimension-agnostic inference \citep{kim2020dimension, wasserman2020universal} and sample-splitting.
%    \item Some optimization literature Arun mentioned to me before \citep{seri2004confidence, vogel2008universal, banholzer2022rates, mak1999monte}.
%    \item Nonparametric confidence sets. Instead of performing ``honest'' inference over sets (statistician chooses), we perform inference on the minimizer/maximizer of some criteria. 
%\end{itemize}
%
%\begin{example}[Random regression function]
%	The observation is an IID sample $(X_1, Y_1) \ldots (X_n, Y_n)$ from a distribution taking values in $\mathcal{X} \times \mathcal{Y}$ where $\mathcal{Y}\subseteq \mathbb{R}$. The data follows the regression model structure such that $y = f_0(X) + \varepsilon$ with $\mathbb{E}[\varepsilon \mid X]=0$ and $\mathbb{E}[\varepsilon^2 \mid X]< \infty$ almost surely. The target of interest can be a squared loss minimizer over a nonparametric function space $\mathcal{F}$ such as 
%	\begin{align}
%		f_* := \argmin_{f\in\mathcal{F}}\, \mathbb{E}\left[(Y-f(X))^2\right]\nonumber
%	\end{align}
%\end{example}
%\begin{example}[Cube-root asymptotics]
%	
%\end{example}
%\begin{example}[Classification]
%	\begin{align}
%		f_* := \argmin_{f\in\mathcal{F}}\, \mathbb{E}\left[1\{Y =f(X)\}\right]\nonumber
%	\end{align}
%\end{example}
The present study examines the inference for the parameter defined as the solution to an optimization problem, commonly referred to as M-estimation, which arises in broad statistical applications. Let $\mathcal{P}$ be a set of probability measures on a measurable space $(\Omega, \mathcal{S})$ with a $\sigma$-algebra $\mathcal{S}$. Let $Z_1, \ldots, Z_n \in \mathcal{Z}$ be a sequence of identically distributed random variables, following an unknown data-generating distribution $P \in\mathcal{P}$. We emphasize that independence is \emph{not} assumed unless explicitly stated otherwise. Given a metric space $(\Theta, \|\cdot\|)$ and a ``criterion'' function $\M: \Theta \times \mathcal{P} \mapsto \mathbb{R}$, the goal of an M-estimation problem is to identify an element $\theta(P) \in \Theta$, which minimizes (or maximizes) the mapping $\theta \mapsto \M(\theta, P)$. Equivalently, the aim is to estimate 
\begin{equation}\label{eq:def-m-functional}
    \theta(P):= \argmin_{\theta \in \Theta}\, \M(\theta, P).
\end{equation}
The uniqueness of the solution has not yet been assumed, and $\theta(P)$ in~\eqref{eq:def-m-functional} denotes the set of minimizers. The primary objective of this manuscript is the construction of an \emph{honest} confidence set for the $P$-dependent minimizer such that 
\begin{equation}\label{eq:def-honest-ci}
    \inf_{P \in \mathcal{P}}\, \mathbb{P}_P (\theta(P) \in \widehat{\mathrm{CI}}_{n,\alpha}) \ge 1-\alpha
\end{equation}
where $\mathbb{P}_P(\cdot)$ denotes the probability of an event under distribution $P$. 

Commonly used confidence set procedures include (1) the Wald methods based on the limiting distribution of a studied estimator, and (2) the resampling approaches. Both methods require an estimator $\widehat{\theta}_n$ such that for a suitable rate of convergence $r_n$, diverging to $\infty$, $r_n(\widehat{\theta}_n - \theta(P))$ converges in distribution. The Wald methods assume a parametric structure on the limiting distribution and use the quantiles of the estimated parametric limiting distribution to construct the confidence sets. The second (resampling) approach non-parametrically estimates the limiting distribution by resampling the available data. From the extensive study of both approaches in the literature, we know of numerous settings in which the corresponding confidence sets might not satisfy the guarantee of honest inference~\eqref{eq:def-honest-ci}. In particular, if the weak convergence of the normalized estimator is not ``continuous'' in $P$, the honest validity guarantee may fail for both Wald and resampling techniques~\citep{Andrews2000, andrews2010asymptotic, cattaneo2020bootstrap, cattaneo2023bootstrap}. An example of such ``continuity'' condition is the regularity of an estimator~\citep[Sec. 8.5]{van2000asymptotic}. We refer to the settings where such ``continuity'' condition fails (or equivalently, the estimator is ill-behaved) as irregular problems. It may be helpful to clarify that we consider cases where the functional $\theta(P)$ or estimator $\widehat{\theta}_n$ considered is ill-behaved to be irregular.

Inference for M-estimation problems that induce non-standard or irregular asymptotics is a particularly active area of research in econometrics \citep{geyer1994asymptotics, Ketz2018,Horowitz2019, Hsieh2022, Li2024}. This list is far from exhaustive. To the best of our knowledge, existing methods typically are tailored to specific classes of regularities. For instance, \citet{Li2024} proposed a general inferential framework for stochastic optimization, allowing for potentially nonsmooth and non-convex objective functions; however, their approach requires knowledge of the estimator's convergence rate, which depends on unknown regularity, and the quantile of a complex random object must be estimated. \citet{vogel2008universal} proposes a method closely related to the one in this manuscript; however, their corresponding confidence set often requires stronger regularity assumptions for validity, particularly, with respect to the complexity of $\Theta$. \cite{dey2024anytime} and \cite{park2023robust} consider inferential procedures based on the sample-splitting; however, they both require stronger assumptions than those in this manuscript for validity. 
% Additionally, a key contribution of this manuscript is the analysis of adaptive convergence rates, which is limited in the references above. Concretely, Theorems~\ref{thm:concentration-width} and \ref{thm:concentration-width-unbounded} establish the convergence rates, which depend on the local properties of the optimization problem near the optimum. These results represent a significant advancement in the field of honest and adaptive inference.

This manuscript proposes a simpler approach to inference based on the defining property of the functional and sample-splitting. Sample-splitting has seen renewed interest in recent times for complicated inference problems in several works~\citep{Robins2006, wasserman2020universal, angelopoulos2023prediction, park2023robust, kim2020dimension, dey2024anytime}. By the defining property, we mean~\eqref{eq:def-m-functional}, which yields the functional as a minimizer of some population quantity. The proposed method at an intuitive level can be derived in two steps as follows: (1) Because $\theta(P)$ minimizes $\theta\mapsto \mathbb{M}(\theta, P)$, we know that $\theta(P)$ is contained in $\{\theta:\, \mathbb{M}(\theta, P) \le \mathbb{M}(\widehat{\theta}, P)\}$ for any $\widehat{\theta}$ in the parameter space; (2) if $\theta\mapsto\widehat{\mathbb{M}}_n(\theta)$ is an estimator of $\mathbb{M}(\theta, P)$, then it is reasonable to expect that $\theta(P)$ would also be contained in $\{\theta:\, \widehat{\mathbb{M}}_n(\theta) \le \widehat{\mathbb{M}}_n(\widehat{\theta}_n) + \gamma_n\}$ for some ``appropriate'' $\gamma_n$. See Section~\ref{sec:method} for a precise description of the proposed method. This idea is not new and can be found, for example, in~\cite{vogel2008universal}. Our contribution to this idea is twofold. We find a dimension/complexity-agnostic and data-driven $\gamma_n$ to provide asymptotic validity; this is made possible by constructing $\widehat{\mathbb{M}}_n(\cdot)$ and $\widehat{\theta}_n$ on two independent datasets. We analyze the width/diameter of the proposed confidence set under mild conditions and prove rate adaptivity in some examples. The conditions we adopt for width analysis are comparable to those employed in studying the convergence rate of the M-estimator.  We believe these results represent a significant advancement in the field of honest and adaptive inference.

% The proposed procedure is summarized as follows: (1) split the data into two parts; (2) use the first half to construct an \emph{arbitrary} estimator $\widehat\theta_1$ of $\theta(P)$; and (3) using the second half, obtain the lower confidence bound $\mathbb{M}(\theta, P) - \mathbb{M}(\widehat\theta_1, P) \ge L_{n,\alpha}(\theta, \widehat \theta_1)$  (see the definition \eqref{eq:lower-bound}). The final confidence set is defined as $\{\theta \in \Theta \, : \, L_{n,\alpha}(\theta, \widehat \theta_1) \le 0\}$. Intuitively, we exclude $\theta$ from the confidence set if it performs statistically ``worse" than the initial estimator $\widehat\theta_1$. 

The proposed approach offers great flexibility and robustness compared to traditional methods of inference. First, the validity of the method is agnostic to the choice of the initial estimator $\widehat\theta_n$, and more importantly, it does not require any guarantees on its convergence rate or the existence of a limiting distribution. Second, our method does not require knowledge of the convergence rate of the estimator. This is a significant improvement over traditional methods because in irregular problems the rate of convergence is impossible to estimate uniformly consistently. Third, it can accommodate constrained parameter spaces or (data-independent) regularization penalties with no additional modifications; this is because our method is based on thresholding the (real-valued) objective function. Note that the limiting distributions of constrained M-estimators can be significantly complicated~\citep{wang1996asymptotics}.

This flexibility and generality come with a price in two aspects. Although we provide conditions under which the proposed confidence set shrinks to a singleton at the optimal rate adaptively, our confidence set can be larger than the traditional ones due to sample splitting. Moreover, the shape of the confidence set is controlled by the shape of the objective function. Unlike traditional methods that control the shape of the confidence set by considering an appropriate statistic, our confidence set can be non-convex or even disconnected depending on the (estimated) objective function. It might be worth pointing out that, in regular cases, our confidence set will approximately be an ellipsoid in similarity to the likelihood ratio confidence set. Furthermore, we note that the universal inference procedure of~\cite{wasserman2020universal} also shares the same drawbacks.

In summary, the confidence set proposed in this manuscript remains valid even in high-dimensional or irregular problems where the standard approach exhibits non-standard asymptotics. The following statistical problems are a few examples in which inference remains difficult to date and the proposed confidence set provides a simple solution.
\begin{enumerate}
    \item \textbf{High-dimensional Linear Regression}: Inference for ordinary least squares (OLS) remains challenging when the dimension $d$ increases with the sample size $n$. In particular, \citet{mammen1993bootstrap} and \citet{cattaneo2019two} establish that the standard OLS estimator has a bias of order $d/n^{1/2}$, resulting in a shortage of valid inferential methods when $d \gg n^{1/2}$. Recently, \citet{cattaneo2019two} and \citet{chang2023inference} have proposed methods based on explicit bias correction, regaining validity in some regimes $d \gg n^{1/2}$; however, these methods still impose some constraints on the growth condition of $d$. Sections~\ref{sec:mean} and \ref{sec:ols} show that our confidence set is asymptotically valid for any growth rate of the dimension with a width tending to zero as long as $d/n\to 0$. 
    \item \textbf{Cube-root Estimators}: Certain families of M-estimation share a common structure known as cube-root asymptotics \citep{kim1990cube}. Notable examples include Manski’s maximum score estimator \citep{manski1975maximum, manski1985semiparametric,horowitz1992smoothed,delgado2001subsampling}, the Grenander estimator \citep{grenander1956theory, sen2010inconsistency, westling2020unified, cattaneo2023bootstrap}, and classification in machine learning \citep{mohammadi2005asymptotics}. In these problems, the M-estimator converges at $n^{-1/3}$ rate whose limit process involves unknown infinite-dimensional objects, making inference difficult. In particular, classical empirical bootstrap is known to be inconsistent for these problems \citep{sen2010inconsistency, patra2018consistent}; \citet{cattaneo2020bootstrap, cattaneo2023bootstrap} recently proposed a modified resampling procedure for cube root problems. Section~\ref{sec:manski} provides new inferential results related to a prototypical example in this class.
    \item \textbf{Non-smooth Objective}: Many common criterion functions in \eqref{eq:def-m-functional} can be written as $\M(\theta, P) \equiv \E_P[m_{\theta}(Z)]$ where $m_{\theta}(Z)$ is often referred to as a ``loss" function. When $\theta \mapsto m_{\theta}$ is non-smooth, the limiting distribution of an estimator can be non-standard unless additional regularity conditions hold \citep{smirnov1952limit, knight1998limiting}. One well-known example is quantile estimation whose limiting distribution depends on the unknown smoothness of the cumulative distribution function (CDF) associated with $P$. While distribution-free finite sample valid confidence intervals exist for the quantiles, we study the behavior of our confidence set in this problem in Section~\ref{sec:quantile}.  
    \item \textbf{Constrained Optimization}: The parameter space $\Theta$ in \eqref{eq:def-m-functional} can incorporate structural constraints, such as sparsity, monotonicity, convexity, and boundedness \citep{ wang1996asymptotics, candes2007dantzig, li2015geometric, royset2020variational}. Confidence sets under such constraints have been explored in the literature \citep{geyer1994asymptotics}, particularly within the operations research literature \citep{vogel2008confidence, vogel2008universal, vogel2017confidence, vogel2019universal}. Our confidence set remains valid under such structural constraints.
\end{enumerate}

Finally, our procedure shares similar goals to \citet{Robins2006}, who developed an adaptive confidence set for a given nonparametric statistical model. Although both methods employ sample-splitting, they differ significantly. First, the parameter of interest in this manuscript is defined as the solution of the optimization problem and does not require the specification of the statistical model. In contrast, the construction in \citet{Robins2006} hinges on quantifying the estimation error $\|\theta-\widehat\theta_n\|$, which depends on the choice of the norm, the statistical model, and involves complex variance estimation based on U-statistics. Furthermore, the nature of adaptation also differs. \citet{Robins2006} focus on the adaptation to submodels within a specified statistical model, whereas our approach considers the instance-specific adaptation, tailored to the local geometry of the optimization landscape around the optimum $\theta(P)$.

The remainder of this manuscript is organized as follows. Section~\ref{sec:method} formally defines the proposed procedure within a general optimization framework. Section~\ref{sec:lowerbounds} establishes the foundational theorems on the validity and width of the proposed confidence set. Section~\ref{sec:application} provides an analysis of the confidence set proposed in statistical applications whose inference has been considered challenging. We end the manuscript with a few concluding remarks in Section~\ref{sec:conclusions}.

\paragraph{Notation.} We adopt the following convention. For two real numbers $a$ and $b$, we set $a \vee b = \max\{a, b\}$ and $a \wedge b = \min\{a, b\}$. For $x \in \mathbb{R}^d$, we write $\|x\|_2 = \sqrt{x^\top x}$. In particular, we define the unit sphere with respect to $\|\cdot\|_2$ such that $\mathbb{S}^{d-1} = \{u \in \mathbb{R}^d \, : \, \|u\|_2 =1\}$. Given a square matrix $A \in \mathbb{R}^{d\times d}$, its trace, the smallest and the largest eigenvalues are denoted by $\mathrm{tr}(A)$, $\lambda_{\min}(A)$ and $\lambda_{\max}(A)$ respectively. For a real-valued function $f : \Omega \mapsto \mathbb{R}$, its supremum norm is denoted by $\|f\|_\infty := \sup_{x \in\Omega}|f(x)|$. A standard indicator function is denoted by $\mathbf{1}\{\cdot\}$, i.e., $\mathbf{1}\{x\in A\} = 1$ if $x\in A$ and $0$ if $x\notin A$. For any deterministic sequences $\{x_n\}_{n \ge 1}$ and $\{r_n\}_{n \ge 1}$, we denote $x_n = O(r_n)$ if there exists a universal constant $C>0$ such that $|x_n| \le C|r_n|$ for all $n$ larger than some $N$. Similarly, we denote $x_n = O_P(r_n)$ if, for any $\varepsilon>0$, there exists a constant $C_\varepsilon>0$ such that $\mathbb{P}(|x_n| \le C_\varepsilon|r_n|) \le \varepsilon$ for all $n$ larger than some $N_\varepsilon$.
We denote $x_n = o(r_n)$ if $x_n/r_n \to 0$ and $x_n = o_p(r_n)$ if $x_n/r_n \overset{p}{\to} 0$ where $\overset{p}{\to}$ denotes convergence in probability.
% \kt{Add motivation below}
% The challenge arises since $\M(\theta, P)$ is often unavailable as it requires the knowledge of $P$. The estimator $\widehat \theta$ of $\theta(P)$ is often obtained as the solution of $\argmin_{\theta \in \Theta}\M_n(\theta, P)$ where $\M_n(\theta, P)$ is an estimator of $\M(\theta, P)$. Heuristically, one hopes this realized optimization problem suitably approximates the original one. The literature has established sufficient conditions for the consistency of the estimator $\widehat \theta$ of $\theta(P)$, its rate of convergence, and its weak convergence to a limiting process. The weak convergence of $\widehat \theta$ can be non-standard---it can be characterized as the $\argmin$ (or $\argmax$) of the stochastic process with a deterministic drift whose convergence rates may involve unknown parameters. Instead of analyzing the limiting behaviors of a particular estimator, such as $\widehat \theta$, we exploit the structure of the functional $P \mapsto \argmin_{\theta \in \Theta} \M(\theta, P)$ to perform the inference. This section outlines a simple procedure for constructing a confidence set for $\theta(P)$ by leveraging the sample splitting. 

% \subsection{Literature review}

==> main/lower-bound.tex <==
\section{Construction of Lower Confidence Bounds}\label{sec:lowerbounds}
Section~\ref{sec:method} establishes that the inference on $\theta(P)$, as defined in \eqref{eq:def-m-functional}, can be reduced to the construction of the upper and lower confidence bounds, satisfying \eqref{eq:lower-bound} and \eqref{eq:upper-bound}. Furthermore, Remark~\ref{remark:the-role-U} suggests that a valid confidence set can be obtained without estimating the upper confidence bound as the upper bound only plays a role in improving the statistical power. Therefore, the primary focus is on constructing the lower confidence bound, which is essential for ensuring validity. This section presents two general approaches for developing the lower confidence bounds.

Throughout, we introduce an additional structure to the M-estimation shared by many problems such that $\M(\theta, P)$ corresponds to the expectation of some ``loss" function. Formally, we define a measurable function $m_\theta : \mathcal{Z} \mapsto \mathbb{R}$ indexed by $\theta \in \Theta$. We consider the minimization of $m_\theta$ under the expectation with respect to $P$ such that 
\begin{align*}
    \theta(P) := \argmin_{\theta\in\Theta}\, \M(\theta, P) = \argmin_{\theta\in\Theta}\, \int m_\theta(z)\, dP(z).
\end{align*}
For example, taking $m_{\theta}(Y,X) := (Y-\theta^\top X)^2$ with $\Theta \equiv \mathbb{R}^d$ corresponds to linear regression while taking $m_{\theta}(Z) := -\log P(Z; \theta)$ for a parametrized family of likelihood functions $P(Z; \theta)$ yields maximum likelihood estimation. This definition arises in many popular situations; however, it does exclude certain classes of M-estimation problems. For example, there are problems when $\M(\theta, P)$ is defined as U-statistics or higher-order U-statistics \citep{bose2018u, diciccio2022clt}, U-quantile \citep{choudhury1988generalized}, and other problems where $\M(\theta, P)$ involves nuisance parameters, such as Cox proportional hazard models \citep{cox1972regression}. Although the general results in Section~\ref{sec:method} still apply to these problems, detailed investigations of these applications are left for future research.

We introduce the definitions and notation that we frequently refer to. For any $n \in \mathbb{N}$ and the identically distributed observation $Z_1, \ldots, Z_n \in D_2$, the empirical measure is defined as $\mathbb{P}_n := n^{-1}\sum_{i=1}^n \delta_{Z_i}$ where $\delta_z$ is the Dirac measure at $z$. For any measure $P$ and $P$-integrable function, we set $Pf = \int f dP$. In particular, $\mathbb{P}_n f$ means $n^{-1} \sum_{i=1}^n f(Z_i)$. The empirical process is defined as the centered and normalized process, which is denoted by $ \mathbb{G}_n f := n^{1/2}(\mathbb{P}_n-P)f$. For notational convenience, we also denote by $\E_P[\cdot]$ the expectation under $P$. Given an arbitrary initial estimator $\widehat\theta_1$, it follows that 
\begin{align*}
    \M(\theta, P)-\M(\widehat \theta_1, P) = P(m_\theta-m_{\widehat{\theta}_1})\quad \mbox{and}\quad
   \M(\theta, \mathbb{P}_n)-\M(\widehat \theta_1, \mathbb{P}_n) = \mathbb{P}_n (m_\theta-m_{\widehat{\theta_1}}).
\end{align*}

\subsection{Construction by concentration inequalities}
As discussed in Section~\ref{sec:method}, we can derive the lower confidence bound by concentration inequalities. In particular, replacing $\M(\theta, P)$ with $P m_{\theta}$ and $\widehat{\mathbb{M}}_n(\theta)$ with $\mathbb{P}_n m_{\theta}$, it suffices to establish the following inequality:
\begin{align*}
    &\mathbb{P}_P\big((\mathbb{P}_n-P)(m_{\theta}-m_{\widehat \theta_1}) > t(\alpha_1, \theta, \widehat \theta_1) \mid D_1\big) \le \alpha_1.
\end{align*}
There is a wide range of concentration inequalities for this purpose. We refer to \citet{Boucheron2013Concentration} for a glossary of classical results and \citet{hao2019bootstrapping, ramdas2023randomized, waudby2024estimating, bates2021distribution} for more recent developments. As an illustration, we may consider the one-sided empirical Bernstein inequality \citep{maurer2009empirical}, established below:
\begin{example}[Empirical Bernstein inequality]\label{prop:bernstein}
Suppose $Z_1, \ldots, Z_n$ are independent and identically distributed (IID) according to $P$, and 
	\begin{align}
		\|m_{\theta_1}-m_{\theta_2}\|_\infty \le  B_0 \quad \mbox{for all} \quad \theta_1, \theta_2 \in \Theta. \label{eq:uniform-boundedness}
	\end{align}
 Denoting the sample variance of $m_{\theta_1}-m_{\theta_2}$ by
	\begin{align}\label{eq:sample-variance}
		\widehat \sigma_{\theta_1, \theta_2}^2 := \frac{1}{n-1}\sum_{i=1}^n \left\{(m_{\theta_1}-m_{\theta_2})(Z_i) - \mathbb{P}_n(m_{\theta_1}-m_{\theta_2})\right\}^2,
	\end{align}
the one-sided empirical Bernstein inequality implies that
	\begin{align}
		\mathbb{P}_P\left((\mathbb{P}_n-P)(m_{\theta(P)}-m_{\widehat \theta_1}) > \sqrt{\frac{2\widehat \sigma^2_{\theta, \widehat\theta_1} \log(2/\alpha_1)}{n}} + \frac{7B_0\log(2/\alpha_1)}{3(n-1)}\mid D_1\right) \le \alpha_1.
	\end{align}
	Hence, the concentration inequality-based confidence set becomes 
	\begin{align}
    &\widehat{\mathrm{CI}}^{\mathrm{E.B.}}_{n,\alpha} \nonumber\\
    &\quad := \left\{\theta \in \Theta \, : \, \mathbb{P}_n(m_{\theta}-m_{\widehat \theta_1})\le \sqrt{\frac{2\widehat \sigma^2_{\theta, \widehat\theta_1} \log(2/\alpha_1)}{n}} + \frac{7B_0\log(2/\alpha_1)}{3(n-1)}+\big(0 \wedge U_{n,\alpha_2}(\theta, \widehat \theta_1; D_2)\big)\right\}.\label{eq:eb-confidence-set-def}
\end{align}
\end{example}
The validity of the confidence set can be established without any additional assumptions, as shown in the following theorem.
\begin{theorem}\label{thm:validity-concentration}
Assume that $Z_1, \ldots, Z_n$ are IID according to $P \in \mathcal{P}$. Suppose \eqref{eq:upper-bound} and~\eqref{eq:uniform-boundedness} hold.
Then for any fixed $n\ge 1$, and $\alpha_1, \alpha_2\in(0, 1)$,
    \begin{align*}
\inf_{P\in\mathcal{P}}\, \mathbb{P}_P(\theta(P) \in \widehat{\mathrm{CI}}^{\mathrm{E.B.}}_{n,\alpha}) \ge 1-\alpha_1-\alpha_2. 
    \end{align*}
\end{theorem}
This theorem is a simple corollary of Theorem~\ref{thm:validity}. The conditional probability $\mathbb{P}_P(\cdot|D_1)$ is replaced by the marginal probability $\mathbb{P}_P(\cdot)$ since the lower bound no longer depends on $D_1$. 

Next, we establish the rate at which the confidence set shrinks. As discussed in Remark~\ref{remark:unique-opt}, the convergence rate of the set requires the uniqueness of the optimizer $\theta(P)$. Below, we assume that $\theta(P)$ is a unique point in $\Theta$ such that the following assumptions hold:
	\begin{enumerate}[label=\textbf{(A\arabic*)},leftmargin=2cm]
    \item \label{as:margin} There exist constants $c_0, \beta \ge 0$ such that 
    % \kt{Let $\mathcal{C} : B(0, 1) \mapsto \mathbb{R}_+$ and $\mathrm{dir}(t):= t\mapsto t/\|t\|$}
    \begin{align*}
        \mathbb{C}_P(\theta) = P (m_\theta - m_{\theta(P)}) \ge c_0\|\theta-\theta(P)\|^{1+\beta}\quad \mbox{for all} \quad \theta \in \Theta.
    \end{align*}
    % \kt{\begin{align*}
    %     \mathbb{C}_P(\theta) = P (m_\theta - m_{\theta(P)}) \ge \mathcal{C}(\mathrm{dir}(\theta-\theta(P)))\|\theta-\theta(P)\|^{1+\beta}\quad \mbox{for all} \quad \theta \in \Theta.
    % \end{align*}}
    % \item \kt{I think we can prove with A1 but only locally} There exists $\delta_0 >0$ such that for all $\|\theta-\theta(P)\|\le \delta_0$, $\E_P (m_\theta - m_{\theta(P)}) \ge \|\theta-\theta(P)\|^{1+\beta}$ for some $\beta \ge 0$.
    \item \label{as:local-entropy}There exists a function $\phi_n : \mathbb{R}_+ \mapsto \mathbb{R}$ such that 
    \begin{align}
    	\left\{\E_P \left[\sup_{\|\theta-\theta(P)\| < \delta}|\mathbb{G}_n (m_\theta - m_{\theta(P)})| \right] \vee \sup_{\|\theta-\theta(P)\| \le \delta }\left(P(m_{\theta}-m_{\theta(P)})^2 \right)^{1/2}\right\}\le  \phi_n(\delta)\label{eq:maximal-inequality}
    \end{align}
    for every $n\ge 1$. Furthermore, $\phi_n(x)/x^q$ is non-increasing for some $q < 1+\beta$.
    % \kt{\begin{align}
    % 	\left\{\E_P \left[\sup_{\|\theta-\theta(P)\| < \delta}|\mathbb{G}_n \frac{m_\theta - m_{\theta(P)}}{\mathcal{C}(\mathrm{dir}(\theta-\theta(P)))}| \right] \vee \sup_{\|\theta-\theta(P)\| \le \delta }\frac{\left(P(m_{\theta}-m_{\theta(P)})^2 \right)^{1/2}}{\mathcal{C}(\mathrm{dir}(\theta-\theta(P)))}\right\}\le  \phi_n(\delta)\label{eq:maximal-inequality}
    % \end{align}}
    % \item \label{as:variance} There exists a function $\nu_n : \mathbb{R}_+ \mapsto \mathbb{R}$ and constant $\tau > 0$ such that  
    % \begin{align}
    % 	\sup_{\|\theta-\theta(P)\| \le \delta_n }\E_P(m_{\theta}-m_{\theta(P)})^2 \le \nu_n^2(\delta_n).
    % \end{align} 
    % for every $n\ge 1$ and $\delta_n \le \tau$. Furthermore, $\nu_n(x)/x^q$ is non-increasing for $q < 2+2\beta$.
    \item \label{as:rate-initial-estimator} 
    For every $n \ge 1$, there exists a random variable $s_n$ such that the initial estimator satisfies
    \begin{align}
        n^{-1/2}\sqrt{P (m_{\widehat\theta_1}-m_{\theta(P)})^2} + \mathbb{C}_P(\widehat{\theta}_1) \le s_n.
    \end{align}
\end{enumerate}
The parameter $\beta$ in \ref{as:margin} links the optimization problem at hand to the curvature within the parameter space. This condition also implies that $\theta(P)$ is a strong global minimizer of $\theta\mapsto\mathbb{M}(\theta, P)$~\citep{drusvyatskiy2013tilt}. The modulus $\phi_n$ in \ref{as:local-entropy} quantifies the complexity of the parameter space $\Theta$ and serves as an upper bound on the variance of the loss function near $\theta(P)$. In particular, the first part of inequality \eqref{eq:maximal-inequality} is known in the literature as the maximal inequality with its upper bound $\phi_n(\cdot)$ reflecting the complexity of $\Theta$. Finally, \ref{as:rate-initial-estimator} pertains to the rate of convergence of the initial estimator. The convergence rate of the proposed confidence set depends on all these terms; such geometric structures are commonly used to establish the convergence rates of M-estimators, as discussed in Theorem 3.2.5 of~\cite{van1996weak}. These conditions are also used in \citet{kim1990cube} in the estimation context to explain the differences between M-estimators in the regular and irregular cases. 
% \kt{
\begin{remark}
   The ``curvature assumption" \ref{as:margin} is stated for all $\theta \in \Theta$. However, in most cases, this holds only locally in some neighborhood of the optimum $\theta(P)$---See Section~\ref{sec:quantile} for a concrete example. Relaxing \ref{as:margin} to its local analog is not trivial. For example, when \ref{as:margin} holds locally and $\Theta$ is unbounded, the conditions above may not be sufficient to claim that the proposed confidence set is bounded. To this end, we envision the use of the naive confidence set $\widehat{\mathrm{CI}}_n^{\dagger}$ in~\eqref{eq:anti-conservative-confidence-set} with a potentially inconsistent $\widehat{\theta}_1$ to first obtain a bounded confidence set and then consider the intersection of $\widehat{\mathrm{CI}}_{n,\alpha}$ with $\widehat{\mathrm{CI}}_n^{\dagger}$ to obtain a provably bounded confidence set. This intersection allows us to weaken assumptions~\ref{as:margin} and~\ref{as:local-entropy} by restricting to a bounded subset of $\Theta$, even if $\Theta$ is unbounded to start with. 
   % The existence of a uniformly bounded confidence set can hold both practical and theoretical significance. Practically, intersecting this bounded confidence set with a potentially unbounded one can prevent trivial results where the confidence set covers all possible parameters. Theoretically, the fact that the confidence set is bounded aids the analysis of the empirical process term based on the so-called peeling devices, as it only needs to consider a finite partition of the parameter space.
\end{remark}


We now establish a bound on the diameter of the confidence set. For any set $A$ equipped with a metric $\|\cdot\|$, the diameter of $A$ is denoted by $\mathrm{Diam}_{\|\cdot\|}(A) := \sup\{\|a-b\|\, :\, a, b\in A\}$. The following theorem provides the high probability bound on the diameter of our confidence set constructed using a concentration inequality-based lower confidence bound.
\begin{theorem}\label{thm:concentration-width}Assume that $Z_1, \ldots, Z_n$ are IID according to $P \in \mathcal{P}$. Assume $\theta(P)$ is a unique solution of \eqref{eq:def-m-functional} that satisfies \ref{as:margin}--\ref{as:rate-initial-estimator}. Given $c_0$ and $\beta$ in \ref{as:margin} and the modulus $\phi_n$ in \ref{as:local-entropy}, we define $r_n$ as any value that satisfies
\begin{align}
    r_n^{-2} \phi_n(c_0^{-1/(1+\beta)}r_n^{2/(1+\beta)}) \le n^{1/2}. \label{rq:define-rn}
\end{align}
Then, for any $n\ge 1$ and $\varepsilon > 0$, there exists a constant $\mathfrak{C}$, depending on $\alpha, \beta, B_0, \varepsilon$ such that 
\begin{align*}
\mathbb{P}_P\left(\mathrm{Diam}_{\|\cdot\|}\big(\widehat{\mathrm{CI}}^{\mathrm{E.B.}}_{n,\alpha}\big)\le \mathfrak{C}c_0^{-1/(1+\beta)}(r_n^{2/(1+\beta)} + (B_0/n)^{1/(1+\beta)} + s_n^{1/(1+\beta)})\right) \ge 1-\varepsilon.
\end{align*}
\end{theorem}
The proof is provided in Section~\ref{sec:proof-concentration-width} of the supplement. In summary, Theorem~\ref{thm:concentration-width} states that the diameter of the set $\widehat{\mathrm{CI}}^{\mathrm{E.B.}}_{n,\alpha}$ depends on four key factors: (1) the curvature of the optimization problem,  (2) the complexity of $\Theta$, (3) the variance of the loss function near $\theta(P)$, and (4) the quality of $\widehat \theta_1$.  


\subsection{Construction by the central limit theorem}\label{sec:clt-based-ci}
This section discusses an alternative approach to construct the lower confidence bound, given by \eqref{eq:lower-bound}, based on the central limit theorem (CLT). Let $\widehat \sigma^{2}_{\theta(P), \widehat\theta_1}$ be the sample variance of $(m_{\theta(P)}-m_{\widehat \theta_1})(Z_i)$, given by \eqref{eq:sample-variance}, and $\Phi(t)$ be the cumulative distribution function of the standard normal random variable. We define the Kolmogorov-Smirnov distance as
\begin{align}\label{eq:be-approximation}
	\Delta_{n,P} := \sup_{t\in\mathbb{R}} \left|\mathbb{P}_P\left(\widehat\sigma^{-1}_{\theta(P), \widehat\theta_1} \mathbb{G}_n(m_{\theta(P)}-m_{\widehat \theta_1})\le t \mid D_1 \right )-\Phi(t)\right|. 
\end{align}
We will shortly discuss the upper bound for $\Delta_{n,P}$ based on the Berry–Esseen bound for studentized statistics \citep{bentkus1996berry, Bentkus1996}. The lower confidence bound is defined as 
\begin{align*}
	L^{\mathrm{CLT}}_{n, \alpha_1}(\theta, \widehat \theta_1; D_2):= \mathbb{P}_n (m_\theta-m_{\widehat{\theta}_1})-n^{-1/2}z_{\alpha_1} \widehat\sigma_{\theta, \widehat\theta_1}
\end{align*}
where $z_{\alpha}$ is the $1-\alpha$-th quantile of a standard normal distribution. The corresponding confidence set is given by 
	\begin{equation}
    \widehat{\mathrm{CI}}^{\mathrm{CLT}}_{n,\alpha} := \left\{\theta \in \Theta \, : \, \mathbb{P}_n(m_{\theta}-m_{\widehat \theta_1})\le n^{-1/2}z_{\alpha_1} \widehat\sigma_{\theta, \widehat\theta_1}+\big(0 \wedge U_{n,\alpha_2}(\theta, \widehat \theta_1; D_2)\right\}.\label{eq:general-set-gaussian}
\end{equation}
The validity of this set follows immediately in view of \eqref{eq:be-approximation} and Theorem~\ref{thm:validity}.
\begin{theorem}\label{thm:vlt-validity-basic}
    Assume that $Z_1, \ldots, Z_n$ are IID according to $P \in \mathcal{P}$. Suppose \eqref{eq:upper-bound}  holds. Then for any fixed $n\ge 1$,
    \begin{align*}
\inf_{P\in\mathcal{P}}\, \mathbb{P}_P(\theta(P) \in \widehat{\mathrm{CI}}^{\mathrm{CLT}}_{n,\alpha}|D_1) \ge 1-\alpha_1-\alpha_2- \sup_{P\in\mathcal{P}}\,\Delta_{n,P}. 
    \end{align*}
\end{theorem}
The proof is provided in Section~\ref{sec:proof-vlt-validity-basic} of the supplement. Comparing two expressions \eqref{eq:eb-confidence-set-def} and \eqref{eq:general-set-gaussian}, we can observe that the CLT-based method always yields a smaller confidence set, since the leading constant for the $n^{-1/2}$ term in~\eqref{eq:eb-confidence-set-def} is $\sqrt{2\log(2/\alpha)} > z_{\alpha}$ for any $\alpha \in (0,1)$. This shows a strong practical advantage of the CLT-based confidence set. However, the CLT-based method compromises the validity for a finite sample size because $\sup_{P\in\mathcal{P}}\Delta_{n,P}$ might at best be close to zero as $n\to\infty$. In the following, we discuss sufficient conditions, based on~\cite{katz1963note}, \cite{bentkus1996berry}, and~\cite{Bentkus1996}, under which $\sup_{P\in\mathcal{P}}\Delta_{n,P}$ converges to zero.
\begin{lemma}\label{prop:clt-valid}Assume $Z_1, \ldots, Z_n$ is IID, generated from $P$. Define a centered random variable 
\begin{align}\label{def:W-rv}
    W_i := m_{\theta(P)}(Z_i)-m_{\widehat \theta_1}(Z_i) - P(m_{\theta(P)} - m_{\widehat \theta_1}) \quad \mbox{for}\quad  1 \le i \le n
\end{align}
and let $B^2 := \E_P[W_1^2|D_1]$. Then  
	% \begin{align}
	% 	\Delta_{n,P} &\le C \left ( \E_P[W_1^2 1\{W_1^2 > nS\}] S^{-1} +  n^{-1/2}\E_P[|W_1|^3 1\{W_1^2 \le  nS\}] S^{-3/2} \right)\label{eq:bentkus-result}
	% \end{align}
 	\begin{align}
		\Delta_{n,P} &\le \min\left\{1, C \E_P\left[\frac{W_1^2}{B^2} \min\left\{1, \frac{|W_1|}{n^{1/2}B}\right\}\bigg| D_1 \right]\right\} \label{eq:bentkus-result}
	\end{align}
	for some universal constant $C > 0$. 
\end{lemma}
This result is a direct consequence of Corollary 1.1 of \cite{bentkus1996berry}. To ensure the validity of the proposal, we require that the right-hand term of \eqref{eq:bentkus-result} converge to zero.
\begin{theorem}\label{thm:validity-BE}
 Assume that $Z_1, \ldots, Z_n$ are IID according to $P \in \mathcal{P}$. Suppose \eqref{eq:upper-bound} holds, and 
 \begin{align}\label{eq:condition-bentkus}
     \sup_{P\in\mathcal{P}}\,\E_P\left[\frac{W_1^2}{B^2} \min\left\{1, \frac{|W_1|}{n^{1/2}B}\right\}\, \bigg| D_1\right] = o_p(1)\quad \text{as $n \longrightarrow \infty$}.
 \end{align}
Then
 \begin{align*}
     \inf_{P \in \mathcal{P}}\, \mathbb{P}_P(\theta(P) \in \widehat{\mathrm{CI}}^{\mathrm{CLT}}_{n,\alpha}) \ge 1-\alpha_1-\alpha_2 - o(1)\quad\mbox{as}\quad n\to\infty.
 \end{align*}
\end{theorem}
This theorem is an immediate consequence of combining Theorem~\ref{thm:vlt-validity-basic} and Lemma~\ref{prop:clt-valid}. In particular, the conditional probability $\mathbb{P}_P(\cdot | D_1)$ can be replaced by the marginal probability $\mathbb{P}_P(\cdot)$ because $\Delta_{n,P}$ can be bounded by the minimum of one and the left-hand side of~\eqref{eq:condition-bentkus}. Section~\ref{sec:uniform-validity-condition} provides a further discussion on condition~\eqref{eq:condition-bentkus}. 

We now establish bounds on the diameter of the CLT-based confidence set. First, we introduce an additional assumption to allow for unbounded loss functions.
\begin{enumerate}[label=\textbf{(A\arabic*)},leftmargin=2cm]\setcounter{enumi}{3}
\item \label{as:square-process} There exists a function $\omega_n : \mathbb{R}_+ \mapsto \mathbb{R}$ such that 
    \begin{align}
    	\E_P \left[\sup_{\|\theta-\theta(P)\| < \delta}|\mathbb{G}_n (m_\theta - m_{\theta(P)})^2| \right]\le  \omega^2_n(\delta)\label{eq:maximal-inequality-2}
    \end{align}
    for every $n\ge 1$. Furthermore, $\omega_n(x)/x^q$ is non-increasing for some $q < 1+\beta$.
\end{enumerate}
Assumption \ref{as:square-process} resembles \ref{as:local-entropy}, but instead, quantifies the growth rate of the expectation of the localized \emph{squared} empirical processes. As $m_{\theta}$ is unbounded, the growth rates of the moduli $\phi_n$ and $\omega_n$ may depend on the concentration properties of $(m_\theta - m_{\theta(P)})(Z_i)$, characterized through, for instance, sub-Weibull tails or the number of the available moments. Such arguments often require specific case-by-case analysis. Following Section 3.2 of \citet{van1996weak}, we present the general result in terms of the growth rate of $\omega_n$, allowing for the theorem to apply without specific conditions on $m_\theta - m_{\theta(P)}$. The theorem is provided as follows:
\begin{theorem}\label{thm:concentration-width-unbounded}
Assume that $Z_1, \ldots, Z_n$ are IID according to $P\in \mathcal{P}$. Assume $\theta(P)$ is a unique solution of \eqref{eq:def-m-functional} that satisfies \ref{as:margin}--\ref{as:square-process}. Given $c_0$ and $\beta$ in \ref{as:margin}, the moduli $\phi_n$ and $\omega_n$ in \ref{as:local-entropy} and \ref{as:square-process}, we define $r_n$ and $u_n$ as any values that satisfy
\begin{align}
    r_n^{-2} \phi_n(c_0^{-1/(1+\beta)}r_n^{2/(1+\beta)}) \le n^{1/2}\quad \text{and} \quad u_n^{-2} \omega_n(c_0^{-1/(1+\beta)}u_n^{2/(1+\beta)}) \le n^{3/4}. \label{rq:define-rn-un}
\end{align}
Then, for any $n\ge 1$ and $\varepsilon > 0$, there exists a constant $\mathfrak{C}$, depending on $\alpha, \beta, \varepsilon$ such that 
\begin{align*}
\mathbb{P}_P\left(\mathrm{Diam}_{\|\cdot\|}\big(\widehat{\mathrm{CI}}^{\mathrm{CLT}}_{n,\alpha}\big)\le \mathfrak{C}c_0^{-1/(1+\beta)}(r_n^{2/(1+\beta)} + u_n^{2/(1+\beta)} +  s_n^{1/(1+\beta)})\right) \ge 1-\varepsilon.
\end{align*}
% % \[\mathbb{P}_P\left(\widehat{\mathrm{CI}}^{\mathrm{E.B.}}_{n,\alpha} \subseteq B_{\|\cdot\|}(\theta(P); \gamma_n)\right) \ge \varepsilon \quad \mbox{with probability greater than } 1-\varepsilon.\]
% where
% % \begin{align}
% % 	\gamma_n := \mathfrak{C}\left(r_n^{2/(1+\beta)} \vee n^{-1/(2+2\beta-\nu)}\vee n^{-1/(1+\beta)} \vee \Gamma^{1/(1+\beta)}_n(\widehat\theta, \theta(P))\right) \quad \mbox{and}
% % 	\end{align}
%  \begin{align}
% 	\gamma_n := \left(r_n^{2/(1+\beta)} + n^{-1/(2+2\beta-\nu)}+ n^{-1/(1+\beta)} +(n^{-1/2}s_n^{-\nu/2} )^{1/(1+\beta)}\right).
% 	\end{align}
\end{theorem}
The proof is provided in Section~\ref{sec:proof-concentration-width-unbounded} of the supplement.
\begin{remark}
The CLT-based confidence set remains useful even when $m_{\theta}$ is uniformly bounded. In such cases, Theorem~\ref{thm:concentration-width-unbounded} yields the same rate as Theorem~\ref{thm:concentration-width} since we can simply take $\omega_n = \phi_n$ using the contraction inequality (Theorem 4.12 of \citet{ledoux2013probability}). Although the rates are identical, the validity must be verified since there exist uniformly bounded random variables for which the CLT does not hold. A classical example is when $W_1, \ldots, W_n$ are IID Bernoulli random variables with success probability $p$ such that $np\longrightarrow \lambda$. In this case, the condition \eqref{eq:bentkus-result} fails.
\end{remark}
\begin{remark}
    While it is common to impose light-tail assumptions, such as the sub-Gaussian tail for $m_{\theta}-m_{\theta(P)}$, to obtain $\omega_n$ for unbounded processes, Lemma~\ref{lemma:moment-bounds} in Section~\ref{sec:technical-lemma} of the supplement offers general construction of $\omega_n$ under much weaker assumptions. This is achieved through a truncation argument, which is a proof device frequently employed in the literature. See similar results, for instance, Proposition 3.1 of \citet{gine2000exponential} and Proposition B.1 of \citet{kuchibhotla2022least}.
\end{remark}

\subsection{On the validity of the CLT-based method}\label{sec:uniform-validity-condition}
Section~\ref{sec:clt-based-ci} outlines the construction of the confidence set based on the CLT whose (asymptotic) validity is guaranteed so long as the Gaussian approximation tends to zero as $n \longrightarrow \infty$. 
% Theorem~\ref{thm:validity-BE} and the conditions therein only provide the validity statement conditioning on $D_1$. It is, however, impractical to assume $D_1$ to be fixed for statistical purposes. See Figure 2 in \citet{kim2020dimension} for a visual illustration. 
Verification of~\eqref{eq:condition-bentkus} can be difficult when $\widehat{\theta}_1$ is consistent for $\theta(P)$ because the variance $B^2$ in Lemma~\ref{prop:clt-valid} converges to zero under consistency of $\widehat{\theta}_1$.
This section provides sufficient conditions for the validity to hold. The results of this section are frequently used in the statistical applications presented in
Section~\ref{sec:application}. 

For any real-valued random variable $X$, we write $\|X\|_p = (\mathbb{E}[|X|^p])^{1/p}$ for any $p > 0$.
\begin{definition}[Uniform Lindeberg condition]
    A distribution $Q$ supported on (a subset of) $\mathbb{R}^d, d\ge1$ is said to satisfy the {\em uniform Lindeberg condition} (ULC) if a random variable $H\sim Q$  satisfies  
    \begin{align}
        \lim_{\kappa \to \infty}\, \sup_{t \in \mathbb{R}^d}\,  \E\left[\frac{\langle t, H \rangle^2}{\|\langle t, H \rangle\|_{2}^2} \min\left\{1, \frac{|\langle t, H \rangle|}{\kappa \|\langle t, H \rangle\|_{2}}\right\}\right]  = 0.
    \end{align}
    In particular, a class of distributions $\mathcal{Q}$ is said to satisfy the ULC if   
    \label{eq:validity-condition-clt}
     \begin{align}
        \lim_{\kappa \to \infty}\,\sup_{Q\in\mathcal{Q}}\, \sup_{t \in \mathbb{R}^d}\,  \E_Q\left[\frac{\langle t, H \rangle^2}{\|\langle t, H \rangle\|_{2}^2} \min\left\{1, \frac{|\langle t,H\rangle|}{\kappa \|\langle t, H \rangle\|_{2}}\right\}\right]  = 0.
    \end{align}
\end{definition}
% We emphasize that both supremums are taken outside of the expectation. 
Importantly, the uniform Lindeberg condition does not require strong moment assumptions on $Q$ such as the finite third moments.
% Recalling Lemma~\ref{prop:clt-valid}, we need to verify the upper bound on the corresponding object in terms of the random variable $W \in \mathbb{R}$ defined as \eqref{def:W-rv}.
The proposition below provides the first-order approximation result, which becomes useful for many statistical applications. 
\begin{proposition}\label{prop:first-order-linearization}
    Suppose that there exists a $\delta_0 > 0$ and a $P$-dependent\footnote{We mean that the distribution of $H_i$ depends on $P$.} mean-zero random variable/vector $H_i$ such that
       \begin{align}
    	\frac{\E_P[W_1- \langle  \theta - \theta(P), H_1 \rangle ]^2}{\E_P[\langle  \theta - \theta(P), H_1 \rangle^2]} \le  \varphi(\|\theta - \theta(P)\|) \quad \text{for all} \quad \|\theta - \theta(P)\| < \delta_0\label{eq:qmd2}
    \end{align}
    where $\varphi:\mathbb{R}_+\to\mathbb{R}_+$ is continuous and $\varphi(0) = 0$. Then, for any $P\in\mathcal{P}$,
    \begin{align*}
        \E_P\left[\frac{W_1^2}{B^2} \min\left\{1, \frac{|W_1|}{n^{1/2}B}\right\}\right] &\lesssim  \inf_{\delta < \delta_0}\left\{\varphi(\delta) + \varphi^{1/2}(\delta) + \mathbb{P}_P(\|\widehat\theta_1 - \theta(P)\| > \delta)\right\}\\
        &\quad +  \sup_{t \in \mathbb{R}^d}\,\E_P\left[\frac{\langle  t, H_1 \rangle^2}{\|\langle t, H_1 \rangle\|_{2}^2} \min\left\{1, \frac{|\langle  t, H_1 \rangle|}{n^{1/2}\|\langle t, H_1 \rangle\|_{2}}\right\}\right]
    \end{align*}
where $B^2 = \E_P[W^2_1|D_1]$. In particular, if $\widehat{\theta}_1$ is uniformly (in $P\in\mathcal{P}$) consistent for $\theta(P)$ and $H$ satisfies ULC uniformly over $P\in\mathcal{P}$, then the left hand side converges to zero as $n\to\infty$.
\end{proposition}
The proof is provided in Section~\ref{sec:proof-first-order-linearization} of the supplement. Intuitively, the random variable $H_1$ serves as the gradient of $W_1$ with respect to $\theta$ (evaluated at $\theta(P)$) so that $W_1 \approx \langle  \theta - \theta(P), H_1 \rangle$. The approximation defined in \eqref{eq:qmd2} is a quantitative version of the quadratic mean differentiability~\citep[Lemma 3.2.19]{van1996weak}, which is weaker than the pointwise differentiability. The role of the uniform Lindeberg condition is clearer in this context: when the first-order approximation in the sense of \eqref{eq:qmd2} is available, it suffices to verify the uniform Lindeberg condition for the random sequence $\{H_i\}_{i=1}^n$ instead of directly inspecting $\{W_i\}_{i=1}^n$. The upper bound of this proposition no longer involves conditioning on $D_1$, but instead, requires the consistency of the initial estimator $\widehat \theta_1$. Although this aspect may be stringent compared to the confidence set based on concentration inequalities, which remained valid even when $\widehat\theta_1$ is not consistent, such consistency is not a necessary condition for the validity of the CLT-based confidence sets---see Remark~\ref{remark:consistency} in this regard. The following proposition provides sufficient conditions under which uniform Lindeberg condition is satisfied. 
\begin{definition}[$L_{2+\delta}$-$L_2$ norm equivalence]\label{as:l4-l2}
    A mean-zero random variable/vector $H$ satisfies the uniform $L_{2+\delta}$-$L_2$ norm equivalence with a constant $L \ge 1$ if 
\begin{align}
    \sup_{P \in \mathcal{P}}\,\sup_{t \in \mathbb{R}^d}\, \frac{\|\langle t, H \rangle\|_{2+\delta}}{\|\langle t, H \rangle\|_{2}} \le L \quad \text{for some} \quad \delta \in (0,1].\label{eq:norm-equivalence-def}
\end{align}
\end{definition}
\begin{definition}[Uniform integrability under standardization]\label{as:unifrom-integrable}
    A mean-zero random variable/vector $H$ is uniformly integrable under standardization if it satisfies
\begin{align}
   \lim_{\kappa \to \infty}\, \sup_{P \in \mathcal{P}}\,\sup_{t \in \mathbb{R}^d}\,\E_P\left[\frac{\langle t, H\rangle^2}{\|\langle t, H \rangle\|_{2}^2}\mathbf{1}\left\{\frac{\langle t, H\rangle^2}{\|\langle t, H \rangle\|_{2}^2} > \kappa \right\}\right] \longrightarrow 0.\label{eq:unif-integrable-def}
\end{align}
\end{definition}
\begin{proposition}\label{prop:suff-cond-for-CLT}
    The following statement holds:
    \begin{align*}
        \eqref{eq:norm-equivalence-def} \Longrightarrow \eqref{eq:unif-integrable-def} \Longrightarrow \mathrm{Uniform \, Lindeberg \, condition}.
    \end{align*}
\end{proposition}

Proposition~\ref{prop:suff-cond-for-CLT} is standard in the CLT literature, and for the reader's convenience, we provide proof in Section~\ref{sec:proof-suff-cond-for-CLT} of the supplement.

\begin{remark}[On $L_{2+\delta}$-$L_2$ norm equivalence assumption]\label{remark:norm-equiv}The $L_{2+\delta}$-$L_2$ norm equivalence, with a particular emphasis on $\delta=2$, is a widely employed structure in the literature of high-dimensional covariance matrix estimation \citep{minsker2018sub, mendelson2020robust} and high-dimensional least squares \citep{oliveira2016lower, catoni2016pac, mourtada2022distribution}. 
This assumption is considerably less restrictive than imposing the
sub-Gaussianity of $X$ since any such $X$ satisfies the $L_{2+\delta}$-$L_2$ norm equivalence with $\delta\ge2$. Remarks 2.19, 2.20 and Figure S.7 of \cite{patil2022mitigating} provide useful discussion and visual comparison of different norm equivalence assumptions. 
\end{remark}

\begin{remark}[On consistency of the initial estimator]\label{remark:consistency}
    Proposition~\ref{prop:first-order-linearization} establishes the validity of the confidence set in terms of the assumption on $H$, which is often easily verified in many statistical problems. This is achieved by requiring the consistency of the initial estimator. However, the existence of such an estimator may be harder to establish depending on the specific problem at hand \citep{royset2020variational}. Importantly, we emphasize that the consistency of the estimator, even for some applications provided below, is not necessary. This requirement can be relaxed under alternative assumptions on the data-generating distribution that may be slightly more difficult to verify. 
    % As alternative evidence, we provide the existence of the conservative confidence set when the initial estimator may be inconsistent in Section~\ref{sec:bounded-set} of the supplement. Combining such a confidence set with the proposed set may regain validity under the inconsistent initial estimator.
\end{remark}

==> main/method.tex <==
\section{Construction of the Confidence Set}\label{sec:method}
%In the following, we suppress the dependency of $\M$ on $P$ from its notation when it is clear from the context.
% As $\M$ is often unknown, we obtain an estimator $\widehat \theta_1_n$ of $\theta(P)$, which minimizes $\theta$ over a stochastic process $\M_n(\theta)$ instead. This task is formalized as the following optimization problem: 
% \begin{align*}
% \theta(P) := \argmin_{\theta \in \Theta} \M(\theta)\quad \text{and}\quad
% \widehat\theta_n := \argmin_{\theta \in \Theta} \M_n(\theta; Z_1, \ldots, Z_n)
% \end{align*}
% where $Z_1, \ldots, Z_n$ is a sequence of random variables that take values in a measurable space $(\mathcal{Z}, \mathcal{S})$ with a $\sigma$-algebla $\mathcal{S}$. The observations $Z_1, \ldots, Z_n$ do not need to be independent or identically distributed.
% The parameter $\theta(P)$ is a global minimizer of the program with respect to the unknown criterion. As the limiting criterion mapping is typically not available, the optimization seeks to minimize a random function $\theta \mapsto \M_n(\theta)$. 

% Many statistical applications consider the following special case of the optimization program described above. Let a random variable $Z$ take a value in a measurable space $(\mathcal{Z}, \mathcal{S})$ with a $\sigma$-algebla $\mathcal{S}$. Let $Z_1, \ldots, Z_n$ be a sequence of observed random variables following unknown data-generating distribution $P$. For each $\theta \in \Theta$, we define a criterion function $m_\theta : \mathcal{Z} \mapsto \mathbb{R}$, and the corresponding M-estimation is defined as
% \begin{align*}
% \theta(P) := \argmin_{\theta \in \Theta} \int m_\theta(z)\, dP(z) \quad \text{and}\quad
% \widehat\theta := \argmin_{\theta \in \Theta} \frac{1}{n}\sum_{i=1}^n m_\theta(Z_i).
% \end{align*}
% where $\E_0$ denotes the expectation under $P$. Notable examples of this framework are the maximum likelihood estimators and the ordinary least squares estimators.
Given an identically, but not necessarily independently, distributed observation $Z_1, \ldots, Z_N$, we construct two sets of observations $D_1:= \{Z_i: i \in \mathcal{I}_1\}$ and $D_2:= \{Z_i : i \in \mathcal{I}_2\}$, where $\mathcal{I}_1$ and $\mathcal{I}_2$ are the disjoint partitions of $\{1, \ldots, N\}$. First, we construct \textit{any} estimator of $\theta(P)$ using $D_1$, defining $\widehat \theta_1 := \widehat \theta_1(D_1) \in \Theta$. We use the first data only to obtain an initial estimator and remain agnostic to the choice of $\widehat \theta_1$. Given this estimator $\widehat \theta_1$, we construct a confidence set using the second data $D_2$. Throughout the manuscript, we denote by $n$ the cardinality of $D_2$ as we primarily use $D_2$ for the inferential task.

As stated in Section~\ref{sec:introduction}, our confidence set is based on the defining property of $\theta(P)$. Our ideal (unactionable) confidence set is 
\[
\widetilde{\mathrm{CI}} := \left\{\theta\in\Theta:\, \mathbb{M}(\theta, P) - \mathbb{M}(\widehat{\theta}_1, P) \le 0\right\}.
\]
From this, it might be tempting to consider the set
\begin{equation}\label{eq:anti-conservative-confidence-set}
\widehat{\mathrm{CI}}^\dagger_{n} := \left\{\theta\in\Theta:\, \widehat{\mathbb{M}}_n(\theta) - \widehat{\mathbb{M}}_n(\widehat{\theta}_1) \le 0\right\},
\end{equation}
where $\theta\mapsto\widehat{\mathbb{M}}_n(\theta)$ is an estimator of $\mathbb{M}(\theta, P)$ based on $D_2$. If $\widehat{\theta}_1$ is consistent for $\theta(P)$, then the confidence set in~\eqref{eq:anti-conservative-confidence-set} may not have valid coverage, and if $\widehat{\theta}_1$ is not consistent for $\theta(P)$, then this confidence set may not shrink to a singleton as the sample size increases. Nevertheless, we can prove the following result on the coverage validity of the confidence set in~\eqref{eq:anti-conservative-confidence-set}, and this can be useful to find a ``small'' set that contains $\theta(P)$. To state the result, for any $\theta, \theta'\in\Theta$, consider
\begin{equation}\label{eq:notation-MSE-curvature}
    \begin{split}
        \mathbb{V}_P(\theta, \theta') ~&:=~ \mathbb{E}_P[|(\widehat{\mathbb{M}}_n - \mathbb{M})(\theta) - (\widehat{\mathbb{M}}_n - \mathbb{M})(\theta')|^2] \quad\mbox{and}\\
        \mathbb{C}_P(\theta) ~&:=~ \mathbb{M}(\theta, P) - \mathbb{M}(\theta(P), P).
    \end{split}
\end{equation}
The quantity $\mathbb{C}_P(\theta)$ represents the curvature of the M-estimation problem. It quantifies the hardness of ``estimating'' $\theta(P)$. Note that $\mathbb{V}_P(\theta, \theta')$ and $\mathbb{C}_P(\theta)$ are defined for non-stochastic $\theta, \theta'\in\Theta$ and if evaluated at a random point $\widehat{\theta}_1\in\Theta$, these should be considered as random variables.
\begin{theorem}\label{thm:coverage-anti-conservative-confidence-set}
    For any initial estimator $\widehat{\theta}_1$ computed on $D_1$, and any estimator $\widehat{\mathbb{M}}_n(\cdot)$ of $\mathbb{M}(\cdot, P)$ computed on $D_2$, we have
    \[
    \mathbb{P}_P\left(\theta(P) \notin \widehat{\mathrm{CI}}_{n}^{\dagger}\right) ~\le~ \mathbb{E}_P\left[\frac{\mathbb{V}_P(\theta(P), \widehat{\theta}_1)}{\mathbb{V}_P(\theta(P), \widehat{\theta}_1) + \mathbb{C}_P^2(\widehat{\theta}_1)}\right] \le 1.
    \]
    In particular, if $\mathbb{V}_P(\theta(P), \widehat{\theta}_1)/\mathbb{C}_P^2(\widehat{\theta}_1) = o_p(1)$ uniformly over all $P\in\mathcal{P}$, then $\widehat{\mathrm{CI}}_n^{\dagger}$ is an asymptotically uniformly valid confidence interval of confidence 1. 
\end{theorem}
The proof of Theorem~\ref{thm:coverage-anti-conservative-confidence-set} is provided in Section~\ref{appsec:proof-of-coverage-anti-conservative} and is based on Cantelli's inequality~\citep{pinelis2010between}. Observe that uniqueness of $\theta(P)$ is not required in Theorem~\ref{thm:coverage-anti-conservative-confidence-set}. Moreover, the miscoverage bound depends naturally on two aspects of the M-estimation problem: (1) the estimation error of $\widehat{\mathbb{M}}_n(\cdot)$ captured by the mean squared error $\mathbb{V}_P(\cdot, \cdot)$; and (2) the curvature of the problem $\mathbb{C}_P(\cdot)$. Note that, by the definition of $\theta(P)$, $\mathbb{C}_P(\theta) \ge 0$ for all $\theta\in\Theta$. The miscoverage bound is non-decreasing in the estimation error and non-increasing in the curvature of the problem. Because the definition of the confidence set does not depend on any target coverage, the confidence set provides an agnostic bound. To understand the behavior of the miscoverage bound, consider the case when $\mathbb{M}(\theta, P) = \mathbb{E}_P[m_{\theta}(Z)]$ for a loss function $m_{\theta}(Z)$ and $\widehat{\mathbb{M}}_n(\theta) = \sum_{i=1}^n m_{\theta}(Z_i)/n$, $\mathbb{V}_P(\theta, \theta') = \mbox{Var}(m_{\theta}(Z) - m_{\theta'}(Z))/n$. If $n\mathbb{C}_P^2(\widehat{\theta}_1)$ diverges to infinity in probability, while $\mbox{Var}(m_{\theta}(Z) - m_{\widehat{\theta}_1}(Z)|\widehat{\theta}_1)$ is bounded away from zero as $n\to\infty$, then the confidence set in~\eqref{eq:anti-conservative-confidence-set} has an asymptotic confidence of 1. For the special case of loss functions satisfying the so-called Bernstein condition~\citep[Def. 2.6]{bartlett2006empirical} with parameters $(\beta, B)$ with $\beta\in(0, 1]$, i.e., $\mathbb{E}_P[(m_{\theta}(Z) - m_{\theta(P)}(Z))^2] \le B(\mathbb{C}_P(\theta))^{\beta}$, this divergence condition is satisfied if $(n/B)^{1/(2-\beta)}\mathbb{C}_P(\widehat{\theta}_1)$ diverges to infinity in probability as $n\to\infty.$ Note that this divergence condition can be trivially satisfied by taking an inconsistent estimator $\widehat{\theta}_1$ of $\theta(P)$, and the resulting confidence set would be a (non-shrinking) bounded set, in most cases. 

For finer control on the coverage guarantee, we modify the confidence set in~\eqref{eq:anti-conservative-confidence-set} as follows. 
% Our procedure is based on the following idea: rather than analyzing the limiting behavior of $\widehat \theta_1$, inference can be performed by directly constructing the lower confidence bound of $\M(\theta(P), P) - \M(\widehat \theta_1, P)$. Denoting the lower bound of $\theta \mapsto \M(\theta, P) - \M(\widehat \theta_1, P)$ by $\theta \mapsto L(\theta, \widehat \theta_1)$, the definition of M-estimation as the minimizer implies the following:
% \begin{align}
% 	\M(\theta(P), P) - \M(\widehat \theta_1, P) \le 0\,  \Longrightarrow L(\theta(P), \widehat \theta_1) \le 0, \quad \mbox{for all}\quad  \widehat \theta_1 \in \Theta \quad \mbox{almost surely}.
% \end{align}
% Hence, the preimage of $\{L(\theta, \widehat \theta_1)\le 0\}$ under the mapping $\theta \mapsto L(\theta, \widehat \theta_1)$ contains $\theta(P)$ with probability one. In order to satisfy the definition \eqref{eq:def-honest-ci}, we only need the probabilistic lower bound $\widehat L(\theta, \widehat \theta_1)$ such that 
% \[\M(\theta(P), P) - \M(\widehat \theta_1, P) \ge \widehat L(\theta(P), \widehat \theta_1) \quad \mbox{with probability greater than}\quad  1-\alpha.\]
% In other words, we need to construct the lower confidence bound of $\M(\theta(P), P) - \M(\widehat \theta_1, P)$. 
Define random mappings $\theta \mapsto L_{n,\alpha_1}(\theta, \widehat \theta_1; D_2)$ and $\theta \mapsto U_{n,\alpha_2}(\theta, \widehat \theta_1; D_2)$ based on the dataset $D_2$, satisfying the following properties:
\begin{align}\label{eq:lower-bound}
	\inf_{P\in\mathcal{P}}\, \mathbb{P}_{P}\left( -\mathbb{C}_P(\widehat{\theta}_1) \geq L_{n,\alpha_1}(\theta(P), \widehat \theta_1; D_2) \mid D_1 \, \right)\ge 1-\alpha_1
\end{align} 
and
\begin{align}\label{eq:upper-bound}
	\inf_{P\in\mathcal{P}}\,\mathbb{P}_{P}\left( -\mathbb{C}_P(\widehat{\theta}_1) \le  U_{n,\alpha_2}(\theta(P), \widehat \theta_1; D_2) \mid D_1\, \right)\ge 1-\alpha_2
\end{align} 
for any $n\ge 1$ and $\alpha_1, \alpha_2 \in (0,1)$. The final confidence set for $\theta(P)$ is defined as:
\begin{equation}\label{eq:confidence-set}
    \widehat{\mathrm{CI}}_{n,\alpha} := \left\{\theta \in \Theta \, : \,  L_{n,\alpha_1}(\theta, \widehat \theta_1; D_2) \le (0 \wedge U_{n,\alpha_2}(\theta, \widehat \theta_1; D_2))\right\}
\end{equation}
where $\alpha := (\alpha_1, \alpha_2)$. In particular, if $\alpha_2 = 0$, then $U_{n,\alpha_2}(\theta(P), \widehat{\theta}_1; D_2)$ can be taken to be zero because the definition of $\theta(P)$ implies $-\mathbb{C}_P(\widehat{\theta}_1) \le 0$ almost surely, and this yields
\begin{equation}\label{eq:CI-without-upper-bound}
\widehat{\mathrm{CI}}_{n,\alpha} := \left\{\theta\in\Theta:\, L_{n,\alpha}(\theta, \widehat{\theta}_1; D_2) \le 0\right\}.
\end{equation}
The following theorem establishes the validity guarantee for the proposed confidence set. 
\begin{theorem}\label{thm:validity}
    Fix $n\ge1$, and assume \eqref{eq:lower-bound} and \eqref{eq:upper-bound} to hold. Then, 
    \begin{align*}
\inf_{P\in\mathcal{P}}\, \mathbb{P}_P(\theta(P) \in \widehat{\mathrm{CI}}_{n,\alpha} \mid D_1) \ge 1-\alpha_1-\alpha_2. 
    \end{align*}
\end{theorem}
The proof of Theorem~\ref{thm:validity} can be found in Section~\ref{appsec:proof-of-validity}. In situations where constructing a confidence set for $\theta(P)$ seems challenging, it may initially appear puzzling that our proposed approach involves building a (lower) confidence bound for $-\mathbb{C}_P(\widehat{\theta}_1) = \mathbb{M}(\theta(P), P) - \mathbb{M}(\widehat{\theta}_1, P)$. However, recognizing that the confidence set~\eqref{eq:confidence-set} relies on the random mapping $\theta \mapsto L_{n,\alpha_1}(\theta, \widehat{\theta}_1; D_2)$, it is helpful to reinterpret condition~\eqref{eq:lower-bound} as
\begin{equation}\label{eq:reinterpret-lower-upper}
    \begin{split}
        \inf_{P\in\mathcal{P}}\,\inf_{\theta,\theta'\in\Theta}\,\mathbb{P}_P\big(\mathbb{M}(\theta, P) - \mathbb{M}(\theta', P) \ge L_{n,\alpha_1}(\theta, \theta'; D_2)\,\big|\,D_1\big) \ge 1-\alpha_1.
    % \inf_{P\in\mathcal{P}}\,\inf_{\theta,\theta'\in\Theta}\,\mathbb{P}_P\big(\mathbb{M}(\theta, P) - \mathbb{M}(\theta', P) \le U_{n,\alpha_2}(\theta, \theta'; D_2)\,\big|\,D_1\big) \ge 1-\alpha_2.
    \end{split}
\end{equation}
In other words, we need to construct a lower confidence bound for $\mathbb{M}(\theta, P) - \mathbb{M}(\theta', P)$ for every (non-stochastic) pair $\theta, \theta'\in\Theta$. For instance, if $\mathbb{M}(\theta, P) = \mathbb{E}_P[m_{\theta}(Z)]$, then $\mathbb{M}(\theta, P) - \mathbb{M}(\theta', P) = \mathbb{E}_P[m_{\theta}(Z) - m_{\theta'}(Z)]$ for which lower confidence bound can be constructed by the central limit theorem.
Because the mapping $\theta \mapsto \M(\theta, P) - \M(\widehat \theta_1, P)$ is always real-valued regardless of the complexity of $\Theta$, it is conceivable that the lower confidence limit in~\eqref{eq:reinterpret-lower-upper} can be constructed without any reference to the complexity of $\Theta$. This is in stark contrast to the ``classical'' inferential approach based on the weak convergence of $r_n(\widehat \theta_1-\theta(P))$ to some limit process, which often depends heavily on the complexity of $\Theta$. 

Comparing the definitions of $\widehat{\mathrm{CI}}_{n}^{\dagger}$ in~\eqref{eq:anti-conservative-confidence-set} and $\widehat{\mathrm{CI}}_{n,\alpha}$ in~\eqref{eq:confidence-set}, one can interpret the naive confidence set in~\eqref{eq:anti-conservative-confidence-set} as using the estimator $\widehat{\mathbb{M}}_n(\theta) - \widehat{\mathbb{M}}_n(\widehat{\theta}_1)$ as $L_{n,\alpha}(\theta, \widehat{\theta}_1; D_2)$. This, in general, does not satisfy the guarantee~\eqref{eq:lower-bound}. In the following section, we consider two methods for constructing lower confidence bounds satisfying~\eqref{eq:lower-bound}: one based on concentration inequalities under the assumption of bounded loss function and the other based on central limit theorem. Both lower bounds are of the form
\[
L_{n,\alpha}(\theta, \widehat{\theta}_1; D_2) = \widehat{\mathbb{M}}_n(\theta) - \widehat{\mathbb{M}}_n(\widehat{\theta}_1) - t(\alpha, \theta, \theta'),
\]
for some non-negative function $t(\cdot, \cdot, \cdot)$. With such non-negativity, it is clear that $\widehat{\mathrm{CI}}_{n,\alpha} \supseteq \widehat{\mathrm{CI}}_{n}^{\dagger}$.

% The remainder of this manuscript centers around the constructions of lower confidence bounds  \eqref{eq:lower-bound}. We provide the first example based on concentration inequalities. Let $\mathbb{M}_n(\theta; D_2)$ be an estimator of $\mathbb{M}(\theta, P)$ based on $D_2$, satisfying:
% \begin{align}
%     &\mathbb{P}_P\big(\{\mathbb{M}_n(\theta; D_2)-\mathbb{M}_n(\widehat\theta_1; D_2)\}-\{\mathbb{M}(\theta, P)-\mathbb{M}(\widehat\theta_1, P)\} > t(\alpha_1, \theta, \widehat \theta_1) \mid D_1\big) \le \alpha_1 \label{eq:concentraion-inequality} 
% \end{align}
% where $t(\alpha_1, \theta, \widehat \theta_1)$ is a constant depending on $\alpha_1, \theta$ and $\widehat \theta_1$. Once this concentration inequality is established, we can define the lower confidence bound as 
% \begin{align*}
% 	L^{\mathrm{C.E.}}_{n,\alpha_1}(\theta, \widehat \theta_1; D_2):= \mathbb{M}_n(\theta; D_2)-\mathbb{M}_n(\widehat\theta_1; D_2)-t(\alpha_1, \theta, \widehat \theta_1).
% \end{align*}
% It may be instructive to verify the condition \eqref{eq:lower-bound}. We introduce the short-hand notation $\mathbb{M}_n(\theta) \equiv \mathbb{M}_n(\theta; D_2)$ and $\mathbb{M}_P(\theta)\equiv \mathbb{M}(\theta, P)$. It then follows 
% \begin{align*}
%     &\mathbb{P}_P(\{\mathbb{M}_n(\theta(P))-\mathbb{M}_n(\widehat\theta_1)\}-\{\mathbb{M}_P(\theta(P))-\mathbb{M}_P(\widehat\theta_1)\} > t(\alpha_1, \theta(P), \widehat \theta_1) \mid D_1) \le \alpha_1   \\
%     & \qquad\Longleftrightarrow \mathbb{P}_P(\M_P(\theta(P))-\M_P(\widehat \theta_1)\ge \mathbb{M}_n(\theta(P))-\mathbb{M}_n(\widehat\theta_1)-t(\alpha_1, \theta(P), \widehat \theta_1)\mid D_1) \ge 1-\alpha_1 \\
%     & \qquad\Longleftrightarrow \mathbb{P}_P(\M_P(\theta(P))-\M_P(\widehat \theta_1) \ge L^{\mathrm{C.E.}}_{n,\alpha_1}(\theta(P), \widehat \theta_1; D_2)\mid D_1) \ge 1-\alpha_1.
% \end{align*}
% The corresponding confidence set is thus given by 
% \begin{equation}\label{eq:concentration-based-ci}
%     \widehat{\mathrm{CI}}_{n,\alpha} := \left\{\theta \in \Theta \, : \, \mathbb{M}_n(\theta; D_2)-\mathbb{M}_n(\widehat\theta_1; D_2)\le t(\alpha_1, \theta, \widehat \theta_1)+\big(0 \wedge U_{n,\alpha_2}(\theta, \widehat \theta_1; D_2)\big)\right\}.
% \end{equation}

\begin{remark}\label{remark:the-role-U}
The upper and lower confidence bounds play asymmetric roles. While the lower confidence bound is crucial for the validity, the upper confidence bound serves to improve the statistical power. As noted above, the upper confidence bound \eqref{eq:upper-bound}, in fact, holds trivially by setting $U_{n,\alpha_2}(\theta(P), \widehat \theta_1; D_2) = 0$ and $\alpha_2=0$. We emphasize that \eqref{eq:lower-bound} and \eqref{eq:upper-bound} are only required to hold at $\theta(P)$, and it is generally true that $L_{n,\alpha_1}(\theta, \widehat \theta_1; D_2) > U_{n,\alpha_2}(\theta, \widehat \theta_1; D_2)$ for some $\theta \in \Theta$. As a result, we have $ \{\theta \in \Theta : L_{n,\alpha_1}(\theta, \widehat \theta_1; D_2) \le U_{n,\alpha_2}(\theta, \widehat \theta_1; D_2)\} \subsetneq \Theta$, and thus 
	\begin{align}
		\widehat{\mathrm{CI}}_{n,\alpha} &:= \{L_{n,\alpha_1}(\theta, \widehat \theta_1; D_2) \le 0\} \cap  \{L_{n,\alpha_1}(\theta, \widehat \theta_1; D_2) \le U_{n,\alpha_2}(\theta, \widehat \theta_1; D_2)\} \nonumber\\
  &\subsetneq \{L_{n,\alpha_1}(\theta, \widehat \theta_1; D_2) \le 0\},\nonumber
	\end{align}
leading to a non-trivial shrinkage of the confidence set when $U_{n,\alpha_2}(\theta(P), \widehat \theta_1; D_2) < 0$.
\end{remark}
% \begin{remark}\label{remark:consgtrain}The proof of Theorem~\ref{thm:validity} does not use any structure of $\Theta$, and only the fact that 
% 	\[\mathbb{M}(\theta(P), P) - \mathbb{M}(\widehat\theta_1, P) \le 0.\]
% Hence, the confidence set for the constrained M-estimation can be obtained analogously. Let $K \subsetneq \Theta$ be a (strict) subset whose elements adhere to certain properties such as sparsity or shape constraints. Then the set
% 	\begin{equation}
%     \widehat{\mathrm{CI}}^K_{n,\alpha} := \left\{\theta \in K \, : \,  L_{n,\alpha_1}(\theta, \widehat \theta_1; D_2) \le (0 \wedge U_{n,\alpha_2}(\theta, \widehat \theta_1; D_2))\right\}
% \end{equation}
% remains $1-\alpha_1-\alpha_2$-level confidence set as long as $\theta(P) \in K$. This result remains to hold when $\theta(P)$ lies on the boundary of $K$. 
% \end{remark}
\begin{remark}\label{remark:unique-opt}
    The validity of the confidence set is established even when the optimizer $\theta(P)$ in \eqref{eq:def-m-functional} is not uniquely identified. In such cases, the resulting confidence set will contain all points that minimize \eqref{eq:def-m-functional}, and consequently will not converge to a singleton set. In order to establish the convergence rate of the diameter of the confidence set, we assume the uniqueness of the optimizer. Formal statements are provided as Theorems~\ref{thm:concentration-width} and \ref{thm:concentration-width-unbounded} below.
\end{remark}
%Suppose we construct the $1-\alpha/2$ level confidence set defined as \eqref{eq:confidence-set} based on the second data set, call it $\widehat{\mathrm{CI}}_{n,\alpha}^{(2)}$, and swap the role of the datasets and construct $\widehat{\mathrm{CI}}_{n,\alpha}^{(1)}$. Then $\Tilde{C}_n := \widehat{\mathrm{CI}}_{n,\alpha}^{(1)} \cap \widehat{\mathrm{CI}}_{n,\alpha}^{(2)}$ is the valid $\alpha$-level confidence set. 
%\begin{align*}
%    \mathbb{P}(\theta(P) \not\in \Tilde{C}_n) = \mathbb{P}(\{\theta(P) \not\in \widehat{\mathrm{CI}}_{n,\alpha}^{(1)}\} \cup \{\theta(P) \not\in \widehat{\mathrm{CI}}_{n,\alpha}^{(2)}\}) \le \mathbb{P}(\theta(P) \not\in \widehat{\mathrm{CI}}_{n,\alpha}^{(1)}) + \mathbb{P}(\theta(P) \not\in \widehat{\mathrm{CI}}_{n,\alpha}^{(2)}) \le \alpha/2 + \alpha/2
%\end{align*}
% \kt{The proof of Theorem~\ref{thm:validity} uses the fact that $\theta(P)$ is a global minimizer of $\mathbb{M}_\theta(P)$ and leaves the structure of $\Theta$ or $\mathbb{M}_\theta(P)$ unspecified. Therefore we only use the fact that 
% \[\mathbb{P}(\{\widehat L_{n,\alpha_1}(\theta(P)) > 0\}\cap\mathcal{A}_n) \le \mathbb{P}(M_{\theta(P)}(P) - M_{\widehat \theta_1}(P) > 0),\]
% which cannot be stated with equality without further assumptions about $M(\widehat{\theta})$ or $M(\theta(P))$. As a result, the confidence set $\widehat{C}_n$ remains valid but is often not exact even when \eqref{eq:lower-bound} holds with an equality. 
% }


==> main/proof.tex <==
  \begin{center}
  \Large {\bf Supplement to ``Bridging Root-$n$ and Non-standard Asymptotics:\, Dimension-agnostic Adaptive Inference in M-Estimation''}
  \end{center}
       
\begin{abstract}
This supplement contains the proofs of all the main results in the paper and some supporting lemmas. 
\end{abstract}
\section{Proof of Theorem~\ref{thm:coverage-anti-conservative-confidence-set}}\label{appsec:proof-of-coverage-anti-conservative}
% \begin{proof}[Proof of Theorem~\ref{thm:coverage-anti-conservative-confidence-set}]
We denote by $\M(\theta) \equiv \M(\theta, P)$ for any $\theta \in \Theta$. Note that
\begin{align*}
    &\mathbb{P}_P\left(\theta(P) \notin \widehat{\mathrm{CI}}_{n}^{\dagger}\right)\\ ~&\qquad\le~ \mathbb{P}_P(\widehat{\mathbb{M}}_n(\theta(P)) > \widehat{\mathbb{M}}_n(\widehat{\theta}_1))\\
    &\qquad=~ \mathbb{E}_P[\mathbb{P}_P((\widehat{\mathbb{M}}_n - \mathbb{M})(\theta(P)) - (\widehat{\mathbb{M}}_n - \mathbb{M})(\widehat{\theta}_1) > \mathbb{M}(\widehat{\theta}_1) - \mathbb{M}(\theta(P))|\widehat{\theta}_1)] \\
    ~&\qquad\le~ \mathbb{E}_P\left[\frac{\mathbb{E}_P[|(\widehat{\mathbb{M}}_n - \mathbb{M})(\theta(P)) - (\widehat{\mathbb{M}}_n - \mathbb{M})(\widehat{\theta}_1)|^2|\widehat{\theta}_1]}{\mathbb{E}_P[|(\widehat{\mathbb{M}}_n - \mathbb{M})(\theta(P)) - (\widehat{\mathbb{M}}_n - \mathbb{M})(\widehat{\theta}_1)|^2|\widehat{\theta}_1] + (\mathbb{M}(\widehat{\theta}_1) - \mathbb{M}(\theta(P)))^2}\right],
\end{align*}
where the last inequality follows from Cantelli's inequality~\citep{pinelis2010between}.
% \end{proof}
\section{Proof of Theorem~\ref{thm:validity}}\label{appsec:proof-of-validity}
% \begin{proof}[\bfseries{Proof of Theorem~\ref{thm:validity}}]
Let $P$ be an arbitrary distribution in $\mathcal{P}$.
Conditioning on $D_1$, such that $\widehat \theta_1$ is considered deterministic, we define following events:
\begin{align}
	\mathcal{A}_n &:= \{\M(\theta(P), P) - \M(\widehat \theta_1, P) \geq  L_{n,\alpha_1}(\theta(P), \widehat \theta_1; D_2)\} \quad \mathrm{and}\nonumber\\
	\mathcal{B}_n &:= \{\M(\theta(P), P) - \M(\widehat \theta_1, P) \leq  U_{n,\alpha_2}(\theta(P), \widehat \theta_1; D_2)\}.\nonumber
\end{align}
We further observe that
\begin{equation}
	\begin{aligned}
		\label{eq:validity-int-step}
	&\{\theta(P)\notin\widehat{\mathrm{CI}}_{n,\alpha}\}\cap\mathcal{A}_n\cap\mathcal{B}_n \\
 &\qquad= \{ L_{n,\alpha_1}(\theta(P), \widehat \theta_1; D_2) >(0\wedge U_{n,\alpha_2}(\theta(P), \widehat \theta_1; D_2)) \}\cap\mathcal{A}_n \cap\mathcal{B}_n \\
	&\qquad\subseteq \{\M(\theta(P), P) - \M(\widehat \theta_1, P)> (0 \wedge U_{n,\alpha_2}(\theta(P), \widehat \theta_1; D_2))\} \cap \mathcal{B}_n.
	\end{aligned}
\end{equation}
The last event has probability zero under $\mathbb{P}_{P}( \cdot | D_1)$ since $\theta(P)$ is the minimizer of $\theta \mapsto \mathbb{M}(\theta, P)$ and thus $\mathbb{M}(\theta(P), P) \le  \mathbb{M}(\theta, P)$ holds $P$-almost surely for any $\theta \in \Theta$. When $U_{n,\alpha_2}(\theta(P), \widehat \theta_1; D_2) < 0$, the probability under $\mathbb{P}_{P}(\cdot | D_1)$ remains zero after taking the intersection with $\mathcal{B}_n$. Hence, we have 
\begin{align*}
&\mathbb{P}_{P}(\theta(P) \notin\widehat{\mathrm{CI}}_{n,\alpha} \mid D_1) \\
&\qquad\le \mathbb{P}_{P}(\{\theta(P)\notin \widehat{\mathrm{CI}}_{n,\alpha}\}\cap\mathcal{A}_n\cap\mathcal{B}_n\mid D_1) + \mathbb{P}_{P}(\mathcal{A}_n^c\mid D_1)+ \mathbb{P}_{P}(\mathcal{B}_n^c\mid D_1)\\
&\qquad= \mathbb{P}_{P}(\mathcal{A}_n^c\mid D_1) + \mathbb{P}_{P}(\mathcal{B}_n^c\mid D_1).
\end{align*}
Finally, we conclude the claim by the fact that $\mathbb{P}_{P}(\mathcal{A}_n^c\mid D_1) \le \alpha_1$ by \eqref{eq:lower-bound} and $\mathbb{P}_{P}(\mathcal{B}_n^c\mid D_1) \le \alpha_2$ by \eqref{eq:upper-bound} uniformly for all $P \in \mathcal{P}$.
% \end{proof}
\section{Proof of Theorem~\ref{thm:concentration-width}}\label{sec:proof-concentration-width}
Without loss of generality, we set $U_{n,\alpha_2}(\theta, \widehat \theta_1; D_2) = 0$, which only enlarges the confidence set and hence the following result remains to hold. Any element $\theta \in \Theta$ in the confidence set, defined as \eqref{eq:eb-confidence-set-def}, satisfies the following:
	\begin{align*}
		&\mathbb{P}_n (m_\theta-m_{\widehat{\theta}_1}) \le \sqrt{\frac{2\widehat \sigma^2_{\theta, \widehat\theta_1} \log(2/\alpha)}{n}} + \frac{7B_0\log(2/\alpha)}{3(n-1)}\\
		% &\qquad \Longleftrightarrow (\mathbb{P}_n-P) (m_\theta-m_{\widehat{\theta}_1}) \le -P (m_\theta-m_{\widehat{\theta}_1}) + \sqrt{\frac{2\widehat \sigma^2_{\theta, \widehat\theta_1} \log(2/\alpha)}{n}} + \frac{7B_0\log(2/\alpha)}{3(n-1)}\\
		% &\qquad \Longleftrightarrow P (m_\theta-m_{\widehat{\theta}_1}) \le -(\mathbb{P}_n-P) (m_\theta-m_{\widehat{\theta}_1}) + \sqrt{\frac{2\widehat \sigma^2_{\theta, \widehat\theta_1} \log(2/\alpha)}{n}} + \frac{7B_0\log(2/\alpha)}{3(n-1)}\\
		&\qquad \Longleftrightarrow P (m_\theta-m_{\theta(P)})+P(m_{\theta(P)}-m_{\widehat{\theta}_1}) \\
		&\qquad\qquad\le -(\mathbb{P}_n-P) (m_\theta-m_{\theta(P)}+m_{\theta(P)}-m_{\widehat{\theta}_1}) + \sqrt{\frac{2\widehat \sigma^2_{\theta, \widehat\theta_1} \log(2/\alpha)}{n}} + \frac{7B_0\log(2/\alpha)}{3(n-1)}.
	\end{align*}

Now the original confidence set is contained $P$-almost surely in the following supersets: 
	\begin{align*}
		&\bigg\{\theta \in \Theta : P (m_\theta-m_{\theta(P)})+P(m_{\theta(P)}-m_{\widehat{\theta}_1}) \\
		&\qquad\left.\le -(\mathbb{P}_n-P) (m_\theta-m_{\theta(P)}+m_{\theta(P)}-m_{\widehat{\theta}_1}) +\sqrt{\frac{2\widehat \sigma^2_{\theta, \widehat\theta_1} \log(2/\alpha)}{n}} + \frac{7B_0\log(2/\alpha)}{3(n-1)}\right\}\\
		& \subseteq \bigg\{\theta \in \Theta : P (m_\theta-m_{\theta(P)})\\
		&\qquad\left.\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)}) +   \sqrt{\frac{2\widehat \sigma^2_{\theta, \theta(P)} \log(2/\alpha)}{n}} + \frac{7B_0\log(2/\alpha)}{3(n-1)} + \Gamma_n(\widehat\theta_1, \theta(P))\right\}\\
		& \subseteq \bigg\{\theta \in \Theta : c_0\|\theta-\theta(P)\|^{1+\beta}\\
  &\qquad\left.\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)}) +   \sqrt{\frac{2\widehat \sigma^2_{\theta, \theta(P)} \log(2/\alpha)}{n}} + \frac{7B_0\log(2/\alpha)}{3(n-1)} + \Gamma_n(\widehat\theta_1, \theta(P))\right\}
	\end{align*}
	where 
	\[\Gamma_n(\widehat\theta_1, \theta(P)) := |\mathbb{P}_n(m_{\widehat{\theta}_1}-m_{\theta(P)}) |+\sqrt{\frac{2\widehat \sigma^2_{\widehat\theta_1, \theta(P)} \log(2/\alpha)}{n}}\]
 and the last step uses \ref{as:margin}.
Furthermore, we have
\begin{align*}
    \widehat \sigma^2_{\theta, \theta(P)} \le \mathbb{P}_n (m_{\theta}-m_{\theta(P)})^2
\end{align*}
and hence 
\begin{align*}
    \frac{\widehat \sigma^2_{\theta, \theta(P)}}{n} \le  \frac{1}{n}\left(n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta(P)})^2 + P (m_{ \theta}-m_{\theta(P)})^2\right).
\end{align*}
Using this result, the confidence set can be further contained in 
\begin{align*}
    &\bigg\{\theta \in \Theta : c_0\|\theta-\theta(P)\|^{1+\beta}\\
    &\qquad\left.\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)}) +   \sqrt{\frac{2\widehat \sigma^2_{\theta, \theta(P)} \log(2/\alpha)}{n}} + \frac{7B_0\log(2/\alpha)}{3(n-1)} + \Gamma_n(\widehat\theta_1, \theta(P))\right\}\\
    &\qquad\subseteq \bigg\{\theta \in \Theta : c_0\|\theta-\theta(P)\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)}). \\
    &\left.\qquad \qquad\qquad\qquad+   \sqrt{\frac{2\log(2/\alpha)n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta(P)})^2}{n}}\right.
    \left.  +\sqrt{\frac{2\log(2/\alpha)P (m_{ \theta}-m_{\theta(P)})^2 }{n}} \right.\\
    &\qquad \qquad\qquad\qquad+ \frac{7B_0\log(2/\alpha)}{3(n-1)} + \Gamma_n(\widehat\theta_1, \theta(P))\bigg\}\\
    &\qquad =: \overline{\mathrm{CI}}_{n, \alpha}.
\end{align*}
We analyze the superset $\overline{\mathrm{CI}}_{n, \alpha}$. Given $c_0$ and $\beta$ in \ref{as:margin} and the function $\phi_n$ in \ref{as:local-entropy}, we define $r_n$ as any value that satisfies 
\begin{align*}
    r_n^{-2} \phi_n(c_0^{-1/(1+\beta)}r_n^{2/(1+\beta)}) \le n^{1/2}.
\end{align*}
We define
\begin{align*}
    \mathrm{R}_M := 2^{M/(1+\beta)} c_0^{-1/(1+\beta)}\left(r_n^{2/(1+\beta)} +  r_n^{1/(1+\beta)} (B_0/n)^{1/(2+2\beta)}+ \left\{\Gamma'_n(\widehat\theta_1, \theta(P))\right\}^{1/(1+\beta)}\right)
\end{align*}
where 
\begin{align*}
    \Gamma_n'(\widehat\theta_1, \theta(P)) := \frac{7B_0\log(2/\alpha)}{3(n-1)} + \Gamma_n(\widehat\theta_1, \theta(P)).
\end{align*}
The constant $M > 0$ will be specified later. We denote by $B_{\|\cdot\|}(\theta; r)$ a $\|\cdot\|$-ball centered at $\theta$ with radius $r \ge 0$. 
We consider the partition of the parameter space $\Theta$ into the intersection with the ball 
\begin{align*}
    \Theta \cap B_{\|\cdot\|}(\theta(P); \mathrm{R}_M) \quad \mathrm{and}\quad \Theta \cap B_{\|\cdot\|}^c(\theta(P), \mathrm{R}_M)
\end{align*}
where 
\begin{align*}
    B_{\|\cdot\|}^c(\theta(P); \mathrm{R}_M) := \{\theta \in \Theta \,:\, \|\theta-\theta(P)\| > \mathrm{R}_M\}.
\end{align*}
Thus far, we have shown that $\widehat{\mathrm{CI}}^{\mathrm{E.B.}}_{n,\alpha} \subseteq \overline{\mathrm{CI}}_{n,\alpha}$. We now consider the following elementary result:
\begin{align*}
     \widehat{\mathrm{CI}}^{\mathrm{E.B.}}_{n,\alpha} \subseteq \overline{\mathrm{CI}}_{n,\alpha} \subseteq B_{\|\cdot\|}(\theta(P);\mathrm{R}_M) \,\Longleftrightarrow \, \overline{\mathrm{CI}}_{n,\alpha} \cap B^c_{\|\cdot\|}(\theta(P); \mathrm{R}_M) = \emptyset.
\end{align*}
Therefore to claim that, with high probability, the set $\widehat{\mathrm{CI}}^{\mathrm{E.B.}}_{n,\alpha}$ is contained in the ball $B_{\|\cdot\|}(\theta(P); \mathrm{R}_M)$ (and hence the diameter is less than $2\mathrm{R}_M$), we need to establish that $\overline{\mathrm{CI}}_{n,\alpha}$ intersects with $B^c_{\|\cdot\|}(\theta(P); \mathrm{R}_M)$ with an arbitrarily small probability. 

Below, we adopt the notation $\mathbb{P}^{1}_P \equiv \mathbb{P}_P(\cdot \mid D_1)$, meaning that probability should be regarded as conditioning on $D_1$ under the distribution $P$. We now establish the existence of $M$ large enough such that for 
$\|\theta-\theta(P)\| > \mathrm{R}_M$,
\begin{align*}
    \mathbb{P}^{1}_P\bigg(c_0\|\theta-\theta(P)\|^{1+\beta}&\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)}) +   \sqrt{\frac{2\log(2/\alpha)n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta(P)})^2}{n}}\\
    &\qquad +\sqrt{\frac{2\log(2/\alpha)P (m_{ \theta}-m_{\theta(P)})^2 }{n}} +\Gamma_n'(\widehat\theta_1, \theta(P))\bigg)\le \varepsilon.
\end{align*}
It follows that 
\begin{align*}
    &\mathbb{P}^{1}_P\bigg(c_0\|\theta-\theta(P)\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)}) +   \sqrt{\frac{2\log(2/\alpha)n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta(P)})^2}{n}}\\
    &\qquad\qquad\qquad\qquad \qquad+\sqrt{\frac{2\log(2/\alpha)P (m_{ \theta}-m_{\theta(P)})^2 }{n}} +\Gamma_n'(\widehat\theta_1, \theta(P))\bigg)\\
    &\qquad \le \mathbb{P}^{1}_P\left(4^{-1}c_0\|\theta-\theta(P)\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)}) \right) \\
    &\qquad\qquad + \mathbb{P}^{1}_P\left(4^{-1}c_0\|\theta-\theta(P)\|^{1+\beta}\le  \sqrt{\frac{2\log(2/\alpha)n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta(P)})^2}{n}}\right) \\
    &\qquad\qquad + \mathbb{P}^{1}_P\left(4^{-1}c_0\|\theta-\theta(P)\|^{1+\beta}\le  \sqrt{\frac{2\log(2/\alpha)P (m_{ \theta}-m_{\theta(P)})^2 }{n}}\right)\\
    &\qquad\qquad + \mathbb{P}^{1}_P\left(4^{-1}c_0\|\theta-\theta(P)\|^{1+\beta}\le \Gamma_n'( \widehat\theta_1, \theta(P))\right)\\
    &\qquad =: \mathbf{I}  + \mathbf{II} + \mathbf{III} + \mathbf{IV}.   
\end{align*}
The last term is trivially controlled since 
\begin{align}
    \mathbf{IV} &= \mathbb{P}^{1}_P\left(4^{-1}c_0\|\theta-\theta(P)\|^{1+\beta} \le \Gamma_n(\widehat\theta_1, \theta(P))\right)\nonumber\\ &\le \mathbb{P}^{1}_P\left(4^{-1}c_0\mathrm{R}_M^{1+\beta}\le \Gamma_n(\widehat\theta_1, \theta(P))\right)\nonumber \\
    &\le \mathbb{P}^{1}_P\left(4^{-1}2^{M}\Gamma_n'(\widehat\theta_1, \theta(P))\le \Gamma_n'(\widehat\theta_1, \theta(P))\right)\nonumber \\
    &\le 4 \cdot 2^{-M}\label{eq:term1}
\end{align}
by Markov inequality and the fact that $\Gamma_n'(\widehat\theta_1, \theta(P))$ is deterministic under $\mathbb{P}^{1}_P(\cdot)$.
The last display becomes less than $\varepsilon/8$ for $M$ large enough. 
% We consider a ball 
% \begin{align*}
%     &\|\theta(P) - \theta\| \\
%     &\qquad \ge 2^M \left(r_n^{2/(1+\beta)} +  r_n^{1/(1+\beta)}n^{-1/(2+2\beta)} B_0^{1/(2+2\beta)}+ \sqrt{\frac{2 P(m_{\theta}-m_{\theta(P)})^2 \log(2/\alpha)}{n-1}}+\frac{7B_0\log(2/\alpha)}{3(n-1)}+ \Gamma_n(\widehat\theta_1, \theta(P))\right)
% \end{align*}
% $\|\theta(P) - \theta\| \ge 2^M r_n^{2/(1+\beta)}$ and (2) $\|\theta(P) - \theta\| < 2^M r_n^{2/(1+\beta)}$ with the constant $M$ to be specified later. Under the case (1), we claim that 
% \[\mathbb{P}\left(\|\theta-\theta(P)\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)})+   \sqrt{\frac{2\widehat \sigma^2_{\theta, \theta(P)} \log(2/\alpha)}{n}} + \frac{7B_0\log(2/\alpha)}{3(n-1)} + \Gamma_n(\widehat\theta_1, \theta(P))\right) \le \varepsilon.\]
% Furthermore, we have
% We thus have
% \begin{align*}
%     &\mathbb{P}\left(\|\theta-\theta(P)\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)})+   \sqrt{\frac{2\widehat \sigma^2_{\theta, \theta(P)} \log(2/\alpha)}{n}} + \frac{7B_0\log(2/\alpha)}{3(n-1)} + \Gamma_n(\widehat\theta_1, \theta(P))\right)\\
%     &\qquad \le \mathbb{P}\left(3^{-1}\|\theta-\theta(P)\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)})\right)\\
%     &\qquad\qquad + \mathbb{P}\left(3^{-1}\|\theta-\theta(P)\|^{1+\beta}\le \sqrt{\frac{2n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta(P)})^2 \log(2/\alpha)}{n-1}} \right)\\
%     &\qquad \qquad +\mathbb{P}\left(3^{-1}\|\theta-\theta(P)\|^{1+\beta}\le\sqrt{\frac{2 P(m_{\theta}-m_{\theta(P)})^2 \log(2/\alpha)}{n-1}}+\frac{7B_0\log(2/\alpha)}{3(n-1)}+ \Gamma_n(\widehat\theta_1, \theta(P))\right)
% \end{align*}

% First, we reduce the analysis into 
% \begin{align*}
%     &\mathbb{P}\left(\|\theta-\theta(P)\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)})+   \sqrt{\frac{2\widehat \sigma^2_{\theta, \theta(P)} \log(2/\alpha)}{n}} + \frac{7B_0\log(2/\alpha)}{3(n-1)} + \Gamma_n(\widehat\theta_1, \theta(P))\right)\\
%     &\qquad \le \mathbb{P}\left(4^{-1}\|\theta-\theta(P)\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)})\right)+ \mathbb{P}\left(4^{-1}\|\theta-\theta(P)\|^{1+\beta}\le \sqrt{\frac{2\widehat \sigma^2_{\theta, \theta(P)} \log(2/\alpha)}{n}} \right)\\
%     &\qquad \qquad +\mathbb{P}\left(4^{-1}\|\theta-\theta(P)\|^{1+\beta}\le\frac{7B_0\log(2/\alpha)}{3(n-1)}\right)+ \mathbb{P}\left(4^{-1}\|\theta-\theta(P)\|^{1+\beta}\le \Gamma_n(\widehat\theta_1, \theta(P))\right)
% \end{align*}
Moving onto the term $\mathbf{I}$, we first observe that 
\begin{align*}
    \mathbf{I} &=\mathbb{P}^{1}_P\left(4^{-1}c_0\|\theta-\theta(P)\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)}) \mbox{ for } \|\theta-\theta(P)\| \ge \mathrm{R}_M \right) \\
     &\le \mathbb{P}^{1}_P\left(4^{-1}c_0\|\theta-\theta(P)\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)}) \mbox{ for } \|\theta-\theta(P)\| \ge 2^{M/(1+\beta)}c_0^{-1/(1+\beta)}r_n^{2/(1+\beta)} \right).
\end{align*}
We define the ``shell": 
\[S_j = \{\theta \in \Theta : 2^{j}c_0^{-1/(1+\beta)}r_n^{2/(1+\beta)} \le \|\theta-\theta(P)\| < 2^{j+1}c_0^{-1/(1+\beta)}r_n^{2/(1+\beta)}\}\]
for each $j  \in \{0\} \cup \mathbb{N}$. It then follows that 
\begin{align}
	&\mathbb{P}^{1}_P(4^{-1}c_0\|\theta-\theta(P)\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)}) \, \textrm{ for some $\theta$, i.e.,}\, \|\theta(P) - \theta\| \ge 2^M c_0^{-1/(1+\beta)}r_n^{2/(1+\beta)})\nonumber \\
 &\qquad \le \mathbb{P}^{1}_P(\exists\, (j \ge M, \theta \in S_j) : 4^{-1}c_0\|\theta-\theta(P)\|^{1+\beta}\le |n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)})|) \nonumber\\
 &\qquad \le \sum_{j=M}^\infty \mathbb{P}^{1}_P(\exists \, \theta \in S_j : 4^{-1}c_0\|\theta-\theta(P)\|^{1+\beta}\le |n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)})|)\nonumber\\
 &\qquad \le \sum_{j=M}^\infty \mathbb{P}^{1}_P\left(4^{-1}2^{j(1+\beta)}r_n^{2}\le \sup_{\theta \in S_j}|n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)})|\right)\nonumber\\
 &\qquad \le 4\sum_{j=M}^\infty 2^{-j(1+\beta)}r_n^{-2}n^{-1/2}\mathbb{E}_P\left[ \sup_{\theta \in S_j}|\mathbb{G}_n(m_\theta-m_{\theta(P)})|\right]\nonumber\\
 &\qquad \le 4\sum_{j=M}^\infty n^{-1/2}2^{-j(1+\beta)}r_n^{-2}\phi_n(2^{j+1}c_0^{-1/(1+\beta)}r_n^{2/(1+\beta)})\nonumber \\
 &\qquad \le 4\sum_{j=M}^\infty n^{-1/2}2^{-j(1+\beta)}r_n^{-2}2^{q(j+1)}\phi_n(c_0^{-1/(1+\beta)}r_n^{2/(1+\beta)})\nonumber\\
 &\qquad \le 4\sum_{j=M}^\infty 2^{-j(1+\beta)}2^{q(j+1)} = 4\cdot 2^{\beta+1}\sum_{j=M}^\infty 2^{-(j+1)(1+\beta-q)}.\label{eq:term2}
\end{align}
By assumption \ref{as:local-entropy} that $q < 1+\beta$, the last display becomes less than $\varepsilon/8$ for $M$ large enough, depending on $\beta$ and $q$.

The term $\mathbf{II}$ can similarly be controlled as:
\begin{align*}
    \mathbf{II}&=\mathbb{P}^{1}_P\left(4^{-1}c_0\|\theta-\theta(P)\|^{1+\beta}\le \sqrt{\frac{2\log(2/\alpha)n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta(P)})^2}{n}}\mbox{ for } \|\theta-\theta(P)\| \ge \mathrm{R}_M \right) \\
     &\le \mathbb{P}^{1}_P\left(4^{-1}c_0\|\theta-\theta(P)\|^{1+\beta}\le \sqrt{\frac{2\log(2/\alpha)n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta(P)})^2}{n}}\right.\\
     &\qquad\qquad\qquad\qquad\left. \mbox{ for } \|\theta-\theta(P)\| \ge 2^{M/(1+\beta)}c_0^{-1/(1+\beta)}r_n^{1/(1+\beta)}n^{-1/(2+2\beta)} B_0^{1/(2+2\beta)} \right)\\
     &\le \mathbb{P}^{1}_P\left(4^{-1}c_0\|\theta-\theta(P)\|^{1+\beta}\le \sqrt{\frac{2\log(2/\alpha)n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta(P)})^2}{n}}\right.\\
     &\qquad\qquad\qquad\qquad\left. \mbox{ for } \|\theta-\theta(P)\| \ge 2^{M/(1+\beta)}c_0^{-1/(1+\beta)}(r_n \vee n^{-1/2})^{1/(1+\beta)}n^{-1/(2+2\beta)} B_0^{1/(2+2\beta)} \right).
\end{align*}
We denote by $\bar{r}_n := (r_n \vee n^{-1/2})$ where $r_n$ is the solution of the equation given by \eqref{rq:define-rn}. We now define the ``shell": 
\begin{align*}
    S'_j = \{\theta \in \Theta &: 2^{j}c_0^{-1/(1+\beta)}\bar{r}_n^{1/(1+\beta)}n^{-1/(2+2\beta)} B_0^{1/(2+2\beta)}  \\
    &\qquad \le \|\theta-\theta(P)\| < 2^{j+1}c_0^{-1/(1+\beta)}\bar{r}_n^{1/(1+\beta)}n^{-1/(2+2\beta)} B_0^{1/(2+2\beta)}\}
\end{align*}
for each $j  \in \{0\} \cup \mathbb{N}$. It follows that 
\begin{align*}
	&\mathbb{P}^{1}_P\left(4^{-1}c_0\|\theta-\theta(P)\|^{1+\beta}\le \sqrt{\frac{2\log(2/\alpha)n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta(P)})^2}{n}}\right.\\
     &\qquad\qquad\qquad\qquad\qquad\left. \mbox{ for } \|\theta-\theta(P)\| \ge 2^{M/(1+\beta)}c_0^{-1/(1+\beta)}\bar{r}_n^{1/(1+\beta)}n^{-1/(2+2\beta)} B_0^{1/(2+2\beta)} \right)\\
 &\qquad \le \mathbb{P}^{1}_P\left(\exists\, (j \ge M, \theta \in S'_j) : 4^{-1}c_0\|\theta-\theta(P)\|^{1+\beta}\le \sqrt{\frac{2\log(2/\alpha)n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta(P)})^2}{n}}\right) \\
 &\qquad = \mathbb{P}^{1}_P\left(\exists\, (j \ge M, \theta \in S'_j) : 4^{-2}(2\log(2/\alpha))^{-1}c_0^2\|\theta-\theta(P)\|^{2+2\beta}\le \left|\frac{n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta(P)})^2}{n}\right|\right)\\
 % &\qquad \le \sum_{j=M}^\infty \mathbb{P}^{1}_P(\exists \, \theta \in S_j : 3^{-1}\|\theta-\theta(P)\|^{1+\beta}\le |n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)})|)\\
 &\qquad \le \sum_{j=M}^\infty \mathbb{P}^{1}_P\left(4^{-2}(2\log (2/\alpha))^{-1}2^{j(2+2\beta)}\bar{r}_n^{2}n^{-1} B_0\le \sup_{\theta \in S_j'}\left|\frac{n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta(P)})^2}{n}\right|\right)\\
 &\qquad \le 32\log (2/\alpha)\sum_{j=M}^\infty 2^{-j(2+2\beta)}\bar{r}_n^{-2}B_0^{-1}n^{-1/2}\mathbb{E}_P\left[ \sup_{\theta \in S_j'}|\mathbb{G}_n(m_{ \theta}-m_{\theta(P)})^2|\right].
\end{align*}
Now, we observe that
\begin{align*}
    \mathbb{E}_P\left[ \sup_{\theta \in S_j'}|\mathbb{G}_n(m_{ \theta}-m_{\theta(P)})^2|\right] = B_0^2\mathbb{E}_P\left[ \sup_{\theta \in S_j'}\left|\mathbb{G}_n\left(\frac{m_{ \theta}-m_{\theta(P)}}{B_0}\right)^2\right|\right]
\end{align*}
and the mapping $t\mapsto t^2$ is $2$-Lipschitz on $t \in [-1,1]$. Hence, by the contraction inequality, for instance, Theorem 4.12 of \cite{ledoux2013probability} or Corollary 3.2.2 of \cite{gine2021mathematical}, we obtain 
\begin{align*}
    B_0^2\mathbb{E}_P\left[ \sup_{\theta \in S_j'}\left|\mathbb{G}_n\left(\frac{m_{ \theta}-m_{\theta(P)}}{B_0}\right)^2\right|\right] \le 2 B_0\mathbb{E}_P\left[ \sup_{\theta \in S_j'}\left|\mathbb{G}_n (m_{ \theta}-m_{\theta(P)})\right|\right].
\end{align*}
To complete the argument, we have
\begin{align}
    &32\log (2/\alpha)\sum_{j=M}^\infty 2^{-j(2+2\beta)}\bar{r}_n^{-2}B_0^{-1}n^{-1/2}\mathbb{E}_P\left[ \sup_{\theta \in S_j'}|\mathbb{G}_n(m_{ \theta}-m_{\theta(P)})^2|\right]\nonumber\\
    &\qquad \le 64 \log (2/\alpha)\sum_{j=M}^\infty 2^{-j(2+2\beta)}\bar{r}_n^{-2}n^{-1/2}\mathbb{E}_P\left[ \sup_{\theta \in S_j'}|\mathbb{G}_n(m_{ \theta}-m_{\theta(P)})|\right].\label{eq:term3}
\end{align}
We now have that 
\begin{align*}
    &\bar{r}_n^{-2}n^{-1/2}\mathbb{E}_P\left[ \sup_{\theta \in S_j'}|\mathbb{G}_n(m_{ \theta}-m_{\theta(P)})|\right] \\
    &\qquad \le \bar{r}_n^{-2}n^{-1/2}\phi_n(2^{j+1}c_0^{-1/(1+\beta)}\bar{r}_n^{1/(1+\beta)}n^{-1/(2+2\beta)} B_0^{1/(2+2\beta)})\\
    &\qquad\le \bar{r}_n^{-2}n^{-1/2}2^{q(j+1)}B_0^{q/(2+2\beta)}n^{-q/(2+2\beta)} \bar{r}_n^{-q/(1+\beta)}\phi_n(c_0^{-1/(1+\beta)}\bar{r}_n^{2/(1+\beta)}).
\end{align*}

When $r_n \le n^{-1/2}$, we have $\bar{r}_n = n^{-1/2}$ and thus 
\begin{align*}
   &\bar{r}_n^{-2}n^{-1/2} 2^{q(j+1)}B_0^{q/(2+2\beta)}n^{-q/(2+2\beta)} \bar{r}_n^{-q/(1+\beta)}\phi_n(c_0^{-1/(1+\beta)}\bar{r}_n^{2/(1+\beta)}) \\
   &\qquad = n\cdot n^{-1/2}2^{q(j+1)}B_0^{q/(2+2\beta)}\phi_n(c_0^{-1/(1+\beta)}n^{-1/(1+\beta)}) \le 2^{q(j+1)}B_0^{q/(2+2\beta)}
\end{align*}
where the last inequality follows since 
$\phi_n(t^{2/(1+\beta)})/t^2$ is strictly decreasing and thus 
\begin{align*}
    nc_0\phi_n(c_0^{-1/(1+\beta)}n^{-1/(1+\beta)}) &\le c_0\phi_n(c_0^{-1/(1+\beta)}r_n^{2/(1+\beta)})/r_n^2 \le c_0n^{1/2}.
\end{align*}
Hence $ n\phi_n(c_0^{-1/(1+\beta)}n^{-1/(1+\beta)}) \le n^{1/2}$.
On the other hand, when $r_n \ge n^{-1/2}$, we have $\bar{r}_n = r_n$. It further follows that $\bar{r}_n \ge n^{-1/2} \Leftrightarrow n^{1/2}\bar{r}_n \ge 1$, and we can bound $n^{-q/(2+2\beta)} r_n^{-q/(1+\beta)} = (n^{1/2}r_n)^{-q/(1+\beta)}$ by one. The rest of the argument is identical to the earlier derivation and the last summation in \eqref{eq:term3} can be bounded as 
\begin{align*}
    &64\log (2/\alpha)\sum_{j=M}^\infty 2^{-j(2+2\beta)}\bar{r}_n^{-2}n^{-1/2}\mathbb{E}_P\left[ \sup_{\theta \in S_j'}|\mathbb{G}_n(m_{ \theta}-m_{\theta(P)})|\right] \\
    &\qquad \le 64\log (2/\alpha)\sum_{j=M}^\infty 2^{-j(2+2\beta)}2^{q(j+1)}B_0^{q/(2+2\beta)},
\end{align*}
which can be made smaller than $\varepsilon/8$ for $M$ large enough, depending on $\alpha$, $\beta$ and $B_0$. 

Finally, the third term can be bounded as 
\begin{align*}
    \mathbf{III}&=\mathbb{P}^{1}_P\left(4^{-1}c_0\|\theta-\theta(P)\|^{1+\beta}\le  \sqrt{\frac{2\log(2/\alpha)P (m_{ \theta}-m_{\theta(P)})^2 }{n}}\mbox{ for } \|\theta-\theta(P)\| \ge \mathrm{R}_M \right) \\
    & \le  \mathbb{P}^{1}_P\bigg(4^{-2}c_0^2\|\theta-\theta(P)\|^{2+2\beta}\le  \frac{2\log(2/\alpha)P (m_{ \theta}-m_{\theta(P)})^2 }{n}\\
    &\qquad \qquad\qquad \qquad\mbox{ for } \|\theta-\theta(P)\| \ge 2^{M/(1+\beta)}c_0^{-1/(1+\beta)}r_n^{2/(1+\beta)} \bigg).
\end{align*}
By repeating the analogous peeling argument over the shell
\[S_j = \{\theta \in \Theta : 2^{j}c_0^{-1/(1+\beta)}r_n^{2/(1+\beta)} \le \|\theta-\theta(P)\| < 2^{j+1}c_0^{-1/(1+\beta)}r_n^{2/(1+\beta)}\}\]
for each $j  \in \{0\} \cup \mathbb{N}$, it follows that 
\begin{align}
	&\mathbb{P}^{1}_P\bigg(4^{-2}c_0^2\|\theta-\theta(P)\|^{2+2\beta}\le  \frac{2\log(2/\alpha)P (m_{ \theta}-m_{\theta(P)})^2 }{n}\mbox{ for } \|\theta-\theta(P)\| \ge 2^{M/(1+\beta)}c_0^{-1/(1+\beta)}r_n^{2/(1+\beta)} \bigg)\nonumber \\
 %    &\qquad \le \mathbb{P}^{1}_P\bigg(\exists\, (j \ge M, \theta \in S_j) :4^{-2}\|\theta-\theta(P)\|^{2+2\beta}\le  \frac{2\log(2/\alpha)P (m_{ \theta}-m_{\theta(P)})^2 }{n} \bigg)\nonumber \\
 % % &\qquad \le \mathbb{P}^{1}_P(\exists\, (j \ge M, \theta \in S_j) : 3^{-1}\|\theta-\theta(P)\|^{1+\beta}\le |n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)})|) \nonumber\\
 % &\qquad \le \sum_{j=M}^\infty \mathbb{P}^{1}_P\bigg(4^{-2}\|\theta-\theta(P)\|^{2+2\beta}\le \frac{2\log(2/\alpha)P (m_{ \theta}-m_{\theta(P)})^2 }{n}\bigg)\nonumber\\
 %  &\qquad \le \sum_{j=M}^\infty \mathbb{P}^{1}_P\bigg(\exists \, \theta \in S_j : 4^{-2}\|\theta-\theta(P)\|^{2+2\beta}\le \frac{2\log(2/\alpha)P (m_{ \theta}-m_{\theta(P)})^2 }{n}\bigg)\nonumber\\
 % &\qquad \le \sum_{j=M}^\infty \mathbb{P}^{1}_P\left(4^{-2}2^{j(2+2\beta)}t_n^{2}\le \sup_{\theta \in S_j}\left|\frac{2\log(2/\alpha)P (m_{ \theta}-m_{\theta(P)})^2 }{n}\right|\right)\nonumber\\
 % &\qquad \le 32\log(2/\alpha)\sum_{j=M}^\infty 2^{-j(2+2\beta)}t_n^{-2}n^{-1}\sup_{\theta \in S_j}\left|P (m_{ \theta}-m_{\theta(P)})^2\right|\nonumber\\
  &\qquad \le 32\log(2/\alpha)\sum_{j=M}^\infty 2^{-j(2+2\beta)}2^{2q(j+1)}r_n^{-4}n^{-1}\phi^2_n(c_0^{-1/(1+\beta)}r_n^{2/(1+\beta)})\nonumber\\
 &\qquad \le 32\log(2/\alpha)\sum_{j=M}^\infty 2^{-j(2+2\beta)}2^{2q(j+1)} \le 32\log(2/\alpha)  2^{(1+\beta)}\sum_{j=M}^\infty 2^{-2(j+1)\{(1+\beta)-q\}}.\label{eq:term4}
\end{align}
Since $q < 1+\beta$, the last expression can be smaller than $\varepsilon/8$ for large $M$ enough, depending on $\alpha$ and $\beta$.
% By assumption \ref{as:local-entropy} that $q < 1+\beta$, the last display is less than $\varepsilon/3$ for $M$ large enough. 
% Under the case (2), we claim that with probability at least $1-\varepsilon$,
% \[n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)}) \le C_\varepsilon r_n^{2} \]
% with a constant $C_\varepsilon$ only depending on $\varepsilon > 0$. Similarly to the above derivation, we have 
% \begin{align}
%     &\mathbb{P}(2^{K+Mq} r_n^2 < -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)}) \, \textrm{ for some $\theta$, i.e.,}\, \|\theta(P) - \theta\| < 2^M r_n^{2/(1+\beta)})\\
%     &\qquad \le \mathbb{P}\left(2^{K+Mq} r_n^2 < \sup_{\|\theta(P) - \theta\| < 2^M r_n^{2/(1+\beta)}}\, |n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)})|\right)\\
%     &\qquad \le 2^{-K-Mq}r_n^{-2}n^{-1/2}\phi_n(2^{M}r_n^{2/(1+\beta)})\\
%     &\qquad \le 2^{-K}.\label{eq:term2}
% \end{align}

Finally, let $M$ be a large constant only depending on $\varepsilon$, $\alpha$, $\beta$ and $B_0$ such that \eqref{eq:term1},\eqref{eq:term2},\eqref{eq:term3} and \eqref{eq:term4} become smaller than $\varepsilon/8$ respectively. Then with probability at least $1-\varepsilon/2$, it holds that 
\begin{align*}
    &\bigg\{\theta \in \Theta : c_0\|\theta-\theta(P)\|^{1+\beta}\\
    &\qquad\qquad \left.\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)}) +   \sqrt{\frac{2\widehat \sigma^2_{\theta, \theta(P)} \log(2/\alpha)}{n}} + \frac{7B_0\log(2/\alpha)}{3(n-1)} +\Gamma_n(\widehat\theta_1, \theta(P))\right\} \\
    & \qquad \subseteq \left\{\theta \in \Theta : \|\theta-\theta(P)\|^{1+\beta}\le \mathfrak{C} c_0^{-1}\left(r_n^{2} +  r_n n^{-1/2} B_0^{1/2}+ n^{-1} B_0+\Gamma_n(\widehat\theta_1, \theta(P))\right)\right\}
\end{align*}
where the constant $\mathfrak{C}$ depends on $\varepsilon$, $\alpha$, $\beta$ and $B_0$. Since all terms in the last display are non-negative, we have 
\begin{align*}
    &c_0^{-1/(1+\beta)}\left(r_n^{2} +  r_n n^{-1/2} B_0^{1/2}+n^{-1} B_0+\Gamma_n(\widehat\theta_1, \theta(P))\right)^{1/(1+\beta)}\\
    &\qquad \le c_0^{-1/(1+\beta)}\left\{r_n^{2/(1+\beta)} + \left(r_n n^{-1/2} B_0^{1/2}\right)^{1/(1+\beta)}+n^{-1/(1+\beta)} B_0^{1/(1+\beta)}+\Gamma^{1/(1+\beta)}_n(\widehat\theta_1, \theta(P))\right\}.
\end{align*}
Furthermore, it follows 
\begin{align*}
    r_n^{2/(1+\beta)} + \left(r_n n^{-1/2} B_0^{1/2}\right)+n^{-1/(1+\beta)} B_0^{1/(1+\beta)} \le 2\left( r_n^{2/(1+\beta)} +n^{-1/(1+\beta)} B_0^{1/(1+\beta)}\right)
\end{align*}
since the middle term is always smaller than one of the other two. Putting all results together, we conclude the claim such that \[\widehat{\mathrm{CI}}^{\mathrm{E.B.}}_{n,\alpha} \subseteq B_{\|\cdot\|}(\theta(P); \mathrm{R}_n)\]
with probability greater than $1-\varepsilon/2$
where
\begin{align*}
	\mathrm{R}_n := \mathfrak{C}c_0^{-1/(1+\beta)}\left(r_n^{2/(1+\beta)} + (B_0/n)^{1/(1+\beta)} + \Gamma^{1/(1+\beta)}_n(\widehat\theta, \theta(P))\right).
	\end{align*}

This result is stated under the conditional probability on $D_1$. The only term that remains random is $\Gamma^{1/(1+\beta)}_n(\widehat\theta, \theta(P))$. We establish that there exists $S_\varepsilon$ such that  
\begin{align*}
\mathbb{P}_P(\Gamma^{1/(1+\beta)}_n(\widehat\theta, \theta(P)) \ge S_\varepsilon) \le \varepsilon/2.
\end{align*}
We observe that 
 \begin{align*}
&\mathbb{P}_P(\Gamma^{1/(1+\beta)}_n(\widehat\theta, \theta(P)) \ge S_\varepsilon) \\
     &\qquad = \mathbb{P}_P(\Gamma_n(\widehat\theta, \theta(P)) \ge S_\varepsilon^{1+\beta}) \\
     &\qquad\le \mathbb{P}_P(|\mathbb{P}_n(m_{\widehat{\theta}_1}-m_{\theta(P)}) | \ge S_\varepsilon^{1+\beta}/2) + \mathbb{P}_P(n^{-1/2}\widehat \sigma_{\widehat\theta_1, \theta(P)}\ge S_\varepsilon^{1+\beta}/2).
 \end{align*}
 The first term can be bounded by the Markov's inequality as
 \begin{align*}
    &\mathbb{P}_P(|\mathbb{P}_n(m_{\widehat{\theta}_1}-m_{\theta(P)}) - P(m_{\widehat{\theta}_1}-m_{\theta(P)}) + P(m_{\widehat{\theta}_1}-m_{\theta(P)})| \ge S_\varepsilon^{1+\beta}/2) \\
    &\qquad \le\frac{2(\mathbb{E}_P|\frac{1}{n}\sum_{i=1}^n m_{\widehat{\theta}_1}-m_{\theta(P)}|^2)^{1/2} + 2\E_P(m_{\widehat{\theta}_1}-m_{\theta(P)})}{S_\varepsilon^{1+\beta}}\\&\qquad =\frac{2\sqrt{\mathbb{E}_P(m_{\widehat{\theta}_1}-m_{\theta(P)})^2}}{n^{1/2}S_\varepsilon^{1+\beta}} + \frac{2|\mathbb{E}_P(m_{\widehat{\theta}_1}-m_{\theta(P)})|}{S_\varepsilon^{1+\beta}}.
 \end{align*}
 Similarly, we have 
  \begin{align*}
    \mathbb{P}_P(n^{-1/2}\widehat \sigma_{\widehat\theta_1, \theta(P)}\ge S_\varepsilon^{1+\beta}/2) \le \frac{4\mathbb{E}_P (m_{\widehat\theta_1}-m_{\theta(P)})^2}{nS_\varepsilon^{2+2\beta}}.
 \end{align*}

Hence by defining $S_\varepsilon = C_\varepsilon s_n$ where $s_n$ is defined as \ref{as:rate-initial-estimator} and $C_\varepsilon$ is a constant, only depending on the $\varepsilon$, it follows that 
 \begin{align*}
     \Gamma^{1/(1+\beta)}_n(\widehat\theta, \theta(P)) &\le C_\varepsilon \left(n^{-1/2}\sqrt{\mathbb{E}_P (m_{\widehat\theta_1}-m_{\theta(P)})^2} + |\mathbb{E}_P(m_{\widehat{\theta}_1}-m_{\theta(P)})|\right)^{1/(1+\beta)} \le C_\varepsilon  s_n^{1/(1+\beta)}.
 \end{align*}
Choosing $C_\varepsilon$ large enough, we can obtain 
\begin{align*}
\mathbb{P}_P(\Gamma^{1/(1+\beta)}_n(\widehat\theta, \theta(P)) \ge S_\varepsilon) = \mathbb{P}_P(\Gamma^{1/(1+\beta)}_n(\widehat\theta, \theta(P)) \ge C_\varepsilon s_n) \le \varepsilon/2.
\end{align*}
Hence, we conclude the claim such that \[\widehat{\mathrm{CI}}^{\mathrm{E.B.}}_{n,\alpha} \subseteq B_{\|\cdot\|}(\theta(P); \mathrm{R}_n)\]
with probability greater than $1-\varepsilon$
where
\begin{align*}
	\mathrm{R}_n := \mathfrak{C}c_0^{-1/(1+\beta)}\left(r_n^{2/(1+\beta)} + (B_0/n)^{1/(1+\beta)} + s_n^{1/(1+\beta)}\right).
\end{align*}

% Next, we consider the case when \ref{as:cond2} holds. Again, by an analogous derivation to the proof of Proposition~\ref{prop:clt-valid}, we obtain for $\delta \in (0,1]$, 
% \begin{align*}
% 	&\mathbb{E}_P[\dot m_t^2 \mathbf{1}\{\dot m_t^2 > n\dot M_t\}] \dot M_t^{-1} +  n^{-1/2}\mathbb{E}_P[|\dot m_t|^3 \mathbf{1}\{\dot m_t^2 \le  n\dot M_t\}] \dot M_t^{-3/2}\\
%  &\qquad \le  2n^{-\delta/2}\left(\frac{\mathbb{E}_P[\dot m_t^{2+\delta}]^{1/(2+\delta)}}{\mathbb{E}_P[\dot m_t^2]^{1/2}}\right)^{2+\delta}.
% \end{align*}
% Hence under \ref{as:cond2}, we obtain 
% \begin{align*}
% 	\Delta_{n,P} \le C(\varepsilon + n^{-\delta/2}L^{2+\delta} + \mathbf{1}\{\|\widehat{\theta}-\theta(P)\| \ge C_\varepsilon\}). 
% \end{align*}
% This concludes the claim. 
\section{Proof of Theorem~\ref{thm:vlt-validity-basic}}\label{sec:proof-vlt-validity-basic}
We verify the condition \eqref{eq:lower-bound}, which follows as 
\begin{align}
    &\Phi(z_{\alpha_1}) = 1-\alpha_1\nonumber  \\
    &\qquad \Longleftrightarrow \Phi(z_{\alpha_1})-\mathbb{P}_P\left(\widehat\sigma^{-1}_{\theta(P), \widehat\theta_1} \mathbb{G}_n(m_{\theta(P)}-m_{\widehat \theta_1}) \le z_{\alpha_1}\mid D_1\right) \nonumber \\
    &\qquad\qquad +\mathbb{P}_P\left(\widehat\sigma^{-1}_{\theta(P), \widehat\theta_1} \mathbb{G}_n(m_{\theta(P)}-m_{\widehat \theta_1}) \le z_{\alpha_1}\mid D_1\right)= 1-\alpha_1\nonumber \\
    & \qquad\Longrightarrow \mathbb{P}_P\left(\widehat\sigma^{-1}_{\theta(P), \widehat\theta_1} \mathbb{G}_n(m_{\theta(P)}-m_{\widehat \theta_1}) \le z_{\alpha_1}\mid D_1\right) \ge 1-\alpha_1-\Delta_{n,P}\nonumber \\
    & \qquad\Longleftrightarrow \mathbb{P}_P\left((\mathbb{P}_n-P)(m_{\theta(P)}-m_{\widehat \theta_1}) \le n^{-1/2}z_{\alpha_1}\widehat\sigma_{\theta(P), \widehat\theta_1}.\mid D_1\right) \ge 1-\alpha_1-\Delta_{n,P}\nonumber \\
    & \qquad\Longleftrightarrow \mathbb{P}_P(\M(\theta(P), P)-\M(\widehat \theta_1, P) \ge L^{\mathrm{CLT}}_{n,\alpha_1}(\theta(P), \widehat \theta_1; D_2)\mid D_1) \ge 1-\alpha_1-\Delta_{n,P}.\nonumber
\end{align}
The result follows from Theorem~\ref{thm:validity}.
\section{Proof of Theorem~\ref{thm:concentration-width-unbounded}}\label{sec:proof-concentration-width-unbounded}
The general structure of the proof is identical to the proof of Theorem~\ref{thm:concentration-width}. By an analogous argument, the CLT-based confidence is contained almost surely by the superset as follows:
\begin{align*}
&\widehat{\mathrm{CI}}^{\mathrm{CLT}}_{n,\alpha}\subseteq \left\{\theta \in \Theta : c_0\|\theta-\theta(P)\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)}) +   \sqrt{\frac{z_{\alpha}n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta(P)})^2}{n}}\right.\\
    &\left.\qquad \qquad\qquad\qquad\qquad \qquad  +\sqrt{\frac{z_{\alpha}P (m_{ \theta}-m_{\theta(P)})^2 }{n}} + \Gamma_n(\widehat\theta_1, \theta(P))\right\}=: \widetilde{\mathrm{CI}}_{n, \alpha}.
	\end{align*}
	where 
	\[\Gamma_n(\widehat\theta_1, \theta(P)) := |\mathbb{P}_n(m_{\widehat{\theta}_1}-m_{\theta(P)}) |+\sqrt{\frac{z_{\alpha}\widehat \sigma^2_{\widehat\theta_1, \theta(P)} }{n}}.\]
 The main difference from the proof of Theorem~\ref{thm:concentration-width-unbounded} is that we can no longer use the contraction inequality to control the squared process. We now define the ``shell": 
\[S'''_j = \{\theta \in \Theta : 2^{j}c_0^{-1/(1+\beta)}u_n^{2/(1+\beta)} \le \|\theta-\theta(P)\| < 2^{j+1}c_0^{-1/(1+\beta)}u_n^{2/(1+\beta)}\}\]
for each $j  \in \{0\} \cup \mathbb{N}$. Then, it follows that 
\begin{align*}
	&\mathbb{P}^{1}_P\left(4^{-1}c_0\|\theta-\theta(P)\|^{1+\beta}\le \sqrt{\frac{z_{\alpha}n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta(P)})^2}{n}}\right.\\
     &\qquad\qquad\qquad\qquad\qquad\left. \mbox{ for } \|\theta-\theta(P)\| \ge 2^{M/(1+\beta)}c_0^{-1/(1+\beta)}u_n^{1/(1+\beta)} \right)\\
 &\qquad \le \mathbb{P}^{1}_P\left(\exists\, (j \ge M, \theta \in S'_j) : 4^{-1}c_0\|\theta-\theta(P)\|^{1+\beta}\le \sqrt{\frac{z_{\alpha}n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta(P)})^2}{n}}\right) \\
 &\qquad = \mathbb{P}^{1}_P\left(\exists\, (j \ge M, \theta \in S'_j) : 4^{-2}c_0^2q^{-1}_{1-\alpha}\|\theta-\theta(P)\|^{2+2\beta}\le \left|\frac{n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta(P)})^2}{n}\right|\right)\\
 % &\qquad \le \sum_{j=M}^\infty \mathbb{P}^{1}_P(\exists \, \theta \in S_j : 4^{-2}c_0^2\|\theta-\theta(P)\|^{1+\beta}\le |n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)})|)\\
 &\qquad \le \sum_{j=M}^\infty \mathbb{P}^{1}_P\left(4^{-2}q^{-1}_{1-\alpha}2^{-2j(1+\beta)}u_n^{4}\le \sup_{\theta \in S_j'}\left|\frac{n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta(P)})^2}{n}\right|\right)\\
 &\qquad \le 16z_{\alpha} \sum_{j=M}^\infty 2^{2j(1+\beta)}u_n^{-4}n^{-3/2}\mathbb{E}_P\left[ \sup_{\theta \in S_j'}|\mathbb{G}_n(m_{ \theta}-m_{\theta(P)})^2|\right]\\
 &\qquad \le 16z_{\alpha}  \sum_{j=M}^\infty 2^{-2j(1+\beta)}2^{2q(j+1)}u_n^{-4}n^{-3/2}\omega^2_n(c_0^{-1/(1+\beta)}u_n^{2/(1+\beta)})\\
 &\qquad \le 16z_{\alpha}  2^{(1+\beta)}\sum_{j=M}^\infty 2^{-2(j+1)\{(1+\beta)-q\}}.
\end{align*}
By the assumption $q < 1-\beta$, the last series is summable and thus can be made smaller than $\varepsilon$ for $M$ large enough. Then with probability at least $1-\varepsilon/2$, it holds that 
\begin{align*}
    &\widehat{\mathrm{CI}}^{\mathrm{CLT}}_{n,\alpha}\subseteq \left\{\theta \in \Theta : \|\theta-\theta(P)\|^{1+\beta}\le \mathfrak{C}c_0^{-1} \left(r_n^{2} +  u_n^2 +\Gamma_n(\widehat\theta_1, \theta(P))\right)\right\}
\end{align*}
where the constant $\mathfrak{C}$ depends on $\varepsilon$, $\alpha$ and $\beta$. We note that the dependence of $\mathfrak{C}$ 
 on $B_0$ is dropped as this was introduced in the proof of Theorem~\ref{thm:concentration-width} as a consequence of the contraction inequality. The rest of the proof is identical to that of Theorem~\ref{thm:concentration-width}.
\section{Proof of Proposition~\ref{prop:first-order-linearization}}\label{sec:proof-first-order-linearization}
Fix $P \in \mathcal{P}$. 
% We adopt the notation $\E_P^1[\cdot] \equiv \E_P[\cdot | D_1]$ for convenience. 
Beginning with the statement of Theorem~\ref{thm:validity-BE}, it is immediate that
\begin{align*}
	&\mathbb{P}_P(\theta(P) \in \widehat{\mathrm{CI}}^{\mathrm{CLT}}_{n, \alpha} \mid D_1)\\
	 &\qquad\ge 1-\alpha_1-\alpha_2-\Delta_{n,P}\\
	&\qquad \ge 1-\alpha_1-\alpha_2-C\left ( \mathbb{E}_P[W_1^2 \mathbf{1}\{W_1^2 > nB^2\}] B^{-2} +  n^{-1/2}\mathbb{E}_P[|W_1|^3 \mathbf{1}\{W_1^2 \le  nB^2\}] B^{-3} \right)
\end{align*}
where $C$ is a universal constant and $B^2 = \E_P^1[W_1^2]$ and the second inequality follows from Proposition~\ref{prop:clt-valid}. We now provide the upper bounds on two terms in the parenthesis. 

First, by adding and subtracting terms, we obtain 
\begin{align*}
	\mathbb{E}_P\left[\frac{W_1^2}{B^2} \mathbf{1}\left\{\frac{W_1^2}{B^2} > n\right\}  \right] & = \mathbb{E}_P\left[\frac{W_1^2}{B^2} \mathbf{1}\left\{\frac{W_1^2}{B^2} > n\right\}  \right]\\
 &\qquad- \mathbb{E}_P\left[\frac{\langle t,H_1\rangle^2}{\mathbb{E}_P\langle t,H_1\rangle^2} \mathbf{1}\left\{\frac{\langle t,H_1\rangle^2}{\mathbb{E}_P\langle t,H_1\rangle^2} > n\right\}  \right]\\
	&\qquad +  \mathbb{E}_P\left[\frac{\langle t,H_1\rangle^2}{\mathbb{E}_P\langle t,H_1\rangle^2} \mathbf{1}\left\{\frac{\langle t,H_1\rangle^2}{\mathbb{E}_P\langle t,H_1\rangle^2} > n\right\}  \right]
	\end{align*}
We invoke technical Lemma~\ref{lemma:moment-bounds} provided below to control the approximation term. The equation \eqref{eq:qmd2} implies that there exists $\varphi$ such that 
\begin{align*}
	\mathbb{E}_P[|W_1 - \langle \widehat{\theta}_1-\theta(P),H_1\rangle|^2] \le \varphi(\|\widehat{\theta}_1-\theta(P)\|) \mathbb{E}_P \langle \widehat{\theta}_1-\theta(P),H_1\rangle^2
\end{align*}
holds for all $\widehat{\theta}_1$ such that $\|\widehat{\theta}_1-\theta(P)\| < \delta_0$. Hence, by the second statement of Lemma~\ref{lemma:moment-bounds}, 
\begin{align*}
	&\mathbb{E}_P\left[\frac{W_1^2}{B^2} \mathbf{1}\left\{\frac{W_1^2}{B^2} > n\right\}\right]- \mathbb{E}_P\left[\frac{\langle t,H_1\rangle^2}{\mathbb{E}_P\langle t,H_1\rangle^2} \mathbf{1}\left\{\frac{\langle t,H_1\rangle^2}{\mathbb{E}_P\langle t,H_1\rangle^2} > n\right\}\right]\leq 16 (\varphi(\delta) + \varphi^{1/2}(\delta)).
\end{align*}
assuming $\|\widehat{\theta}_1-\theta(P)\| < \delta$ for any $0 < \delta < \delta_0$. Similarly, by the third statement of Lemma~\ref{lemma:moment-bounds},
\begin{align*}
    &n^{-1/2}\mathbb{E}_P\left[\frac{|W_1|^3}{B^3} \mathbf{1}\left\{\frac{W_1^2}{B^2} \le  n\right\}\right] -  n^{-1/2}\mathbb{E}_P\left[\frac{|\langle t,H_1\rangle|^3}{(\mathbb{E}_P\langle t,H_1\rangle^2)^{3/2}} \mathbf{1}\left\{\frac{\langle t,H_1\rangle^2}{\mathbb{E}_P\langle t,H_1\rangle^2} \le n\right\}\right] \\
    &\qquad \le 16 (\varphi(\delta) + \varphi^{1/2}(\delta)).
\end{align*}
% \begin{align*}
% 	&n^{-1/2}\mathbb{E}_P[|W_1|^3 \mathbf{1}\{W_1^2 \le  nS\}] S^{-3/2}\\
% 	& \qquad - n^{-1/2}\mathbb{E}_P[\langle t,H\rangle^3 \mathbf{1}\{\langle t,H\rangle^2 > nP\langle t,H\rangle^2\}] (P\langle t,H\rangle)^{-3/2} \\
%  &\qquad \le  16 (\varepsilon + \varepsilon^{1 / 2})
% \end{align*}
% assuming $\|\widehat{\theta}_1-\theta(P)\| < C_\varepsilon$. Putting together, we have
% \begin{align*}
% 	&\mathbb{E}_P[W_1^2 \mathbf{1}\{W_1^2 > nS\}] S^{-1} +  n^{-1/2}\mathbb{E}_P[|W_1|^3 \mathbf{1}\{W_1^2 \le  nS\}] S^{-3/2} \\
% 	&\qquad \le 32(\varepsilon + \varepsilon^{1 / 2}) + \mathbb{E}_P[\langle t,H\rangle^2 \mathbf{1}\{\langle t,H\rangle^2 > nP\langle t,H\rangle^2\}] (P\langle t,H\rangle)^{-1}\\
% 	&\qquad\qquad + n^{-1/2}\mathbb{E}_P[\langle t,H\rangle^3 \mathbf{1}\{\langle t,H\rangle^2 > nP\langle t,H\rangle^2\}] (P\langle t,H\rangle)^{-3/2}
% \end{align*}
% when $\|\widehat{\theta}_1-\theta(P)\| < C_\varepsilon$.
We thus obtain for any $0 < \delta < \delta_0$, 
\begin{align*}
	\Delta_{n,P} &= \Delta_{n,P} \mathbf{1}\{{\|\widehat{\theta}_1-\theta(P)\| < \delta}\} + \Delta_{n,P} \mathbf{1}\{{\|\widehat{\theta}_1-\theta(P)\| \ge \delta}\} \\
	&\le C\bigg(32(\varphi(\delta) + \varphi^{1/2}(\delta)) +\mathbf{1}\{{\|\widehat{\theta}_1-\theta(P)\| \ge \delta}\} \\
 &\qquad + \mathbb{E}_P[\langle t,H_1\rangle^2 \mathbf{1}\{\langle t,H_1\rangle^2 > n\E_P\langle t,H_1\rangle^2\}] (\E_P\langle t,H_1\rangle)^{-1}\\
	&\qquad + n^{-1/2}\mathbb{E}_P[\langle t,H_1\rangle^3 \mathbf{1}\{\langle t,H_1\rangle^2 > n\E_P\langle t,H_1\rangle^2\}] (\E_P\langle t,H_1\rangle)^{-3/2} \bigg)\\
	&= C\bigg(32(\varphi(\delta) + \varphi^{1/2}(\delta)) +  \mathbf{1}\{{\|\widehat{\theta}_1-\theta(P)\| \ge \delta}\} \\
 &\qquad + \mathbb{E}_P\left[\frac{\langle t,H_1\rangle^2}{\E_P^1\langle t,H_1\rangle^2} \left\{1 \wedge n^{-1/2}\frac{|\langle t,H_1\rangle|}{\sqrt{\E_P^1\langle t,H_1\rangle^2}}\right\}\right] \bigg).
\end{align*}
where we use the trivial bound of $\Delta_{n,P} \le 1$ in the case when $\|\widehat{\theta}_1-\theta(P)\| \ge \delta$. By taking the supremum over $\|t\|=1$, we conclude 
\begin{align*}
    \sup_{P\in \mathcal{P}}\, \E_{P}[\Delta_{n,P}] &\lesssim \sup_{P\in \mathcal{P}}\, \sup_{\|t\|=1}\E_P\left[\frac{\langle t,H_1\rangle^2}{P\langle t,H_1\rangle^2} \left\{1 \wedge n^{-1/2}\frac{|\langle t,H_1\rangle|}{\sqrt{P\langle t,H_1\rangle^2}}\right\}\right] \\
    &\qquad + \varphi(\delta) + \varphi^{1/2}(\delta) +   \sup_{P\in \mathcal{P}}\,\mathbb{P}_P(\|\widehat{\theta}_1-\theta(P)\| \ge \delta)
\end{align*}
for any $0 \le \delta < \delta_0$.

\section{Proof of Proposition~\ref{prop:suff-cond-for-CLT}}\label{sec:proof-suff-cond-for-CLT}
We fix $P \in \mathcal{P}$ and $t \in \mathbb{R}^d$. We denote by $Z_t:=\langle t, Z\rangle$, which is a real-valued mean-zero random variable and $B_t = (\E_P[Z_t^2])^{1/2}$. First, we prove $\eqref{eq:unif-integrable-def}\Longrightarrow$ uniform Lindeberg condition. We observe that 
% \begin{align}
    % &\E_P\left[\frac{Z_t^2}{B_t^2} \left\{1 \wedge \frac{|Z_t|}{n^{1/2}B_t}\right\}\right] \nonumber\\
    % &\qquad = \E_P\left[\frac{Z_t^2}{B_t^2} \mathbf{1}\left\{n^{1/2}B_t < |Z_t|\right\}\right] + n^{-1/2}\E_P\left[\frac{|Z_t|^3}{B_t^3} \mathbf{1}\left\{n^{1/2}B_t > |Z_t|\right\}\right]\label{eq:mid-step}\\
    % &\qquad = \E_P\left[\frac{Z_t^2}{B_t^2} \mathbf{1}\left\{n^{1/2}B_t < |Z_t|\right\}\right] + n^{-1/2}\E_P\left[\frac{|Z_t|^3}{B_t^3} \mathbf{1}\left\{\varepsilon n^{1/2}B_t > |Z_t|\right\}\right]\nonumber\\
    % &\qquad\qquad + n^{-1/2}\E_P\left[\frac{|Z_t|^3}{B_t^3} \mathbf{1}\left\{ n^{1/2}B_t > |Z_t| > \varepsilon n^{1/2}B_t\right\}\right]\nonumber\\
    % &\qquad \le \E_P\left[\frac{Z_t^2}{B_t^2} \mathbf{1}\left\{n^{1/2}B_t < |Z_t|\right\}\right] + \varepsilon\E_P\left[\frac{|Z_t|^2}{B_t^2} \mathbf{1}\left\{\varepsilon n^{1/2}B_t > |Z_t|\right\}\right]\nonumber\\
    % &\qquad\qquad + \E_P\left[\frac{|Z_t|^2}{B_t^2} \mathbf{1}\left\{ n^{1/2}B_t > |Z_t| > \varepsilon n^{1/2}B_t\right\}\right]\nonumber\\
    % &\qquad \le \varepsilon + \E_P\left[\frac{|Z_t|^2}{B_t^2} \mathbf{1}\left\{ |Z_t| > \varepsilon n^{1/2}B_t\right\}\right]\nonumber
% \end{align}
\begin{align}
    &\E_P\left[\frac{Z_t^2}{B_t^2} \left\{1 \wedge \frac{|Z_t|}{\kappa B_t}\right\}\right] \nonumber\\
    &\qquad = \E_P\left[\frac{Z_t^2}{B_t^2} \mathbf{1}\left\{1 > \frac{|Z_t|}{\kappa B_t}\right\}\right] + \kappa^{-1}\E_P\left[\frac{|Z_t|^3}{B_t^3} \mathbf{1}\left\{1 \le \frac{|Z_t|}{\kappa B_t}\right\}\right]\label{eq:mid-step}\\
    % &\qquad = \inf_{\varepsilon > 0}\,\left\{\E_P\left[\frac{Z_t^2}{B_t^2} \mathbf{1}\left\{\varepsilon > \frac{|Z_t|}{\kappa B_t}\right\}\right] + \E_P\left[\frac{|Z_t|^3}{B_t^3} \mathbf{1}\left\{\varepsilon  \le \frac{|Z_t|}{\kappa B_t}\right\}\right]\right\}\label{eq:mid-step-2}\\
    &\qquad = \E_P\left[\frac{Z_t^2}{B_t^2} \mathbf{1}\left\{\kappa B_t < |Z_t|\right\}\right] + \kappa^{-1}\E_P\left[\frac{|Z_t|^3}{B_t^3} \mathbf{1}\left\{\varepsilon \kappa B_t > |Z_t|\right\}\right]\nonumber\\
    &\qquad\qquad + \kappa^{-1}\E_P\left[\frac{|Z_t|^3}{B_t^3} \mathbf{1}\left\{ \kappa B_t > |Z_t| > \varepsilon \kappa B_t\right\}\right]\nonumber\\
    &\qquad \le \E_P\left[\frac{Z_t^2}{B_t^2} \mathbf{1}\left\{\kappa B_t < |Z_t|\right\}\right] + \varepsilon\E_P\left[\frac{|Z_t|^2}{B_t^2} \mathbf{1}\left\{\varepsilon \kappa B_t > |Z_t|\right\}\right]\nonumber\\
    &\qquad\qquad + \E_P\left[\frac{|Z_t|^2}{B_t^2} \mathbf{1}\left\{ \kappa B_t > |Z_t| > \varepsilon \kappa B_t\right\}\right]\nonumber\\
    &\qquad \le \varepsilon + \E_P\left[\frac{|Z_t|^2}{B_t^2} \mathbf{1}\left\{ |Z_t| > \varepsilon \kappa B_t\right\}\right]\nonumber
\end{align}
for any $\varepsilon > 0$. Hence we have
\begin{align*}
    &\sup_{P\in \mathcal{P}}\, \sup_{\|t\|=1}\, \E_P\left[\frac{Z_t^2}{B_t^2} \left\{1 \wedge \frac{|Z_t|}{\kappa B_t}\right\}\right] \le \sup_{P\in \mathcal{P}}\, \sup_{\|t\|=1}\,\left(\varepsilon + \E_P\left[\frac{|Z_t|^2}{B_t^2} \mathbf{1}\left\{ |Z_t| > \varepsilon \kappa B_t\right\}\right]\right).
\end{align*}
Assuming uniform integrability under standardization, the last display tends to zero as $\kappa \longrightarrow \infty$ for fixed $\varepsilon > 0$, and then we take $\varepsilon \longrightarrow 0$.

Next, we prove $\eqref{eq:norm-equivalence-def} \Longrightarrow \eqref{eq:unif-integrable-def}$. This follows since 
\begin{align*}
   \sup_{P\in \mathcal{P}}\, \sup_{\|t\|=1}\,\E_P\left[\frac{|Z_t|^2}{B_t^2} \mathbf{1}\left\{ |Z_t| >  \kappa B_t\right\}\right] &\le \sup_{P\in \mathcal{P}}\, \sup_{\|t\|=1}\,\E_P\left[\frac{|Z_t|^{2+\delta}}{\kappa^\delta B_t^{2+\delta}} \mathbf{1}\left\{ |Z_t| >  \kappa B_t\right\}\right] \\
    &\le \kappa^{-\delta/(2+\delta)}\sup_{P\in \mathcal{P}}\, \sup_{\|t\|=1}\,\left ( \frac{\E_P[|Z_t|^{2+\delta}]^{1/(2+\delta)}}{\E_P[Z_t^2]^{1/2}}\right)^{2+\delta} \longrightarrow 0
\end{align*}
as $\kappa \longrightarrow \infty$. Hence the uniform integrability is implied. These two results establish 
\begin{align*}
        \eqref{eq:norm-equivalence-def} \Longrightarrow \eqref{eq:unif-integrable-def} \Longrightarrow \mathrm{Uniform \, Lindeberg \, condition}.
    \end{align*}
    
In fact, \eqref{eq:norm-equivalence-def} implies a stronger result than the uniform Lindeberg condition. To see this, we begin from \eqref{eq:mid-step} above and obtain
\begin{align*}
    &\E_P\left[\frac{Z_t^2}{B_t^2} \mathbf{1}\left\{\kappa B_t < |Z_t|\right\}\right] + \kappa^{-1}\E_P\left[\frac{|Z_t|^3}{B_t^3} \mathbf{1}\left\{\kappa B_t > |Z_t|\right\}\right] \le 2 \kappa^{-\delta}\left ( \frac{\E_P[|Z_t|^{2+\delta}]^{1/(2+\delta)}}{\E_P[Z_t^2]^{1/2}}\right)^{2+\delta}.
\end{align*}
Hence we have
\begin{align*}
    &\sup_{P\in \mathcal{P}}\, \sup_{\|t\|=1}\, \E_P\left[\frac{Z_t^2}{B_t^2} \left\{1 \wedge \frac{|Z_t|}{\kappa B_t}\right\}\right] \le L^{2+\delta} \kappa^{-\delta} \longrightarrow 0
\end{align*}
as $\kappa \to \infty$ under the $L_{2+\delta}$-$L_2$ norm equivalence. Hence not only does the last expression tend to zero, but the rate of convergence is given by $O(\kappa^{-\delta})$.
%  	\begin{align*}
% 		&\left ( \mathbb{E}_P[W_1^2 \mathbf{1}\{W_1^2 > nS\}] S^{-1} +  n^{-1/2}\mathbb{E}_P[|W_1|^3 \mathbf{1}\{W_1^2 \le  nS\}] S^{-3/2} \right) \\
%   &\qquad \le C \left (\varepsilon +  \E_P[W_1^2 \mathbf{1}\{W_1^2 > \varepsilon^2 nS\}] S^{-1}  \right).
% 	\end{align*}
%  This holds trivially for $\varepsilon > 1$ and thus we focus on $\varepsilon < 1$. First, we observe that 
%  \begin{align*}
%      &\mathbb{E}_P[W_1^2 \mathbf{1}\{W_1^2 > nS\}] S^{-1} +  n^{-1/2}\mathbb{E}_P[|W_1|^3 \mathbf{1}\{W_1^2 \le  nS\}] S^{-3/2}\\
%      &\qquad = \mathbb{E}_P[W_1^2 \mathbf{1}\{W_1^2 > nS\}] S^{-1} +  n^{-1/2}\mathbb{E}_P[|W_1|^3 \mathbf{1}\{W_1^2 \le \varepsilon^2 nS\}] S^{-3/2} \\
%      &\qquad\qquad + n^{-1/2}\mathbb{E}_P[|W_1|^3 \mathbf{1}\{\varepsilon^2 nS < W_1^2 \le  nS\}] S^{-3/2}\\
%      &\qquad \le  \mathbb{E}_P[W_1^2 \mathbf{1}\{W_1^2 > nS\}] S^{-1} +  \varepsilon\mathbb{E}_P[|W_1|^2 \mathbf{1}\{W_1^2 \le \varepsilon^2 nS\}] S^{-1} \\
%      &\qquad\qquad + \mathbb{E}_P[|W_1|^2 \mathbf{1}\{\varepsilon^2 nS < W_1^2 \le  nS\}] S^{-1}\\
%      &\qquad \le  2\left(\varepsilon + \mathbb{E}_P[|W_1|^2 \mathbf{1}\{\varepsilon^2 nS < W_1^2\}] S^{-1}\right).
%  \end{align*}
% This concludes the claim. 

% Finally, for any $\delta \in (0,1]$, 
%  	\begin{align*}
% 		&\left ( \mathbb{E}_P[W_1^2 \mathbf{1}\{W_1^2 > nS\}] S^{-1} +  n^{-1/2}\mathbb{E}_P[|W_1|^3 \mathbf{1}\{W_1^2 \le  nS\}] S^{-3/2} \right) \\
%   &\qquad = \left ( \mathbb{E}_P[W_1^2 \mathbf{1}\{W_1^\delta > n^{\delta/2}S^{\delta/2}\}] S^{-1} +  n^{-1/2}\mathbb{E}_P[|W_1|^3 \mathbf{1}\{W_1^{1-\delta} \le  n^{(1-\delta)/2}S^{(1-\delta)/2}\}] S^{-3/2} \right)\\
%   &\qquad \le 2 n^{-\delta/2}\left ( \frac{\E_P[|W_1|^{2+\delta}]^{1/(2+\delta)}}{\E_P[W_1^2]^{1/2}}\right)^{2+\delta}
% 	\end{align*}
%  by Markov inequality. This concludes the claim. 

% This result is identical to equation (1.5) of \citet{bentkus1996berry}. We provide the proof for completeness. We first introduce several notations. For each $\theta \in \Theta$ and $P\in \mathcal{P}$, we define 
% \begin{align*}
% 	W_i &:= m_{\theta}(Z_i) - m_{\theta(P)}(Z_i) - P(m_{\theta}-m_{\theta(P)}), \\
% 	S_n &:= \sum_{i=1}^n \mathrm{Var}(W_i), \quad	Y_i := S_n^{-1/2} W_i \mathbf{1}\{W_i^2\le S_n\}, \quad 	M := \sum_{i=1}^n \mathrm{Var}(Y_i),  \\
% 	\Pi &:= \sum_{i=1}^n \mathbb{P}_P(W_i^2 > S_n),\quad  \Upsilon := M^{-1/2}\sum_{i=1}^n|\mathbb{E}_P Y_i|, \quad\mbox{and}\quad  \Lambda := M^{-3/2}\sum_{i=1}^n\mathbb{E}_P |Y_i|^3.
% \end{align*}
% Although all terms depend on $P$, we omit its dependence from the notation. Then Corollary 1.1 of \citet{bentkus1996berry} states that there exists a universal constant $C$ such that  
% \[\Delta_{n, P} \le C(\Pi+ \Upsilon + \Lambda).\]
% Furthermore, we observe that 
% \begin{align*}
% 	\Pi &= \sum_{i=1}^n \mathbb{P}_P(W_i^2 > S_n) = \sum_{i=1}^n \mathbb{P}_P(W_i^2 \mathbf{1}\{W_i^2 > S_n\} > S_n) \le \sum_{i=1}^n \mathbb{E}_P[W_i^2 \mathbf{1}\{W_i^2 > S_n\}] S_n^{-1} 
% \end{align*}
% by the Markov inequality. Similarly, we also have 
% \begin{align*}
% 	|\mathbb{E}_P Y_i| &= |\mathbb{E}_P [S_n^{-1/2} W_i \mathbf{1}\{W_i^2\le S_n\}]| \\
%  &= |\mathbb{E}_P  S_n^{-1} W_i - \mathbb{E}_P S_n^{-1/2} W_i  \mathbf{1}\{W_i^2 > S_n\}| \\
%  &= S_n^{-1/2} |\mathbb{E}_P W_i  \mathbf{1}\{W_i^2 > S_n\}| \\
% 	&\le S_n^{-1/2} (\mathbb{E}_P |W_i|^2  \mathbf{1}\{W_i^2 > S_n\})^{1/2} \mathbb{P}_P^{1/2}(W_i^2 \mathbf{1}\{W_i^2 > S_n\}> S_n) \\
%  &= \mathbb{E}_P[W_i^2 \mathbf{1}\{W_i^2 > S_n\}] S_n^{-1} 
% 	\end{align*}
% where we use the fact that $\E_P[W_i]=0$ and the inequality follows by Cauchy-Schwarz inequality. It also follows that
% \begin{align*}
% 	\mathbb{E}_P |Y_i|^3 &= \mathbb{E}_P | S_n^{-1/2} W_i \mathbf{1}\{W_i^2\le S_n\} |^3 = S_n^{-3/2} \mathbb{E}_P | W_i|^3 \mathbf{1}\{W_i^2\le S_n\}.
% \end{align*}

% Finally, we have
% \begin{align*}
% 		\mathrm{Var}(Y_i) &= \mathbb{E}_P Y_i^2 - (\mathbb{E}_P Y_i)^2 \\
%   &= S_n^{-1} \mathbb{E}_P W_i^2 \mathbf{1}\{W_i^2\le S_n\} - S_n^{-1} (\mathbb{E}_P W_i \mathbf{1}\{W_i^2\le S_n\})^2 \\
% 		&= S_n^{-1} \mathbb{E}_P W_i^2 - S_n^{-1} \mathbb{E}_P W_i^2 \mathbf{1}\{W_i^2> S_n\} - S_n^{-1} (\mathbb{E}_P W_i \mathbf{1}\{W_i^2\le S_n\})^2\\
% 		&\ge S_n^{-1} \mathbb{E}_P W_i^2 - 2 S_n^{-1} \mathbb{E}_P W_i^2 \mathbf{1}\{W_i^2> S_n\},
% \end{align*}
% and hence 
% \begin{align*}
% 	M \ge \sum_{i=1}^n S_n^{-1} \mathbb{E}_P W_i^2 - 2 S_n^{-1} \mathbb{E}_P W_i^2 \mathbf{1}\{W_i^2> S_n\} = 1 - 2 S_n^{-1} \sum_{i=1}^n\mathbb{E}_P W_i^2 \mathbf{1}\{W_i^2> S_n\}.
% \end{align*}

% It is without loss of generality to assume that $S_n^{-1} \sum_{i=1}^n\mathbb{E}_P W_i^2 \mathbf{1}\{W_i^2> S_n\}  \le 1/4$ since the following statement holds with $C > 4$ trivially. We thus have 
% \begin{align}
% 	\Delta_{n,P} &\le C(\Pi+ \Upsilon + \Lambda)\nonumber\\
%  &\le C\left ( \sum_{i=1}^n \mathbb{E}_P[W_i^2 \mathbf{1}\{W_i^2 > S_n\}] S_n^{-1} +  \sum_{i=1}^n \mathbb{E}_P[|W_i|^3 \mathbf{1}\{W_i^2 \le  S_n\}] S_n^{-3/2} \right)\nonumber\\
%  &= C\left ( \mathbb{E}_P[W_1^2 \mathbf{1}\{W_1^2 > nS\}] S^{-1} +  n^{-1/2}\mathbb{E}_P[|W_1|^3 \mathbf{1}\{W_1^2 \le  nS\}] S^{-3/2} \right)\label{eq:last-term-prop2}
% %	\\
% %	&= C\left ( \sum_{i=1}^n \mathbb{E}[W_i^2 \mathbf{1}\{W_i^2 > S_n^2\}] S_n^{-2} +  \sum_{i=1}^n \mathbb{E}[|W_i|^3 \mathbf{1}\{W_i^2 \le  \varepsilon^2 S_n^2\}] S_n^{-3} + \sum_{i=1}^n \mathbb{E}[|W_i|^3 \mathbf{1}\{\varepsilon^2 S_n^2 < W_i^2 \le  S_n^2\}] S_n^{-3}\right)\\
% %	&\le C\left ( \sum_{i=1}^n \mathbb{E}[W_i^2 \mathbf{1}\{W_i^2 > S_n^2\}] S_n^{-2} +  \varepsilon + \sum_{i=1}^n \mathbb{E}[|W_i|^2 S_n \mathbf{1}\{\varepsilon^2 S_n^2 < W_i^2 \le  S_n^2\}] S_n^{-3}\right)\\
% %	&\le C\left ( \varepsilon + \sum_{i=1}^n \mathbb{E}[|W_i|^2 \mathbf{1}\{W_i^2 > \varepsilon^2 S_n^2 \}] S_n^{-2}\right)
% \end{align}
% where the last step follows since $W_1, \ldots, W_n$ is an IID observation. 

% We provide two ways to further control \eqref{eq:last-term-prop2}. 
% For the ease of notation, we denote by 
% \[\dot m_t \equiv \langle t, \dot m_{\theta(P)}\rangle \quad \mbox{and} \quad  \dot M_t \equiv P \langle t, \dot m_{\theta(P)}\rangle^2.\]

% First, we analyze the case when \ref{as:cond1} holds. For $\varepsilon< 1/16$, we observe that  
% \begin{align*}
% 	&\mathbb{E}_P[\langle t, \dot m_{\theta(P)}\rangle^2 \mathbf{1}\{\langle t, \dot m_{\theta(P)}\rangle^2 > nP\langle t, \dot m_{\theta(P)}\rangle^2\}] (P\langle t, \dot m_{\theta(P)}\rangle^2)^{-1}\\
% 	&\qquad \le  C\left(\varepsilon  +\mathbb{E}_P[\dot m_t^2 \mathbf{1}\{ \dot m_t^2 \ge  n\varepsilon^2 \dot M_t \}] \dot M_t^{-1}\right)
% \end{align*}
% by an analogous derivation to the proof of Proposition~\ref{prop:clt-valid}.
% Hence under \ref{as:cond1}, we obtain 
% \begin{align*}
% 	\Delta_{n,P} \le C(\varepsilon + \mathbf{1}\{\|\widehat{\theta}-\theta(P)\| \ge  C_\varepsilon\}) 
% \end{align*}
% for all $n \ge N_\varepsilon$, depending on $\varepsilon$.

\section{Statistical Applications}\label{sec:proof-applications}
This section contains all proofs associated with the statistical applications. We first provide notations to which we frequently refer. For any set $\Theta$ equipped with a metric $\|\cdot\|$, and any $\varepsilon > 0$, an $\varepsilon$-covering number $\mathcal{N}(\varepsilon,\Theta, \|\cdot\|)$ of $\Theta$ relative to the metric $\|\cdot\|$ is defined as the minimal number of $\|\cdot\|$-balls of radius less than or equal to $\varepsilon$ required for covering $\Theta$. On the other hands, the $\varepsilon$-bracketing number $\mathcal{N}_{[\,]}(\varepsilon,\Theta, \|\cdot\|)$ is the minimal number of ``brackets" such that $[L, U] := \{f : L \le f \le U\}$ of size $\|U-L\|\le \varepsilon$ required for covering $\Theta$. In particular, we consider when $\Theta$ contains measurable functions of observations $Z_1\, \ldots, Z_n \in \mathcal{Z}$ and let $Q$ be any  discrete probability measure on $Z_1\, \ldots, Z_n$. We define an envelop function $F$ of the class $\Theta$ as $F := z\mapsto \sup_{f\in\Theta}|f(z)|$. The uniform entropy numbers of $\Theta$ relative to $L_r$ is defined as 
\begin{align*}
    J(\delta, \Theta, L_r) := \sup_{Q}\int_{0}^\delta \sqrt{1 + \log N(\varepsilon\|F\|_{Q, r}, \Theta, L_r(Q))}\, d\varepsilon
\end{align*}
where $\|f\|_{Q,r} := \left(\sum_{i=1}^n f^r(z_i)Q(z_i)\right)^{1/r}$. Similarly, the bracketing entropy integral is defined as 
\begin{align*}
    J_{[\, ]}(\delta, \Theta, \|\cdot\|) := \int_{0}^\delta \sqrt{1 + \log N_{[\,]}(\varepsilon, \Theta, \|\cdot\|)}\, d\varepsilon,
\end{align*}
crucially without taking the supremum over $Q$ and $\varepsilon$ is not normalized by the norm of the envelop function. We use the following result from \citet{van2011local}:
\begin{theorem}[Theorem 2.1 of \citet{van2011local}]\label{thm:local-maximal-ineq}
    Let $\mathcal{F}$ be a collection of $P$-square integrable functions equipped with an envelop function $F \le 1$. If $\mathbb{E}_P f^2 \le t^2 \mathbb{E}_P F^2$, for every $f$ and some $t \in (0,1)$, then 
    \begin{align*}
        \E_P\, \left[\sup_{f \in \mathcal{F}}\, |\mathbb{G}_n f|\right] \lesssim J(t, \mathcal{F}, L_2)\left(1+ \frac{J(t, \mathcal{F}, L_2)}{t^2 \sqrt{n}\|F\|_{P,2}}\right) \|F\|_{P, 2}
    \end{align*}
    where the expectation should be regarded as an outer expectation (Chapter 1.2 of \citet{van1996weak}) when the content inside is not measurable. 
\end{theorem}
An analogous result under the bracketing entropy integral is also available:
\begin{theorem}[Theorem 2.14.17' of \citet{van1996weak}]\label{thm:local-maximal-ineq-bracket}
    Let $\mathcal{F}$ be a collection of $P$-square integrable functions equipped with an envelop function $F \le M$. If $\mathbb{E}_P f^2 \le t^2 \mathbb{E}_P F^2$, for every $f$ and some $t \in (0,1)$, then 
    \begin{align*}
        \E_P\, \left[\sup_{f \in \mathcal{F}}\, |\mathbb{G}_n f|\right] \lesssim J_{[\, ]}(t, \mathcal{F}, L_2(P))\left(1+ \frac{J_{[\, ]}(t, \mathcal{F}, L_2(P))}{t^2 \sqrt{n}}M\right) 
    \end{align*}
    where the expectation should be regarded as an outer expectation (Chapter 1.2 of \citet{van1996weak}) when the content inside is not measurable. 
\end{theorem}

\subsection{High-dimensional mean estimation}
% In this example, we take $m_{\theta}(z) := \|z-\theta\|^2$.
\begin{proof}[\bfseries{Proof of Theorem~\ref{thm:mean-ci-validity}}]
Throughout, we treat $\|\cdot\|\equiv\|\cdot\|_2$. We provide the sufficient condition under which $\Delta_{n,P}$ tends to zero as $n \longrightarrow \infty$. Observe that 
    \begin{align*}
        W_i &= m_{\widehat\theta_1}-m_{\theta(P)} - P(m_{\widehat\theta_1}-m_{\theta(P)})\\
        &= 2(X-\theta(P))^\top(\widehat\theta_1-\theta(P))\\
        &= 2t^\top (X-\theta(P))\|\widehat\theta_1-\theta(P)\|\quad \text{for} \quad t \in \mathbb{S}^{d-1}
    \end{align*}
    and $B^2 = \E_P[W_i^2] = 4\|\widehat\theta_1-\theta(P)\|^2 P(t^\top (X-\theta(P)))^2$. This is an example where the linearization in the form of \eqref{eq:qmd2} holds \textit{exactly}. In the context of Proposition~\ref{prop:first-order-linearization}, we can take $\varphi \equiv 0$ and $\delta \longrightarrow \infty$. Alternatively, by directly inspecting the upper bound in Lemma~\ref{prop:clt-valid}, we obtain
	% \begin{align}
	% 	\Delta_{n,P} &\le C \left ( \E_P[W_1^2 1\{W_1^2 > nS\}] S^{-1} +  n^{-1/2}\E_P[|W_1|^3 1\{W_1^2 \le  nS\}] S^{-3/2} \right)\label{eq:bentkus-result}
	% \end{align}
 	\begin{align*}
		\Delta_{n,P} &\le C_0 \E_P\left[\frac{W_1^2}{B^2} \left\{1 \wedge n^{-1/2}\frac{|W_1|}{B}\right\}\bigg|D_1\right] \\
  &=C_0  \E_P\left[\frac{\langle t, X-\theta(P)\rangle^2}{B_t^2} \left\{1 \wedge n^{-1/2}\frac{|\langle t, X-\theta(P)\rangle|}{B_t}\right\}\bigg|D_1\right] \\
  &\le C_0  \sup_{t\in\mathbb{S}^{d-1}}\,\E_P\left[\frac{\langle t, X-\theta(P)\rangle^2}{B_t^2} \left\{1 \wedge n^{-1/2}\frac{|\langle t, X-\theta(P)\rangle|}{B_t}\right\}\right] 
	\end{align*}
 where $B_t = \E_P\langle t, X-\theta(P)\rangle^2$
	for some universal constant $C_0 > 0$. Hence under the uniform Lindeberg condition on $X-\theta(P)$, we obtain $\sup_{P\in\mathcal{P}}\, \Delta_{n,P} \longrightarrow 0$ as $n \longrightarrow \infty$. This result does not require the consistency of the initial estimator. We conclude the claim in view of Theorem~\ref{thm:validity-BE}.
\end{proof}
\begin{proof}[\bfseries{Proof of Theorem~\ref{thm:mean-ci-width}}]
    Throughout, we treat $\|\cdot\|\equiv\|\cdot\|_2$. The proof proceeds by verifying conditions required for Theorem~\ref{thm:concentration-width-unbounded}. First, we check \ref{as:margin}. We observe for any $\theta \in \Theta$, 
    \begin{align*}
    m_{\theta}-m_{\theta(P)} := \|X-\theta\|^2 - \|X-\theta(P)\|^2 = 2(X-\theta)^\top(\theta-\theta(P)) + \|\theta-\theta(P)\|^2
\end{align*}
and $P(m_{\theta}-m_{\theta(P)}) =  \|\theta-\theta(P)\|^2$. Thus \ref{as:margin} holds (with an equality) with $\beta=1$ and $c_0=1$. Next, we check \ref{as:local-entropy}. For any $\theta$ such that $\|\theta-\theta(P)\| \le \delta$, we have 
    \begin{align*}
        \sup_{\|\theta-\theta(P)\| \le \delta}\, |\|X-\theta\|^2 - \|X-\theta(P)\|^2| &\le \sup_{\|\theta-\theta(P)\| \le \delta}\, 2|\big(X-\theta(P)\big)^\top (\theta(P)-\theta)| + \delta^2\\
        &= 2\delta \sup_{u \in \mathbb{S}^{d-1}}\,|u^\top (X-\theta(P))|  + \delta^2\\
        &= 2\delta \|X-\theta(P)\|  + \delta^2.
    \end{align*}
    \kt{\begin{align*}
        \sup_{\|\theta-\theta(P)\| \le \delta}\, |m_{\theta}-m_{\theta(P)} - P(m_{\theta}-m_{\theta(P)})| &\le \sup_{\|\theta-\theta(P)\| \le \delta}\, 2|\big(X-\theta(P)\big)^\top (\theta(P)-\theta)| \\
        &= 2\delta \sup_{u \in \mathbb{S}^{d-1}}\,|u^\top (X-\theta(P))|  \\
        &= 2\delta \|X-\theta(P)\|.
    \end{align*}}
   Hence, we obtain 
    \begin{align*}
    	\E_P \left[\sup_{\|\theta-\theta(P)\| < \delta}|\mathbb{G}_n (m_\theta - m_{\theta(P)})| \right]&\le \left(\E_P \sup_{\|\theta-\theta(P)\| < \delta}|m_{\theta}-m_{\theta(P)}|^2\right)^{1/2}\\
     &\le2\delta\left(\E_P\|X-\theta(P)\|^2\right)^{1/2} + 2\delta^2.
    \end{align*}
    \kt{\begin{align*}
    	\E_P \left[\sup_{\|\theta-\theta(P)\| < \delta}|\mathbb{G}_n (m_\theta - m_{\theta(P)})| \right]&\le n^{-1/2}\E_P \left[\left|\sum_{i=1}^n 2\delta \|X_i-\theta(P)\|\right| \right]\\
        &\le2\delta\left(\E_P\|X-\theta(P)\|^2\right)^{1/2}.
    \end{align*}}
    Similarly, we have 
    \begin{align*}
    P(m_{\theta}-m_{\theta(P)})^2 &\le 4\E_P|(X-\theta)^\top(\theta-\theta(P))|^2 + 2\|\theta-\theta(P)\|^4\\
    &\le 4\|\theta-\theta(P)\|^2\E_P\|X-\theta(P)\|^2  + 2\|\theta-\theta(P)\|^4.
\end{align*}
As a result, we can choose $\phi_n$ in \ref{as:local-entropy} as
\begin{align*}
    \phi_n(\delta) = 2\delta\left(\E_P\|X-\theta(P)\|^2\right)^{1/2} + 2\delta^2.
\end{align*}
\kt{\begin{align*}
    &\E_P \left[\sup_{\|\theta-\theta(P)\| < \delta}|\mathbb{G}_n (m_\theta - m_{\theta(P)})| \right] \vee \sqrt{P(m_{\theta}-m_{\theta(P)})^2}\\
    &\qquad \le 2\delta\left(\E_P\|X-\theta(P)\|^2\right)^{1/2} + \sqrt{2}\delta^2 = \phi_n(\delta).
\end{align*}}
For $\omega_n$ in \ref{as:square-process}, we invoke Lemma~\ref{prop:squared-Gn} in Section~\ref{sec:technical-lemma}.
From the earlier derivation, it is immediate that the local envelope can be defined as 
\begin{align*}
     M_\delta(x)= \sup_{\|\theta-\theta(P)\| \le \delta}\, |(m_{\theta}-m_{\theta(P)})(x)|\le  2\delta \|x-\theta(P)\|  + \delta^2.
\end{align*}
Lemma~\ref{prop:squared-Gn} implies 
\begin{align*}
    &\E_P\left[\sup_{\|\theta-\theta(P)\| < \delta}\, |\mathbb{G}_n(m_{\theta}-m_{\theta(P)} )^2|\right] \\
    &\qquad \le C\left\{ n^{1/2} \left(\mathbb{E}_P M_\delta^2 \right)+ \left(\mathbb{E}_PM_\delta^2\right)^{1/2}\E_P \left[\sup_{\|\theta-\theta(P)\| < \delta}\, \left|\sum_{i=1}^n \varepsilon_i (m_{\theta}-m_{\theta(P)})\right|\right]\right\}\\
    &\qquad \le C\left\{ n^{1/2} \left(\mathbb{E}_P M_\delta^2 \right)+ \left(n\mathbb{E}_PM_\delta^2\right)^{1/2}\delta\left(\E_P\|X-\theta(P)\|^2\right)^{1/2}\right\}\\
    &\qquad \le Cn^{1/2} \left(\delta^2 \E_P\|X-\theta(P)\|^2  + \delta^4\right).
\end{align*}
As a result, we can choose $\omega_n$ in \ref{as:square-process} as
\begin{align*}
    \omega_n(\delta) = \sqrt{Cn^{1/2} \left(\delta^2 \E_P\|X-\theta(P)\|^2  + \delta^4\right)}.
\end{align*}

It now remains the solve the inequalities in Theorem~\ref{thm:concentration-width-unbounded}. First,
\begin{align*}
    2r_n^{-1}\left(\E_P\|X-\theta(P)\|^2\right)^{1/2} \le n^{1/2} \implies r_n  \ge 2\left(\frac{\E_P\|X-\theta(P)\|^2}{n}\right)^{1/2} = 2\left(\frac{\mathrm{tr}(\Sigma)}{n}\right)^{1/2}.
\end{align*}
When $r_n \le 1$, this term dominates (up to a constant) and thus the inequality in \eqref{rq:define-rn} is satisfied as long as $\mathrm{tr}(\Sigma) \le n$. Similarly, we arrive at
\begin{align*}
    &u_n^{-2}\sqrt{Cn^{1/2} \left(u_n^2 \E_P\|X-\theta(P)\|^2  + u_n^4\right)} \le n^{3/4} \\
    &\qquad\implies u_n  \ge \left(\frac{C\E_P\|X-\theta(P)\|^2}{n}\right)^{1/2} = \left(\frac{C\mathrm{tr}(\Sigma)}{n}\right)^{1/2}
\end{align*}
assuming $\mathrm{tr}(\Sigma) \le n$. Thus by Theorem~\ref{thm:concentration-width-unbounded}, 
\begin{align*}
    &r_n^{2/(1+\beta)} + u_n^{2/(1+\beta)} +s_n^{1/(1+\beta)} = C\left\{\left(\frac{\mathrm{tr}(\Sigma) }{n}\right)^{1/2} +s_n^{1/2}\right\}.
\end{align*}
This concludes the first result.

Next, we assess the requirement for $s_n$ as defined in \ref{as:rate-initial-estimator}. First, for fixed $\widehat \theta_1$, we have
\begin{align*}
    \left(P(m_{\widehat\theta_1}-m_{\theta(P)})^2\right)^{1/2} &\le 2\left(\mathrm{tr}(\Sigma)\|\widehat\theta_1-\theta(P)\|^2\right)^{1/2}  + \left(2\|\widehat\theta_1-\theta(P)\|^4\right)^{1/2}.
\end{align*}
Assuming that $\mathbb{P}_P(\|\widehat\theta_1-\theta(P)\|^2 \ge C_\varepsilon \mathrm{tr}(\Sigma)/n) \le \varepsilon$, we choose $C_\varepsilon$ such that an event $\Omega := \{\|\widehat\theta_1-\theta(P)\|^2 < C_\varepsilon \mathrm{tr}(\Sigma)/n\}$ holds with probability greater than $1-\varepsilon/2$. Then, conditioning on $\Omega$, we have
\begin{align*}
    \E_P\|X-\widehat\theta_1\|^2 - \E_P\|X-\theta(P)\|^2 =  \|\widehat\theta_1-\theta(P)\|^2 \le \frac{C_1\mathrm{tr}(\Sigma)}{n},
\end{align*}
and this implies  
\begin{align*}
    s_n^{1/2} \le 2\left(\frac{\mathrm{tr}(\Sigma)\|\widehat\theta_1-\theta(P)\|^2}{n}\right)^{1/4}  + \left(\frac{2\|\widehat\theta_1-\theta(P)\|^4}{n}\right)^{1/4} + \left(\frac{C_1\mathrm{tr}(\Sigma)}{n}\right)^{1/2}
\end{align*}
with probability greater than $1-\varepsilon/2$. Thus as long as the initial estimation satisfies
\begin{align*}
    \|\widehat\theta_1-\theta(P)\|^2 \lesssim \frac{\mathrm{tr}(\Sigma)}{n} \quad \text{and} \quad \|\widehat\theta_1-\theta(P)\|^4 \lesssim \frac{\mathrm{tr}^2(\Sigma)}{n},
\end{align*}
in high probability, we can claim $ s_n^{1/2} =O_P( \sqrt{\mathrm{tr}(\Sigma)/n})$. In particular, the requirement of $\|\widehat\theta_1-\theta(P)\|^2 \lesssim \mathrm{tr}(\Sigma)/n$ in high probability suffices. To see this, we obtain the following from the first result of this theorem:
\begin{align*}
\mathbb{P}_P\left(\mathrm{Diam}_{\|\cdot\|}\big(\widehat{\mathrm{CI}}_{n,\alpha}^{\mathrm{mean}}\big)\le \mathfrak{C}\left\{\left(\frac{\mathrm{tr}(\Sigma)}{n}\right)^{1/2} + s_n^{1/2}\right\}\right) \ge 1-\varepsilon/2.
\end{align*}
Then, it follows that
\begin{align*}
&\mathbb{P}_P\left(\mathrm{Diam}_{\|\cdot\|}\big(\widehat{\mathrm{CI}}_{n,\alpha}^{\mathrm{mean}}\big)\le \mathfrak{C}\left\{\left(\frac{\mathrm{tr}(\Sigma)}{n}\right)^{1/2} + s_n^{1/2}\right\}\right) \\
&\qquad \le \mathbb{P}_P\left(\mathrm{Diam}_{\|\cdot\|}\big(\widehat{\mathrm{CI}}_{n,\alpha}^{\mathrm{mean}}\big)\le \mathfrak{C}\left\{\left(\frac{\mathrm{tr}(\Sigma)}{n}\right)^{1/2} + s_n^{1/2}\right\}\bigg| \Omega\right)\mathbb{P}_P(\Omega) + \mathbb{P}_P(\Omega^c) \\
&\qquad \le \mathbb{P}_P\left(\mathrm{Diam}_{\|\cdot\|}\big(\widehat{\mathrm{CI}}_{n,\alpha}^{\mathrm{mean}}\big)\le \mathfrak{C}\left\{\left(\frac{\mathrm{tr}(\Sigma)}{n}\right)^{1/2} + s_n^{1/2}\right\}\bigg| \Omega\right) + \frac{\varepsilon}{2}.
\end{align*}
On the event $\Omega$ for $n \ge C_\varepsilon$, it is implies that 
\begin{align*}
    \|\widehat\theta_1-\theta(P)\|^4 \le \mathrm{tr}(\Sigma)\|\widehat\theta_1-\theta(P)\|^2 \le \frac{C_\varepsilon \mathrm{tr}^2(\Sigma)}{n}
\end{align*}
hence the required probabilistic upper bound on $\|\widehat\theta_1-\theta(P)\|^4$ is implied. We thus conclude 
\begin{align*}
\mathbb{P}_P\left(\mathrm{Diam}_{\|\cdot\|}\big(\widehat{\mathrm{CI}}_{n,\alpha}^{\mathrm{mean}}\big)\le \mathfrak{C}\left(\frac{\mathrm{tr}(\Sigma)}{n}\right)^{1/2}\right) \ge 1-\varepsilon
\end{align*}
when the requirements for $\widehat \theta_1$ are satisfied.

% for some universal constant $C$, the second term does not dominate. To see the second condition, we have 
% \begin{align*}
%     \mathbb{P}_P(\|\widehat\theta_1-\theta(P)\|^2 > C_\varepsilon \mathrm{tr}^2(\Sigma)) \le \frac{C}{C_\varepsilon n \mathrm{tr}(\Sigma)}
% \end{align*}
% and thus with high probability, $\|\widehat\theta_1-\theta(P)\|^2 \le C_\varepsilon \mathrm{tr}^2(\Sigma)$, which concludes that 
% \begin{align*}
%     n^{-1/4}s_n^{1/2} \le  \frac{C_\varepsilon\mathrm{tr}(\Sigma)}{n}
% \end{align*}
% with probability at least $1-\varepsilon$.
\end{proof}

%  and 


% Hence we take $\phi(\delta) = 2\delta \E_P\|Z-\theta(P)\|$. Note that $\E_P\|Z-\theta(P)\| \le \sqrt{\sum_{j=1}^d \sigma^2_{jj}} \asymp \sqrt{d}$.

% \begin{align*}
%     M_\delta := \sup_{\|\theta-\theta(P)\| < \delta} |m_{\theta}-m_{\theta(P)}| &\le \sup_{\|\theta-\theta(P)\| < \delta}2|(Z-\theta)^\top(\theta-\theta(P))| + \delta^2\\
%     &\le 2\|Z-\theta(P)\| \delta + \delta^2
% \end{align*}
% and 
% \begin{align*}
%     \left(\E_P[M_\delta^2]\right)^{1/2} \le 2\delta \left(\E_P\|Z-\theta(P)\|^2\right)^{1/2} + 2\delta^2
% \end{align*}
% We also have 
% \begin{align*}
%     \omega_n(\delta) \le n^{1/2}\left(2\delta^2 \E_P\|Z-\theta(P)\|^2 + 2\delta^4\right) 
% \end{align*}

% \begin{align*}
%     r_n^{-2}\phi_n(r_n) \le n^{1/2} &\implies 2r_n^{-1} \E_P\|Z-\theta(P)\| \le n^{1/2}
% \end{align*}
% Thus we have $r_n \le \frac{\E_P\|Z-\theta(P)\|}{n^{1/2}}$

% % \begin{proof}[\bfseries{Proof of Proposition~\ref{prop:mean-ci}}]
% First, we observe that 
% \begin{align*}
% 	P(m_{\theta(P)}-m_{\widehat\theta_1}) &= \mathbb{E}_P[\|Z-\theta(P)\|_2^2-\|Z-\widehat{\theta}_1\|_2^2]\\
% 	&= \mathbb{E}_P[\|Z-\theta(P)\|_2^2-\|Z-\theta(P)+\theta(P)-\widehat{\theta}_1\|_2^2]\\
% 	&= \mathbb{E}_P[\|Z-\theta(P)\|_2^2-\|Z-\theta(P)\|_2^2-2(Z-\theta(P))^\top(\theta(P) - \widehat\theta_1)-\|\theta(P)-\widehat{\theta}_1\|_2^2]\\
% 	&= \mathbb{E}_P[-2(Z-\theta(P))^\top(\theta(P) - \widehat\theta_1)]-\|\theta(P)-\widehat{\theta}_1\|_2^2\\
% 	&= -\|\theta(P)-\widehat{\theta}_1\|_2^2.
% \end{align*}
% Hence, we have $U_{n,\alpha_2}(\theta(P), \widehat \theta_1; D_2) \equiv -\|\theta(P)-\widehat{\theta}_1\|_2^2$ with $\alpha_2=0$. 

% Next, denoting by $\overline Z_n$ the sample mean of the observations in $D_2$, we obtain
% \begin{align*}
% 	&\mathbb{P}_n(m_{\theta}-m_{\widehat{\theta}_1}) \\
% 	&\qquad = n^{-1}\sum_{i=1}^n[\|Z_i-\theta\|_2^2-\|Z_i-\widehat{\theta}_1\|_2^2] \\
% 	&\qquad= n^{-1}\sum_{i=1}^n[\| Z_i-\overline Z_n+\overline Z_n-\theta\|_2^2-\|Z_i-\overline Z_n+\overline Z_n-\widehat{\theta}_1\|_2^2] \\
% 	&\qquad= n^{-1}\sum_{i=1}^n 2\langle Z_i-\overline Z_n, \overline Z_n-\theta\rangle + \|\overline Z_n-\theta\|_2^2-2\langle Z_i-\overline Z_n, \overline Z_n-\widehat\theta_1\rangle -\|\overline Z_n-\widehat\theta_1\|_2^2\\
% 	&\qquad=  \|\overline Z_n-\theta\|_2^2-\|\overline Z_n-\widehat\theta_1\|_2^2\\
% 	&\qquad=  \|\overline Z_n-\theta\|_2^2-\|\overline Z_n-\theta+\theta-\widehat\theta_1\|_2^2\\
% 	&\qquad=  -2\langle \overline Z_n-\theta, \theta-\widehat\theta_1 \rangle -\|\theta-\widehat\theta_1\|_2^2.
% \end{align*}
% It also follows that 
% \begin{align*}
% 	\widehat \sigma^{2}_{\theta, \widehat\theta_1} &= n^{-1}\sum_{i=1}^n[\|Z_i-\theta\|_2^2-\|Z_i-\widehat{\theta}_1\|_2^2-\mathbb{P}_n(m_{\theta}-m_{\widehat{\theta}_1})]^2\\
% 	&= n^{-1}\sum_{i=1}^n[2\langle Z_i-\overline Z_n, \overline Z_n-\theta\rangle-2\langle Z_i-\overline Z_n, \overline Z_n-\widehat\theta_1\rangle]^2\\
% 	&= 4n^{-1}\sum_{i=1}^n\langle Z_i-\overline Z_n, \widehat\theta_1-\theta\rangle^2 = 4\|\widehat{\theta} - \theta\|_{\widehat \Sigma}^2
% 	\end{align*}
% where $\widehat \Sigma := n^{-1}\sum_{i=1}^n(Z_i-\overline Z_n)(Z_i-\overline Z_n)^\top$ and $\|x\|_A = \sqrt{x^\top A x}$. Hence, we conclude 
% 	\begin{align*}
%     \widehat{\mathrm{CI}}^{\mathrm{Mean}}_{n,\alpha} &:= \left\{\theta \in \mathbb{R}^d \, : \, \mathbb{P}_n(m_{\theta}-m_{\widehat \theta_1})\le n^{-1/2}z_{\alpha} \widehat\sigma_{\theta, \widehat\theta_1}+\big(0 \wedge U_{n,\alpha_2}(\theta, \widehat \theta_1; D_2)\right\}\\
%     &= \left\{\theta \in \mathbb{R}^d \, : \, -2\langle \overline Z_n-\theta, \theta-\widehat\theta_1 \rangle -\|\theta-\widehat\theta_1\|_2^2\le 2n^{-1/2}z_{\alpha} \|\widehat{\theta} - \theta\|_{\widehat \Sigma}-\|\theta-\widehat{\theta}_1\|_2^2\right\}\\
%     &= \left\{\theta \in \mathbb{R}^d \, : \, \langle \overline Z_n-\theta, \widehat\theta_1 -\theta\rangle \le n^{-1/2}z_{\alpha} \|\widehat{\theta} - \theta\|_{\widehat \Sigma}\right\}.
% \end{align*}
% This concludes the claim.
% \end{proof}
% \kt{Proof of validity}
% \begin{proof}
% First, we observe that 
% \begin{align*}
% 	W_i &= m_{\theta(P)}(Z_i) - m_{\widehat \theta_1}(Z_i) - P(m_{\theta(P)} - m_{\widehat \theta_1})\\
% 	&\qquad = \|Z_i-\theta(P)\|_2^2-\|Z_i-\widehat \theta\|_2^2-P(m_{\theta(P)}-m_{\widehat\theta_1})\\
% 	&\qquad = -2(Z_i-\theta(P))^\top(\theta(P) - \widehat\theta_1)-\|\theta(P)-\widehat \theta_1\|_2^2+\|\theta(P)-\widehat \theta_1\|_2^2\\
% 	&\qquad = -2(Z_i-\theta(P))^\top(\theta(P) - \widehat\theta_1).
% \end{align*}
% The random variable $W_i$ has mean zero and the variance is given by 
% \begin{align*}
%     P_0 W_i^2 = 4(\theta(P) - \widehat\theta_1)^\top \Sigma_P (\theta(P) - \widehat\theta_1)
% \end{align*}
% where $\Sigma$ is a covariance matrix. We verify the condition for the validity, which is 
% \begin{align*}
%     &\mathbb{E}_P\left[\frac{W_i^2}{4(\theta(P) - \widehat\theta_1)^\top \Sigma_P (\theta(P) - \widehat\theta_1)}\left\{1 \wedge n^{-1/2}\frac{|W_i|}{2\|\theta(P) - \widehat\theta_1\|_{\Sigma_P}}\right\}\right] \\
%     & \qquad\le \mathbb{E}_P\left[\sup_{\|t\|=1}\frac{t^\top (Z_i-\theta(P))  (Z_i-\theta(P))^\top t}{t^\top \Sigma_P t}\left\{1 \wedge n^{-1/2}\frac{|t^\top (Z_i-\theta(P))|}{\|t\|_{\Sigma_P}}\right\}\right]
% \end{align*}
% \end{proof}
% \begin{proof}[\bfseries{Proof of Proposition~\ref{prop:clt-valid}}]
%     We observe that 
% \begin{align*}
% 	&m_{\theta(P)} - m_{\widehat \theta_1} - P(m_{\theta(P)} - m_{\widehat \theta_1})\\
% 	&\qquad = \|Z-\theta(P)\|_2^2-\|Z-\widehat \theta\|_2^2-P(m_{\theta(P)}-m_{\widehat\theta_1})\\
% 	&\qquad = -2(Z-\theta(P))^\top(\theta(P) - \widehat\theta_1)-\|\theta(P)-\widehat \theta_1\|_2^2+\|\theta(P)-\widehat \theta_1\|_2^2\\
% 	&\qquad = -2(Z-\theta(P))^\top(\theta(P) - \widehat\theta_1)
% \end{align*}
% Thus the function $\dot m_{\theta(P)}$ in \ref{as:qmd+lindeberg} corresponds exactly with $Z\mapsto -2(Z-\theta(P))$. Hence under \ref{as:mean-est1}, Theorem~\ref{thm:validity-BE} implies for all $n > N_\varepsilon$ 
% \begin{align*}
%      &\mathbb{P}_P(\theta(P) \in \widehat{\mathrm{CI}}^{\mathrm{Mean}}_{n,\alpha}\mid D_1) \ge 1-\alpha-C\left(\varepsilon + \mathbf{1}\{\|\widehat\theta_1-\theta(P)\| \ge C_\varepsilon\}\right)\\
%      &\qquad \Longrightarrow\mathbb{P}_P(\theta(P) \in \widehat{\mathrm{CI}}^{\mathrm{Mean}}_{n,\alpha}) \ge 1-\alpha-C\left(\varepsilon + \mathbb{P}_P(\|\widehat\theta_1-\theta(P)\| \ge C_\varepsilon)\right)\\
%      &\qquad \Longrightarrow\inf_{P\in\mathcal{P}}\, \mathbb{P}_P(\theta(P) \in \widehat{\mathrm{CI}}^{\mathrm{Mean}}_{n,\alpha}) \ge 1-\alpha-C\left(\varepsilon + \sup_{P\in\mathcal{P}}\, \mathbb{P}_P(\|\widehat\theta_1-\theta(P)\| \ge C_\varepsilon)\right).
% \end{align*}
% We conclude the claim since the last term converges uniformly in probability in a sense that 
% \[\lim_{n\longrightarrow\infty}\, \sup_{P\in\mathcal{P}}\, \mathbb{P}_P(\|\widehat\theta_1-\theta(P)\| \ge C_\varepsilon)) = 0\]
% in view of \eqref{eq:uniform-convergence}. Derivation under \ref{as:mean-est2} is analogous by the result of Theorem~\ref{thm:validity-BE}.
% \end{proof}

% \begin{proof}[\bfseries{Proof of Proposition~\ref{prop:width-mean}}]
% Let $\theta := \widehat{\theta}_1 + h u \in\widehat{\mathrm{CI}}^{\mathrm{Mean}}_{n,\alpha}$ for $u \in \mathbb{S}^{d-1}$ and $h \in \mathbb{R}$. For such an element, it must hold that 
% 	\begin{align*}
% &\langle \overline Z_n-\theta, \widehat\theta_1 -\theta\rangle \le n^{-1/2}z_{\alpha} \|\widehat{\theta}_1 - \theta\|_{\widehat \Sigma}\\
% 		&\qquad \Longleftrightarrow (\widehat{\theta}_1 + h u-\overline{Z}_n)^\top hu\le n^{-1/2}z_{\alpha} |h|(u^\top \widehat \Sigma u)^{1/2}\\
% 		&\qquad \Longleftrightarrow (\widehat{\theta}_1 -\overline{Z}_n)^\top hu + h^2\le n^{-1/2}z_{\alpha} |h|(u^\top \widehat \Sigma u)^{1/2}.
% 	\end{align*}
% 	We now consider cases depending on the sign of $h$. When $h \ge 0$, we have 
% 	\begin{align*}
% 		&(\widehat{\theta}_1 -\overline{Z}_n)^\top hu + h^2\le n^{-1/2}z_{\alpha} |h|(u^\top \widehat \Sigma u)^{1/2} \\
% 		&\qquad \Longleftrightarrow  h\le n^{-1/2}z_{\alpha} (u^\top \widehat \Sigma u)^{1/2} - (\widehat{\theta}_1 -\overline{Z}_n)^\top u.
% 	\end{align*}
% 	By the assumption that $h \ge 0$, we arrive the upper bound 
% 	\begin{align*}
% 		h\le \left(n^{-1/2}z_{\alpha} (u^\top \widehat \Sigma u)^{1/2} - (\widehat{\theta}_1 -\overline{Z}_n)^\top u\right)_+
% 	\end{align*}
% 	where $(t)_+$ denotes $(t \vee 0)$. Similarly for $h \le 0$, the analogous derivation implies that 
% 	\begin{align*}
% 		h\ge -\left(n^{-1/2}z_{\alpha} (u^\top \widehat \Sigma u)^{1/2} + (\widehat{\theta}_1 -\overline{Z}_n)^\top u\right)_+.
% 	\end{align*}

% We define the width of the confidence set $\mathrm{CI}$ in the direction of $u$ as 
% \begin{align*}
%     \mathrm{Width}_u(\mathrm{CI}) := \sup_{\theta_1, \theta_2 \in \mathrm{CI}} |u^\top\theta_1-u^\top\theta_2|.
% \end{align*}
% Hence the width of the confidence set $\widehat{\mathrm{CI}}^{\mathrm{Mean}}_{n,\alpha}$ in the direction of $u$ is exactly given by 
% 	\begin{align*}
% 		\left(n^{-1/2}z_{\alpha} (u^\top \widehat \Sigma u)^{1/2} - (\widehat{\theta}_1 -\overline{Z}_n)^\top u\right)_+ + \left(n^{-1/2}z_{\alpha} (u^\top \widehat \Sigma u)^{1/2} + (\widehat{\theta}_1 -\overline{Z}_n)^\top u\right)_+.
% 	\end{align*}
	
% 	We can simplify the above display by observing that 
% 	\begin{align*}
% 		&\mathrm{Width}_u(\widehat{\mathrm{CI}}^{\mathrm{Mean}}_{n,\alpha}) \\
%   &\qquad := \begin{cases}
% 			2n^{-1/2}z_{\alpha} (u^\top \widehat \Sigma u)^{1/2} & \text{when $n^{-1/2}z_{\alpha} (u^\top \widehat \Sigma u)^{1/2} \ge |(\widehat{\theta}_1 -\overline{Z}_n)^\top u|$}\\
% 			n^{-1/2}z_{\alpha} (u^\top \widehat \Sigma u)^{1/2} + (\widehat{\theta}_1 -\overline{Z}_n)^\top u & \text{when $n^{-1/2}z_{\alpha} (u^\top \widehat \Sigma u)^{1/2} <(\widehat{\theta}_1 -\overline{Z}_n)^\top u$}\\
% 			n^{-1/2}z_{\alpha} (u^\top \widehat \Sigma u)^{1/2} - (\widehat{\theta} -\overline{Z}_n)^\top u & \text{when $n^{-1/2}z_{\alpha} (u^\top \widehat \Sigma u)^{1/2} < -(\widehat{\theta}_1 -\overline{Z}_n)^\top u$}
% 		\end{cases}.
% 	\end{align*}
% 	Simplifying the cases above, we obtain 
% 	\begin{align*}\mathrm{Width}_u(\widehat{\mathrm{CI}}^{\mathrm{Mean}}_{n,\alpha}) = n^{-1/2}z_{\alpha} (u^\top \widehat \Sigma u)^{1/2} + \left\{n^{-1/2}z_{\alpha} (u^\top \widehat \Sigma u)^{1/2} \vee |(\widehat{\theta}_1 -\overline{Z}_n)^\top u|\right\}.
% 	\end{align*}
% 	As a special case of $u \equiv e_j$, it implies 
% 	\begin{align*}
% 		\mathrm{Width}_{e_j}(\widehat{\mathrm{CI}}^{\mathrm{Mean}}_{n,\alpha}) = n^{-1/2}z_{\alpha} \widehat \Sigma_{jj}^{1/2} + \left\{n^{-1/2}z_{\alpha} \widehat \Sigma_{jj}^{1/2} \vee |\widehat{\theta}_{1,j} -\overline{Z}_{n,j}|\right\}
% 	\end{align*}
%  where $X_j$ denotes the $j$th coordinate when $X\in\mathbb{R}^d$ and $A_{jj}$ denotes the $j$th diagonal element when $A\in\mathbb{R}^{d\times d}$. Thus for any $\theta \in \widehat{\mathrm{CI}}^{\mathrm{Mean}}_{n,\alpha}$, it must hold that 
%  \begin{align*}
%      \|\theta-\widehat\theta_1\| &= \left(\sum_{j=1}^d e_j^\top|\theta-\widehat\theta_1|^2\right)^{1/2}\\
%      &\le \left(\sum_{j=1}^d \left|n^{-1/2}z_{\alpha} \widehat \Sigma_{jj}^{1/2} + \left\{n^{-1/2}z_{\alpha} \widehat \Sigma_{jj}^{1/2} \vee |\widehat{\theta}_{1,j} -\overline{Z}_{n,j}|\right\}\right|^2\right)^{1/2}\\
%      &\le \left(\sum_{j=1}^d \left|2n^{-1/2}z_{\alpha} (\widehat \Sigma_{jj}^{1/2}- \Sigma_{jj}^{1/2}+ \Sigma_{jj}^{1/2}) + |\widehat{\theta}_{1,j} -\overline{Z}_{n,j}|\right|^2\right)^{1/2}
%  \end{align*}
%  where $\Sigma:=\E_P(Z-\E_P[Z])(Z-\E_P[Z])^\top$. By triangle inequality, we conclude
%  \begin{align*}
%      &\|\theta-\widehat\theta_1\|\le 2n^{-1/2}z_{\alpha}\left(\sum_{j=1}^d(\widehat \Sigma_{jj}^{1/2}-\Sigma_{jj}^{1/2})^2\right)^{1/2}+2n^{-1/2}z_{\alpha}\left(\sum_{j=1}^d \Sigma_{jj}\right)^{1/2}+\|\widehat{\theta} - \overline{Z}_n\|_2.
%  \end{align*}
% 	% Let $w(\widehat{\textrm{CI}}^{\textrm{Mean}}_{n,\alpha})$ be a $d$-dimensional vector of width in each canonical basis, 
% 	% \begin{align}
% 	% 	w(\widehat{\textrm{CI}}^{\textrm{Mean}}_{n,\alpha}) := (\textrm{Width}_1(\widehat{\textrm{CI}}^{\textrm{Mean}}_{n,\alpha}), \ldots, \textrm{Width}_d(\widehat{\textrm{CI}}^{\textrm{Mean}}_{n,\alpha}))^\top
% 	% \end{align}
% 	% then 
% 	% \begin{align}
% 	% 	\|w(\widehat{\textrm{CI}}^{\textrm{Mean}}_{n,\alpha})\|_2 &= \left(\sum_{j=1}^d \textrm{Width}^2_j(\widehat{\textrm{CI}}^{\textrm{Mean}}_{n,\alpha}) \right)^{1/2}\\
% 	% &= \left(\sum_{j=1}^d \left( n^{-1/2}z_{\alpha} \widehat \Sigma_{jj}^{1/2} + \left\{n^{-1/2}z_{\alpha} \widehat \Sigma_{jj}^{1/2} \vee |\widehat{\theta}_j -\bar Z_j|\right\}\right)^2 \right)^{1/2}\\
% 	% &\le \left(\sum_{j=1}^d \left( 2n^{-1/2}z_{\alpha} (\widehat \Sigma_{jj}^{1/2}-\Sigma_{jj}^{1/2}+\Sigma_{jj}^{1/2}) + |\widehat{\theta}_j -\bar Z_j|\right)^2 \right)^{1/2}\\
% 	% &\le 2n^{-1/2}z_{\alpha}\left(\sum_{j=1}^d(\widehat \Sigma_{jj}^{1/2}-\Sigma_{jj}^{1/2})^2\right)^{1/2}+2n^{-1/2}z_{\alpha}\left(\sum_{j=1}^d \Sigma_{jj}\right)^{1/2}+\|\widehat{\theta} - \bar Z\|_2 
% 	% \end{align}
%  % by the triangle inequality.
% 	% \kt{Assuming $\sigma_j$ is bounded, we can show that the above inequality is $O_p(\sqrt{d/n} + \|\widehat{\theta} - \theta(P)\|_2 )$}
	
% 	% We also have that 
% 	% \begin{align}
% 	% 		\|w(\widehat{\textrm{CI}}^{\textrm{Mean}}_{n,\alpha})\|_\infty &= \max_{1\le j \le d} \, |\textrm{Width}_j(\widehat{\textrm{CI}}^{\textrm{Mean}}_{n,\alpha})|\\
% 	% &=  \max_{1\le j \le d}\,  \left|n^{-1/2}z_{\alpha} \widehat \Sigma_{jj}^{1/2} + \left\{n^{-1/2}z_{\alpha} \widehat \Sigma_{jj}^{1/2} \vee |\widehat{\theta}_j -\bar Z_j|\right\}\right|\\
% 	% &\le \max_{1\le j \le d}\, \left|2n^{-1/2}z_{\alpha} \widehat \Sigma_{jj}^{1/2} + |\widehat{\theta}_j -\bar Z_j|\right|\\
% 	% 	&\le 2n^{-1/2}z_{\alpha}\max_{1\le j \le d}\,|\widehat \Sigma_{jj}^{1/2} - \Sigma_{jj}^{1/2}| +2n^{-1/2}z_{\alpha}\max_{1\le j \le d}\,| \Sigma_{jj}^{1/2}|+\|\widehat{\theta} - \bar Z\|_\infty
% 	% \end{align}

% \end{proof}
% \begin{align}
% 	&\|Z-\theta(P)\|_2^2-\|Z-\widehat{\theta}_1\|_2^2-P(m_{\theta(P)}-m_{\widehat\theta_1})\\
% 	&\qquad = -2(Z-\theta(P))^\top(\theta(P) - \widehat\theta_1)-\|\theta(P)-\widehat{\theta}_1\|_2^2+-\|\theta(P)-\widehat{\theta}_1\|_2^2\\
% 	&\qquad = -2(Z-\theta(P))^\top(\theta(P) - \widehat\theta_1)
% \end{align}
%  \begin{align}
%      \mathbb{P}_P(\theta(P) \in \widehat{\textrm{CI}}^{\textrm{CLT}}_{n,\alpha}\mid D_1) \ge 1-\alpha_1-\alpha_2-C\left(\varepsilon + \mathbf{1}\{\|\widehat\theta_1-\theta(P)\| \ge C_\varepsilon\}\right)
%  \end{align}
%   where $C$ is a universal constant. 
% On the other hand, assuming \eqref{eq:lower-bound}, \eqref{eq:upper-bound} and  \ref{as:cond2}, 
%   \begin{align}
%      \mathbb{P}_P(\theta(P) \in \widehat{\textrm{CI}}^{\textrm{CLT}}_{n,\alpha}\mid D_1) \ge 1-\alpha_1-\alpha_2-C\left(\varepsilon +n^{-\delta/2}L^{2+\delta} + \mathbf{1}\{\|\widehat\theta_1-\theta(P)\| \ge C_\varepsilon\}\right).
%  \end{align}


% Therefore, we have the exact upper bound $U_n(\theta, \widehat\theta_1; D_2) = -\|\theta-\widehat{\theta}_1\|_2^2$ with $\alpha_2=0$. 


% Therefore, the confidence set is given by 
% \begin{align}
%     &\left\{\theta \in \Theta \, : \, \mathbb{P}_n(m_{\theta}-m_{\widehat{\theta}})\le n^{-1/2}z_{\alpha} \sigma_{\theta, \widehat\theta_1}+\big(0 \wedge U_n(\theta, \widehat{\theta}; D_2)\right\}\\
%     &\qquad =  \left\{\theta \in \Theta \, : \, -2\langle \overline Z_n-\theta, \theta-\widehat\theta_1 \rangle -\|\theta-\widehat\theta_1\|_2^2\le 2n^{-1/2}z_{\alpha} \|\widehat{\theta} - \theta\|_{\widehat \Sigma}-\|\theta(P)-\widehat{\theta}\|_2^2\right\}\\
%     &\qquad =  \left\{\theta \in \Theta \, : \, \langle \overline Z_n-\theta, \widehat\theta_1 - \theta\rangle \le n^{-1/2}z_{\alpha} \|\widehat{\theta} - \theta\|_{\widehat \Sigma}\right\}
% \end{align}




% \begin{align}
% 	&\|Z-\theta(P)\|_2^2-\|Z-\widehat{\theta}\|_2^2-P(m_{\theta(P)}-m_{\widehat\theta_1})\\
% 	&\qquad = -2(Z-\theta(P))^\top(\theta(P) - \widehat\theta_1)-\|\theta(P)-\widehat{\theta}\|_2^2+-\|\theta(P)-\widehat{\theta}\|_2^2\\
% 	&\qquad = -2(Z-\theta(P))^\top(\theta(P) - \widehat\theta_1)
% \end{align}
% Hence the function $\dot m_{\theta(P)}(Z) = -2(Z-\theta(P))$ satisfies to 

%It is without loss of generality to assume that $B_n^{-2} \sum_{i=1}^n\mathbb{E} X_i^2 \mathbf{1}\{X_i^2> B_n^2\}  \le 1/4$ since otherwise the below hold with $C > 4$ trivially. We thus have 
%\begin{align}
%	\delta_n &\le C\left (  \right) \\
%	&= C\left ( \sum_{i=1}^n \mathbb{E}[X_i^2 \mathbf{1}\{X_i^2 > B_n^2\}] B_n^{-2} +  \sum_{i=1}^n \mathbb{E}[|X_i|^3 \mathbf{1}\{X_i^2 \le  \varepsilon^2 B_n^2\}] B_n^{-3} + \sum_{i=1}^n \mathbb{E}[|X_i|^3 \mathbf{1}\{\varepsilon^2 B_n^2 < X_i^2 \le  B_n^2\}] B_n^{-3}\right)\\
%	&\le C\left ( \sum_{i=1}^n \mathbb{E}[X_i^2 \mathbf{1}\{X_i^2 > B_n^2\}] B_n^{-2} +  \varepsilon + \sum_{i=1}^n \mathbb{E}[|X_i|^2 B_n \mathbf{1}\{\varepsilon^2 B_n^2 < X_i^2 \le  B_n^2\}] B_n^{-3}\right)\\
%	&\le C\left ( \varepsilon + \sum_{i=1}^n \mathbb{E}[|X_i|^2 \mathbf{1}\{X_i^2 > \varepsilon^2 B_n^2 \}] B_n^{-2}\right)
%\end{align}
%
%An easier sufficient condition to deal with is 
%\begin{align}
%	\sum_{i=1}^n \mathbb{E}[X_i^2 \mathbf{1}\{X_i^2 > B_n^2\}] B_n^{-2} \le \sum_{i=1}^n \mathbb{E} \left[X_i^2 \frac{|X_i|^{\delta}}{B_n^{\delta}}\right] B_n^{-2} = \sum_{i=1}^n \mathbb{E}|X_i|^{2+\delta} B_n^{-(2+\delta)}
%\end{align}
%and 
%\begin{align}
%	\sum_{i=1}^n \mathbb{E}[|X_i|^3 \mathbf{1}\{X_i^2 \le  B_n^2\}] B_n^{-3} \le \sum_{i=1}^n \mathbb{E}|X_i|^{2+\delta} B_n^{-(2+\delta)}
%\end{align}
%Thus we have 
%\begin{align}
%	\delta_n \le C\sum_{i=1}^n \mathbb{E}|X_i|^{2+\delta} B_n^{-(2+\delta)}
%\end{align}
%We thus have two options. To get a Berry-Esseeen,
%%\begin{itemize}
%%	\item For some $\delta \in (0,1]$, we have $\mathbb{E}_{P_i}|X_i|^{2+\delta} < \infty$ for all distributions $\{P_i\}_{i=1}^n$.
%%\end{itemize}
%To get asymptotic control only, we need 
%\[\frac{\sum_{i=1}^n \mathbb{E}_i |X_i|^{2+\delta}}{(\sum_{i=1}^n \mathbb{E}_i |X_i|^{2})^{(2+\delta)/2}} = \left(\frac{(\sum_{i=1}^n \mathbb{E}_i |X_i|^{2+\delta})^{1/(2+\delta)}}{(\sum_{i=1}^n \mathbb{E}_i |X_i|^{2})^{1/2}}\right)^{2+\delta} \longrightarrow 0\]
%We note that under IID we have
%\[n^{-\delta/2}\left(\frac{(\mathbb{E} |Y|^{2+\delta})^{1/(2+\delta)}}{(\mathbb{E} |Y|^{2})^{1/2}}\right)^{2+\delta} \longrightarrow 0\]
%Hence, we need $L_{2+\delta}$-$L_2$ norm equivalence. 
\subsection{Misspecified linear regression}
% This section includes all proofs for the result presented in Section~\ref{sec:ols}.
\begin{proof}[\bfseries{Proof of Theorem~\ref{thm:LR-valid}}]
Throughout, we treat $\|\cdot\|\equiv\|\cdot\|_2$. First, observe that 
\begin{align*}
	W_i&=m_{\theta_P} - m_{\widehat \theta_1} - P(m_{\theta_P} - m_{\widehat \theta_1})\\
	& = (Y_i-\theta_P^\top X_i)^2-(Y_i-\widehat \theta_1^\top X_i)^2-P(m_{\theta_P}-m_{\widehat\theta_1})\\
	& = -2(Y_i-\theta_P^\top X)(\theta_P - \widehat\theta_1)^\top X-\{(\theta_P-\widehat \theta_1)^\top X_i\}^2+\E_P \{X_i^\top(\theta_P - \widehat \theta_1)\}^2.
	% &\qquad = -2(Y-\theta_P^\top X)(\theta_P - \widehat\theta)^\top X - \{(\theta_P-\widehat \theta)^\top X\}^2+\E \{X^\top(\theta_P - \widehat \theta)\}^2
\end{align*}
\textcolor{red}{
The uncentered R.V. $W'_i$
\begin{align*}
	W_i'&=m_{\theta_P} - m_{\widehat \theta_1}\\
	& = (Y_i-\theta_P^\top X_i)^2-(Y_i-\widehat \theta_1^\top X_i)^2\\
	& = -2(Y_i-\theta_P^\top X)(\theta_P - \widehat\theta_1)^\top X-\{(\theta_P-\widehat \theta_1)^\top X_i\}^2.
\end{align*}
Denoting $\widehat t := (\theta_P-\widehat \theta_1)$, we have 
\begin{align*}
	W_i'&=-\begin{bmatrix}
    2\xi_i, & X_i^\top \widehat t 
\end{bmatrix}\begin{bmatrix}
    X_i^\top \widehat t \\ X_i^\top \widehat t 
\end{bmatrix}
\end{align*}
and 
\begin{align*}
    \mathrm{Var}[W']
    &=  4\E[\xi_i^2({\widehat t}^\top X_i)^2] + \E[(\widehat t^\top X_i)^4] + 4\E[\xi_i(\widehat t^\top X_i)^3]-(\widehat t^\top  \Gamma_P \widehat t)^2.
\end{align*}
Can I find a sufficient condition for 
\begin{align*}
    \E_P\left[\frac{(W'-\mathbb{E}_P[W'])^2}{ \mathrm{Var}[W']} \min\left\{1, \frac{|W'-\mathbb{E}_P[W']|}{n^{1/2} (\mathrm{Var}[W'])^{1/2}}\right\}\, \bigg|\, \widehat t\right] = o_P(1)
\end{align*}
When $\|\widehat t\| = o_P(1)$, the same result from linear regression applies. We are interested in the case when $\|\widehat t\| = O_P(1)$. 
\begin{align*}
    \mathrm{Var}[W']
    &=  4\E[\xi_i^2({\widehat t}^\top X_i)^2] + \E[(\widehat t^\top X_i)^4] + 4\E[\xi_i(\widehat t^\top X_i)^3]-\E[(\widehat t^\top X_i)^2] \\
    & \ge 
\end{align*}
}
Taking $H := -2X(Y-\theta_P^\top X)$, the equation \eqref{eq:qmd2} corresponds to
    \begin{align*}
    &\frac{\E_P[m_{\widehat\theta_1} - m_{\theta_P} -P(m_{\widehat\theta_1}-m_{\theta_P})- \langle  \widehat\theta_1 - \theta_P, H \rangle ]^2}{\E_P \langle \widehat\theta_1-\theta_P, H \rangle^2 } \\
    &\qquad \le   \frac{\E_P\big[\{(\theta_P- \widehat\theta_1)^\top X\}^2+\E_P [\{X^\top(\theta_P -  \widehat\theta_1)\}^2] \big]^2}{4\E_P[\E_P[\xi_i^2|X_i](X^\top(\theta_P -  \widehat\theta_1))^2]} \\
    % &\qquad \le  \sigma_0^2\frac{P[\{(\theta_P- \widehat\theta_1)^\top X\}^4]+[P \{X^\top(\theta_P -  \widehat\theta_1)\} ]^4}{2\E_P[(X^\top(\theta_P -  \widehat\theta_1))^2]}\\
    &\qquad \le  \frac{\E_P[\{(\theta_P- \widehat\theta_1)^\top X\}^4]}{\underbar{$\sigma$}^2\E_P[\{(\theta_P- \widehat\theta_1)^\top X\}^2]}\le  \underbar{$\sigma$}^{-2}L^4 \|\theta_P- \widehat\theta_1\|^2\lambda_{\max}(\Gamma_P)
    \end{align*}
where the last inequality uses \ref{as:linreg-moment-covariate}. With the choice 
\begin{align*}
    \varphi(\|\theta_P-\widehat\theta_1\|) = \underbar{$\sigma$}^{-2}L^4 \lambda_{\max}(\Gamma_P)\|\widehat\theta_1-\theta_P\|^2,
\end{align*}
Proposition~\ref{prop:first-order-linearization} holds with $H :=-2X\xi$, which states that 
\begin{align*}
    \sup_{P\in\mathcal{P}}\, \Delta_{n,P} &\lesssim \underbar{$\sigma$}^{-2}L^4 \lambda_{\max}(\Gamma_P)\varepsilon^2 +\underbar{$\sigma$}^{-1}L^2 \lambda^{1/2}_{\max}(\Gamma_P)\varepsilon +  \sup_{P\in\mathcal{P}}\,\mathbb{P}_P(\|\widehat\theta_1 - \theta_P\| > \varepsilon) \\
    &\qquad + \sup_{P\in\mathcal{P}}\, \sup_{\|t\|=1}\,\E_P\left[\frac{\langle  t, 2X\xi \rangle^2}{\E_P\langle t, 2X\xi \rangle^2} \left\{1 \wedge n^{-1/2}\frac{|\langle  t, 2X\xi \rangle|}{\E_P\langle t, 2X\xi \rangle}\right\}\right].
    \end{align*}
Thus under the uniform Lindeberg condition on $X\xi$ and the assumptions stated in the theorem, we conclude $ \sup_{P\in\mathcal{P}}\, \Delta_{n,P} \longrightarrow 0$ by taking $n \longrightarrow \infty$ and then $\varepsilon \longrightarrow 0$. We conclude the claim in view of Theorem~\ref{thm:validity-BE}.
\end{proof}
\begin{proof}[\bfseries{Proof of Theorem~\ref{thm:LR-ci-width}}]Throughout, we treat $\|\cdot\|\equiv\|\cdot\|_2$.
We verify conditions required for Theorem~\ref{thm:concentration-width-unbounded}. First, we check \ref{as:margin}. We observe that 
\begin{align*}
    m_{\theta}-m_{\theta_P} = (Y-\theta^\top X)^2 - (Y-\theta_P^\top X)^2 &= 2(Y-\theta_P^\top X)(\theta_P^\top X-\theta^\top X) + (\theta_P^\top X-\theta^\top X)^2\\
    &= 2\xi X^{\top}(\theta_P - \theta) + ((\theta_P-\theta)^{\top}X)^2.
\end{align*}
Taking the expectation under $P$ and the fact that $\E_P(Y-\theta_P^\top X)X = \E_P[\xi X] = 0$, we obtain 
\begin{align*}
    P(m_{\theta}-m_{\theta_P}) = \E_P (\theta_P^\top X-\theta^\top X)^2  = \|\theta_P-\theta\|^2\E_P  u^\top(XX^\top)u
\end{align*}
for any $u \in \mathbb{S}^{d-1}$. By the assumption that the gram matrix (i.e., $\E_P(XX^\top)$) is invertible, its eigenvalue is bounded away from zero. Hence we have 
\begin{align*}
    P(m_{\theta}-m_{\theta_P}) \ge \lambda_{\min}(\Gamma_P) \|\theta_P-\theta\|^2,
\end{align*}
which implies that \ref{as:margin} is satisfied with $\beta=1$ and $c_0 = \lambda_{\min}(\Gamma_P)$. 
\textcolor{red}{
\begin{align*}
    P(m_{\theta}-m_{\theta_P}) = \E_P (\theta_P^\top X-\theta^\top X)^2  = \|\theta_P-\theta\|^2_{\Gamma_P}
\end{align*}
which implies that \ref{as:margin} is satisfied with $\beta=1$ and $c_0 = 1$. 
}
Next, we check \ref{as:local-entropy}. First, we note that 
\begin{align*}
    \sup_{\|\theta-\theta_P\|\le \delta} |(Y-\theta^\top X)^2 - (Y-\theta_P^\top X)^2| &\le \sup_{\|\theta-\theta_P\|\le \delta}\left\{2|\xi(\theta_P^\top X-\theta^\top X) | + |(\theta_P^\top X-\theta^\top X)^2|\right\}\\
    &\le \sup_{\|\theta-\theta_P\|\le \delta}\left\{2|(\theta_P-\theta)^\top \xi X |\right\} + \sup_{\|\theta-\theta_P\|\le \delta}\left\{|(\theta_P-\theta)^\top X|^2\right\}\\
    &= 2\delta\|\xi X\|+ \delta^2 \|XX^\top\|_{\mathrm{op}}.
    % &= 2\delta|\xi|\|X\| + \delta^2\|X\|^2.
\end{align*}
\textcolor{red}{
\begin{align*}
    &\sup_{\|\theta-\theta_P\|_{\Gamma_P}\le \delta} |(Y-\theta^\top X)^2 - (Y-\theta_P^\top X)^2| \\
    &\qquad \le \sup_{\|\theta-\theta_P\|_{\Gamma_P}\le \delta}\left\{2|\xi(\theta_P^\top X-\theta^\top X) | + |(\theta_P^\top X-\theta^\top X)^2|\right\}\\
    &\qquad \le \sup_{\|\theta-\theta_P\|_{\Gamma_P}\le \delta}\left\{2|(\theta_P-\theta)^\top \Gamma_P^{1/2}\Gamma_P^{-1/2}\xi X |\right\} + \sup_{\|\theta-\theta_P\|_{\Gamma_P}\le \delta}\left\{|(\theta_P-\theta)^\top \Gamma_P^{1/2}\Gamma_P^{-1/2}X|^2\right\}\\
    &\qquad = 2\delta\|\Gamma_P^{-1/2}\xi X\|+ \delta^2 \|\Gamma_P^{-1/2}XX^\top\Gamma_P^{-1/2}\|_{\mathrm{op}}.
    % &= 2\delta|\xi|\|X\| + \delta^2\|X\|^2.
\end{align*}
}
by the fact that the dual norm of $\|\cdot\|_2$ is itself. Here, $\|\cdot\|_{\mathrm{op}}$ denotes the operator norm. Note that the last expression can be taken as our local envelope function. It then follows that 
\begin{align*}
    \E_P \left[\sup_{\|\theta-\theta_P\| < \delta}|\mathbb{G}_n (m_\theta - m_{\theta_P})| \right] 
    &\le 2\E_P\left[\sup_{\|\theta-\theta_P\| < \delta}|\mathbb{G}_n[\xi X]^{\top}(\theta - \theta_P)|\right]\\ 
    &\quad+ \E_P\left[\sup_{\|\theta - \theta_P\| < \delta}|(\theta - \theta_P)^{\top}\mathbb{G}_n[XX^{\top}](\theta - \theta_P)|\right]\\
    &= 2\delta\E_P[\|\mathbb{G}_n[\xi X]\|] + \delta^2\E_P[\|\mathbb{G}_n[XX^{\top}]\|_{\mathrm{op}}].
    % 2\delta\left(\E_P \|\xi X\|^2\right)^{1/2} + 2^{1/2}\delta^2\left(\E_P\|X\|^4\right)^{1/2}.
\end{align*}
\textcolor{red}{
\begin{align*}
    &\E_P \left[\sup_{\|\theta-\theta_P\|_{\Gamma_P}< \delta}|\mathbb{G}_n (m_\theta - m_{\theta_P})| \right] 
    \\
    &\qquad\le 2\E_P\left[\sup_{\|\theta-\theta_P\|_{\Gamma_P} < \delta}|\mathbb{G}_n[\xi X]^{\top}\Gamma_P^{-1/2}\Gamma_P^{1/2}(\theta - \theta_P)|\right]\\ 
    &\qquad\qquad+ \E_P\left[\sup_{\|\theta - \theta_P\|_{\Gamma_P} < \delta}|(\theta - \theta_P)^{\top}\Gamma_P^{1/2}\Gamma_P^{-1/2}\mathbb{G}_n[XX^{\top}]\Gamma_P^{1/2}\Gamma_P^{-1/2}(\theta - \theta_P)|\right]\\
    &\qquad= 2\delta\E_P[\|\mathbb{G}_n[\Gamma_P^{-1/2}\xi X]\|] + \delta^2\E_P[\|\Gamma_P^{-1/2}\mathbb{G}_n[XX^{\top}]\Gamma_P^{-1/2}\|_{\mathrm{op}}].
\end{align*}
}
Observe that
\[
\mathbb{E}_P[\|\mathbb{G}_n[\xi X]\|] \le (\mathbb{E}[\|\mathbb{G}_n[\xi X]\|^2])^{1/2} \le (\mathbb{E}_P[|\xi|^2\|X\|^2])^{1/2} = \overline{\sigma}(\mbox{tr}(\Gamma_P))^{1/2}.\]
\textcolor{red}{
\begin{align*}
\mathbb{E}_P[\|\mathbb{G}_n[\Gamma_P^{-1/2}\xi X]\|] &\le (\mathbb{E}[\|\mathbb{G}_n[\xi \Gamma_P^{-1/2}X]\|^2])^{1/2} \\
&\le (\mathbb{E}_P[|\xi|^2\|\Gamma_P^{-1/2}X\|^2])^{1/2} = \overline{\sigma}(\mbox{tr}(\Gamma_P^{-1/2}\Gamma_P\Gamma_P^{-1/2}))^{1/2}=\overline{\sigma}d^{1/2}.
\end{align*}
}
% \kt{
% Let $u = (u_*^\top \Gamma_P^{-1}u_*)^{-1/2}\Gamma_P^{-1/2}u_*$ (This satisfies $\|u\|^2=(u_*^\top \Gamma_P^{-1}u_*)^{-1} u_*^\top\Gamma_P^{-1}u_*=1$)
% \begin{align*}
%     \mathbb{E}_P\left[\sup_{\|u\|\le 1}\frac{|u^\top \xi X |}{u^\top \Gamma_P u} \right]&=\mathbb{E}_P\left[\sup_{\|u_*\|\le 1}\frac{(u_*^\top \Gamma_P^{-1}u_*)^{-1/2}|u_*^\top \xi \Gamma_P^{-1/2}X |}{ (u_*^\top \Gamma_P^{-1}u_*)^{-1}u_*^\top \Gamma_P^{-1/2}\Gamma_P \Gamma_P^{-1/2}u_*} \right]\\&= \mathbb{E}_P\left[\sup_{\|u_*\|\le 1}(u_*^\top \Gamma_P^{-1}u_*)^{1/2}|u_*^\top \xi \Gamma_P^{-1/2}X |\right]\le\overline{\sigma}\|\Gamma_P^{-1/2}\|\big(\E_P\| \Gamma_P^{-1/2}X\|^2\big)^{1/2}
%     % \\&= \overline{\sigma}\|\Gamma_P^{-1/2}\|\big(\E_P\Gamma_P^{-1/2}XX^\top \Gamma_P^{-1/2}\big)^{1/2} = \overline{\sigma}\sqrt{\sum_{j=1}^d e_j^\top \Gamma_P^{-1}e_j } = \overline{\sigma}\mathrm{tr}^{1/2}(\Gamma_P^{-1})
% \end{align*}
% }
% {\color{red}You would have to apply Theorem I of~\url{https://arxiv.org/pdf/1506.04711} to bound the second term on the right hand side.}
From Theorem I of~\cite{tropp2016expected}, we get
\begin{equation}
\mathbb{E}_P[\|\mathbb{G}_n[XX^{\top}]\|_{\mathrm{op}}] \le C\sqrt{\log(d)v(X)} + C\frac{\log(d)}{n^{1/2}}\left(\mathbb{E}[\max_{1\le i\le n}\|X_i\|^4]\right)^{1/2},\label{eq:matrix-bernstein}
\end{equation}
\textcolor{red}{
\begin{equation}
\mathbb{E}_P[\|\mathbb{G}_n[\Gamma_P^{-1/2}XX^{\top}\Gamma_P^{-1/2}]\|_{\mathrm{op}}] \le C\sqrt{\log(d)v(X)} + C\frac{\log(d)}{n^{1/2}}\left(\mathbb{E}[\max_{1\le i\le n}\|\Gamma_P^{-1/2}X_i\|^4]\right)^{1/2}
\end{equation}
}
for some universal constant $C$. Here
\[
v(X) = \left\|\frac{1}{n}\sum_{i=1}^n \mathbb{E}\left[(X_iX_i^{\top} - \Gamma_P)(X_iX_i^{\top}-\Gamma_P)\right]\right\|_{\mathrm{op}}.
\]
We bound two terms of the upper bound in \eqref{eq:matrix-bernstein}. 
For the second term, we observe
\begin{align*}\left(\mathbb{E}[\max_{1\le i\le n}\|X_i\|^4]\right)^{1/2} &\le \left(\mathbb{E}\left[\max_{1\le i\le n}\|X_i\|^{q_x}\right]\right)^{2/q_x} \le n^{2/q_x}\left(\mathbb{E}[\|X_i\|^{q_x}]\right)^{2/q_x}\\
&= n^{2/q_x}\left(\mathbb{E}[\sum_{j=1}^d (e_j^\top X_i)^{q_x}]\right)^{2/q_x} \le n^{2/q_x}d^{2/q_x}L^2\lambda_{\max}(\Gamma_P).
\end{align*}
\textcolor{red}{
\begin{align*}\left(\mathbb{E}[\max_{1\le i\le n}\|\Gamma_P^{-1/2}X_i\|^4]\right)^{1/2} &\le \left(\mathbb{E}\left[\max_{1\le i\le n}\|\Gamma_P^{-1/2}X_i\|^{q_x}\right]\right)^{2/q_x} \le n^{2/q_x}\left(\mathbb{E}[\|\Gamma_P^{-1/2}X_i\|^{q_x}]\right)^{2/q_x}\\
&= n^{2/q_x}\left(\mathbb{E}[\sum_{j=1}^d (e_j^\top \Gamma_P^{-1/2}X_i)^{q_x}]\right)^{2/q_x} \le n^{2/q_x}d^{2/q_x}L^2.
\end{align*}
where the last step follows by the similar assumption as 
Assumption 2.c of \citet{chang2023inference}.
}
where the last step follows by \ref{as:linreg-moment-covariate}. Next, we observe
\begin{align*}
    \mathbb{E}\left[(X_iX_i^{\top} - \Gamma_P)(X_iX_i^{\top}-\Gamma_P)\right] &= \mathbb{E}\left[X_iX_i^{\top}X_iX_i^{\top} - \Gamma_PX_iX_i^{\top} -X_iX_i^{\top}\Gamma_P + \Gamma_P^2\right]\\
    & = \mathbb{E}\left[\|X_i\|^2X_iX_i^{\top} - \Gamma_P^2\right].
\end{align*}
\textcolor{red}{
\begin{align*}
    &\mathbb{E}\left[(\Gamma_P^{-1/2}X_iX_i^{\top}\Gamma_P^{-1/2} - I_d)(\Gamma_P^{-1/2}X_iX_i^{\top}\Gamma_P^{-1/2}-I_d)\right] \\
    &\qquad = \mathbb{E}\left[\Gamma_P^{-1/2}X_iX_i^{\top}\Gamma_P^{-1/2}\Gamma_P^{-1/2}X_iX_i^{\top}\Gamma_P^{-1/2} - 2\Gamma_P^{-1/2}X_iX_i^{\top}\Gamma_P^{-1/2} + I_d\right]\\
    &\qquad = \mathbb{E}\left[\|\Gamma_P^{-1/2}X_i\|^2\Gamma_P^{-1/2}X_iX_i^{\top} \Gamma_P^{-1/2}- I_d\right].
\end{align*}
}
The operator norm can be controlled as
\begin{align*}
    \left\|\frac{1}{n}\sum_{i=1}^n \mathbb{E}\left[(X_iX_i^{\top} - \Gamma_P)(X_iX_i^{\top}-\Gamma_P)\right]\right\|_{\mathrm{op}} &\le \frac{1}{n}\sum_{i=1}^n \left\|\mathbb{E}\left[(X_iX_i^{\top} - \Gamma_P)(X_iX_i^{\top}-\Gamma_P)\right]\right\|_{\mathrm{op}}\\
    &= \frac{1}{n}\sum_{i=1}^n \sup_{\|u\|=1}| \mathbb{E}\left[\|X\|^2|u^\top X_i|^2\right] - u^\top\Gamma_P^2u|\\
    &\le \frac{1}{n}\sum_{i=1}^n \sup_{\|u\|=1}\sqrt{ \mathbb{E}\|X\|^4\mathbb{E}|u^\top X_i|^4}\\
    &\le dL^4\lambda_{\max}^2(\Gamma_P),
\end{align*}
\textcolor{red}{
\begin{align*}
    &\left\|\frac{1}{n}\sum_{i=1}^n \mathbb{E}\left[(\Gamma_P^{-1/2}X_iX_i^{\top}\Gamma_P^{-1/2} - I_d)(\Gamma_P^{-1/2}X_iX_i^{\top}\Gamma_P^{-1/2}-I_d)\right]\right\|_{\mathrm{op}}\\
    &\qquad \le \frac{1}{n}\sum_{i=1}^n \left\|\mathbb{E}\left[(\Gamma_P^{-1/2}X_iX_i^{\top}\Gamma_P^{-1/2} - I_d)(\Gamma_P^{-1/2}X_iX_i^{\top}\Gamma_P^{-1/2}-I_d)\right]\right\|_{\mathrm{op}}\\
    &\qquad= \frac{1}{n}\sum_{i=1}^n \sup_{\|u\|=1}| \mathbb{E}\left[\|\Gamma_P^{-1/2}X_i\|^2|u^\top \Gamma_P^{-1/2}X_i|^2\right] - u^\top I_du|\\
    &\qquad\le \frac{1}{n}\sum_{i=1}^n \sup_{\|u\|=1}\sqrt{ \mathbb{E}\|\Gamma_P^{-1/2}X\|^4\mathbb{E}|u^\top \Gamma_P^{-1/2}X_i|^4}\le dL^4,
\end{align*}
}
where the last step follows by \ref{as:linreg-moment-covariate} since $q_x \ge 4$. We thus obtain
\begin{align*}
\mathbb{E}_P[\|\mathbb{G}_n[XX^{\top}]\|_{\mathrm{op}}] &\le C\sqrt{d \log d}L^2\lambda_{\max}(\Gamma_P) + C\frac{d^{2/q_x} \log d}{n^{1/2 - 2/q_x}}L^2\lambda_{\max}(\Gamma_P).
\end{align*}
\textcolor{red}{
\begin{align*}
\mathbb{E}_P[\|\mathbb{G}_n[\Gamma_P^{-1/2}XX^{\top}\Gamma_P^{-1/2}]\|_{\mathrm{op}}]&\le C\sqrt{d \log d}L^2 + C\frac{d^{2/q_x} \log d}{n^{1/2 - 2/q_x}}L^2.
\end{align*}
}
From the earlier derivation, it also follows that 
\begin{align*}
    P(m_{\theta}-m_{\theta_P})^2 &\le 4\E_P|\xi(\theta_P^\top X-\theta^\top X) |^2 + 2 \E_P|(\theta_P-\theta)^\top X|^4  \\
    &\le 4\|\theta_P-\theta\|^2\sup_{u\in\mathbb{S}^{d-1}}\,\E_P |u^\top \xi X|^2 + 2\|\theta_P-\theta\|^4\sup_{u\in\mathbb{S}^{d-1}}\, \E_P  (u^\top X)^4 \\
    &\le 4\|\theta_P-\theta\|^2\E_P \|\xi X\|^2 + 2\|\theta_P-\theta\|^4 L^4 \lambda^2_{\max}(\Gamma_P).
\end{align*}
\textcolor{red}{\begin{align*}
    P(m_{\theta}-m_{\theta_P})^2 &\le 4\E_P|\xi(\theta_P^\top X-\theta^\top X) |^2 + 2 \E_P|(\theta_P-\theta)^\top X|^4  \\
    &\le 4\|\theta_P-\theta\|_{\Gamma_P}^2\sup_{u\in\mathbb{S}^{d-1}}\,\E_P |u^\top \xi \Gamma_P^{-1/2}X|^2 + 2\|\theta_P-\theta\|_{\Gamma_P}^4\sup_{u\in\mathbb{S}^{d-1}}\, \E_P  (u^\top \Gamma_P^{-1/2}X)^4 \\
    &\le 4\|\theta_P-\theta\|_{\Gamma_P}^2\E_P \|\xi\Gamma_P^{-1/2} X\|^2 + 2\|\theta_P-\theta\|_{\Gamma_P}^4 L^4.
\end{align*}}
Hence, we can take 
\begin{align*}
    \phi(\delta) = C\overline{\sigma}\left(\mathrm{tr}(\Gamma_P)\right)^{1/2} \delta+ CL^2\lambda_{\max}(\Gamma_P)\delta^2\sqrt{d\log d}\left[1 + \frac{d^{2/q_x-1/2}\sqrt{ \log d}}{n^{1/2 - 2/q_x}}\right]
\end{align*}
\textcolor{red}{\begin{align*}
    \phi(\delta) = C\overline{\sigma}d^{1/2} \delta+ CL^2\delta^2\sqrt{d\log d}\left[1 + \frac{d^{2/q_x-1/2}\sqrt{ \log d}}{n^{1/2 - 2/q_x}}\right]
\end{align*}}
in \ref{as:local-entropy}. The first term dominates when 
\begin{align*}
    &\overline{\sigma}\left(\mathrm{tr}(\Gamma_P)\right)^{1/2} \delta \ge \sqrt{d\log d}L^2\lambda_{\max}(\Gamma_P)\delta^2\left[1 + \sqrt{\frac{\log d}{(nd)^{1 - 4/q_x}}}\right]\\&\qquad\Rightarrow \delta \le \left(\frac{\overline{\sigma}\left(\mathrm{tr}(\Gamma_P)\right)^{1/2}}{L^2\lambda_{\max}(\Gamma_P)}\right)\left(\frac{1}{\sqrt{d\log d}(1 + \sqrt{\log d/(nd)^{1 - 4/q_x}})}\right)\\&\qquad\Rightarrow \delta \le \left(\frac{\overline{\sigma}}{L^2\lambda^{1/2}_{\max}(\Gamma_P)}\right)\left(\frac{(nd)^{1/2 - 2/q_x}}{\log d}\right) = \mathfrak{C}_P\left(\frac{(nd)^{1/2 - 2/q_x}}{\log d}\right)
\end{align*}
\textcolor{red}{
\begin{align*}
    &\overline{\sigma}d^{1/2} \delta \ge \sqrt{d\log d}L^2\delta^2\left[1 + \sqrt{\frac{\log d}{(nd)^{1 - 4/q_x}}}\right]\\&\qquad\Rightarrow \delta \le \left(\frac{\overline{\sigma}d^{1/2}}{L^2}\right)\left(\frac{1}{\sqrt{d\log d}(1 + \sqrt{\log d/(nd)^{1 - 4/q_x}})}\right)\\&\qquad\Rightarrow \delta \le \frac{\overline{\sigma}}{L^2}\left(\frac{(nd)^{1/2 - 2/q_x}}{\log d}\right) = \mathfrak{C}_P\left(\frac{(nd)^{1/2 - 2/q_x}}{\log d}\right)
\end{align*}
}
where $\mathfrak{C}_P = \overline{\sigma}/(L^2\lambda^{1/2}_{\max}(\Gamma_P))$. \textcolor{red}{$\mathfrak{C}_P = \overline{\sigma}/L^2$.}
We verify this condition at the end for the choice of $\delta$. Provided that $\delta$ satisfies this inequality, we can take $\phi(\delta) = 2C\overline{\sigma}\left(\mathrm{tr}(\Gamma_P)\right)^{1/2} \delta$. \textcolor{red}{$\phi(\delta) = C\overline{\sigma}d^{1/2} \delta$.}

% {\color{red}You can bound the right hand side in terms of the dimension and $L$. You cannot get a dimension-free bound, as far as I can tell. Also, once we assume the minimum eigenvalue of $\Gamma_P$ as non-zero, the result is not dimension-free because it constraints the dimension to be no larger than $n$.}
% We can bound 

% {\color{red}\bf This inequality is wrong, you are taking the supremum out of the expected value.} We thus obtain 
% \begin{align*}
%     \E_P \left[\sup_{\|\theta-\theta_P\| < \delta}|\mathbb{G}_n (m_\theta - m_{\theta_P})| \right]&\le 2\delta\left(\E_P \|\xi X\|^2\right)^{1/2} + 2^{1/2}L^2 \lambda_{\max}(\Gamma_P)\delta^2.
% \end{align*}
Finally, we verify \ref{as:square-process} by invoking Lemma~\ref{prop:squared-Gn}. The local envelope is defined as 
\begin{align*}
     M_\delta(x)= \sup_{\|\theta-\theta(P)\| \le \delta}\, |(m_{\theta}-m_{\theta(P)})(x)|\le   2\delta\|\xi X\|+ \delta^2 \|X\|^2,
\end{align*}
\textcolor{red}{\begin{align*}
     M_\delta(x)= \sup_{\|\theta-\theta(P)\|_{\Gamma_P} \le \delta}\, |(m_{\theta}-m_{\theta(P)})(x)|\le   2\delta\|\Gamma_P^{-1/2}\xi X\|+ \delta^2 \|\Gamma_P^{-1/2}XX^\top \Gamma_P^{-1/2}\|_{\mathrm{op}},
\end{align*}}
and 
\begin{align*}
    \E_PM_\delta^2 \le 4\delta^2\E_P\|\xi X\|^2+ 2\delta^4 \E_P\|XX^\top\|^2_{\mathrm{op}}.
\end{align*}
\textcolor{red}{
\begin{align*}
    \E_PM_\delta^2 \le 4\delta^2\E_P\|\Gamma_P^{-1/2}\xi X\|^2+ 2\delta^4 \E_P\|\Gamma_P^{-1/2}XX^\top\Gamma_P^{-1/2}\|^2_{\mathrm{op}}.
\end{align*}
}
From assumption~\ref{as:linreg-moment-covariate} and the earlier derivation,
\[
\E_P\|XX^\top\|^2_{\mathrm{op}}\le C\left(d \log dL^4\lambda^2_{\max}(\Gamma_P) + d^{4/q_x} (\log d)^2L^4\lambda^2_{\max}(\Gamma_P)\right)
\]
\textcolor{red}{
\[
\E_P\|\Gamma_P^{-1/2}XX^\top\Gamma_P^{-1/2}\|^2_{\mathrm{op}}\le C\left(d \log dL^4 + d^{4/q_x} (\log d)^2L^4\right)
\]
}
% A similar application of Theorem I of~\cite{tropp2016expected} implies
% \begin{align*}
% \E_P\|XX^\top\|^2_{\mathrm{op}} &\le 2C\log(d)v(X) + 2C\log^2(d)\mathbb{E}\|X\|^4 \\
% &\le 2C\log(d)d^{1/2}L^4\lambda_{\max}^2(\Gamma_P) + 2C\log^2(d)dL^4\lambda^2_{\max}(\Gamma_P)\\
% &\le  2C\log^2(ed)dL^4\lambda^2_{\max}(\Gamma_P)\label{eq:matrix-bernstein2}
% \end{align*}
By Lemma~\ref{prop:squared-Gn}, 
\begin{align*}
    \omega^2_n(\delta)& \le Cn^{1/2} \left\{  \delta^2\overline{\sigma}^2\mbox{tr}(\Gamma_P)+\delta^4(\log d)^2dL^4\lambda^2_{\max}(\Gamma_P)\right.\\
&\qquad\left.+\delta\overline{\sigma}\mbox{tr}^{1/2}(\Gamma_P)\phi(\delta) +\delta^2(\log d)d^{1/2}L^2\lambda_{\max}(\Gamma_P)\phi(\delta)\right\}\\
& \le Cn^{1/2} \left\{  \delta^2\overline{\sigma}^2\mbox{tr}(\Gamma_P)+\delta\overline{\sigma}\mbox{tr}^{1/2}(\Gamma_P)\phi(\delta) \right\}\\
& \le 2Cn^{1/2}  \delta^2\overline{\sigma}^2\mbox{tr}(\Gamma_P)
\end{align*}
\textcolor{red}{\begin{align*}
    \omega^2_n(\delta)& \le Cn^{1/2} \left\{  \delta^2\overline{\sigma}^2d+\delta^4(\log d)^2dL^4+\delta\overline{\sigma}d^{1/2}\phi(\delta) +\delta^2(\log d)d^{1/2}L^2\phi(\delta)\right\}\\
& \le Cn^{1/2} \left\{  \delta^2\overline{\sigma}^2d+\delta\overline{\sigma}d^{1/2}\phi(\delta) \right\}\\
& \le 2Cn^{1/2}  \delta^2\overline{\sigma}^2d
\end{align*}}
where the second and third lines follow provided that $\mathfrak{C}_P (nd)^{1/2-2/q_x}\log^{-1}(d)\ge\delta$.
It thus remains to solve equations \eqref{rq:define-rn-un} to derive the convergence rate. First, recalling that $\beta=1$ and $c_0 = \lambda_{\min}(\Gamma_P)$ \textcolor{red}{$c_0 = 1$}, we have 
\begin{align*}
    &C\overline{\sigma}\lambda^{-1/2}_{\min}(\Gamma_P)\left(\mathrm{tr}(\Gamma_P)\right)^{1/2} r_n^{-1} \le n^{1/2}
     \Longleftrightarrow r_n \ge C\overline{\sigma}\lambda^{-1/2}_{\min}(\Gamma_P)\left(\mathrm{tr}(\Gamma_P)/n\right)^{1/2}
\end{align*}
\textcolor{red}{\begin{align*}
    &C\overline{\sigma}d^{1/2} r_n^{-1} \le n^{1/2}
     \Longleftrightarrow r_n \ge C\overline{\sigma}\left(d/n\right)^{1/2}
\end{align*}}
and 
\begin{align*}
&C\overline{\sigma}\lambda^{-1/2}_{\min}(\Gamma_P)\left(\mathrm{tr}(\Gamma_P)\right)^{1/2} u_n^{-1} \le n^{1/2}
     \Longleftrightarrow u_n \ge C\overline{\sigma}\lambda^{-1/2}_{\min}(\Gamma_P)\left(\mathrm{tr}(\Gamma_P)/n\right)^{1/2}.
\end{align*}
\textcolor{red}{\begin{align*}
    &C\overline{\sigma}d^{1/2} u_n^{-1} \le n^{1/2}
     \Longleftrightarrow u_n \ge C\overline{\sigma}\left(d/n\right)^{1/2}
\end{align*}}
Finally, we verify $r_n, u_n \le \mathfrak{C}_P (nd)^{1/2-2/q_x}\log^{-1}(d)$. This is satisfied when 
\begin{align*}
&\overline{\sigma}\lambda^{-1/2}_{\min}(\Gamma_P)\left(\mathrm{tr}(\Gamma_P)/n\right)^{1/2} \le \mathfrak{C}_P (nd)^{1/2-2/q_x}\log^{-1}(d) \\
&\qquad \Rightarrow \left(L^2\lambda_{\max}(\Gamma_P) \lambda_{\min}^{-1}(\Gamma_P)d^{2/q_x}\log(d)\right)^{q_x/(q_x-2)}\le n.
\end{align*}
\textcolor{red}{
\begin{align*}
&\overline{\sigma}\left(d/n\right)^{1/2} \le \mathfrak{C}_P (nd)^{1/2-2/q_x}\log^{-1}(d)\Rightarrow \left(L^2d^{2/q_x}\log(d)\right)^{q_x/(q_x-2)}\le n.
\end{align*}
}
Thus the inequality in \eqref{rq:define-rn-un} is satisfied when $n \ge \left(L^2\lambda_{\max}(\Gamma_P) \lambda_{\min}^{-1}(\Gamma_P)d^{2/q_x}\log(d)\right)^{q_x/(q_x-2)}$. \textcolor{red}{$n \ge \left(L^2d^{2/q_x}\log(d)\right)^{q_x/(q_x-2)}$} We note from the fact that $q_x \ge 4$, we can derive the condition under the least-favorable case, which is $n \ge L^4\lambda^2_{\max}(\Gamma_P)\lambda_{\min}^{-2}(\Gamma_P)d (\log d)^2$ \textcolor{red}{$n \ge L^2d (\log d)^2$}. As $q_x \to \infty$, we have $n \ge L^2\lambda_{\max}(\Gamma_P)\lambda_{\min}^{-1}(\Gamma_P) (\log d)$. However the assumption $\lambda_{\min}(\Gamma_P) \ge \underbar{$\lambda$} > 0$ still requires $n \ge d$.
% Furthermore, we have 
% \begin{align*}
%     \E_P \|\xi X\|^2 &= \E_P \lef t[\xi^2 \sum_{j=1}^d (e_j^\top X_j)^2\right]  \\
%     &= \E_P \left[ \sum_{j=1}^d (e_j^\top X_j)^2\E_P\left[\xi^2 \mid X_1,\ldots, X_n\right]\right]\le \overline{\sigma}^2 \E_P \left[ \sum_{j=1}^d (e_j^\top X_j)^2\right] = \overline{\sigma}^2 \mathrm{tr}(\Gamma_P).
% \end{align*}
Finally by Theorem~\ref{thm:concentration-width-unbounded},
\begin{align*}
    &c_0^{-1/(1+\beta)}\left(r_n^{2/(1+\beta)} + u_n^{2/(1+\beta)}+s_n^{1/(1+\beta)}\right)= C\left\{\left(\frac{\overline{\sigma}^2 \mathrm{tr}(\Gamma_P)}{\lambda^2_{\min}(\Gamma_P)n}\right)^{1/2}+\left(\frac{s_n}{\lambda_{\min}(\Gamma_P)}\right)^{1/2}\right\}
\end{align*}
\textcolor{red}{
\begin{align*}
    &c_0^{-1/(1+\beta)}\left(r_n^{2/(1+\beta)} + u_n^{2/(1+\beta)}+s_n^{1/(1+\beta)}\right)= C\left\{\left(\frac{\overline{\sigma}^2 d}{n}\right)^{1/2}+s_n^{1/2}\right\}
\end{align*}
}
for some universal constant $C$. This concludes the first result. 


We consider the requirement for $s_n$ defined as \ref{as:rate-initial-estimator}. First, for fixed $\widehat\theta_1$,
\begin{align*}
    P(m_{\widehat\theta_1}-m_{\theta_P})^2 &\lesssim \|\widehat\theta_1-\theta_P\|^2\E_P \|\xi X\|^2 +L^4 \lambda^2_{\max}(\Gamma_P)\|\widehat\theta_1-\theta_P\|^4.
\end{align*}
We also have
\begin{align*}
    \E_P(Y-\widehat\theta_1^\top X)^2 - \E_P(Y-\theta_P^\top X)^2 &\le \lambda_{\max}(\Gamma_P)\|\widehat\theta_1-\theta(P)\|^2.
\end{align*}
The remaining argument is analogous to the proof of Theorem~\ref{thm:mean-ci-width}. 
\begin{align*}
    &n^{-1/2}\sqrt{P (m_{\widehat\theta_1}-m_{\theta(P)})^2} + \mathbb{C}_P(\widehat{\theta}_1) \\
    &\qquad \le n^{-1/2} \|\widehat\theta_1-\theta_P\|\big(\E_P \|\xi X\|^2\big)^{1/2} + (n^{-1/2}L^2+1)\lambda_{\max}(\Gamma_P)\|\widehat\theta_1-\theta_P\|^2 \\
    &\qquad \le n^{-1/2} \overline{\sigma}(\mbox{tr}(\Gamma_P))^{1/2}\|\widehat\theta_1-\theta_P\| + 2L^2\lambda_{\max}(\Gamma_P)\|\widehat\theta_1-\theta_P\|^2 := s_n.
\end{align*}
Conditioning on the event where $\|\widehat\theta_1 - \theta_P\|_2^2 \le C_\varepsilon\overline{\sigma}^2\mathrm{tr}(\Gamma_P)/(n\lambda^2_{\min}(\Gamma_P))$, we obtain 
\begin{align*}
    \frac{s_n}{\lambda_{\min}(\Gamma_P)} &=\frac{ \overline{\sigma}(\mbox{tr}(\Gamma_P))^{1/2}\|\widehat\theta_1-\theta_P\|  }{n^{1/2}\lambda_{\min}(\Gamma_P)} + \frac{2L^2\lambda_{\max}(\Gamma_P)\|\widehat\theta_1-\theta_P\|^2}{\lambda_{\min}(\Gamma_P)}\\
    &\le\frac{ C_\varepsilon^{1/2} \overline{\sigma}^2\mbox{tr}(\Gamma_P)  }{n\lambda^2_{\min}(\Gamma_P)} + \left(\frac{2L^2\lambda_{\max}(\Gamma_P)}{\lambda_{\min}(\Gamma_P)}\right)\frac{ C_\varepsilon \overline{\sigma}^2\mbox{tr}(\Gamma_P)  }{n\lambda^2_{\min}(\Gamma_P)}
\end{align*}
% \begin{align*}
%     s_n/\lambda_{\min}(\Gamma_P) &\le \frac{C_\varepsilon\overline{\sigma}^2 \mathrm{tr}(\Gamma_P)}{n\lambda_{\min}(\Gamma_P)} + \frac{2L^2\lambda_{\max}(\Gamma_P)C_\varepsilon\overline{\sigma}^2\mathrm{tr}(\Gamma_P)}{n\lambda_{\min}(\Gamma_P)}\left(\frac{L^4\lambda^2_{\max}(\Gamma_P)}{n\lambda^2_{\min}(\Gamma_P)}\right)^{1/4} \|\widehat\theta_1-\theta(P)\|\\
%     &\qquad + \left(\frac{\lambda_{\max}(\Gamma_P)}{n\lambda_{\min}(\Gamma_P)}\right)^{1/2}\|\widehat\theta_1-\theta(P)\|\\
%     &\lesssim \left(\frac{\overline{\sigma}^4 \mathrm{tr}^2(\Gamma_P)}{n^2\lambda^2_{\min}(\Gamma_P)}\right)^{1/4}  + \left(\frac{L^4\lambda^2_{\max}(\Gamma_P)\overline{\sigma}^4 \mathrm{tr}^2(\Gamma_P)}{n^3\lambda^2_{\min}(\Gamma_P)}\right)^{1/4}  + \left(\frac{\lambda_{\max}(\Gamma_P)\overline{\sigma}^2 \mathrm{tr}(\Gamma_P)}{n\lambda_{\min}(\Gamma_P)}\right)^{1/2}\\
%     &\lesssim \left(\frac{\overline{\sigma}^4 \mathrm{tr}^2(\Gamma_P)}{n^2\lambda^2_{\min}(\Gamma_P)}\right)^{1/4}  + \left(\frac{L^4\lambda^2_{\max}(\Gamma_P)\overline{\sigma}^2 \mathrm{tr}(\Gamma_P)}{n^2\lambda^2_{\min}(\Gamma_P)}\right)^{1/4}  + \left(\frac{\lambda_{\max}(\Gamma_P)\overline{\sigma}^2 \mathrm{tr}(\Gamma_P)}{n\lambda_{\min}(\Gamma_P)}\right)^{1/2}\\
%     % &\lesssim \left(\frac{\overline{\sigma}^2 \mathrm{tr}(\Gamma_P)  + \overline{\sigma} \mathrm{tr}^{1/2}(\Gamma_P)L^2\lambda_{\max}(\Gamma_P) +L^4\lambda^2_{\max}(\Gamma_P)}{n\lambda_{\min}(\Gamma_P)}\right)^{1/2}\\
%     &\lesssim \left(\frac{\overline{\sigma}^2 \mathrm{tr}(\Gamma_P)  \vee L^4\lambda^2_{\max}(\Gamma_P)}{n\lambda_{\min}(\Gamma_P)}\right)^{1/2}.  
% \end{align*}
Then for $C_\varepsilon$ large enough, we conclude
\begin{align*}
\mathbb{P}_P\left(\mathrm{Diam}_{\|\cdot\|}\big(\widehat{\mathrm{CI}}_{n,\alpha}^{\mathrm{LR}}\big)\le \mathfrak{C}\left(\frac{L^2\lambda_{\max}(\Gamma_P)\overline{\sigma}^2\mathrm{tr}(\Gamma_P)}{n\lambda^3_{\min}(\Gamma_P)}\right)^{1/2}\right) \ge 1-\varepsilon
\end{align*}
when the requirements for $\widehat \theta_1$ are satisfied.
\end{proof}
% \begin{proof}[\bfseries{Proof of Proposition~\ref{prop:ols-ci-def}}]
%     First, we observe that 
%     \begin{align*}
%         \E_P[m_{\theta_P} - m_{\widehat \theta_1}] &= \E_P[(Y-\theta_P^\top X)^2 - (Y-\widehat\theta_1^\top X)^2]\\
% 	&= \E_P[(Y-\theta_P^\top X)^2 - (Y-\theta_P^\top X+\theta_P^\top X-\widehat\theta_1^\top X)^2]\\
% 	&= -\E_P[\{(\theta_P-\widehat\theta_1)^\top X\}^2].
%     \end{align*}
%     Hence, we have $U_{n,\alpha_2}(\theta_P, \widehat\theta_1; D_2) \equiv -\E_P[\{(\theta_P-\widehat\theta_1)^\top X\}^2]$ with $\alpha_2=0$.     Since this term involves $P$, we need to estimate them. We consider the empirical mean 
%     \begin{align*}
%         \frac{1}{n}\sum_{i=1}^n [\{(\theta_P-\widehat\theta_1)^\top X_i\}^2], 
%     \end{align*}


%     Next, denoting by $\overline{\theta}_n$ the ordinary least square based on $D_2$, defined as \eqref{eq:ols-definition-d2}, we obtain 
%     \begin{align*}
%         \mathbb{P}_n(m_{\theta}-m_{\widehat\theta_1})
% &= n^{-1}\sum_{i=1}^n[(Y_i-\overline{\theta}_n^\top X_i + \overline{\theta}_n^\top X_i-\theta^\top X_i)^2 - (Y_i-\overline{\theta}_n^\top X_i + \overline{\theta}_n^\top X_i-\widehat\theta_1^\top X_i)^2]\\
% 	&= n^{-1}\sum_{i=1}^n[2(Y_i-\overline{\theta}_n^\top X_i)(\widehat\theta_1-\theta)^\top X_i + \{(\overline{\theta}_n-\theta)^\top X_i\}^2-\{(\overline{\theta}_n-\widehat\theta_1)^\top X_i\}^2]\\
%  &= n^{-1}\sum_{i=1}^n[\{(\overline{\theta}_n-\theta)^\top X_i\}^2-\{(\overline{\theta}_n-\theta+\theta-\widehat\theta_1)^\top X_i\}^2]\\
% 	&= -2n^{-1}\sum_{i=1}^n\{(\overline{\theta}_n-\theta)^\top X_i\}\{(\theta-\widehat\theta_1)^\top X_i\}-n^{-1}\sum_{i=1}^n\{(\theta-\widehat\theta_1)^\top X_i)\}^2\\
% 	&= -2(\overline{\theta}_n-\theta)^\top\widehat \Sigma (\theta-\widehat\theta_1)-n^{-1}\sum_{i=1}^n\{(\theta-\widehat\theta_1)^\top X_i)\}^2
%  \end{align*}
%  where $\widehat \Sigma := n^{-1}\sum_{i=1}^n X_i X_i^\top$.
%  Hence, we conclude 
% 	\begin{align*}
%     \widehat{\mathrm{CI}}^{\mathrm{OLS}}_{n,\alpha} &:= \left\{\theta \in \mathbb{R}^d \, : \, \mathbb{P}_n(m_{\theta}-m_{\widehat \theta_1})\le n^{-1/2}z_{\alpha} \widehat\sigma_{\theta, \widehat\theta_1}+\big(0 \wedge U_{n,\alpha_2}(\theta, \widehat \theta_1; D_2)\right\}\\
%     &= \bigg\{\theta \in \mathbb{R}^d \, : \,  -2(\overline{\theta}_n-\theta)^\top\widehat \Sigma (\theta-\widehat\theta_1)-n^{-1}\sum_{i=1}^n\{(\theta-\widehat\theta_1)^\top X_i)\}^2\\
%     &\qquad \qquad \le n^{-1/2}z_{\alpha} \widehat\sigma_{\theta, \widehat\theta_1}-n^{-1}\sum_{i=1}^n\{(\theta-\widehat\theta_1)^\top X_i)\}^2\bigg\}\\
%     &= \left\{\theta \in \mathbb{R}^d \, : 2(\overline{\theta}_n-\theta)^\top\widehat \Sigma (\widehat\theta_1-\theta) \le n^{-1/2}z_{\alpha} \widehat\sigma_{\theta, \widehat\theta_1}\right\}
% \end{align*}
% where $\sigma_{\widehat\theta_1, \theta}^2 := \mathbb{P}_n \big(m_{\theta} - m_{\widehat\theta_1}-\mathbb{P}_n(m_{\theta} - m_{\widehat\theta_1})\big)^2$.
% \end{proof}
% \begin{proof}[\bfseries{Proof of Proposition~\ref{prop:ols-validity}}]


% \kt{I want to use Chebyshev to show that $\alpha_2 = o_P(1)$. I thin for this, we need to slightly overestimate $U_{n,\alpha_2}(\theta, \widehat \theta_1; D_2)$}
% Hence under \ref{as:ols-est1}, Theorem~\ref{thm:validity-BE} implies for all $n > N_\varepsilon$ 
% \begin{align*}
%      &\mathbb{P}_P(\theta(P) \in \widehat{\mathrm{CI}}^{\mathrm{OLS}}_{n,\alpha}\mid D_1) \ge 1-\alpha-C\left(\varepsilon + \mathbf{1}\{\|\widehat\theta_1-\theta(P)\| \ge C_\varepsilon\}\right)\\
%      &\qquad \Longrightarrow\mathbb{P}_P(\theta(P) \in \widehat{\mathrm{CI}}^{\mathrm{OLS}}_{n,\alpha}) \ge 1-\alpha-C\left(\varepsilon + \mathbb{P}_P(\|\widehat\theta_1-\theta(P)\| \ge C_\varepsilon)\right)\\
%      &\qquad \Longrightarrow\inf_{P\in\mathcal{P}}\, \mathbb{P}_P(\theta(P) \in \widehat{\mathrm{CI}}^{\mathrm{OLS}}_{n,\alpha}) \ge 1-\alpha-C\left(\varepsilon + \sup_{P\in\mathcal{P}}\, \mathbb{P}_P(\|\widehat\theta_1-\theta(P)\| \ge C_\varepsilon)\right).
% \end{align*}
% We conclude the claim since the last term converges uniformly in probability in a sense that 
% \[\lim_{n\longrightarrow\infty}\, \sup_{P\in\mathcal{P}}\, \mathbb{P}_P(\|\widehat\theta_1-\theta(P)\| \ge C_\varepsilon)) = 0\]
% in view of \eqref{eq:uniform-convergence}. Derivation under \ref{as:ols-est2} is analogous by the result of Theorem~\ref{thm:validity-BE}.
% \end{proof}
% \begin{proof}[\bfseries{Proof of Proposition~\ref{prop:ols-width}}]
% First, the standard deviation can be bounded by 
% \begin{align*}
% 	 \widehat\sigma_{\theta, \widehat \theta_1} &\le  \left(\frac{1}{n}\sum_{i=1}^n \left(m_{\theta} - m_{\widehat\theta_1}\right)^2\right)^{1/2}\\
% 	  &=  \left(\frac{1}{n}\sum_{i=1}^n \left(2(Y_i-\overline{\theta}_n^\top X_i)(\widehat\theta_1-\theta)^\top X_i-2(\overline{\theta}_n-\theta)^\top X_i(\theta-\widehat\theta_1)^\top X_i-(\theta^\top X_i-\widehat\theta_1^\top X_i)^2\right)^2\right)^{1/2}\\
% 	  &\le   2\left(\frac{1}{n}\sum_{i=1}^n \left((Y_i-\overline{\theta}_n^\top X_i)(\widehat\theta_1-\theta)^\top X_i\right)^2 \right)^{1/2}\\
% 	  &\qquad +  2\left(\frac{1}{n}\sum_{i=1}^n \left((\overline{\theta}_n-\theta)^\top X_i(\theta-\widehat\theta_1)^\top X_i\right)^2 \right)^{1/2}+  \left(\frac{1}{n}\sum_{i=1}^n \left(\theta^\top X_i-\widehat\theta_1^\top X_i\right)^4 \right)^{1/2}.
% \end{align*}
% Denoting the empirical error variable as $\overline\xi_i := Y_i - \overline{\theta}_n^\top X_i$, we have 
% \begin{align*}
% 	|\overline\xi_i(\widehat\theta_1-\theta)^\top X_i| = |\overline\xi_i(\widehat\theta_1-\theta)^\top \widehat{\Sigma}^{1/2}I_d\widehat{\Sigma}^{-1/2} X_i| \le |\overline\xi_i|\|\theta-\widehat\theta_1\|_{\widehat \Sigma} \| \widehat{\Sigma}^{-1/2}X_i\|.
% \end{align*}
% Using this result, the first term can be bounded by
% \begin{align*}
%     2\left(\frac{1}{n}\sum_{i=1}^n \left((Y_i-\overline{\theta}_n^\top X_i)(\widehat\theta_1-\theta)^\top X_i\right)^2 \right)^{1/2}&= 2\left(\frac{1}{n}\sum_{i=1}^n \left(\overline\xi_i(\widehat\theta_1-\theta)^\top X_i\right)^2 \right)^{1/2}\\ 
%     &\le 2\|\theta-\widehat\theta_1\|_{\widehat \Sigma} \left(\frac{1}{n}\sum_{i=1}^n \overline\xi_i^2 \| \widehat{\Sigma}^{-1/2}X_i\|^2 \right)^{1/2}.
% \end{align*}

% Next, we observe 
% \begin{align*}
% 	|(\theta-\widehat\theta_1)^\top X_i| = |(\theta-\widehat\theta_1)^\top \widehat{\Sigma}^{1/2}I_d\widehat{\Sigma}^{-1/2} X_i| \le \|\theta-\widehat\theta_1\|_{\widehat \Sigma} \| \widehat{\Sigma}^{-1/2}X_i\|
% \end{align*}
% by the Cauchy–Schwarz inequality. Hence, we have
% \begin{align*}
% 	 \left(\frac{1}{n}\sum_{i=1}^n \left(\theta^\top X_i-\widehat\theta_1^\top X_i\right)^4 \right)^{1/2} \le \|\theta-\widehat\theta_1\|_{\widehat \Sigma}^2 \left(\frac{1}{n}\sum_{i=1}^n\| \widehat{\Sigma}^{-1/2}X_i\|^4 \right)^{1/2}.
% \end{align*}

% The second term can be bounded by
% \begin{align*}
% 	&2\left(\frac{1}{n}\sum_{i=1}^n \left((\overline{\theta}_n^\top X_i-\theta^\top X_i)(\theta^\top X_i-\widehat\theta_1^\top X_i)\right)^2 \right)^{1/2} \\
% 	&\qquad =2\left(\frac{1}{n}\sum_{i=1}^n \left((\overline{\theta}_n^\top X_i-\widehat\theta_1^\top X_i+\widehat\theta_1^\top X_i-\theta^\top X_i)(\theta^\top X_i-\widehat\theta_1^\top X_i)\right)^2 \right)^{1/2} \\
% 	% &\qquad \le 2\left(\frac{1}{n}\sum_{i=1}^n \left((\widehat\theta_1^\top X_i-\theta^\top X_i)(\theta^\top X_i-\widehat\theta_1^\top X_i)\right)^2 \right)^{1/2} \\
%  % &\qquad\qquad+ 2\left(\frac{1}{n}\sum_{i=1}^n \left((\overline{\theta}_n^\top X_i-\widehat\theta_1^\top X_i)(\theta^\top X_i-\widehat\theta_1^\top X_i)\right)^2 \right)^{1/2} \\
% 	&\qquad \le 2\left(\frac{1}{n}\sum_{i=1}^n (\widehat\theta_1^\top X_i-\theta^\top X_i)^4 \right)^{1/2}+ 2\left(\frac{1}{n}\sum_{i=1}^n \left((\overline{\theta}_n^\top X_i-\widehat\theta_1^\top X_i)(\theta^\top X_i-\widehat\theta_1^\top X_i)\right)^2 \right)^{1/2}\\
% 	&\qquad = 2\|\theta-\widehat\theta_1\|_{\widehat \Sigma}^2 \left(\frac{1}{n}\sum_{i=1}^n\| \widehat{\Sigma}^{-1/2}X_i\|^4 \right)^{1/2} + 2\left(\|\widehat\theta_1-\overline{\theta}_n\|_{\widehat \Sigma}\|\widehat\theta_1-\theta\|_{\widehat \Sigma} \right).
% \end{align*}
% %Finally, we have 
% %\begin{align*}
% %	|(\theta-\widehat\theta_1)^\top X_i| = |(\theta-\widehat\theta_1)^\top \widehat{\Sigma}^{1/2}I_d\widehat{\Sigma}^{-1/2} X_i| \le \|\theta-\widehat\theta_1\|_{\widehat \Sigma} \| \widehat{\Sigma}^{-1/2}X_i\|
% %\end{align*}
% %by the Cauchy–Schwarz inequality. Hence 
% %\begin{align*}
% %	 \left(\frac{1}{n}\sum_{i=1}^n \left(\theta^\top X_i-\widehat\theta_1^\top X_i\right)^4 \right)^{1/2} \le \|\theta-\widehat\theta_1\|_{\widehat \Sigma}^2 \left(\frac{1}{n}\sum_{i=1}^n\| \widehat{\Sigma}^{-1/2}X_i\|^4 \right)^{1/2}.
% %\end{align*}
% Where the last step follows from 
% \begin{align*}
% 	|(\overline{\theta}_n^\top X_i-\widehat\theta_1^\top X_i)(\theta^\top X_i-\widehat\theta_1^\top X_i)|
% 	& = |(\overline{\theta}_n-\widehat\theta_1)^\top X_iX_i^\top (\theta-\widehat\theta_1)|\\
% 	& = |(\overline{\theta}_n-\widehat\theta_1)^\top X_iX_i^\top \widehat\Sigma^{-1/2} \widehat \Sigma^{1/2}(\theta-\widehat\theta_1)|\\
% 	&\le |(\overline{\theta}_n-\widehat\theta_1)^\top X_iX_i^\top \widehat\Sigma^{-1} X_iX_i^\top (\overline{\theta}_n-\widehat\theta_1)|^{1/2}\|\theta-\widehat\theta_1\|_{ \widehat \Sigma}
% \end{align*}
% and thus
% \begin{align*}
% 	&\left(\frac{1}{n}\sum_{i=1}^n \left((\overline{\theta}_n^\top X_i-\widehat\theta_1^\top X_i)(\theta^\top X_i-\widehat\theta_1^\top X_i)\right)^2 \right)^{1/2}\\
% 	&\qquad \le \left(\frac{1}{n}\sum_{i=1}^n |(\overline{\theta}_n-\widehat\theta_1)^\top X_iX_i^\top \widehat\Sigma^{-1} X_iX_i^\top (\overline{\theta}_n-\widehat\theta_1)|\|\theta-\widehat\theta_1\|^2_{ \widehat \Sigma} \right)^{1/2}\\
% 	&\qquad = \|\theta-\widehat\theta_1\|_{ \widehat \Sigma}\left(\frac{1}{n}\sum_{i=1}^n |(\overline{\theta}_n-\widehat\theta_1)^\top X_iX_i^\top \widehat\Sigma^{-1} X_iX_i^\top (\overline{\theta}_n-\widehat\theta_1)| \right)^{1/2}\\
% 	&\qquad = \|\theta-\widehat\theta_1\|_{ \widehat \Sigma}\|\overline{\theta}_n-\widehat\theta_1\|_{ \widehat \Sigma}.
% \end{align*}
% Putting together, 
% \begin{align*}
% 	 \widehat\sigma_{\theta, \widehat \theta_1} &\le 3\|\theta-\widehat\theta_1\|^2_{\widehat \Sigma} \left(\frac{1}{n}\sum_{i=1}^n\| \widehat{\Sigma}^{-1/2}X_i\|^4 \right)^{1/2} \\
%   &\qquad + 2\left(\|\widehat\theta_1-\overline{\theta}_n\|_{\widehat \Sigma}+ \left(\frac{1}{n}\sum_{i=1}^n \overline\xi_i^2 \| \widehat{\Sigma}^{-1/2}X_i\|^2 \right)^{1/2}\right)  \|\theta-\widehat\theta_1\|_{\widehat \Sigma}.
% \end{align*}

% Furthermore, 
% \begin{align*}
% 	\mathbb{P}_n\{(\overline{\theta}_n-\theta)^\top X\}\{(\theta-\widehat\theta_1)^\top X\} &= \mathbb{P}_n\{(\overline{\theta}_n-\widehat\theta_1 + \widehat\theta_1 - \theta)^\top X\}\{(\theta-\widehat\theta_1)^\top X\}\\
% 	&=\mathbb{P}_n\{(\overline{\theta}_n-\widehat\theta_1)^\top X\}\{(\theta-\widehat\theta_1)^\top X\} + \mathbb{P}_n\{( \widehat\theta_1 - \theta)^\top X\}\{(\theta-\widehat\theta_1)^\top X\}\\
% 	&=\mathbb{P}_n\{(\overline{\theta}_n-\widehat\theta_1)^\top X\}\{(\theta-\widehat\theta_1)^\top X\} - \|\theta -\widehat\theta_1\|_{\widehat \Sigma}^2.
% \end{align*}

% Putting together, we have 
% \begin{align*}
% 	&-2\mathbb{P}_n(\overline{\theta}_n^\top X-\theta^\top X)(\theta^\top X-\widehat\theta_1^\top X)\le n^{-1/2}z_{\alpha} \widehat\sigma_{\theta, \widehat\theta_1} \\
% 	&\qquad \Longrightarrow -2\mathbb{P}_n\{(\overline{\theta}_n-\widehat\theta_1)^\top X\}\{(\theta-\widehat\theta_1)^\top X\} + 2\|\theta -\widehat\theta_1\|_{\widehat \Sigma}^2 \\
% 	&\qquad\qquad\le 2 n^{-1/2}z_{\alpha} \left\{\left(\frac{1}{n}\sum_{i=1}^n \overline\xi_i^2 \| \widehat{\Sigma}^{-1/2}X_i\|^2 \right)^{1/2} + \|\widehat\theta_1-\overline{\theta}_n\|_{\widehat \Sigma}  \right\}\|\widehat\theta_1-\theta\|_{\widehat \Sigma} \\
% 	&\qquad\qquad\qquad + 3n^{-1/2}z_{\alpha} \|\theta-\widehat\theta_1\|_{\widehat \Sigma}^2 \left(\frac{1}{n}\sum_{i=1}^n  \| \widehat{\Sigma}^{-1/2}X_i\|^4 \right)^{1/2}\\
% 	&\qquad \Longrightarrow 0\le 2 n^{-1/2}z_{\alpha} \left\{\left(\frac{1}{n}\sum_{i=1}^n \overline\xi_i^2 \| \widehat{\Sigma}^{-1/2}X_i\|^2 \right)^{1/2} +  \|\widehat\theta_1-\overline{\theta}_n\|_{\widehat \Sigma} \right\}\|\widehat\theta_1-\theta\|_{\widehat \Sigma} \\
% 	&\qquad\qquad\qquad + \left\{3n^{-1/2}z_{\alpha}\left(\frac{1}{n}\sum_{i=1}^n  \| \widehat{\Sigma}^{-1/2}X_i\|^4 \right)^{1/2}-2\right\} \|\theta-\widehat\theta_1\|_{\widehat \Sigma}^2  \\
%  &\qquad\qquad\qquad+ 2\mathbb{P}_n\{(\overline{\theta}_n-\widehat\theta_1)^\top X\}\{(\theta-\widehat\theta_1)^\top X\} \\
% 	&\qquad \Longrightarrow 0\le 2 \left[\|\overline{\theta}_n-\widehat\theta_1\|_{\widehat \Sigma} + n^{-1/2}z_{\alpha} \left\{\left(\frac{1}{n}\sum_{i=1}^n \overline\xi_i^2 \| \widehat{\Sigma}^{-1/2}X_i\|^2 \right)^{1/2} +   \|\widehat\theta_1-\overline{\theta}_n\|_{\widehat \Sigma} \right\}\right]\|\widehat\theta_1-\theta\|_{\widehat \Sigma} \\
% 	&\qquad\qquad\qquad + \left\{3n^{-1/2}z_{\alpha}\left(\frac{1}{n}\sum_{i=1}^n  \| \widehat{\Sigma}^{-1/2}X_i\|^4 \right)^{1/2}-2\right\} \|\theta-\widehat\theta_1\|_{\widehat \Sigma}^2.
% \end{align*}

% We thus conclude that 
% \begin{align*}
% 	\widehat{\mathrm{CI}}^{\mathrm{OLS}}_{n,\alpha} &\subseteq \left\{\|\widehat\theta_1-\theta\|_{\widehat \Sigma}\le \frac{2 \left[(1+n^{-1/2}z_{\alpha})\|\overline{\theta}_n-\widehat\theta_1\|_{\widehat \Sigma} + n^{-1/2}z_{\alpha} \left(\frac{1}{n}\sum_{i=1}^n \overline\xi_i^2 \| \widehat{\Sigma}^{-1/2}X_i\|^2 \right)^{1/2} \right]}{\left[2-3n^{-1/2}z_{\alpha}\left(\frac{1}{n}\sum_{i=1}^n  \| \widehat{\Sigma}^{-1/2}X_i\|^4 \right)^{1/2}\right]_+}\right\}\\
% 	&\subseteq \left\{\|\widehat\theta_1-\theta\|\le \frac{2 \left[(1+n^{-1/2}z_{\alpha})\|\overline{\theta}_n-\widehat\theta_1\|_{\widehat \Sigma} + n^{-1/2}z_{\alpha} \left(\frac{1}{n}\sum_{i=1}^n \overline\xi_i^2 \| \widehat{\Sigma}^{-1/2}X_i\|^2 \right)^{1/2} \right]}{\left[2-3n^{-1/2}z_{\alpha}\left(\frac{1}{n}\sum_{i=1}^n  \| \widehat{\Sigma}^{-1/2}X_i\|^4 \right)^{1/2}\right]_+\lambda^{1/2}_{\min}(\widehat \Sigma)}\right\}
% \end{align*}
% where $\lambda_{\min}(A)$ denotes the smallest eigenvalue of a square matrix $A$.


% % For $X_1, \ldots, X_n \in \mathbb{R}^d$, compute $\hat \Sigma := n^{-1} \sum_{i=1}^n X_i X^\top_i$. Then for any $t \in \mathbb{R}^d$, 
% % \begin{align}
% % 	\frac{1}{n}\sum_{i=1}^n |t^\top X_i|^4 &= \frac{1}{n}\sum_{i=1}^n |t^\top \hat \Sigma^{1/2} \hat \Sigma^{-1/2} X_i|^4\le\|t\|_{\hat \Sigma}^4 \ \frac{1}{n}\sum_{i=1}^n \|X_i\|^4_{\hat \Sigma^{-1}}
% % \end{align}

% % \begin{align}
% % 	\frac{1}{n}\sum_{i=1}^n |t^\top X_i|^4 &= \frac{1}{n}\sum_{i=1}^n |t^\top \hat \Sigma^{1/2} \hat \Sigma^{-1/2} X_iX_i^\top  \hat \Sigma^{-1/2}\hat \Sigma^{1/2}t|^2\\
% % 	&= \|t^\top \hat \Sigma^{1/2} \hat \Sigma^{-1/2} XX^\top  \hat \Sigma^{-1/2}\hat \Sigma^{1/2}t\|_2^2\\
% % 	&= \|t\|^2_{\hat \Sigma} \|\hat \Sigma^{-1/2} XX^\top  \hat \Sigma^{-1/2}\hat \Sigma^{1/2}t\|_{\textrm{op}}^2
% % \end{align}
% \end{proof}

\subsection{Manski's discrete choice model}
In this example, we take 
\[m_{\theta} := (y,x) \mapsto -\frac{1}{2}\, y \cdot \mathrm{sgn}(\theta^\top x).\]
whose envelop function for $m_{\theta}-m_{\theta_P}$ is trivially given by $M=1$. The leading constant $1/2$ is introduced without loss of generality.
\begin{proof}[\bfseries{Proof of Theorem~\ref{thm:manski-width}}]
For any $\theta_1, \theta_2 \in \mathbb{S}^{d-1}$, we define our pseudo-metric as
\begin{align*}
    d_\Delta(\theta_1, \theta_2) := \mathbb{P}_P(\mathrm{sgn}(\theta_1^\top X) \neq \mathrm{sgn}(\theta_2^\top X)).
\end{align*}
Now we consider the following collection of ``localized'' functions:
\begin{align*}
    \mathcal{M}_{\delta}^\Delta := \left\{  \frac{1}{2}\, y \left(\mathrm{sgn}(\theta_P^\top x)-\mathrm{sgn}(\theta^\top x)\right)  \text{ for all }\theta \text{ i.e., } d_\Delta(\theta, \theta_P) \le \delta \text{ and } \theta \in \mathbb{S}^{d-1}\right\}.
\end{align*}
Below, we provide the confidence width in terms of $d_\Delta(\theta_1, \theta_2)$ using Theorem~\ref{thm:concentration-width}. First, we check \ref{as:margin}. Following Proposition 1 of \citet{tsybakov2004optimal} (and similarly for Proposition 2.4 of \citet{mukherjee2021optimal}), we define the set $\mathcal{A}(\theta) := \{x : \mathrm{sgn}(\theta_P^\top X) \neq \mathrm{sgn}(\theta^\top X)\}$ for each $\theta$. It then follows that 
\begin{align*}
   P(m_{\theta}-m_{\theta_P}) &=\frac{1}{2}\E_P\left[ Y \left(\mathrm{sgn}(\theta_P^\top X)-\mathrm{sgn}(\theta^\top X)\right)\right] \\
   &=\int_{\mathcal{A}(\theta)}\, |\E_P[Y |X=x] |P_X(x)\, dx\\
   &\ge 2 \int_{\mathcal{A}(\theta)}\, |\eta_P(x)-1/2|P_X(x)\, dx \\
   &\ge 2\sup_{0 \le t \le t^*}t\mathbb{P}_P\left(|\eta_P(X)-1/2| \ge t \cap X \in \mathcal{A}(\theta)\right)\\
   &\ge 2\sup_{0 \le t \le t^*}t\left(d_\Delta(\theta, \theta_P)-\mathbb{P}_P\left(|\eta_P(X)-0.5| \le t \right)\right)\\
   &\ge 2\sup_{0 \le t \le t^*}t\left(d_\Delta(\theta, \theta_P)- C_0t^{1/\beta} \right).
\end{align*}
The last inequality uses \ref{as:tsybakov}. The optimal choice of $t$ is given by 
\begin{align*}
    t = \begin{cases}
        (1+1/\beta)^{-\beta}C_0^{-\beta}d^\beta_\Delta(\theta, \theta_P) & \text{when}\quad d_\Delta(\theta, \theta_P)\le (1+1/\beta)C_0(t^*)^{1/\beta}\\
        t^* & \text{otherwise.}
    \end{cases}
\end{align*}
Putting together, it follows for all $\theta \in \mathbb{S}^{d-1}$,
    \begin{align*}
        P(m_{\theta}-m_{\theta_P}) &\ge \left(\frac{2}{1+\beta}\right)\frac{d^{1+\beta}_\Delta(\theta, \theta_P)}{ (1+1/\beta)^{\beta}C_0^\beta}\mathbf{1}\left\{d_\Delta(\theta, \theta_P)\le (1+1/\beta)C_0(t^*)^{1/\beta}\right\}\\
        &\qquad +  \left(\frac{2}{1+\beta}\right)t^*d_\Delta(\theta, \theta_P)\mathbf{1}\left\{d_\Delta(\theta, \theta_P)>(1+1/\beta)C_0(t^*)^{1/\beta}\right\}.
    \end{align*}
    % Furthermore, under \ref{as:covariate-manski}, we obtain 
    % \begin{align*}
    %     P(m_{\theta}-m_{\theta(P)}) &\ge C_1\|\theta-\theta_0\|_2^{1+\beta}\mathbf{1}\left\{d_\Delta(\theta, \theta_0)\le (1+1/\beta)C_0(t^*)^{1/\beta}\right\}\\
    %     &\qquad + C_2t^*\|\theta-\theta_0\|_2\mathbf{1}\left\{d_\Delta(\theta, \theta_0)> (1+1/\beta)C_0(t^*)^{1/\beta}\right\}
    % \end{align*}
    % where $C_1$ and $C_2$ depend on $c_0$ and $\beta$. 
    Furthermore, assuming $C_0(t^*)^{1/\beta} > 1$, we conclude 
    \begin{align*}
        P(m_{\theta}-m_{\theta_P})\ge \mathfrak{C} d_\Delta(\theta, \theta_P)^{1+\beta}
    \end{align*}
    for all $\theta\in \mathbb{S}^{d-1}$ and $\mathfrak{C}$ depending on $\beta$ and $C_0$. Next, we derive $\phi_n$ in \ref{as:local-entropy}. We observe that 
    \begin{align*}
        &\E_P \left[\sup_{d_\Delta(\theta, \theta_P) < \delta}|\mathbb{G}_n (m_\theta - m_{\theta_P})| \right] \\
        &\qquad = \E_P\left[\sup_{d_\Delta(\theta, \theta_P) < \delta}\left|\mathbb{G}_n \frac{ y \left(\mathrm{sgn}(\theta_P^\top x)-\mathrm{sgn}(\theta^\top x)\right)}{2}\right| \right]= \E_P\left[\sup_{m \in \mathcal{M}^\Delta_\delta}\left|\mathbb{G}_n m\right| \right],
    \end{align*}
    which we employ Theorem~\ref{thm:local-maximal-ineq} to control. First, we relate the covering number of $\mathcal{M}^\Delta_\delta$ to the VC dimension of the subgraphs of the functions in $\mathcal{M}^\Delta_\delta$. We observe that the subgraph of a function $(x,y) \mapsto y\cdot \{\mathrm{sgn}(\theta_P^\top x)-\mathrm{sgn}(\theta^\top x)\}$ for $y \in \{-1,1\}$ is contained in 
    \begin{align*}
        &\left\{(y,x,t) \, :\, y\{\mathrm{sgn}(\theta_P^\top x)-\mathrm{sgn}(\theta^\top x)\} \ge t\right\} \\
        &\qquad = \{(1, x,t) \, :\,\mathrm{sgn}(\theta_P^\top x)-\mathrm{sgn}(\theta^\top x) \ge t\} \cup \{(-1,x,t) \, :\,\mathrm{sgn}(\theta^\top x)-\mathrm{sgn}(\theta_P^\top x)\ge t\} \\
        &\qquad= \{(1,x,t) \, :\,-\mathrm{sgn}(\theta^\top x) \ge t-\mathrm{sgn}(\theta_P^\top x)\} \cup \{(-1,x,t) \, :\,\mathrm{sgn}(\theta^\top x)\ge t+\mathrm{sgn}(\theta_P^\top x)\}\\
        &\qquad \subseteq \{(1,x,t) \, :\,-\mathrm{sgn}(\theta^\top x) \ge t\} \cup \{(-1,x,t) \, :\,\mathrm{sgn}(\theta^\top x)\ge t\}\\
        &\qquad \subseteq \{(1, x,t) \, :\,\theta^\top x \ge t\} \cup \{(-1, x,t) \, :\,\theta^\top x \ge t\}.
    \end{align*}
    Hence, the set of points that the subgraph of the function space $\mathcal{M}_\delta^\Delta$ can shatter is contained in the set of points that a half-space in $\mathbb{R}^d$ can shatter. Furthermore, the covering number of the VC functions (i.e., whose subgraphs form VC-class of sets) is given by
    \begin{align*}
        N(\varepsilon \|M\|_{L_2(Q)}, \mathcal{M}_\delta^\Delta, L_2(Q)) \le C d (16e)^d \left(\frac{1}{\varepsilon}\right)^{d}
    \end{align*}
    by Theorem 2.6.7 of \citet{van1996weak} for any probabiliry measure $Q$ and $\varepsilon \in (0,1)$ and $C$ is a universal constant. We thus obtain  
    \begin{align*}
        t\mapsto J(t, \mathcal{M}^\Delta_{\delta}, L_2) &= \sup_{Q} \int_{0}^t \sqrt{1+ \log\left(C d (16e)^d \left(\frac{1}{\varepsilon}\right)^{2d}\right)}\, d\varepsilon\\
        &\le  \sup_{Q} \int_{0}^t \sqrt{\mathfrak{C} d + 2d\log\left(\frac{1}{\varepsilon}\right)}\, d\varepsilon \le  \mathfrak{C}t \sqrt{d\log(1/t)}
    \end{align*}
    where $\mathfrak{C}$ is a universal constants that may change line by line. Furthermore, we note that 
    \begin{align*}
        \E_P\left(\frac{y\left(\mathrm{sgn}(\theta_P^\top x)-\mathrm{sgn}(\theta^\top x)\right)}{2}\right)^2  = \mathbb{P}_P\left(\mathrm{sgn}(\theta_P^\top x) \neq \mathrm{sgn}(\theta^\top x)\right) \le \delta.
    \end{align*}
    Thus the condition of Theorem~\ref{thm:local-maximal-ineq} holds with $t^2 = \delta$ and $F=1$. By Theorem~\ref{thm:local-maximal-ineq}, we obtain
    \begin{align}
        \E_P\, \left[\sup_{m \in \mathcal{M}_\delta^\Delta}\, |\mathbb{G}_n m|\right]\lesssim \sqrt{\delta d\log(1/\delta)}\left(1+ \frac{ \sqrt{\delta d\log(1/\delta)}}{\delta \sqrt{n}}\right) = \sqrt{\delta d\log(1/\delta)}+ \frac{d\log(1/\delta)}{\sqrt{n}}.\nonumber
    \end{align}
    We can thus take $\phi_n$ in \ref{as:local-entropy} as
    \begin{align*}
        \delta \mapsto \phi_n(\delta) = \sqrt{\delta d\log(1/\delta)}+ \frac{d\log(1/\delta)}{\sqrt{n}} + \sqrt{\delta} \lesssim \sqrt{\delta d\log(1/\delta)}+ \frac{d\log(1/\delta)}{\sqrt{n}}.
    \end{align*}
    Solving the inequality in Theorem~\ref{thm:concentration-width}, 
    \begin{align*}
        &r_n^{-2} \left(r_n^{1/(1+\beta)} \sqrt{d\log(1/r_n)}+ \frac{d\log(1/r_n)}{\sqrt{n}}\right) \le n^{1/2} \\
        &\qquad \implies r_n \ge \left(\frac{d\log(n/d)}{n}\right)^{(1+\beta)/(2+4\beta)} \vee \left(\frac{d\log(n/d)}{n}\right)^{1/2}\\
        &\qquad \implies r_n^{2/(1+\beta)} \ge \left(\frac{d\log(n/d)}{n}\right)^{1/(1+2\beta)} \vee \left(\frac{d\log(n/d)}{n}\right)^{1/(1+\beta)}.
    \end{align*}    
    Now by Theorem~\ref{thm:concentration-width}, we conclude 
    \begin{align}\label{eq:result-in-delta}
\mathrm{Diam}_{d_\Delta(\cdot)}\big(\widehat{\mathrm{CI}}^{\mathrm{Manski}}_{n,\alpha}\big)\le \mathfrak{C}\left\{\left(\frac{d\log(n/d)}{n}\right)^{1/(1+2\beta)}+ s_n^{1/(1+\beta)}\right\}
\end{align}
with probability greater than $1-\varepsilon$.

Finally, we relate this result to $\|\theta-\theta_P\|_2$ using \ref{as:covariate-manski}. The result established thus far and \ref{as:covariate-manski} together imply that for any $\theta \in \widehat{\mathrm{CI}}^{\mathrm{Manski}}_{n,\alpha}$, 
\begin{align*}
    \|\theta - \theta(P)\|_2 \le c_0^{-1}d_{\Delta}(\theta_1, \theta(P)) \le \mathfrak{C}\left\{\left(\frac{d\log(n/d)}{n}\right)^{1/(1+2\beta)}+ s_n^{1/(1+\beta)}\right\},
\end{align*}
with high probability. This proves the result.
% When $d_\Delta(\theta, \theta_P)>(1+1/\beta)C_0(t^*)^{1/\beta}$, 
% \begin{align*}
%    &\left\{\theta \in \Theta : P_0(m_\theta-m_{\theta(P)})+n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)}) \le    \sqrt{\frac{2\log(2/\alpha)n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta(P)})^2}{n}}\right.\\
%     &\left. \qquad +\sqrt{\frac{2\log(2/\alpha)P (m_{ \theta}-m_{\theta(P)})^2 }{n}} + \frac{7B_0\log(2/\alpha)}{3(n-1)} + \Gamma_n(\widehat\theta_1, \theta(P))\right\}
% \end{align*}
% where the lower bound of the inequality becomes 
% \begin{align*}
%     &P_0(m_\theta-m_{\theta(P)})+n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)}) \\
%     &\qquad \ge P_0(m_\theta-m_{\theta(P)})\left(1-\sup_{d_\Delta(\theta, \theta_0)>(1+1/\beta)C_0(t^*)^{1/\beta}}\, \left|\frac{n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)})}{P_0(m_\theta-m_{\theta(P)})}\right|\right)_+
% \end{align*}
% and 
% \begin{align*}
%     \sup_{d_\Delta(\theta, \theta_0)>(1+1/\beta)C_0(t^*)^{1/\beta}}\, \left|\frac{n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta(P)})}{P_0(m_\theta-m_{\theta(P)})}\right| \le n^{-1/2}C_2^{-1}(1/t^*)\E\left[\sup_{\theta\in \Theta}\, \frac{|m_\theta-m_{\theta(P)}|^2}{d_\Delta(\theta, \theta_0)}\right]
% \end{align*}
\end{proof}

% \subsection{Nonparametric classification}
% In this example, we take $Z:=(X,Y)$ taking values in $X \in \mathcal{X} \subseteq \mathbb{R}^d$ and $Y \in \{0,1\}$. We consider the construction of the ``decision rule", $\theta : \mathcal{X} \mapsto \{0,1\}$, which minimizes the following risk:
% \begin{align}
%     \theta_P := \argmin_{\theta: \mathcal{X} \mapsto \{0,1\}}\, \mathbb{E}_P[\mathbf{1}\{Y \neq \theta(X)\}]
% \end{align}
% where the expectation is taken under the joint distribution between $X$ and $Y$. Following \citet{audibert2007fast}, we consider the family of plug-in classifiers, $\theta(x) := \mathbf{1}\{\eta(x) \ge 1/2\}$, where $\eta$ belongs to a large (nonparametric) class of functions. We can assert that the minimizer of \eqref{eq:classification} corresponds to the Bayes classifier such that 
% \begin{align*}
%     \theta_P(x) := \mathbf{1}\{\eta_P(x) \ge 1/2\} \quad \text{where} \quad \eta_P(x) := \mathbb{P}_P(Y=1 \mid X=x).
% \end{align*}
% Let $\mathcal{H}$ be a set of functions that contains $\eta_P$. For any $\eta \in \mathcal{H}$, we construct a classifier by the plug-in rule $\theta_{\eta}(x) := \mathbf{1}\{\eta(x) \ge 1/2\}$.

% Now we consider a collection of localized functions 
% \begin{align*}
%     \mathcal{M}^\rho_{\delta} := \bigg\{ \mathbf{1}\{y \neq \theta(x)\} - \mathbf{1}\{y \neq \theta_P(x)\}  \text{ for all }\theta \text{ i.e., }  \rho(\theta, \theta_P) \le \delta \bigg\}
% \end{align*}
% where $\rho(\theta, \theta_P) = \mathbb{P}_P(\theta(X)\neq \theta_P(X)) = \|\theta-\theta_P\|_{L_1(P)}$. 
% \begin{proof}[\bfseries{Proof of Theorem~\ref{thm:classificaiton-width}}]
% We verify conditions required for Theorem~\ref{thm:concentration-width}. First, we check \ref{as:margin}. By the analogous derivation as the proof of Theorem~\ref{thm:manski-width} (similarly Lemma 2 of \citet{mammen1999smooth} or Lemma 6.1 of \citet{audibert2007fast}), we conclude 
%     \begin{align*}
%         P(m_{\theta}-m_{\theta(P)})\ge \mathfrak{C}\rho(\theta, \theta_P)^{1+\beta}
%     \end{align*}
% for $C_0(t^*)^{1/\beta} > 1$ with $\mathfrak{C}$ depending on $C_0$ and $\beta$. Next, we assert \ref{as:local-entropy}. Similarly to the proof of \ref{thm:manski-width}, we observe that 
%     \begin{align*}
%         &\E_P \left[\sup_{\rho(\theta, \theta_P) < \delta}|\mathbb{G}_n (m_\theta - m_{\theta(P)})| \right] \\
%         &\qquad = \E_P\left[\sup_{\rho(\theta, \theta_P) < \delta}\left|\mathbb{G}_n  \left(\mathbf{1}\{y \neq \theta(x)\} - \mathbf{1}\{y \neq \theta_P(x)\}\right)\right| \right]= \E_P\left[\sup_{m \in \mathcal{M}^\rho_\delta}\left|\mathbb{G}_n m\right| \right],
%     \end{align*}
%     which we employ Theorem~\ref{thm:local-maximal-ineq-bracket} to control. For any $m \in \mathcal{M}^\rho_\delta$, we have 
% \begin{align*}
%     \E_P m^2 &= \sup_{\rho(\theta, \theta_P) \le \delta}\, \E_P(\mathbf{1}\{Y \neq \theta(X)\}-\mathbf{1}\{Y \neq \theta_P(X)\})^2\\
%     &= \E_P(\mathbf{1}\{\theta_P(X) \neq \theta(X)\}) \le \delta.
% \end{align*}
% Hence the condition of Theorem~\ref{thm:local-maximal-ineq-bracket} holds with $t^2 = \delta$ and $M = 2$.

% For any $m_1, m_2 \in \mathcal{M}^\rho_\delta$ (with each corresponding $\theta$ denoted by $\theta_1,\theta_2$), we have 
% \begin{align*}
%     \|m_1-m_2\|_{L_2(P)} = \sqrt{\mathbb{P}_P(\theta_1(X) \neq \theta_2(X))} \le C_0^{1/2} \|\eta_1-\eta_2\|_\infty^{1/(2\beta)} 
% \end{align*}
% \kt{This is not true. Not sure how to relate.}
% where the inequality follows from Lemma 5.1 of \cite{audibert2007fast}. This implies that 
% \begin{align*}
%     \log N_{[\,]}(\varepsilon, \mathcal{M}^\rho_\delta, L_2(P)) \le \log N_{[\,]}(C_0^{-\beta}\varepsilon^{2\beta}, \mathcal{H}, \|\cdot \|_\infty) \le \mathfrak{C}\varepsilon^{-2\beta\kappa}.
% \end{align*}
% Thus, the bracketing entropy integral is given by 
% \begin{align*}
%     t \mapsto J_{[\, ]}(t, \Theta, \|\cdot\|) &= \int_{0}^t \sqrt{1 + \log N_{[\,]}(\varepsilon, \mathcal{M}^\rho_\delta, L_2(P))}\, d\varepsilon \\
%     &\le \int_{0}^t \sqrt{1 + \mathfrak{C}\varepsilon^{-2\beta\kappa}} \le \mathfrak{C}\left(t + \frac{t^{1-\kappa\beta}}{1-\kappa\beta}\right) 
% \end{align*}
% for $\kappa\beta < 1$.
% By Theorem~\ref{thm:local-maximal-ineq-bracket}, we obtain
%     \begin{align}
%         \E_P\, \left[\sup_{m \in \mathcal{M}_\delta^\rho}\, |\mathbb{G}_n m|\right]\lesssim \left(\sqrt{\delta}  + \delta^{(1-\kappa\beta)/2}\right)\left(1+ \frac{\sqrt{\delta}  + \delta^{(1-\kappa\beta)/2}}{\delta \sqrt{n}}\right).\nonumber
%     \end{align}
%     We can thus take $\phi_n$ in \ref{as:local-entropy} as
%     \begin{align*}
%         \delta \mapsto \phi_n(\delta) &= \left(\sqrt{\delta}  + \delta^{(1-\kappa\beta)/2}\right)\left(1+ \frac{\sqrt{\delta}  + \delta^{(1-\kappa\beta)/2}}{\delta \sqrt{n}}\right) + \sqrt{\delta} \\
%         &\lesssim \delta^{(1-\kappa\beta)/2} + n^{-1/2}\delta^{-\kappa\beta}
%     \end{align*}
%     since $\delta \le 1$. It remains to solve equations in Theorem~\ref{thm:concentration-width} to derive the rate of convergence. First, we have 
% \begin{align*}
%     r_n^{-2}\left\{r_n^{(1-\kappa\beta)/(1+\beta)}\vee n^{-1/2}r_n^{-(2\beta\kappa)/(1+\beta)}\right\} \le n^{1/2} \Longrightarrow r_n \ge n^{-\frac{2(1+\beta+\kappa\beta)}{1+\beta}}.
% \end{align*}
% Hence by Theorem~\ref{thm:concentration-width}, we conclude 
%     \begin{align*}
% \mathrm{Diam}_{\|\cdot\|}\big(\widehat{\mathrm{CI}}^{\mathrm{Class.}}_{n,\alpha}\big)\le \mathfrak{C}\left(n^{-\gamma/((1+\beta)\gamma+d\beta)} + s_n^{1/(1+\beta)}\right)
% \end{align*}
% \kt{
% \begin{align*}
%     r_n^{\frac{-2-2\beta+1-\kappa\beta}{1+\beta}} =r_n^{-\frac{1+2\beta+\kappa\beta}{1+\beta}} \le n^{1/2} \Longrightarrow r_n \ge n^{-\frac{(1+\beta)}{2(1+2\beta+\kappa\beta)}} \Longrightarrow r_n^{2/(1+\beta)} \ge n^{-\frac{1}{1+2\beta+\kappa\beta}} \\
%     r_n^{\frac{-2-2\beta-2\kappa\beta}{1+\beta}} =r_n^{-\frac{2(1+\beta+\kappa\beta)}{1+\beta}} \le n \Longrightarrow r_n \ge n^{-\frac{(1+\beta)}{2(1+\beta+\kappa\beta)}} \Longrightarrow r_n^{2/(1+\beta)} \ge n^{-\frac{1}{1+\beta+\kappa\beta}}
% \end{align*}
% }
% % \begin{align*}
% %     \E_P\left[\sup_{\rho(\theta, \theta_P) < \delta}|\mathbb{G}_n (m_\theta - m_{\theta_P})|\right] &\le 2n^{1/2}\E_P\left[\sup_{\rho(\theta, \theta_P) < \delta}\left|\sum_{i=1}^n \epsilon_i(m_\theta(Z_i) - m_{\theta_P}(Z_i))\right|\right]\\
% %     &\le 2\int_0^{\delta} \sqrt{\log N(\varepsilon, M_{\delta}, \rho)}\, d\varepsilon \\
% %     &\le 2\int_0^{\delta} \sqrt{\log N(C_0^{-1}\varepsilon^{\beta}, \mathcal{H}, \|\cdot\|_\infty)}\, d\varepsilon \\
% %     &\le C\int_0^{\delta} \varepsilon^{-(\beta\gamma/2)} d\varepsilon =  \frac{C}{1-(\beta\gamma/2)} \delta^{1-(\beta\gamma/2)} \quad \text{when} \quad \beta \gamma < 2.
% % \end{align*}
% % Hence we take 
% % \begin{align*}
% %     \phi_n(\delta) = \left\{\frac{C}{1-(\beta\gamma/2)}\delta^{1-(\beta\gamma/2)} \vee \delta^{1/2}\right\}
% % \end{align*}
% % where the transition takes place at $\beta\gamma < 1$. 
% % It remains to solve equations in Theorem~\ref{thm:concentration-width} to derive the rate of convergence. First, we have 
% % \begin{align*}
% %     r_n^{-2}\left\{\frac{C}{1-(\beta\gamma/2)}r_n^{(2-\beta\gamma)/(1+\beta)} \vee r_n^{1/(1+\beta)}\right\} \le n^{1/2} \Longrightarrow r_n \ge \begin{cases}
% %           n^{-\frac{(1+\beta)}{2(1+2\beta)}}& \text{when} \quad \gamma\beta < 1 \\
% %           n^{-\frac{(1+\beta)}{2(\gamma\beta+2\beta)}}& \text{when} \quad 1 \le \gamma\beta < 2
% %     \end{cases}
% % \end{align*}

% \end{proof}

% % \begin{align*}
% %     \mathbb{E}_P[\mathbf{1}\{Y \neq f(X)\}] - \mathbb{E}_P[\mathbf{1}\{Y \neq f_P(X)\}] &= 2\mathbb{E}_P[|\theta_P(X) - 1/2|\mathbf{1}\{f(X) \neq f_P(X)\}]
% % \end{align*}

% % By Lemma 6.1 of \citet{audibert2007fast}, we have 
% % \begin{align*}
% %     \mathbb{E}_P[\mathbf{1}\{Y \neq f(X)\}] - \mathbb{E}_P[\mathbf{1}\{Y \neq f_P(X)\}] &\ge C\left\{\mathbb{P}_X(f(X) \neq f_P(X))\right\}^{1+\beta}
% % \end{align*}
% % \[m_{\theta} := z \mapsto \mathbf{1}(Y \neq \theta(X))\]
% % for any functions $\theta : \mathcal{X} \mapsto \{-1, 1\}$. The $P$-dependent optimizer is now denoted by $\theta_P$. It then immediately holds that 
% % \begin{align*}
% %     \mathbb{P}_P(\theta(X) \neq \theta_P(X)) = \frac{1}{2}\mathbb{E}_P\|\theta-\theta_P\|_1 = \|m_{\theta}-m_{\theta_P}\|_1.
% % \end{align*}
% % The validity of the confidence is again immediate since $\|m_{\theta_1}-m_{\theta_1}\|_\infty \le 2$, and thus we focus on the rate of convergence.
% % \begin{proof}
% %     We verify the conditions required for Theorem~\ref{thm:concentration-width}. First, by Lemma 2 of \citet{mammen1999smooth} and \ref{as:tsybakov}, we obtain 
% %     \begin{align*}
% %         P(m_{\theta}-m_{\theta(P)}) \ge C^{-\beta}\mathbb{P}_P\left(\theta_P(X) \neq \theta(X)\right)^{1+\beta} = \frac{1}{2}C^{-\beta}\|\theta-\theta_P\|_{1,P}.
% %     \end{align*}
% % \end{proof}

\subsection{Quantile estimation without positive densities}
For given $\gamma \in (0,1)$, we consider the quantile loss defined as 
\begin{align*}
    m_{\theta}(x) := \gamma(x-\theta)_+ + (1-\gamma)(\theta-x)_+.
\end{align*}
% Below, we denote by $\theta_P \equiv \theta(P)$.
\begin{proof}[\bfseries{Proof of Theorem~\ref{thm:quantile-validity}}]
Consider the case when $\theta > \theta_P$, then 
    \begin{align*}
    m_{\theta} - m_{\theta_P} 
    & = \gamma(X-\theta)_+ + (1-\gamma)(\theta-X)_+ - \gamma(X-\theta_P)_+ - (1-\gamma)(\theta_P-X)_+\\
    & = (1-\gamma)(\theta-\theta_P) \mathbf{1}\{X \le \theta_P\} 
 -\gamma(\theta-\theta_P)\mathbf{1}\{\theta < X\} \\
 &\qquad\qquad+ \left\{(1-\gamma)(\theta-X)-\gamma(X-\theta_P)\right\} \mathbf{1}\{\theta_P < X \le \theta\}\\
 &=(\theta-\theta_P) \mathbf{1}\{X \le \theta_P\} 
 -\gamma(\theta-\theta_P)(1-\mathbf{1}\{X > \theta_P\})+\gamma(\theta-\theta_P)\mathbf{1}\{\theta_P < X \le \theta\} \\
 &\qquad+ \left\{\theta_P-X +(1-\gamma) (\theta - \theta_P)\right\} \mathbf{1}\{\theta_P < X \le \theta\}\\
    & = (\theta-\theta_P) \mathbf{1}\{X \le \theta_P\} 
 -\gamma(\theta-\theta_P)+\gamma(\theta-\theta_P)\mathbf{1}\{\theta_P < X \le \theta\} \\
 &\qquad+ \left\{\theta_P-X +(1-\gamma) (\theta - \theta_P)\right\} \mathbf{1}\{\theta_P < X \le \theta\}\\
    & = (\theta-\theta_P) \mathbf{1}\{X \le \theta_P\} 
 -\gamma(\theta-\theta_P)+ (\theta-X) \mathbf{1}\{\theta_P < X \le \theta\}.
    \end{align*}
Analogously, we have 
\[m_{\theta} - m_{\theta_P} = \gamma(\theta_P-\theta) - (\theta_P-\theta) \mathbf{1}\{X \le \theta_P\} + (X-\theta) \mathbf{1}\{\theta < X \le \theta_P\}\]
when $\theta_P > \theta$. Taking expectations, we obtain 
\begin{align*}
    P(m_{\theta} - m_{\theta_P}) = \E_P[ (\theta-X) \mathbf{1}\{\theta_P < X \le \theta\}] + \E_P[ (X-\theta) \mathbf{1}\{\theta < X \le \theta_P\}].
\end{align*}
We now define the centered random variable, 
    \begin{align*}
        W_i &= m_{\theta}(X_i)-m_{\theta_P}(X_i) - P( m_{\theta}-m_{\theta_P})\\
        &= (\theta-\theta_P)\left(\mathbf{1}\{X \le \theta_P\}  - \gamma\right) + (\theta-X) \mathbf{1}\{\theta_P < X \le \theta\} + (X-\theta) \mathbf{1}\{\theta < X \le \theta_P\}\\
        &\qquad- \mathbb{E}_P[(\theta-X) \mathbf{1}\{\theta_P < X \le \theta\}]- \mathbb{E}_P[(X-\theta) \mathbf{1}\{\theta < X \le \theta_P\}].
    \end{align*}
    We take $H := \mathbf{1}\{X \le \theta_P\}  - \gamma$ then check \eqref{eq:qmd2} in Proposition~\ref{prop:first-order-linearization}. For $\theta > \theta_P$, this follows
    \begin{align*}
        &\frac{\mathbb{E}_P|W - (\theta-\theta_P)(\mathbf{1}\{X \le \theta_P\}  - \gamma)|^2}{|\theta-\theta_P|^2\E_P(\mathbf{1}\{X \le \theta_P\}  - \gamma)^2} \\
        &\qquad=\frac{\mathbb{E}_P|(\theta-X) \mathbf{1}\{\theta_P < X \le \theta\} - \mathbb{E}_P[(\theta-X) \mathbf{1}\{\theta_P < X \le \theta\}|^2}{|\theta-\theta_P|^2\E_P(\mathbf{1}\{X \le \theta_P\}  - \gamma)^2} \\
        &\qquad \le \frac{2(\theta-\theta_P)^2\mathbb{P}_P(\theta_P < X \le \theta) }{|\theta-\theta_P|^2\gamma(1-\gamma)}\\
        &\qquad\le \frac{2|\mathbb{P}_P(\theta_P < X \le \theta)-M_0|\theta - \theta_P|^{\beta} \mathrm{sgn}(\theta-\theta_P) +M_0|\theta - \theta_P|^{\beta} \mathrm{sgn}(\theta-\theta_P)|}{\gamma(1-\gamma)}\\
        &\qquad\le \frac{2M_1|\theta-\theta_P|^\beta +2M_0|\theta - \theta_P|^{\beta}}{\gamma(1-\gamma)}\le \frac{4M_0|\theta-\theta_P|^\beta }{\gamma(1-\gamma)}
    \end{align*}
    since $M_0 > M_1$. We then repeat the identical argument with $\theta < \theta_P$.
    We use the last display as $\varphi(|\theta-\theta_P|)$ in \eqref{eq:qmd2}.
    % \begin{align}
    % 	\frac{P[W_i- (\theta-\theta_P)\dot{m}_{\theta_P} ]^2}{|\theta-\theta_P|^2} \le 4
    % \end{align}
    Now we introduce the event $\mathcal{E} := \{|\widehat \theta_1 - \theta(P)| < \delta\}$. Then we have
    \begin{align*}
        \mathbb{P}_P(\theta(P) \in \widehat{\mathrm{CI}}^\gamma_{n,\alpha}) &\ge\mathbb{P}_P(\theta(P) \in \widehat{\mathrm{CI}}^\gamma_{n,\alpha} \cap \mathcal{E})-\mathbb{P}_P(\theta(P) \in \widehat{\mathrm{CI}}^\gamma_{n,\alpha} \cap \mathcal{E}^c)\\
        &\ge\mathbb{P}_P(\theta(P) \in \widehat{\mathrm{CI}}^\gamma_{n,\alpha} \cap \mathcal{E})-\mathbb{P}_P(\mathcal{E}^c).
    \end{align*}
    By invoking Proposition~\ref{prop:first-order-linearization} on the event $\mathcal{E} := \{|\widehat \theta_1 - \theta(P)| < \delta\}$, we have for any $\varepsilon < \delta$
\begin{align*}
    \sup_{P\in\mathcal{P}}\, \Delta_{n,P} &\lesssim \frac{4M_0\varepsilon^{\beta}}{\gamma(1-\gamma)} +\left(\frac{4M_0\varepsilon^{\beta}}{\gamma(1-\gamma)}\right)^{1/2} +  \sup_{P\in\mathcal{P}}\,\mathbb{P}_P(\|\widehat\theta_1 - \theta_P\| > \varepsilon) \\
    &\qquad + \sup_{P\in\mathcal{P}}\,\E_P\left[\frac{|\mathbf{1}\{X \le \theta_P\}  - \gamma|^2}{\gamma(1-\gamma)} \left\{1 \wedge \sqrt{\frac{|\mathbf{1}\{X \le \theta_P\}  - \gamma|^2}{n\gamma(1-\gamma)}}\right\}\right]
    \end{align*}
since $B^2 = \E_P(\mathbf{1}\{X \le \theta_P\}  - \gamma)^2 = \gamma(1-\gamma)$. By the trivial upper bound $\Delta_{n,P} \le 1$, it suffices to consider $(4M_0\varepsilon^{\beta})/(\gamma(1-\gamma))\le 1$ and by the assumption that $\delta > \varepsilon$, we have 
\begin{align*}
 \sup_{P\in\mathcal{P}}\,\mathbb{P}_P(\|\widehat\theta_1 - \theta_P\| > \delta) \le  \sup_{P\in\mathcal{P}}\,\mathbb{P}_P(\|\widehat\theta_1 - \theta_P\| > \varepsilon).
\end{align*}
Thus we obtain 
\begin{align*}
    \inf_{P\in\mathcal{P}}\,\mathbb{P}_P(\theta(P) \in \widehat{\mathrm{CI}}^\gamma_{n,\alpha}) \ge 1-\alpha -\sup_{P\in\mathcal{P}}\,\Delta_{n,P}
\end{align*}
where 
\begin{align*}
    \sup_{P\in\mathcal{P}}\Delta_{n,P} &\le C \left( 1\wedge \left(\frac{\varepsilon^{\beta}}{\gamma(1-\gamma)}\right)^{1/2} +  \sup_{P\in\mathcal{P}}\,\mathbb{P}_P(\|\widehat\theta_1 - \theta_P\| > \varepsilon)\right. \\
    &\left.\qquad + \sup_{P\in\mathcal{P}}\,\E_P\left[\frac{|\mathbf{1}\{X \le \theta_P\}  - \gamma|^2}{\gamma(1-\gamma)} \left\{1 \wedge \sqrt{\frac{|\mathbf{1}\{X \le \theta_P\}  - \gamma|^2}{n\gamma(1-\gamma)}}\right\}\right]\right).
\end{align*}
Let $\{q_n\}$ be a positive, non-decreasing sequence such that $q_n \ge 1$ for all $n$ and 
\begin{align*}
\lim_{n\to \infty}\sup_{P\in\mathcal{P}}\,\mathbb{P}_P( q_n\|\widehat\theta_1 - \theta_P\| > \varepsilon) = 0.
\end{align*}
Then, for any fixed $0 < \varepsilon < \delta \le 1$, we have
\begin{align*}
\Delta_{n,P} &\le C\left( 1\wedge \left(\frac{\varepsilon^{\beta}}{q_n^{\beta}\gamma(1-\gamma)}\right)^{1/2} +  \sup_{P\in\mathcal{P}}\,\mathbb{P}_P(q_n\|\widehat\theta_1 - \theta_P\| > \varepsilon) \right.\\
    &\qquad \left.+ \sup_{P\in\mathcal{P}}\,\E_P\left[\frac{|\mathbf{1}\{X \le \theta_P\}  - \gamma|^2}{\gamma(1-\gamma)} \left\{1 \wedge \sqrt{\frac{|\mathbf{1}\{X \le \theta_P\}  - \gamma|^2}{n\gamma(1-\gamma)}}\right\}\right]\right).
\end{align*}
Under the stated assumptions on $\gamma$ and $q_n$, this term tends to zero by taking $n \longrightarrow \infty$ and then taking $\varepsilon \longrightarrow 0$.
\end{proof}
\begin{proof}[\bfseries{Proof of Theorem~\ref{thm:quantile-ci-width}}]
First, we condition on $D_1$ and we take the expectation over $D_1$ at the end. The proof is split into two cases: (1) $|\theta-\theta_P| \le \delta$ and (2) $|\theta-\theta_P| > \delta$ where $\delta > 0$ corresponds to the value defined in \ref{as:cdf-Holder}. Without loss of generality, we assume $\delta < 1$. When \ref{as:cdf-Holder} holds with $\delta > 1$, we set $\delta = 1$. 
First we consider the case (1). We have shown that 
\begin{align*}
    P(m_{\theta} - m_{\theta_P}) = \E_P[ (\theta-X) \mathbf{1}\{\theta_P < X \le \theta\}] + \E_P[ (X-\theta) \mathbf{1}\{\theta < X \le \theta_P\}].
\end{align*}
We observe that $(\theta-X) \mathbf{1}\{\theta_P < X \le \theta\}$ is a non-negative random variable, taking values from $0$ to $\theta-\theta_P$ (when $\theta > \theta_P$). Let $R \in (0,1)$ be an arbitrary constant. Then 
\begin{align*}
    (\theta-X) \mathbf{1}\{\theta_P < X \le \theta\} \ge R(\theta-\theta_P)\mathbf{1}\{\theta_P < X \le \theta_P + (1-R)(\theta-\theta_P)\} 
\end{align*}
and thus 
\begin{align*}
    \E_P[ (\theta-X) \mathbf{1}\{\theta_P < X \le \theta\}]\ge R(\theta-\theta_P)\{F(\theta_P + (1-R)(\theta-\theta_P)) - F(\theta_P)\}.
\end{align*}
When $\theta-\theta_P \le \delta$,
by \ref{as:cdf-Holder}, we can further lower bound the expectation as 
\begin{align*}
    P(m_{\theta} - m_{\theta_P})  &\ge RM_0 (1-R)^{\beta}|\theta-\theta_P|^{1+\beta} - M_1R(1-R)^\beta|\theta-\theta_P|^{1+\beta}\\
    &= (M_0-M_1)R (1-R)^{\beta}|\theta-\theta_P|^{1+\beta}.
\end{align*}

By the assumption that $M_0 > M_1$, we can conclude that 
\begin{align*}
    P(m_{\theta} - m_{\theta_P})  \ge \mathfrak{C} (\theta-\theta_P)^{1+\beta}
\end{align*}
where $\mathfrak{C}$ depends on $M_0$ and $M_1$. 
Repeating the analogous argument for the case with $\theta_P > \theta$, we conclude that 
\begin{align*}
    P(m_{\theta} - m_{\theta_P})  \ge \mathfrak{C} |\theta-\theta_P|^{1+\beta}.
\end{align*}
The rest of the proof is similar to that of Theorem~\ref{thm:concentration-width-unbounded} with small modification that does not alter the main result. First, observe that 
\begin{align*}
    (m_{\theta} - m_{\theta_P})^2 &= \big\{\gamma(\theta_P-\theta) - (\theta_P-\theta) \mathbf{1}\{X \le \theta_P\} + (X-\theta) \mathbf{1}\{\theta < X \le \theta_P\}\big\}^2 \\
    &\le 2(\gamma^2 +2)|\theta_P-\theta|^2,
\end{align*}
and thus we obtain
\begin{align*}
    	\E_P \left[\sup_{\|\theta-\theta_P\| < \delta}|\mathbb{G}_n (m_\theta - m_{\theta_P})| \right] \vee \sup_{\|\theta-\theta_P\| < \delta}\, \sqrt{P(m_{\theta} - m_{\theta_P})^2}\le\sqrt{2}(2+\gamma)\delta =: \phi(\delta).
    \end{align*}
By Lemma~\ref{prop:squared-Gn}, we also obtain 
\begin{align*}
    \omega^2(\delta) = C\left\{ n^{1/2} \left(\mathbb{E}_P M_\delta^2 \right)+ \left(\mathbb{E}_PM_\delta^2\right)^{1/2}\E_P \left[\sup_{m \in \mathcal{M}_{\delta}}\, \left|\sum_{i=1}^n \varepsilon_i m(X_i)\right|\right]\right\} = C\sqrt{2}(2+\gamma)^2n^{1/2}\delta^2.
\end{align*}
It remains to solve equations in Theorem~\ref{thm:concentration-width-unbounded} to derive the rate of convergence. Dropping constants, 
\begin{align*}
    (2+\gamma)r_n^{2/(1+\beta)}r_n^{-2} \le n^{1/2} \Longrightarrow (2+\gamma)^{(1+\beta)/(2\beta)}n^{-(1+\beta)/(4\beta)} \le r_n
\end{align*}
and 
\begin{align*}
    C^{1/2}(2+\gamma)n^{1/4}u_n^{2/(1+\beta)}u_n^{-2} \le n^{3/4} \Longrightarrow C^{(1+\beta)/(4\beta)}(2+\gamma)^{(1+\beta)/(2\beta)}n^{-(1+\beta)/(4\beta)} \le u_n.
\end{align*}
While $\gamma$ may depend on $n$, we observe that 
\begin{align*}
    2^{(1+\beta)/(2\beta)} \le (2+\gamma)^{(1+\beta)/(2\beta)} \le 3^{(1+\beta)/(2\beta)},
\end{align*}
and hence the leading constant does not depend on $n$. Finally by Theorem~\ref{thm:concentration-width-unbounded}, we conclude the width of the confidence set is bounded with probability $1-\varepsilon$ by
\begin{align*}
    &\mathfrak{C}(r_n^{2/(1+\beta)} + u_n^{2/(1+\beta)}+s_n^{1/(1+\beta)})\le \mathfrak{C}\left(\frac{1}{n^{1/2\beta}} + s_n^{1/(1+\beta)}\right)
\end{align*}
with $\mathfrak{C}$ depending on $\alpha, \beta, M_0, M_1$ and $\varepsilon$.


We now consider the case (2). For any $\theta = \theta_P + \ell u$ such that $u \in \{-1, 1\}$ and $\ell > \delta$, we define $\bar\theta = \theta_P + \ell u$. Since $\bar\theta = (1-\delta/\ell)\theta_P + \delta/\ell \theta$, it follows by the convexity of $\theta \mapsto Pm_{\theta}$, 
\begin{align*}
     (1-\delta/\ell) Pm_{\theta_P} - \delta/\ell Pm_{\theta} \ge Pm_{\bar \theta} \Longleftrightarrow  Pm_{\theta}-Pm_{\theta_P}  \ge (\ell/\delta)(Pm_{\bar \theta} -Pm_{\theta_P}) \ge\mathfrak{C}  |\theta-\theta_P|\delta^{\beta}.
\end{align*}
Next, recall for any $\theta \in \Theta$,  
\begin{align*}
	|m_{\theta}-m_{\theta_P}|\le \sqrt{2}(2+\gamma)|\theta-\theta_P| 
\end{align*}
and this implies 
\begin{align*}
	\widehat \sigma_{\theta, \theta_P}^2 \le \mathbb{P}_n|m_{\theta}-m_{\theta_P}|^2 \le 2(2+\gamma)^2|\theta-\theta_P|^2 \quad\textrm{and}\quad  \widehat \sigma_{\widehat\theta_1, \theta_P}^2  \le 2(2+\gamma)^2|\widehat\theta_1-\theta_P|^2.
\end{align*}	
Any $\theta \in \widehat{\mathrm{CI}}_{n,\alpha}^{\gamma}$ satisfies 
\begin{align*}
    &\mathbb{P}_n(m_{\theta} - m_{\widehat{\theta}_1}) - q_{1-\alpha}n^{-1/2}\widehat\sigma_{\theta, \widehat{\theta}_1} \le 0 \\
    &\qquad \Longleftrightarrow P(m_{\theta} - m_{\theta_P}) + (\mathbb{P}_n-P)(m_{\theta} - m_{\theta_P}) \le \mathbb{P}_n(m_{\widehat{\theta}_1} - m_{\theta_P}) + q_{1-\alpha}n^{-1/2}\widehat\sigma_{\widehat{\theta}_1,\theta}\\
    &\qquad \Longrightarrow P(m_{\theta} - m_{\theta_P}) + (\mathbb{P}_n-P)(m_{\theta} - m_{\theta_P}) \\
    &\qquad\qquad \le \mathbb{P}_n(m_{\widehat{\theta}_1} - m_{\theta_P}) + q_{1-\alpha}n^{-1/2}\sqrt{2}(2+\gamma)\left(|\theta-\theta_P|+ |\widehat{\theta}_1-\theta_P|\right)\\
    &\qquad \Longrightarrow P(m_{\theta} - m_{\theta_P}) + (\mathbb{P}_n-P)(m_{\theta} - m_{\theta_P}) \\
    &\qquad\qquad \le \mathbb{P}_n(m_{\widehat{\theta}_1} - m_{\theta_P}) + q_{1-\alpha}n^{-1/2}\sqrt{2}(2+\gamma)\left(|\theta-\theta_P|+ |\widehat{\theta}_1-\theta_P|\right).
\end{align*}
When $|\theta-\theta_P| \ge \delta$, we have $P(m_{\theta} - m_{\theta_P}) > \mathfrak{C}\delta^{\beta+1}$. The lower bound of the above inequality can be written out as 
\begin{align}
	P(m_{\theta} - m_{\theta_P}) + (\mathbb{P}_n-P)(m_{\theta} - m_{\theta_P}) = P(m_{\theta} - m_{\theta_P})\left(1 + \frac{(\mathbb{P}_n-P)(m_{\theta} - m_{\theta_P})}{P(m_{\theta} - m_{\theta_P})}\right).
\end{align}
We claim that the fraction inside of the parenthesis is stochastically bounded when $|\theta-\theta_P| > \delta$. First, we observe that 
\begin{align*}
	\mathbb{E}\left[\sup_{\theta \in \Theta; |\theta-\theta_P| > \delta}\left|\frac{(\mathbb{P}_n-P)(m_{\theta} - m_{\theta_P})}{P(m_{\theta} - m_{\theta_P})}\right|\right]&\le \mathbb{E}\left[\sup_{\theta \in \Theta; |\theta-\theta_P| > \delta}\left|\frac{(\mathbb{P}_n-P)(m_{\theta} - m_{\theta_P})}{\mathfrak{C}|\theta-\theta_P|\delta^{\beta}}\right|\right] \\
    &\le \sqrt{\mathbb{E}\left[\sup_{\theta \in \Theta; |\theta-\theta_P| > \delta}\left|\frac{(\mathbb{P}_n-P)(m_{\theta} - m_{\theta_P})}{\mathfrak{C}|\theta-\theta_P|\delta^{\beta}}\right|^2\right]}\\
	&\le n^{-1/2}\mathfrak{C}^{-1}\delta^{-\beta}\left(\E \left[\sup_{\theta \in \Theta; |\theta-\theta_P| > \delta}\frac{|m_{\theta} - m_{\theta_P}|^2}{|\theta-\theta_P|^2}\right]\right)^{1/2}\\
	&\le n^{-1/2}\mathfrak{C}^{-1}\delta^{-\beta}(2+\gamma).
\end{align*}
Hence by Markov's inequality, we have 
\begin{align}
	\sup_{\theta \in \Theta; |\theta-\theta_P| > \delta}\left|\frac{(\mathbb{P}_n-P)(m_{\theta} - m_{\theta_P})}{P(m_{\theta} - m_{\theta_P})}\right| \le C_{\varepsilon, \beta, M_0, M_1} n^{-1/2}\delta^{-\beta}
	\end{align}
with probability greater than $1-\varepsilon$ for $C_{\varepsilon, \beta, M_0, M_1}$ large enough. Coming back to the inequality, we have 
\begin{align*}
	&P(m_{\theta} - m_{\theta_P}) + (\mathbb{P}_n-P)(m_{\theta} - m_{\theta_P}) \\&\qquad= P(m_{\theta} - m_{\theta_P})\left(1 + \frac{(\mathbb{P}_n-P)(m_{\theta} - m_{\theta_P})}{P(m_{\theta} - m_{\theta_P})}\right)\\
	&\qquad\ge P(m_{\theta} - m_{\theta_P})\left(1 - \sup_{|\theta-\theta_P| > \delta}\left|\frac{(\mathbb{P}_n-P)(m_{\theta} - m_{\theta_P})}{P(m_{\theta} - m_{\theta_P})}\right|\right)_+
	\\
	&\qquad\ge P(m_{\theta} - m_{\theta_P})\left(1 - C_{\varepsilon, \beta, M_0, M_1} n^{-1/2}\delta^{-\beta}\right)_+.
\end{align*}
On the event the inequality holds, and $n \ge 4C^2_{\varepsilon, \beta, M_0, M_1}\delta^{-2\beta}$, we have 
\[P(m_{\theta} - m_{\theta_P}) + (\mathbb{P}_n-P)(m_{\theta} - m_{\theta_P}) \ge 2^{-1}P(m_{\theta} - m_{\theta_P}) \ge2^{-1}\mathfrak{C}\delta^\beta|\theta-\theta_P|. \]
Plugging this result into the expression for the confidence set, we arrive at
\begin{align*}
    &\mathbb{P}_n(m_{\theta} - m_{\widehat{\theta}_1}) - q_{1-\alpha}n^{-1/2}\widehat\sigma_{\theta, \widehat{\theta}} \le 0 \\
    &\qquad \Longrightarrow 2^{-1}\mathfrak{C}\delta^\beta|\theta-\theta_P| \le \mathbb{P}_n(m_{\widehat{\theta}} - m_{\theta_P}) + q_{1-\alpha}n^{-1/2}\sqrt{2}(2+\gamma)\left(|\theta-\theta_P|+ |\widehat{\theta}-\theta_P|\right)\\
    &\qquad \Longrightarrow \left(2^{-1}\mathfrak{C}\delta^\beta-q_{1-\alpha}n^{-1/2}\sqrt{2}(2+\gamma)\right)_+|\theta-\theta_P| \\
    &\qquad\qquad\le \mathbb{P}_n(m_{\widehat{\theta}} - m_{\theta_P}) + q_{1-\alpha}n^{-1/2}\sqrt{2}(2+\gamma)|\widehat{\theta}-\theta_P|.
\end{align*}
Furthermore when $n \ge 16\mathfrak{C}^{-2}\delta^{-2\beta}q^2_{1-\alpha}\sqrt{2}(2+\gamma)^2$, the lower bound becomes strictly positive. Hence, it implies
\begin{align}
	\left(2^{-1}\mathfrak{C}\delta^\beta-q_{1-\alpha}n^{-1/2}\sqrt{2}(2+\gamma)\right)_+|\theta-\theta_P| \ge 2^{-2}\mathfrak{C}\delta^\beta |\theta-\theta_P|.
\end{align}
Putting together, we conclude that for $n \ge (32\mathfrak{C}^{-2}\delta^{-2\beta}q^2_{1-\alpha}(2+\gamma)^2 \vee 4C^2_{\varepsilon, \beta, M_0, M_1}\delta^{-2\beta})$, we have 
\begin{align*}
	|\theta-\theta_P| &\le 4\mathfrak{C}^{-1}\delta^{-\beta}\left(\mathbb{P}_n(m_{\widehat{\theta}} - m_{\theta_P}) + q_{1-\alpha}n^{-1/2}\sqrt{2}(2+\gamma)|\widehat{\theta}-\theta_P|\right)\\
 &\le 8\mathfrak{C}^{-1}\delta^{-\beta} q_{1-\alpha}\sqrt{2}(2+\gamma)|\widehat{\theta}-\theta_P|
\end{align*}
with probability greater than $1-\varepsilon$. 

Summarizing the results we obtained so far, we have shown that there exist constants $C_1, C_2, C_3$ all different but only depend on $\varepsilon, M_0, M_1, \beta$ such that for all $n \ge C_1 \delta^{-2\beta}$, we have 
\begin{align*}
\mathbb{P}_P\left(\mathrm{Diam}_{\|\cdot\|}\big(\widehat{\mathrm{CI}}_{n,\alpha}^{\gamma}\big)\le C_3\tau_n \right) \ge 1-\varepsilon
\end{align*}	
where 
\begin{align*}
    \tau_n = \left(\frac{1}{n^{1/2\beta}} + s_n^{1/(1+\beta)}\right)\mathbf{1}\{|\widehat{\theta}_1-\theta_P| \le C_2 \delta^{1+\beta}\} + \delta^{-\beta}|\widehat{\theta}_1-\theta_P|\mathbf{1}\{|\widehat{\theta}_1-\theta_P| > C_2 \delta^{1+\beta}\}.
\end{align*}
We conclude the first claim.

Next, we verify the requirements for $\widehat\theta_1$. Recalling that $|m_{\theta}-m_{\theta_P}|\lesssim |\theta-\theta_P|$ for any $\theta$. On the other hand, we have $P(m_{\theta} - m_{\theta_P}) \le |\widehat \theta_1 - \theta_P|\mathbb{P}_P(\widehat\theta < X \le \theta_P)$ when $|\widehat \theta_1 - \theta_P | < \delta$. Putting together implies
\begin{align*}
    |m_{\theta}-m_{\theta_P}| + n^{-1/2}\sqrt{P(m_{\widehat\theta_1}-m_{\theta_P})^2} \lesssim |\widehat\theta_1-\theta_P|^{1+\beta} +  \left(\frac{|\widehat\theta_1-\theta_P|^2}{n}\right)^{1/2} = s_n.
\end{align*}
Introducing an event $\mathcal{E}=:\{(\widehat\theta_1-\theta_P)^2 \lesssim n^{-1/\beta}\}$ such that $\mathbb{P}(\mathcal{E}) \ge 1-\varepsilon/2$. On the event $\Omega$, we take $n$ large enough so $|\widehat \theta_1 - \theta_P | < \delta$. We then conclude that $s_n^{1/(1+\beta)} \lesssim n^{-1/2\beta}$ with probability greater than $1-\varepsilon/2$. 

Finally by the first result of this theorem, it holds that 
\begin{align*}
\mathbb{P}_P\left(\mathrm{Diam}_{\|\cdot\|}\big(\widehat{\mathrm{CI}}_{n,\alpha}^{\gamma}\big)\le C_3\tau_n\right) \ge 1-\varepsilon/2
\end{align*}	
Furthermore, observe that 
\begin{align*}
\mathbb{P}_P\left(\mathrm{Diam}_{\|\cdot\|}\big(\widehat{\mathrm{CI}}_{n,\alpha}^{\gamma}\big)\le C_3\tau_n \right) &\le \mathbb{P}_P\left(\mathrm{Diam}_{\|\cdot\|}\big(\widehat{\mathrm{CI}}_{n,\alpha}^{\gamma}\big)\le C_3\tau_n \bigg | \mathcal{E}\right)\mathbb{P}(\mathcal{E}) + \varepsilon/2 \\
&=\mathbb{P}_P\left(\mathrm{Diam}_{\|\cdot\|}\big(\widehat{\mathrm{CI}}_{n,\alpha}^{\gamma}\big)\le \frac{\mathfrak{C}}{n^{1/2\beta}}  \bigg | \mathcal{E}\right)\mathbb{P}(\mathcal{E}) + \varepsilon/2 
\end{align*}
where the second equality holds for all $n \ge (C_2\delta)^{-\beta}$ on $\mathcal{E}$. This concludes the claim.
% \begin{align*}
%     &P(m_{\theta} - m_{\theta_P})^2 \\
%     &\qquad \le 2(\theta-\theta_0)^2 \mathbb{P}_P(Z \le \theta_0) +2\alpha^2(\theta-\theta_0)^2+ 2(\theta-\theta_0)^2 \mathbb{P}_P(\theta_0 < Z \le \theta) \le 6(\theta-\theta_0)^2.
% \end{align*}

% Using the trivial bound on the indicator function, we also obtain the following local envelope:
% \begin{align*}
%     M_\delta:= \sup_{|\theta-\theta_0| < \delta}\, |m_{\theta} - m_{\theta_0}|
%     & \le (2 + \alpha) \delta.
% \end{align*}
% \begin{align*}
% 	\sup_{\theta \in \Theta; |\theta-\theta_0| > \delta}\left|\frac{(\mathbb{P}_n-P)m_{\theta} - m_{\theta_0}}{P(m_{\theta} - m_{\theta_0})}\right| \le \sup_{\theta \in \Theta; |\theta-\theta_0| > \delta}\left|\frac{(\mathbb{P}_n-P)m_{\theta} - m_{\theta_0}}{\mathfrak{C}|\theta-\theta_0|\delta^{\beta}}\right|
% \end{align*}

% Next, when $P(m_{\theta} - m_{\theta_0}) > r_n^2$, we have 
% \begin{align*}
%     & P(m_{\theta} - m_{\theta_0}) + (\mathbb{P}_n-P)(m_{\theta} - m_{\theta_0}) \\
%     &\qquad\qquad \le \mathbb{P}_n(m_{\widehat{\theta}} - m_{\theta_0}) + q_{1-\alpha}n^{-1/2}\|g\|_{L_2(\mathbb{P}_n)}\left(\|\theta-\theta_0\|+ \|\widehat{\theta}-\theta_0\|\right)^\nu\\
%     &\qquad \Longleftrightarrow P(m_{\theta} - m_{\theta_0}) \left(1 + \frac{(\mathbb{P}_n-P)(m_{\theta} - m_{\theta_0})}{P(m_{\theta} - m_{\theta_0})}\right) \\
%     &\qquad\qquad \le \mathbb{P}_n(m_{\widehat{\theta}} - m_{\theta_0}) + q_{1-\alpha}n^{-1/2}\|g\|_{L_2(\mathbb{P}_n)}\left(\|\theta-\theta_0\|+ \|\widehat{\theta}-\theta_0\|\right)^\nu\\
%     &\qquad \Longrightarrow C\left(\|\theta-\theta_0\|^{1+\beta} \wedge \|\theta-\theta_0\|\delta^{\beta}\right) \left(1 - \sup_{\theta \in \Theta; P(m_{\theta} - m_{\theta_0}) > r_n}\left|\frac{(\mathbb{P}_n-P)(m_{\theta} - m_{\theta_0})}{P(m_{\theta} - m_{\theta_0})}\right|\right)_+ \\
%     &\qquad\qquad \le \mathbb{P}_n(m_{\widehat{\theta}} - m_{\theta_0}) + q_{1-\alpha}n^{-1/2}\|g\|_{L_2(\mathbb{P}_n)}\left(\|\theta-\theta_0\|+ \|\widehat{\theta}-\theta_0\|\right)^\nu
% \end{align*}
% For a moment, we assume that 
% \[\sup_{\theta \in \Theta; P(m_{\theta} - m_{\theta_0}) > r_n^2}\left|\frac{(\mathbb{P}_n-P)(m_{\theta} - m_{\theta_0})}{P(m_{\theta} - m_{\theta_0})}\right| \le C_\varepsilon < 1\]
% with probability greater than $1-\varepsilon$. Then we have 
% \begin{align*}
%     &C_\varepsilon\left(\|\theta-\theta_0\|^{1+\beta} \wedge \|\theta-\theta_0\|\delta^{\beta}\right) \le \mathbb{P}_n(m_{\widehat{\theta}} - m_{\theta_0}) \\
%     &\qquad\qquad+ q_{1-\alpha}n^{-1/2}\|g\|_{L_2(P)}\left(\|\theta-\theta_0\|+ \|\widehat{\theta}-\theta_0\|\right)^\nu.
% \end{align*}
% When $\|\theta-\theta_0\| > \delta$, we have 
% \begin{align*}
%     C_\varepsilon\|\theta-\theta_0\|\delta^{\beta} \le \mathbb{P}_n(m_{\widehat{\theta}} - m_{\theta_0}) + q_{1-\alpha}n^{-1/2}\|g\|_{L_2(P)}\left(\|\theta-\theta_0\|+ \|\widehat{\theta}-\theta_0\|\right)^\nu.
% \end{align*}
% Requiring that $\nu \le 1$, we have 
% \begin{align*}
%     &\|\theta-\theta_0\|\left(C_\varepsilon\delta^{\beta}- q_{1-\alpha}n^{-1/2}\|g\|_{L_2(P)}\delta^{\nu-1}\right)_+ \le \mathbb{P}_n(m_{\widehat{\theta}} - m_{\theta_0}) + q_{1-\alpha}n^{-1/2}\|g\|_{L_2(P)}\|\widehat{\theta}-\theta_0\|^\nu\\
%     &\qquad \Longrightarrow \|\theta-\theta_0\| \le \frac{\mathbb{P}_n(m_{\widehat{\theta}} - m_{\theta_0}) + q_{1-\alpha}n^{-1/2}\|g\|_{L_2(P)}\|\widehat{\theta}-\theta_0\|^\nu}{\left(C_\varepsilon\delta^{\beta}- q_{1-\alpha}n^{-1/2}\|g\|_{L_2(P)}\delta^{\nu-1}\right)_+} \wedge T_n
% \end{align*}

% When $\|\theta-\theta_0\| < \delta$, we can use the usual peeling. \kt{This means that \[|m_{\theta}(Z) - m_{\theta_0}(Z)| \le g(Z)\|\theta-\theta_0\|^\nu\] needs to hold only when $\|\theta - \theta_0\| > \delta$}


% \kt{
% We can control 
% \begin{align*}
%     &\left(1 - \sup_{\theta \in \Theta; P(m_{\theta} - m_{\theta_0}) > \mathfrak{C}\delta^{1+\beta}}\left|\frac{(\mathbb{P}_n-P)(m_{\theta} - m_{\theta_0})}{P(m_{\theta} - m_{\theta_0})}\right|\right)_+ \\
%     &\qquad \le  \left(1 - \sup_{\theta \in \Theta; P(m_{\theta} - m_{\theta_0}) > \mathfrak{C}\delta^{1+\beta}}\left|\frac{(\mathbb{P}_n-P)(2 + \alpha) |\theta-\theta_0|}{\mathfrak{C}\delta^\beta|\theta-\theta_0|}\right|\right)_+
% \end{align*}
% \begin{align*}
%     \E\left[\sup_{\theta \in \Theta} \left|(\mathbb{P}_n-P) \frac{m_{\theta}-m_{\theta_0}}{\mathfrak{C}\delta^\beta |\theta-\theta_0|}\right|\right] &\le \sqrt{ \E\left[\sup_{\theta \in \Theta} \left((\mathbb{P}_n-P) \frac{m_{\theta}-m_{\theta_0}}{\mathfrak{C}\delta^\beta |\theta-\theta_0|}\right)^2\right]}\\
%     &=n^{-1/2} 
% \end{align*}
% }

\end{proof}

% \subsection{On the uniform Lindeberg condition}
% This section provides several propositions, which implies the \eqref{eq:validity-condition-clt}
% \begin{proposition}
%     Assume that
% \begin{align*}
%      \underline{M}(Z) \varphi(\|\theta(P)-\theta\|) \le m_{\theta(P)}(Z)-m_{ \theta}(Z) - P(m_{\theta(P)} - m_{\theta}) \le \overline{M}(Z)\varphi(\|\theta(P)-\theta\|)
% \end{align*}
% for all $\theta$ such that $\|\theta-\theta(P)\| \le \delta$ for some $\delta > 0$. Then 
% \end{proposition}
% \begin{proof}
% \begin{align*}
%     \E_P\left[\frac{\langle t, W \rangle^2}{B^2} \left\{1 \wedge n^{-1/2}\frac{|\langle t, W \rangle|}{B}\right\}\right] \le \E_P\left[\frac{\langle t,\overline{M}(Z) \rangle^2}{P \underline{M}^2} \left\{1 \wedge n^{-1/2}\frac{|\langle t, \overline{M} \rangle|}{(P \underline{M}^2)^{1/2}}\right\}\right]
% \end{align*}
% \end{proof}
\section{Technical Lemma}\label{sec:technical-lemma}
We denote the localized collection of functions by 
\begin{align*}
    \mathcal{M}_{\delta} := \{m_\theta(z) - m_{\theta_0}(z)\, : \| \theta - \theta_0\| \le \delta\}
\end{align*}
and let the envelope be denoted by $M_\delta := z \mapsto \sup_{m \in \mathcal{M}_{\delta}}|m(z)|$. The following result provides the upper bound on the expectation of the squared empirical process without requiring the boundedness assumption on the $\mathcal{M}_\delta$. 
\begin{lemma}\label{prop:squared-Gn}
Given $n$ IID random variables, $Z_1, \ldots, Z_n$, the following holds:
    \begin{align*}
        \E_P \left[\sup_{m\in\mathcal{M}_{\delta}}\, |\mathbb{G}_n m^2 |\right] \le  C\left\{ n^{1/2} \left(\mathbb{E}_P M_\delta^2 \right)+ \left(\mathbb{E}_PM_\delta^2\right)^{1/2}\E_P \left[\sup_{m \in \mathcal{M}_{\delta}}\, \left|\sum_{i=1}^n \varepsilon_i m(Z_i)\right|\right]\right\}
    \end{align*}
    where $\{\varepsilon_i\}_{i=1}^n$ is a sequence of independent Rademacher random variables and $C$ is a universal constant.
\end{lemma}
\begin{proof}[\bfseries{Proof of Lemma \ref{prop:squared-Gn}}]
Define a truncation parameter $B := 8 n^{1/2} (\E_P M_\delta^2)^{1/2}$ and let $\{\varepsilon_i\}_{i=1}^n$ be a sequence of independent Rademacher random variables. Then, we have 
    \begin{align*}
    	\E_P \left[\sup_{m \in \mathcal{M}_\delta}\, |\mathbb{G}_n m^2| \right]& = n^{-1/2}\E_P \left[\sup_{m\in\mathcal{M}_{\delta}}\, \left|\sum_{i=1}^n m^2(Z_i) - \mathbb{E}_P m^2\right| \right]\\
     & \le 2n^{-1/2}\E_{P\times \varepsilon} \left[\sup_{m \in \mathcal{M}_\delta}\, \left|\sum_{i=1}^n \varepsilon_i m^2(Z_i)\right|\right]\\
     & \le 2n^{-1/2}\E_{P\times \varepsilon} \left[\sup_{m \in \mathcal{M}_\delta}\, \left|\sum_{i=1}^n \varepsilon_i m^2(Z_i)\mathbf{1}\{M_\delta 
 > B\}\right|\right] \\
 &\qquad+ 2n^{-1/2}\E_{P\times \varepsilon} \left[\sup_{m \in \mathcal{M}_\delta}\, \left|\sum_{i=1}^n \varepsilon_i m^2(Z_i)\mathbf{1}\{M_\delta 
 \le B\}\right|\right].
    \end{align*}
where the second inequality follows from symmetrization (see for instance, Lemma 2.3.1 of \cite{van1996weak}). We now handle two terms separately. For the unbounded part, we have 
\begin{align*}
    &\E_P \left[\sup_{m \in \mathcal{M}_\delta}\, \left|\sum_{i=1}^n \varepsilon_i m^2(Z_i)\mathbf{1}\{M_\delta 
 > B\}\right|\right] \le \E_P \left[\left|\sum_{i=1}^n  M_\delta^2(Z_i)  \mathbf{1}\{M_\delta 
 > B\}\right|\right].
\end{align*}
We apply the Hoffmann-J$\o$rgensen inequality (See Proposition 6.8 of \citet{ledoux2013probability} with $p=1$), which states 
\begin{align*}
    \E_P \left[\left|\sum_{i=1}^n M_\delta^2(Z_i)\mathbf{1}\{M_\delta 
 > B\}\right|\right] \le 8 \left(\mathbb{E}_P\left[\max_{1\le i \le n} M_\delta^2(Z_i)\right] + t_0^2\right)
\end{align*}
for any $t_0$ such that 
\begin{align}\label{eq:condition-for-HJ}
    \mathbb{P}_P\left(\sum_{i=1}^n M_\delta^2(Z_i) \mathbf{1}\{M_\delta 
 > B\} > t_0\right) \le 1/8.
\end{align}

At our truncation level $B$, the result follows with $t_0=0$. We can indeed verify \eqref{eq:condition-for-HJ} by observing 
\begin{align*}
     \mathbb{P}_P\left(\sum_{i=1}^n M_\delta^2 \mathbf{1}\{M_\delta 
 > B\} > 0\right) &\le \mathbb{P}_P\left(\max_{1\le i\le n}M_\delta(Z_i) 
 > B\right) \\
 &\le \frac{\mathbb{E}_P[\max_{1\le i\le n}M_\delta(Z_i) ]}{B}\\
 &\le \frac{\left(\mathbb{E}_P[\sum_{i=1}^n M^2_\delta(Z_i) ]\right)^{1/2}}{B} \le 1/8.
\end{align*}
Hence by the Hoffmann-J$\o$rgensen inequality, we conclude
\begin{align*}
    2n^{-1/2}\E_P \left[\sup_{m \in \mathcal{M}_\delta}\, \left|\sum_{i=1}^n \varepsilon_i m^2(Z_i)\mathbf{1}\{M_\delta 
 > B\}\right|\right] &\le 16n^{-1/2} \mathbb{E}_P\left[\max_{1\le i \le n} |M_\delta(Z_i)|^2\right] \\
 &\le 16n^{1/2} \left(\mathbb{E}_P M_\delta^2\right).
\end{align*}
For the second term, we observe that the entire process is uniformly bounded by $B$. We can thus apply the contraction inequality, such as, Theorem 4.12 of \cite{ledoux2013probability} or Corollary 3.2.2 of \cite{gine2021mathematical}. This in tern implies that 
\begin{align*}
    2n^{-1/2}\E_P \left[\sup_{m \in \mathcal{M}_\delta}\,\left|\sum_{i=1}^n \varepsilon_i m^2(Z_i)\mathbf{1}\{M_\delta 
 \le B\}\right|\right] &\le 4B n^{-1/2}\E_P \left[\sup_{m \in \mathcal{M}_\delta}\,\left|\sum_{i=1}^n \varepsilon_i m(Z_i)\right|\right]\\
 &= 4\left(\mathbb{E}_PM_\delta^2\right)^{1/2}\E_P \left[\sup_{m \in \mathcal{M}_\delta}\,\left|\sum_{i=1}^n \varepsilon_i m(Z_i)\right|\right],
\end{align*}
thus we conclude the claim.
\end{proof}
\begin{lemma}\label{lemma:moment-bounds}
    Suppose that $X$ and $Y$ are the random variables defined on a common measurable space, satisfying $\mathbb{E}|X-Y|^2 \le C \mathbb{E}[X^2]$ with some constant $C>0$.
    Then we have the following three upper bounds:
    \begin{enumerate}
        \item \[\mathbb{E}\left[\left|\frac{X^2}{\mathbb{E}[X^2]}-\frac{Y^2}{\mathbb{E}[Y^2]}\right|\right] \leq 4 (C+ C^{1 / 2})\]
        \item For any $\kappa > 0$,
        \[\mathbb{E}{\left[\frac{X^2}{\mathbb{E}[X^2]} \mathbf{1}\{X^2>\kappa\mathbb{E}[X^2]\}\right]-\mathbb{E}\left[\frac{Y^2}{\mathbb{E}[Y^2]}  \mathbf{1}\{Y^2>\kappa\mathbb{E}[Y^2]\}\right] } \leq  16(C+ C^{1 / 2})\]
        \item For any $\kappa > 0$,
        \[\mathbb{E} {\left[\left(\frac{X^2}{\mathbb{E}[X^2]}\right)^{3/2} \mathbf{1}\{X^2\le \kappa\mathbb{E}[X^2]\}\right]-\mathbb{E}\left[\left(\frac{Y^2}{\mathbb{E}[Y^2]}\right)^{3/2}  \mathbf{1}\{Y^2\le \kappa\mathbb{E}[Y^2]\}\right] } \leq  16 \kappa^{1/2} (C+ C^{1 / 2}).\]
    \end{enumerate}
\end{lemma}
\begin{proof}[\bfseries{Proof of Lemma~\ref{lemma:moment-bounds}}]
    Suppose $X$ and $Y$ are random variables such that $\mathbb{E}|X-Y|^2 \le C \mathbb{E}[X^2]$.
To obtain the first result, we observe that 
\begin{align*}
\mathbb{E}\left[\left|\frac{X^2}{\mathbb{E}[X^2]}-\frac{Y^2}{\mathbb{E}[Y^2]}\right|\right] 
&=\mathbb{E}\left[\left|\frac{X^2 \mathbb{E}[Y^2]-\mathbb{E}[X^2] Y^2}{\mathbb{E}[X^2] \mathbb{E}[Y^2]}\right|\right] \\
&\le \mathbb{E}\left[\left|\frac{(X^2-Y^2) \mathbb{E}[Y^2]}{\mathbb{E}[X^2] \mathbb{E}[Y^2]}\right|\right]+\mathbb{E}\left[\left|\frac{Y^2(\mathbb{E}[Y^2]-\mathbb{E}[X^2])}{\mathbb{E}[X^2] \mathbb{E}[Y^2]}\right|\right] \\
& =\frac{\mathbb{E}[|X^2-Y^2|]}{\mathbb{E}[X^2]}+\frac{|\mathbb{E}[Y^2-X^2]|}{\mathbb{E}[X^2]} \\
&\leq \frac{2\mathbb{E}[|Y^2-X^2|]}{\mathbb{E}[X^2]} 
\end{align*}
by Jensen's inequality. Since $Y^2=(Y-X)^2+2 X(Y-X)+X^2$, we obtain
\begin{align*}
	\mathbb{E}[| Y^2-X^2|] &= \mathbb{E}[|Y-X|^2] +2\mathbb{E}[ X(Y-X)]\\
	&\leq  \mathbb{E}[|Y-X|^2]+2\left(\mathbb{E}[X^2]\right)^{1/2}\left(\mathbb{E}[|Y-X|^2]\right)^{1 / 2}\\
%	&\le  C \mathbb{E}[X^2]+2\left(\mathbb{E}[X^2]\right)^{1/2}\left(C \mathbb{E}[X^2]\right)^{1 / 2}\\
	&\le  C \mathbb{E}[X^2]+2C^{1/2}\mathbb{E}[X^2]
	\end{align*}
by Cauchy-Schwarz inequality. Hence we conclude 
\begin{align*}
	\mathbb{E}\left[\left|\frac{X^2}{\mathbb{E}[X^2]}-\frac{Y^2}{\mathbb{E}[Y^2]}\right|\right] 
\leq \frac{2\mathbb{E}[|Y^2-X^2|]}{\mathbb{E}[X^2]} \le 2C +4C^{1/2}.
\end{align*}
%$$
%\mathbb{E}[| Y^2-X^2|] \leq \mathbb{E}[|X-Y|^2]+2\left(\mathbb{E}[X^2]\right)^{1 / 2}\left(\mathbb{E}\left[\left|Y-X\right|^2\right]\right)^{1 / 2} \text {. }
%$$
%
%Therefore,
%$$
%\mathbb{E}\left[\left|\frac{X^2}{\mathbb{E}[X^2]}-\frac{Y^2}{\mathbb{E}[Y^2]}\right|\right] \leq 2 C+2 C^{1 / 2} .
%$$
%To deal with 
%\begin{align}
%	\mathbb{E}\left[\left|X-Y\right|^2\right] \leq 2 C \mathbb{E}\left[\left|Y\right|^2\right]+2 C \mathbb{E}\left[\left|X-Y\right|^2\right]
%\end{align}
%$$
%\mathbb{E}\left[\left|X-Y\right|^2\right] \leq 2 C \mathbb{E}\left[\left|Y\right|^2\right]+2 C \mathbb{E}\left[\left|X-Y\right|^2\right] \text {. }
%$$
%
%Hence, if $C<1 / 2$, then
%$$
%\mathbb{E}\left[\left|X-Y\right|^2\right] \leq \frac{2 C}{1-2 C} \mathbb{E}\left[\left|Y\right|^2\right] .
%$$
%
%We first provide the $\mathbb{E}\left[\left(X^2 / \mathbb{E}[X^2]\right) 1\left\{X^2 / \mathbb{E}[X^2]>t\right\}\right]$ in terms of $\mathbb{E}\left[\left(Y^2 / \mathbb{E}[Y^2]\right) 1\left\{Y^2 / \mathbb{E}[Y^2]>t\right\}\right]$. First, note that
%$$
%\begin{aligned}
%& \mathbb{E}\left[\left|\frac{X^2}{\mathbb{E}[X^2]}-\frac{Y^2}{\mathbb{E}[Y^2]}\right|\right] \\
%& =\mathbb{E}\left[\left|\frac{X^2 \mathbb{E}[Y^2]-\mathbb{E}[X^2] Y^2}{\mathbb{E}[X^2] \mathbb{E}[Y^2]}\right|\right] \\
%& =\mathbb{E}\left[\left\lfloor\frac{\left(X^2-Y^2\right) \mathbb{E}[Y^2]}{\mathbb{E}[X^2] \mathbb{E}[Y^2]}\right\rceil\right]+\mathbb{E}\left[\left\lfloor\frac{Y^2\left(\mathbb{E}[Y^2]-\mathbb{E}[X^2]\right)}{\mathbb{E}[X^2] \mathbb{E}[Y^2]}\right\rceil\right] \\
%& =\frac{\mathbb{E}\left[\left|X^2-Y^2\right|\right]}{\mathbb{E}[X^2]}+\frac{\left|\mathbb{E}\left[Y^2-X^2\right]\right|}{\mathbb{E}[X^2]} \leq 2 \frac{\mathbb{E}\left[\left|Y^2-X^2\right|\right]}{\mathbb{E}[X^2]} . \\
%&
%\end{aligned}
%$$
%
%Because $Y^2=\left(Y-X\right)^2+2 X\left(Y-X\right)+X^2$, we get
%$$
%\mathbb{E}\left[\mid Y^2-X^2 \|\right] \leq \mathbb{E}\left[\left|X-Y\right|^2\right]+2\left(\mathbb{E}[X^2]\right)^{1 / 2}\left(\mathbb{E}\left[\left|Y-X\right|^2\right]\right)^{1 / 2} \text {. }
%$$
%
%Therefore,
%$$
%\mathbb{E}\left[\left|\frac{X^2}{\mathbb{E}[X^2]}-\frac{Y^2}{\mathbb{E}[Y^2]}\right|\right] \leq 2 C+2 C^{1 / 2} .
%$$
Moving onto the second result, we first denote by $\widetilde{X}=X^2 / \mathbb{E}[X^2]$ and $\widetilde{Y}=Y^2 / \mathbb{E}[Y^2]$. It then follows that 
\begin{align*}
	& \mathbb{E}[\widetilde{X} \mathbf{1}\{\widetilde{X}>\kappa\}]-\mathbb{E}[\widetilde{Y}\mathbf{1}\{\widetilde{Y}>\kappa\}] \\
& \qquad \leq \mathbb{E}[\widetilde{X} \mathbf{1}\{\widetilde{X}>\kappa / 2\}]-\mathbb{E}[\widetilde{Y}\mathbf{1}\{\widetilde{Y}>\kappa\}] \\
& \qquad\leq \mathbb{E}[\widetilde{X} \mathbf{1}\{\widetilde{X}>\kappa / 2, \widetilde{Y}>\kappa\}]+\mathbb{E}[\widetilde{X} \mathbf{1}\{\widetilde{X}>\kappa / 2, \widetilde{Y}\leq \kappa\}] \\
&\qquad\qquad -\mathbb{E}[\widetilde{Y}\mathbf{1}\{\widetilde{Y}>\kappa,\widetilde{X}>\kappa / 2\}]-\mathbb{E}[\widetilde{Y}\mathbf{1}\{\widetilde{Y}>\kappa,\widetilde{X} \leq \kappa / 2\}] \\
& \qquad\leq \mathbb{E}[| \widetilde{X}-\widetilde{Y}|]+\mathbb{E}[\widetilde{X} \mathbf{1}\{\widetilde{X}>\kappa / 2, \widetilde{Y}\leq \kappa\}] \\
&\qquad \leq \mathbb{E}[|\widetilde{X}-\widetilde{Y}|]+\mathbb{E}[(\widetilde{X}-\widetilde{Y}) \mathbf{1}\{\widetilde{X}>\kappa / 2,\widetilde{Y}\leq \kappa\}]+\mathbb{E}[\widetilde{Y} \mathbf{1}\{\widetilde{X}>\kappa / 2,\widetilde{Y}\leq \kappa\}] \\
&\qquad \leq 2 \mathbb{E}[|\widetilde{X}-\widetilde{Y}|]+\kappa \mathbb{E}[\mathbf{1}\{|\widetilde{X}-\widetilde{Y}|>\kappa / 2\}] \\
& \qquad\leq 4 \mathbb{E}[|\widetilde{X}-\widetilde{Y}|].
\end{align*}
Using the first result, the second claim is obtained.

Finally, it follows that 
\begin{align*}
	& \mathbb{E}[\widetilde{X}^{3 / 2} \mathbf{1}\{\widetilde{X} \leq \kappa\}]-\mathbb{E}[\widetilde{Y}^{3 / 2} \mathbf{1}\{\widetilde{Y}\leq \kappa\}] \\
& \qquad\leq \mathbb{E}[\widetilde{X}^{3 / 2} \mathbf{1}\{\widetilde{X} \leq \kappa\}]-\mathbb{E}[\widetilde{Y}^{3 / 2} \mathbf{1}\{\widetilde{Y}\leq \kappa / 2\}] \\
 &\qquad\leq \mathbb{E}[(\widetilde{X}^{3 / 2}-\widetilde{Y}^{3 / 2}) \mathbf{1}\{\widetilde{X} \leq \kappa, \widetilde{Y}\leq \kappa / 2\}] \\
&\qquad\qquad +\mathbb{E}[\widetilde{X}^{3 / 2} \mathbf{1}\{\widetilde{X} \leq \kappa,\widetilde{Y}>\kappa / 2\}]-\mathbb{E}[\widetilde{Y}^{3 / 2} \mathbf{1}\{\widetilde{X}>\kappa,\widetilde{Y}\leq \kappa / 2\}] \\
 &\qquad\leq \frac{3}{2} \kappa^{1 / 2} \mathbb{E}[|\widetilde{Y}-\widetilde{X}|]+\kappa^{3 / 2} \mathbb{P}(|\widetilde{X}-\widetilde{Y}|>\kappa / 2) \\
& \qquad\leq 4 \kappa^{1 / 2} \mathbb{E}[|\widetilde{Y}-\widetilde{X}|].
\end{align*}
Using the first result, the third claim is also obtained.
\end{proof}
% \section{Conservative and Bounded Confidence Sets}\label{sec:bounded-set}
% Suppose $\theta_1, \theta_2\in\Theta$ be such that $\|\theta_1 - \theta_2\| = 1$. Consider a subsample of original data of size $m$ and consider the set
% \[
% \widehat{S}_m := \{\theta:\, \M_m(\theta) \le \max\{\M_m(\theta_1),\, \M_m(\theta_2)\}\}
% \]
% where $\M_m(\theta) = m^{-1}\sum_{i=1}^m m_{\theta}(Z_i)$. Then
% \begin{align*}
% \mathbb{P}_P(\theta(P)\notin \widehat{S}_m) &= \mathbb{P}_P\left(\M_m(\theta(P)) > \M_m(\theta_1),\, \M_m(\theta(P)) > \M_m(\theta_2)\right)\\
% &\le \min_j\left\{\mathbb{P}_P(\M_m(\theta(P)) - \M_m(\theta_j) > 0)\right\}\\
% &\le \min_j\left\{\mathbb{P}_P((\M_m - \M)(\theta(P)) - (\M_m - \M)(\theta_j) > \M(\theta_j) - \M(\theta(P)))\right\}\\
% &\le \min_j\frac{\mbox{Var}((\M_m - \M)(\theta(P)) - (\M_m - \M)(\theta_1))}{\mbox{Var}((\M_m - \M)(\theta(P)) - (\M_m - \M)(\theta_1))+(\M(\theta_j) - \M(\theta(P)))^2}\\
% &\le \min_j\,\frac{\mathbb{E}_P[(m_{\theta(P)} - m_{\theta_j})^2(X)]}{m(\mathbb{E}_P[(m_{\theta(P)} - m_{\theta_j})(X)])^2 + \mbox{Var}(m_{\theta(P)} - m_{\theta_j})} \\
% &\le \frac{\mathfrak{C}_{\theta(P), \theta_1, \theta_2}}{m}
% \end{align*}
% where the third inequality follows by the Cantelli's inequality. Note that $\mathfrak{C}_{\theta(P), \theta_1, \theta_2}$ can be bounded by a constant if $\M(\theta) - \M(\theta(P)) \ge \underline{C}\|\theta - \theta(P)\|$ and $\mathbb{E}_P[(m_{\theta} - m_{\theta(P)})^2(X)] \le \overline{C}\|\theta - \theta(P)\|^2$ for some constants $0 < \underline{C}, \overline{C} < \infty$. These correspond to \ref{as:margin} and \ref{as:local-entropy}. Even if $\M(\theta) - \M(\theta(P)) \ge \underline{C}\|\theta - \theta(P)\|^{1 + \beta}$ for all $\theta$, we can obtain such a constant since 
% \[
% \inf_{\theta(P)}\max_j\{\|\theta_j - \theta(P)\|\} = \frac{1}{2}.
% \]
% Therefore, $\widehat{S}_m$ is a confidence set with coverage converging to one with sample size as long as $m \longrightarrow \infty$. Moreover, the confidence can be boosted by considering two splits of the data and taking the union of the two confidence sets. 

% This strategy can be used to claim that the original proposed confidence interval retains coverage if the initial estimator $\widehat{\theta}_1$ is inconsistent. It is important to note that $\widehat{S}_m$ need not have coverage if we only consider one $\theta_1$ which is close to $\theta(P)$. For example, in linear regression case, the coverage bound could be of the order
% \[
% \frac{\mathbb{E}_P[(Y - X^{\top}\theta(P))^2(X^{\top}(\theta_1 - \theta(P)))^2]}{m(\mathbb{E}_P[(X^{\top}(\theta_1 - \theta(P)))^2])^2},
% \]
% which diverges if $\|\theta_1 - \theta(P)\| \ll m^{-1/2}$.


==> main/validity.tex <==
\section{Proofs}
\subsection{Proof of Theorem~\ref{thm:concentration-width}}

The confidence set based on the empirical Bernstein inequality satisfies the following:
	\begin{align}
		&\mathbb{P}_n (m_\theta-m_{\widehat \theta}) \le \sqrt{\frac{2\widehat \sigma^2_{\theta, \widehat\theta} \log(2/\alpha)}{n}} + \frac{6B_{\theta, \widehat \theta}\log(2/\alpha)}{n}\\
		&\qquad \Longleftrightarrow (\mathbb{P}_n-P_0) (m_\theta-m_{\widehat \theta}) \le -P_0 (m_\theta-m_{\widehat \theta}) + \sqrt{\frac{2\widehat \sigma^2_{\theta, \widehat\theta} \log(2/\alpha)}{n}} + \frac{6B_{\theta, \widehat \theta}\log(2/\alpha)}{n}\\
		&\qquad \Longleftrightarrow P_0 (m_\theta-m_{\widehat \theta}) \le -(\mathbb{P}_n-P_0) (m_\theta-m_{\widehat \theta}) + \sqrt{\frac{2\widehat \sigma^2_{\theta, \widehat\theta} \log(2/\alpha)}{n}} + \frac{6B_{\theta, \widehat \theta}\log(2/\alpha)}{n}\\
		&\qquad \Longleftrightarrow P_0 (m_\theta-m_{\theta_0})+P_0(m_{\theta_0}-m_{\widehat \theta}) \\
		&\qquad\qquad\le -(\mathbb{P}_n-P_0) (m_\theta-m_{\theta_0}+m_{\theta_0}-m_{\widehat \theta}) + \sqrt{\frac{2\widehat \sigma^2_{\theta, \widehat\theta} \log(2/\alpha)}{n}} + \frac{6B_{\theta, \widehat \theta}\log(2/\alpha)}{n}
	\end{align}

	
	Now the confidence set is given by 
	\begin{align}
		&\left\{\theta \in \Theta : P_0 (m_\theta-m_{\theta_0})+P_0(m_{\theta_0}-m_{\widehat \theta}) \right.\\
		&\qquad\left.\le -(\mathbb{P}_n-P_0) (m_\theta-m_{\theta_0}+m_{\theta_0}-m_{\widehat \theta}) +\sqrt{\frac{2\widehat \sigma^2_{\theta, \widehat\theta} \log(2/\alpha)}{n}} + \frac{6B_{\theta, \widehat \theta}\log(2/\alpha)}{n}\right\}\\
		& \subseteq \left\{\theta \in \Theta : P_0 (m_\theta-m_{\theta_0})\right.\\
		&\qquad\left.\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0}) +   \sqrt{\frac{2\widehat \sigma^2_{\theta, \theta_0} \log(2/\alpha)}{n}} + \frac{6B_{\theta,  \theta_0}\log(2/\alpha)}{n} + \Gamma_n(\widehat\theta, \theta_0)\right\}\\
		& \subseteq \left\{\theta \in \Theta : \|\theta-\theta_0\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0}) +   \sqrt{\frac{2\widehat \sigma^2_{\theta, \theta_0} \log(2/\alpha)}{n}} + \frac{6B_{\theta,  \theta_0}\log(2/\alpha)}{n} + \Gamma_n(\widehat\theta, \theta_0)\right\}
	\end{align}
	where 
	\[\Gamma_n(\widehat\theta, \theta_0) := \mathbb{P}_n(m_{\widehat \theta}-m_{\theta_0}) +\sqrt{\frac{2\widehat \sigma^2_{\widehat\theta, \theta_0} \log(2/\alpha)}{n}} + \frac{6B_{\widehat\theta,  \theta_0}\log(2/\alpha)}{n}. \]
Furthermore, we have
\begin{align*}
    \widehat \sigma^2_{\theta, \theta_0} = |n-1|^{-1} \left(\sum_{i=1}^n(m_{\widehat \theta}-m_{\theta_0})^2(Z_i)-n(\bar{m}_{\widehat\theta}-\bar{m}_{\theta_0})^2\right)\le |n-1|^{-1} \sum_{i=1}^n(m_{\widehat \theta}-m_{\theta_0})^2(Z_i)
\end{align*}
and hence 
\begin{align}
    \frac{\widehat \sigma^2_{\theta, \theta_0}}{n} \le \frac{1}{n(n-1)} \sum_{i=1}^n(m_{ \theta}-m_{\theta_0})^2(Z_i) = \frac{1}{n-1}\left(n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta_0})^2 + P_0 (m_{ \theta}-m_{\theta_0})^2\right).
\end{align}
The confidence set can be further contained in 
\begin{align*}
    &\left\{\theta \in \Theta : \|\theta-\theta_0\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0}) +   \sqrt{\frac{2\widehat \sigma^2_{\theta, \theta_0} \log(2/\alpha)}{n}} + \frac{6B_{\theta,  \theta_0}\log(2/\alpha)}{n} + \Gamma_n(\widehat\theta, \theta_0)\right\}\\
    &\qquad\subseteq \left\{\theta \in \Theta : \|\theta-\theta_0\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0}) +   \sqrt{\frac{2\log(2/\alpha)n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta_0})^2}{n-1}}\right.\\
    &\left.\qquad\qquad \qquad\qquad\qquad\qquad \qquad  +\sqrt{\frac{2\log(2/\alpha)P_0 (m_{ \theta}-m_{\theta_0})^2 }{n-1}} + \frac{6B_{\theta,  \theta_0}\log(2/\alpha)}{n} + \Gamma_n(\widehat\theta, \theta_0)\right\}\\
    &\qquad =: \widetilde{\textrm{CI}}_n.
\end{align*}
Given $\beta$ in \ref{as:margin} and the function $\phi_n$ in \ref{as:local-entropy}, we define $r_n$ as any value that satisfies 
\begin{align}
    r_n^{-2} \phi_n(r_n^{2/(1+\beta)}) \le \sqrt{n}.
\end{align}
We now denote by $\mathcal{B}_{\|\cdot\|}(\theta_0, \gamma)$ a $\|\cdot\|$-ball centered at $\theta_0$ with radius $\gamma > 0$. Define
\begin{align}
    \gamma_M := 2^{M/(1+\beta)} \left(r_n^{2/(1+\beta)} +  r_n^{1/(1+\beta)}n^{-1/(2+2\beta)} B_{\theta,  \theta_0}^{1/(2+2\beta)}+ \left\{\Gamma_n(\theta, \widehat\theta, \theta_0)\right\}^{1/(1+\beta)}\right)
\end{align}
where 
\begin{align*}
    \Gamma_n(\theta, \widehat\theta, \theta_0) := \sqrt{\frac{2\log(2/\alpha)P_0 (m_{ \theta}-m_{\theta_0})^2 }{n-1}} + \frac{6B_{\theta,  \theta_0}\log(2/\alpha)}{n} + \Gamma_n(\widehat\theta, \theta_0).
\end{align*}
\kt{I think I need to add absolute value around $\Gamma_n$.}
The constant $M > 0$ will be specified later. Then consider the partition of the parameter space $\Theta$ into 
\begin{align}
    \Theta \cap \mathcal{B}_{\|\cdot\|}(\theta_0, \gamma_M) \textrm{ and } \Theta \cap \mathcal{B}^c_{\|\cdot\|}(\theta_0, \gamma_M).
\end{align}
So far, we have shown that $\widehat{\textrm{CI}}_n \subseteq \widetilde{\textrm{CI}}_n$. We now consider the following elementary result:
\begin{align*}
     \widetilde{\textrm{CI}}_n \subseteq \mathcal{B}_{\|\cdot\|}(\theta_0, \gamma_M) \Longleftrightarrow \widetilde{\textrm{CI}}_n \cap \mathcal{B}^c_{\|\cdot\|}(\theta_0, \gamma_M) = \emptyset.
\end{align*}
In order to claim, with high probability, that the confidence set is contained in the ball $\mathcal{B}_{\|\cdot\|}(\theta_0, \gamma_M)$, we need to establish the existence of $M$ large enough such that for 
$\|\theta-\theta_0\| > \gamma_M$,
\begin{align*}
    \mathbb{P}\left(\|\theta-\theta_0\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0}) +   \sqrt{\frac{2\log(2/\alpha)n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta_0})^2}{n-1}}+\Gamma_n(\theta, \widehat\theta, \theta_0)\right)\le \varepsilon.
\end{align*}
It now follows that 
\begin{align}
    &\mathbb{P}\left(\|\theta-\theta_0\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0}) +   \sqrt{\frac{2\log(2/\alpha)n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta_0})^2}{n-1}}+\Gamma_n(\theta, \widehat\theta, \theta_0)\right)\\
    &\qquad \le \mathbb{P}\left(3^{-1}\|\theta-\theta_0\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0}) \right) \\
    &\qquad\qquad + \mathbb{P}\left(3^{-1}\|\theta-\theta_0\|^{1+\beta}\le  \sqrt{\frac{2\log(2/\alpha)n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta_0})^2}{n-1}}\right)\\
    &\qquad\qquad + \mathbb{P}\left(3^{-1}\|\theta-\theta_0\|^{1+\beta}\le \Gamma_n(\theta, \widehat\theta, \theta_0)\right)
\end{align}

The third term is trivial as 
\begin{align}
    \mathbb{P}\left(3^{-1}\|\theta-\theta_0\|^{1+\beta} \le \Gamma_n(\theta, \widehat\theta, \theta_0)\right) &\le \mathbb{P}\left(3^{-1}\gamma_M^{1+\beta}\le \Gamma_n(\theta, \widehat\theta, \theta_0)\right) \\
    &\le \mathbb{P}\left(3^{-1}2^{M}\Gamma_n(\theta, \widehat\theta, \theta_0)\le \Gamma_n(\theta, \widehat\theta, \theta_0)\right) \\
    &\le 3\cdot 2^{-M}.\label{eq:term1}
\end{align}
The last display can be less than $\varepsilon/3$ for $M$ large enough. 


% We consider a ball 
% \begin{align*}
%     &\|\theta_0 - \theta\| \\
%     &\qquad \ge 2^M \left(r_n^{2/(1+\beta)} +  r_n^{1/(1+\beta)}n^{-1/(2+2\beta)} B_{\theta,  \theta_0}^{1/(2+2\beta)}+ \sqrt{\frac{2 P_0(m_{\theta}-m_{\theta_0})^2 \log(2/\alpha)}{n-1}}+\frac{6B_{\theta,  \theta_0}\log(2/\alpha)}{n}+ \Gamma_n(\widehat\theta, \theta_0)\right)
% \end{align*}
% $\|\theta_0 - \theta\| \ge 2^M r_n^{2/(1+\beta)}$ and (2) $\|\theta_0 - \theta\| < 2^M r_n^{2/(1+\beta)}$ with the constant $M$ to be specified later. Under the case (1), we claim that 
% \[\mathbb{P}\left(\|\theta-\theta_0\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0})+   \sqrt{\frac{2\widehat \sigma^2_{\theta, \theta_0} \log(2/\alpha)}{n}} + \frac{6B_{\theta,  \theta_0}\log(2/\alpha)}{n} + \Gamma_n(\widehat\theta, \theta_0)\right) \le \varepsilon.\]
% Furthermore, we have
% We thus have
% \begin{align*}
%     &\mathbb{P}\left(\|\theta-\theta_0\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0})+   \sqrt{\frac{2\widehat \sigma^2_{\theta, \theta_0} \log(2/\alpha)}{n}} + \frac{6B_{\theta,  \theta_0}\log(2/\alpha)}{n} + \Gamma_n(\widehat\theta, \theta_0)\right)\\
%     &\qquad \le \mathbb{P}\left(3^{-1}\|\theta-\theta_0\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0})\right)\\
%     &\qquad\qquad + \mathbb{P}\left(3^{-1}\|\theta-\theta_0\|^{1+\beta}\le \sqrt{\frac{2n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta_0})^2 \log(2/\alpha)}{n-1}} \right)\\
%     &\qquad \qquad +\mathbb{P}\left(3^{-1}\|\theta-\theta_0\|^{1+\beta}\le\sqrt{\frac{2 P_0(m_{\theta}-m_{\theta_0})^2 \log(2/\alpha)}{n-1}}+\frac{6B_{\theta,  \theta_0}\log(2/\alpha)}{n}+ \Gamma_n(\widehat\theta, \theta_0)\right)
% \end{align*}

% First, we reduce the analysis into 
% \begin{align*}
%     &\mathbb{P}\left(\|\theta-\theta_0\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0})+   \sqrt{\frac{2\widehat \sigma^2_{\theta, \theta_0} \log(2/\alpha)}{n}} + \frac{6B_{\theta,  \theta_0}\log(2/\alpha)}{n} + \Gamma_n(\widehat\theta, \theta_0)\right)\\
%     &\qquad \le \mathbb{P}\left(4^{-1}\|\theta-\theta_0\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0})\right)+ \mathbb{P}\left(4^{-1}\|\theta-\theta_0\|^{1+\beta}\le \sqrt{\frac{2\widehat \sigma^2_{\theta, \theta_0} \log(2/\alpha)}{n}} \right)\\
%     &\qquad \qquad +\mathbb{P}\left(4^{-1}\|\theta-\theta_0\|^{1+\beta}\le\frac{6B_{\theta,  \theta_0}\log(2/\alpha)}{n}\right)+ \mathbb{P}\left(4^{-1}\|\theta-\theta_0\|^{1+\beta}\le \Gamma_n(\widehat\theta, \theta_0)\right)
% \end{align*}
For the first term, we first observe that 
\begin{align}
    &\mathbb{P}\left(3^{-1}\|\theta-\theta_0\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0}) \mbox{ for } \|\theta-\theta_0\| \ge \gamma_M \right) \\
     &\qquad\le \mathbb{P}\left(3^{-1}\|\theta-\theta_0\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0}) \mbox{ for } \|\theta-\theta_0\| \ge 2^{M/(1+\beta)}r_n^{2/(1+\beta)} \right).
\end{align}
We define the ``shell": 
\[S_j = \{\theta \in \Theta : 2^{j}r_n^{2/(1+\beta)} \le \|\theta-\theta_0\| < 2^{j+1}r_n^{2/(1+\beta)}\}\]
for each $j  \in \{0\} \cup \mathbb{N}$. Then, it follows that 
\begin{align}
	&\mathbb{P}(3^{-1}\|\theta-\theta_0\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0}) \, \textrm{ for some $\theta$, i.e.,}\, \|\theta_0 - \theta\| \ge 2^M r_n^{2/(1+\beta)}) \\
 &\qquad \le \mathbb{P}(\exists\, (j \ge M, \theta \in S_j) : 3^{-1}\|\theta-\theta_0\|^{1+\beta}\le |n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0})|) \\
 &\qquad \le \sum_{j=M}^\infty \mathbb{P}(\exists \, \theta \in S_j : 3^{-1}\|\theta-\theta_0\|^{1+\beta}\le |n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0})|)\\
 &\qquad \le \sum_{j=M}^\infty \mathbb{P}\left(3^{-1}2^{j(1+\beta)}r_n^{2}\le \sup_{\theta \in S_j}|n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0})|\right)\\
 &\qquad \le 3\sum_{j=M}^\infty 2^{-j(1+\beta)}r_n^{-2}n^{-1/2}\mathbb{E}\left[ \sup_{\theta \in S_j}|\mathbb{G}_n(m_\theta-m_{\theta_0})|\right]\\
 &\qquad \le 3\sum_{j=M}^\infty n^{-1/2}2^{-j(1+\beta)}r_n^{-2}\phi_n(2^{j+1}r_n^{2/(1+\beta)})\\
 &\qquad \le 3\sum_{j=M}^\infty n^{-1/2}2^{-j(1+\beta)}r_n^{-2}2^{q(j+1)}\phi_n(r_n^{2/(1+\beta)})\\
 &\qquad \le 3\sum_{j=M}^\infty 2^{-j(1+\beta)}2^{q(j+1)}\\
 &\qquad = 3\cdot 2^{\beta+1}\sum_{j=M}^\infty 2^{-(j+1)(1+\beta-q)}.\label{eq:term2}
\end{align}
By assumption \ref{as:local-entropy} that $q < 1+\beta$, the last display is less than $\varepsilon/3$ for $M$ large enough. 

Finally, for the second term, we have 
\begin{align}
    &\mathbb{P}\left(3^{-1}\|\theta-\theta_0\|^{1+\beta}\le \sqrt{\frac{2\log(2/\alpha)n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta_0})^2}{n-1}}\mbox{ for } \|\theta-\theta_0\| \ge \gamma_M \right) \\
     &\qquad\le \mathbb{P}\left(3^{-1}\|\theta-\theta_0\|^{1+\beta}\le \sqrt{\frac{2\log(2/\alpha)n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta_0})^2}{n-1}}\right.\\
     &\qquad\qquad\qquad\qquad\qquad\left. \mbox{ for } \|\theta-\theta_0\| \ge 2^{M/(1+\beta)}r_n^{1/(1+\beta)}n^{-1/(2+2\beta)} B_{\theta,  \theta_0}^{1/(2+2\beta)} \right).
\end{align}
We now define the ``shell": 
\[S'_j = \{\theta \in \Theta : 2^{j}r_n^{1/(1+\beta)}n^{-1/(2+2\beta)} B_{\theta,  \theta_0}^{1/(2+2\beta)} \le \|\theta-\theta_0\| < 2^{j+1}r_n^{1/(1+\beta)}n^{-1/(2+2\beta)} B_{\theta,  \theta_0}^{1/(2+2\beta)}\}\]
for each $j  \in \{0\} \cup \mathbb{N}$. Then, it follows that 
\begin{align}
	&\mathbb{P}\left(3^{-1}\|\theta-\theta_0\|^{1+\beta}\le \sqrt{\frac{2\log(2/\alpha)n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta_0})^2}{n-1}}\right.\\
     &\qquad\qquad\qquad\qquad\qquad\left. \mbox{ for } \|\theta-\theta_0\| \ge 2^{M/(1+\beta)}r_n^{1/(1+\beta)}n^{-1/(2+2\beta)} B_{\theta,  \theta_0}^{1/(2+2\beta)} \right)\\
 &\qquad \le \mathbb{P}\left(\exists\, (j \ge M, \theta \in S'_j) : 3^{-1}\|\theta-\theta_0\|^{1+\beta}\le \sqrt{\frac{2\log(2/\alpha)n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta_0})^2}{n-1}}\right) \\
 &\qquad = \mathbb{P}\left(\exists\, (j \ge M, \theta \in S'_j) : 3^{-2}(2\log(2/\alpha))^{-1}\|\theta-\theta_0\|^{2+2\beta}\le \left|\frac{n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta_0})^2}{n-1}\right|\right)\\
 % &\qquad \le \sum_{j=M}^\infty \mathbb{P}(\exists \, \theta \in S_j : 3^{-1}\|\theta-\theta_0\|^{1+\beta}\le |n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0})|)\\
 &\qquad \le \sum_{j=M}^\infty \mathbb{P}\left(3^{-2}(2\log (2/\alpha))^{-1}2^{j(1+\beta)}r_n^{2}n^{-1} B_{\theta,  \theta_0}\le \sup_{\theta \in S_j}\left|\frac{n^{-1/2}\mathbb{G}_n(m_{ \theta}-m_{\theta_0})^2}{n-1}\right|\right)\\
 &\qquad \le 3^2 \cdot 2\log (2/\alpha)\sum_{j=M}^\infty 2^{-j(1+\beta)}r_n^{-2}\left(\frac{n}{n-1}\right)B_{\theta,  \theta_0}^{-1}n^{-1/2}\mathbb{E}\left[ \sup_{\theta \in S_j}|\mathbb{G}_n(m_{ \theta}-m_{\theta_0})^2|\right].
\end{align}
Now, we observe that
\begin{align*}
    \mathbb{E}\left[ \sup_{\theta \in S_j}|\mathbb{G}_n(m_{ \theta}-m_{\theta_0})^2|\right] = B_{\theta, \theta_0}^2\mathbb{E}\left[ \sup_{\theta \in S_j}\left|\mathbb{G}_n\left(\frac{m_{ \theta}-m_{\theta_0}}{B_{\theta, \theta_0}}\right)^2\right|\right]
\end{align*}
and the mapping $t\mapsto t^2$ is $2$-Lipschitz on $t \in [-1,1]$. Hence, by the contraction inequality, for instance, Theorem 4.12 of \cite{ledoux2013probability} or Corollary 3.2.2 of \cite{gine2021mathematical}, we obtain 
\begin{align*}
    B_{\theta, \theta_0}^2\mathbb{E}\left[ \sup_{\theta \in S_j}\left|\mathbb{G}_n\left(\frac{m_{ \theta}-m_{\theta_0}}{B_{\theta, \theta_0}}\right)^2\right|\right] \le 2 B_{\theta, \theta_0}\mathbb{E}\left[ \sup_{\theta \in S_j}\left|\mathbb{G}_n (m_{ \theta}-m_{\theta_0})\right|\right].
\end{align*}
To complete the argument, we have
\begin{align}
    &3^2 \cdot 2\log (2/\alpha)\sum_{j=M}^\infty 2^{-j(1+\beta)}r_n^{-2}\left(\frac{n}{n-1}\right)B_{\theta,  \theta_0}^{-1}n^{-1/2}\mathbb{E}\left[ \sup_{\theta \in S_j}|\mathbb{G}_n(m_{ \theta}-m_{\theta_0})^2|\right]\\
    &\qquad \le 3^2 \cdot 2^3\log (2/\alpha)\sum_{j=M}^\infty 2^{-j(1+\beta)}r_n^{-2}n^{-1/2}\mathbb{E}\left[ \sup_{\theta \in S_j}|\mathbb{G}_n(m_{ \theta}-m_{\theta_0})|\right]\label{eq:term3}
\end{align}
where the last summation can be arbitrarily small for $M$ large by the same argument from earlier. 
% By assumption \ref{as:local-entropy} that $q < 1+\beta$, the last display is less than $\varepsilon/3$ for $M$ large enough. 
% Under the case (2), we claim that with probability at least $1-\varepsilon$,
% \[n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0}) \le C_\varepsilon r_n^{2} \]
% with a constant $C_\varepsilon$ only depending on $\varepsilon > 0$. Similarly to the above derivation, we have 
% \begin{align}
%     &\mathbb{P}(2^{K+Mq} r_n^2 < -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0}) \, \textrm{ for some $\theta$, i.e.,}\, \|\theta_0 - \theta\| < 2^M r_n^{2/(1+\beta)})\\
%     &\qquad \le \mathbb{P}\left(2^{K+Mq} r_n^2 < \sup_{\|\theta_0 - \theta\| < 2^M r_n^{2/(1+\beta)}}\, |n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0})|\right)\\
%     &\qquad \le 2^{-K-Mq}r_n^{-2}n^{-1/2}\phi_n(2^{M}r_n^{2/(1+\beta)})\\
%     &\qquad \le 2^{-K}.\label{eq:term2}
% \end{align}

Finally, let $M$ be a large constant only depending on $\varepsilon$ such that \eqref{eq:term1},\eqref{eq:term2} and \eqref{eq:term3}  become less than $\varepsilon/3$. Then with probability at least $1-\varepsilon$, it holds that 
\begin{align*}
    &\left\{\theta \in \Theta : \|\theta-\theta_0\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0}) +   \sqrt{\frac{2\widehat \sigma^2_{\theta, \theta_0} \log(2/\alpha)}{n}} + \frac{6B_{\theta,  \theta_0}\log(2/\alpha)}{n} + \Gamma_n(\widehat\theta, \theta_0)\right\} \\
    & \qquad \subseteq \left\{\theta \in \Theta : \|\theta-\theta_0\|^{1+\beta}\right.\\
    &\left.\qquad\qquad\qquad\le C_{\alpha,\varepsilon} \left(r_n^{2} +  r_n n^{-1/2} B_{\theta,  \theta_0}^{1/2}+ n^{-1/2}\{P_0 (m_{ \theta}-m_{\theta_0})^2\}^{1/2}+n^{-1} B_{\theta,  \theta_0}+\Gamma_n(\widehat\theta, \theta_0)\right)\right\}.
\end{align*}

\subsection{Proof of Proposition~\ref{prop:clt-valid}}
This result is identical to equation (1.5) of \citet{bentkus1996berry}. We provide the proof for completeness. We first introduce several notations. For each $\theta \in \Theta$, define 
\begin{align}
	W_i &:= m_{\theta}(Z_i) - m_{\theta_0}(Z_i) - P_0(m_{\theta}-m_{\theta_0}), \\
	S_n^2 &:= \sum_{i=1}^n \textrm{Var}(W_i), \quad	Y_i := S_n^{-1} W_i 1\{W_i^2\le S_n^2\}, \quad 	M^2 := \sum_{i=1}^n \textrm{Var}(Y_i),  \\
	\Pi &:= \sum_{i=1}^n \mathbb{P}(W_i^2 > S_n^2),\quad  \Upsilon := M^{-1}\sum_{i=1}^n|\E Y_i|, \mbox{ and }\  \Lambda := M^{-3}\sum_{i=1}^n\E |Y_i|^3.
\end{align}
Then Corollary 1.1 of \citet{bentkus1996berry} states that there exists a universal constant $C$ such that  
\[\Delta_n \le C(\Pi+ \Upsilon + \Lambda).\]
Furthermore, we observe that 
\begin{align}
	\Pi &= \sum_{i=1}^n \mathbb{P}(W_i^2 > S_n^2) = \sum_{i=1}^n \mathbb{P}(W_i^2 1\{W_i^2 > S_n^2\} > S_n^2) \le \sum_{i=1}^n \E[W_i^2 1\{W_i^2 > S_n^2\}] S_n^{-2} 
\end{align}
by the Markov inequality. Similarly, we also have 
\begin{align}
	|\E Y_i| &= |\E [S_n^{-1} W_i 1\{W_i^2\le S_n^2\}]| \\
 &= |\E  S_n^{-1} W_i - \E S_n^{-1} W_i  1\{W_i^2 > S_n^2\}| \\
 &= S_n^{-1} |\E W_i  1\{W_i^2 > S_n^2\}| \\
	&\le S_n^{-1} (\E |W_i|^2  1\{W_i^2 > S_n^2\})^{1/2} \mathbb{P}^{1/2}(W_i^2 1\{W_i^2 > S_n^2\}> S_n^2) \\
 &= \E[W_i^2 1\{W_i^2 > S_n^2\}] S_n^{-2} 
	\end{align}
where the inequality follows by Cauchy-Schwarz inequality. It also follows that
\begin{align}
	\E |Y_i|^3 &= \E | S_n^{-1} W_i 1\{W_i^2\le S_n^2\} |^3 = S_n^{-3} \E | W_i|^3 1\{W_i^2\le S_n^2\}.
\end{align}

Finally, we have
\begin{align}
		\textrm{Var}(Y_i) &= \E Y_i^2 - (\E Y_i)^2 \\
  &= S_n^{-2} \E W_i^2 1\{W_i^2\le S_n^2\} - S_n^{-2} (\E W_i 1\{W_i^2\le S_n^2\})^2 \\
		&= S_n^{-2} \E W_i^2 - S_n^{-2} \E W_i^2 1\{W_i^2> S_n^2\} - S_n^{-2} (\E W_i 1\{W_i^2\le S_n^2\})^2\\
		&\ge S_n^{-2} \E W_i^2 - 2 S_n^{-2} \E W_i^2 1\{W_i^2> S_n^2\},
\end{align}
and hence 
\begin{align}
	M = \sum_{i=1}^n S_n^{-2} \E W_i^2 - 2 S_n^{-2} \E W_i^2 1\{W_i^2> S_n^2\} = 1 - 2 S_n^{-2} \sum_{i=1}^n\E W_i^2 1\{W_i^2> S_n^2\}.
\end{align}

It is without loss of generality to assume that $S_n^{-2} \sum_{i=1}^n\E W_i^2 1\{W_i^2> S_n^2\}  \le 1/4$ since otherwise the below hold with $C > 4$ trivially. We thus have 
\begin{align}
	\Delta_n &\le C(\Pi+ \Upsilon + \Lambda)\\
 &\le C\left ( \sum_{i=1}^n \E[W_i^2 1\{W_i^2 > S_n^2\}] S_n^{-2} +  \sum_{i=1}^n \E[|W_i|^3 1\{W_i^2 \le  S_n^2\}] S_n^{-3} \right)\\
 &= C\left ( \E[W_1^2 1\{W_1^2 > nS^2\}] S^{-2} +  n^{-1/2}\E[|W_1|^3 1\{W_1^2 \le  nS^2\}] S^{-3} \right)
%	\\
%	&= C\left ( \sum_{i=1}^n \E[W_i^2 1\{W_i^2 > S_n^2\}] S_n^{-2} +  \sum_{i=1}^n \E[|W_i|^3 1\{W_i^2 \le  \varepsilon^2 S_n^2\}] S_n^{-3} + \sum_{i=1}^n \E[|W_i|^3 1\{\varepsilon^2 S_n^2 < W_i^2 \le  S_n^2\}] S_n^{-3}\right)\\
%	&\le C\left ( \sum_{i=1}^n \E[W_i^2 1\{W_i^2 > S_n^2\}] S_n^{-2} +  \varepsilon + \sum_{i=1}^n \E[|W_i|^2 S_n 1\{\varepsilon^2 S_n^2 < W_i^2 \le  S_n^2\}] S_n^{-3}\right)\\
%	&\le C\left ( \varepsilon + \sum_{i=1}^n \E[|W_i|^2 1\{W_i^2 > \varepsilon^2 S_n^2 \}] S_n^{-2}\right)
\end{align}
where the last step follows since $W_1, \ldots, W_n$ is an IID observation. 
\subsection{Proof of Theorem~\ref{thm:validity-BE}}
From the equation \eqref{eq:delta_n-coverage} and Theorem~\ref{thm:validity}, it is immediate that
\begin{align*}
	&\mathbb{P}_0(\theta_0 \in \widehat{C}^{\textrm{Gauss.}}_n \mid D_1)\\
	 &\qquad\ge 1-\alpha_1-\alpha_2-\Delta_n\\
	&\qquad \ge 1-\alpha_1-\alpha_2-C\left ( \E[W_1^2 1\{W_1^2 > nS^2\}] S^{-2} +  n^{-1/2}\E[|W_1|^3 1\{W_1^2 \le  nS^2\}] S^{-3} \right)
\end{align*}
where the second inequality follows from Proposition~\ref{prop:clt-valid}. We now provide the upper bounds on two terms in the parenthesis. 

First, by adding and subtracting terms, we obtain 
\begin{align}
	&\E[W_1^2/S^2 1\{W_1^2/S^2 > n\}] \\
	&\qquad = \E[W_1^2/S^2 1\{W_1^2/S^2 > n\}]- \E[\langle t, \dot m_{\theta_0}\rangle^2 1\{\langle t, \dot m_{\theta_0}\rangle^2 > nP_0\langle t, \dot m_{\theta_0}\rangle^2\}] (P_0\langle t, \dot m_{\theta_0}\rangle)^{-1}\label{eq:term2-approx}\\
	&\qquad\qquad +  \E[\langle t, \dot m_{\theta_0}\rangle^2 1\{\langle t, \dot m_{\theta_0}\rangle^2 > nP_0\langle t, \dot m_{\theta_0}\rangle^2\}] (P_0\langle t, \dot m_{\theta_0}\rangle)^{-1}
	\end{align}
We invoke Lemma~\ref{lemma:moment-bounds} to control \eqref{eq:term2-approx}. \ref{as:qmd+lindeberg} implies that for any $\varepsilon > 0$, there exists $C_\varepsilon$ such that 
\begin{align}
	\E[|W_1 - \langle \widehat \theta-\theta_0, \dot m_{\theta_0}\rangle|^2] \le \varepsilon \| \widehat \theta-\theta_0\|^2  \E \langle t, \dot m_{\theta_0}\rangle^2
\end{align}
holds for all $\widehat \theta$ such that $\|\widehat \theta-\theta_0\| < C_\varepsilon$. We also observe that
\begin{align}
	\E \langle \widehat \theta-\theta_0, \dot m_{\theta_0}\rangle^2 = \|\widehat \theta-\theta_0\|^2 \E \langle t, \dot m_{\theta_0}\rangle^2.
\end{align}
Hence, the second result of Lemma~\ref{lemma:moment-bounds} implies that 
\begin{align}
	\E[W_1^2/S^2 1\{W_1^2/S^2 > n\}]- \E[\langle t, \dot m_{\theta_0}\rangle^2 1\{\langle t, \dot m_{\theta_0}\rangle^2 > nP_0\langle t, \dot m_{\theta_0}\rangle^2\}] (P_0\langle t, \dot m_{\theta_0}\rangle)^{-1} \leq 16 (\varepsilon + \varepsilon^{1 / 2})
\end{align}
assuming $\|\widehat \theta-\theta_0\| < C_\varepsilon$. Similarly, we have 
\begin{align}
	&n^{-1/2}\E[|W_1|^3 1\{W_1^2 \le  nS^2\}] S^{-3} \\
	&\qquad = n^{-1/2}\E[|W_1|^3 1\{W_1^2 \le  nS^2\}] S^{-3}\\
	&\qquad \qquad - n^{-1/2}\E[\langle t, \dot m_{\theta_0}\rangle^3 1\{\langle t, \dot m_{\theta_0}\rangle^2 > nP_0\langle t, \dot m_{\theta_0}\rangle^2\}] (P_0\langle t, \dot m_{\theta_0}\rangle)^{-3/2}\\
	&\qquad\qquad +  n^{-1/2}\E[\langle t, \dot m_{\theta_0}\rangle^3 1\{\langle t, \dot m_{\theta_0}\rangle^2 > nP_0\langle t, \dot m_{\theta_0}\rangle^2\}] (P_0\langle t, \dot m_{\theta_0}\rangle)^{-3/2}
	\end{align}
where the first two terms can be controlled by the third result of Lemma~\ref{lemma:moment-bounds}, which implies that 
\begin{align}
	&n^{-1/2}\E[|W_1|^3 1\{W_1^2 \le  nS^2\}] S^{-3}\\
	& \qquad - n^{-1/2}\E[\langle t, \dot m_{\theta_0}\rangle^3 1\{\langle t, \dot m_{\theta_0}\rangle^2 > nP_0\langle t, \dot m_{\theta_0}\rangle^2\}] (P_0\langle t, \dot m_{\theta_0}\rangle)^{-3/2} \le  16 (\varepsilon + \varepsilon^{1 / 2})
\end{align}
assuming $\|\widehat \theta-\theta_0\| < C_\varepsilon$. Putting together, we have
\begin{align}
	&\E[W_1^2 1\{W_1^2 > nS^2\}] S^{-2} +  n^{-1/2}\E[|W_1|^3 1\{W_1^2 \le  nS^2\}] S^{-3} \\
	&\qquad \le 32(\varepsilon + \varepsilon^{1 / 2}) + \E[\langle t, \dot m_{\theta_0}\rangle^2 1\{\langle t, \dot m_{\theta_0}\rangle^2 > nP_0\langle t, \dot m_{\theta_0}\rangle^2\}] (P_0\langle t, \dot m_{\theta_0}\rangle)^{-1}\\
	&\qquad\qquad + n^{-1/2}\E[\langle t, \dot m_{\theta_0}\rangle^3 1\{\langle t, \dot m_{\theta_0}\rangle^2 > nP_0\langle t, \dot m_{\theta_0}\rangle^2\}] (P_0\langle t, \dot m_{\theta_0}\rangle)^{-3/2}
\end{align}
when $\|\widehat \theta-\theta_0\| < C_\varepsilon$. In the case when $\|\widehat \theta-\theta_0\| \ge C_\varepsilon$, we use the trivial bound of $\Delta_n \le 2$ and thus 
\begin{align}
	\E[\Delta_n] &= \E[\Delta_n 1\{{\|\widehat \theta-\theta_0\| < C_\varepsilon}\}] + \E[\Delta_n 1\{{\|\widehat \theta-\theta_0\| \ge C_\varepsilon}\}] \\
	&\le 32(\varepsilon + \varepsilon^{1 / 2}) + \E[\langle t, \dot m_{\theta_0}\rangle^2 1\{\langle t, \dot m_{\theta_0}\rangle^2 > nP_0\langle t, \dot m_{\theta_0}\rangle^2\}] (P_0\langle t, \dot m_{\theta_0}\rangle)^{-1}\\
	&\qquad + n^{-1/2}\E[\langle t, \dot m_{\theta_0}\rangle^3 1\{\langle t, \dot m_{\theta_0}\rangle^2 > nP_0\langle t, \dot m_{\theta_0}\rangle^2\}] (P_0\langle t, \dot m_{\theta_0}\rangle)^{-3/2}\\
	&\qquad + 2 \mathbb{P}(\|\widehat \theta-\theta_0\| < C_\varepsilon).
\end{align}
Due to the first term $32(\varepsilon + \varepsilon^{1 / 2})$, the statement holds trivial for any $\varepsilon$ such that $\varepsilon > 1/16$. We thus focus on the case when $\varepsilon < 1/16$. 

For the ease of notation, we denote by 
\[\dot m_t = \langle t, \dot m_{\theta_0}\rangle \quad \mbox{and} \quad  \dot M_t = P_0 \langle t, \dot m_{\theta_0}\rangle^2.\]
For $\varepsilon< 1/16$, we observe that  
\begin{align*}
	&\E[\langle t, \dot m_{\theta_0}\rangle^2 1\{\langle t, \dot m_{\theta_0}\rangle^2 > nP_0\langle t, \dot m_{\theta_0}\rangle^2\}] (P_0\langle t, \dot m_{\theta_0}\rangle^2)^{-1}\\
	&\qquad + n^{-1/2}\E[\langle t, \dot m_{\theta_0}\rangle^3 1\{\langle t, \dot m_{\theta_0}\rangle^2 > nP_0\langle t, \dot m_{\theta_0}\rangle^2\}] (P_0\langle t, \dot m_{\theta_0}\rangle^2)^{-3/2}\\
	&\qquad = \E[\dot m_t^2 1\{\dot m_t^2 > n\dot M_t\}] \dot M_t^{-1} +  n^{-1/2}\E[|\dot m_t|^3 1\{\dot m_t^2 \le  n\varepsilon^2\dot M_t\}] \dot M_t^{-3/2}\\
	&\qquad\qquad+n^{-3/2}\E[|\dot m_t|^3 1\{n\varepsilon^2 \dot M_t \le \dot m_t^2 \le  n\dot M_t\}] \dot M_t^{-3/2}\\
	&\qquad \le  \E[\dot m_t^2 1\{\dot m_t^2 > n\dot M_t\}] \dot M_t^{-1} +  \varepsilon  +n^{-1/2}\E[|\dot m_t|^3 1\{n\varepsilon^2 \dot M_t \le \dot m_t^2 \le  n\dot M_t\}] \dot M_t^{-3/2}\\
	&\qquad \le  \E[\dot m_t^2 1\{\dot m_t^2 > n\dot M_t\}] \dot M_t^{-1} +  \varepsilon  +n^{-1/2}\E[|\dot m_t|^2 n^{1/2}S 1\{n\varepsilon^2 \dot M_t \le \dot m_t^2 \le  n\dot M_t\}] \dot M_t^{-3/2}\\
	&\qquad \le  \E[\dot m_t^2 1\{\dot m_t^2 > n\dot M_t\}] \dot M_t^{-1} +  \varepsilon  +\E[\dot m_t^2 1\{ \dot m_t^2 \ge  n\varepsilon^2 \dot M_t \}] \dot M_t^{-1}\\
	&\qquad \le  C\left(\varepsilon  +\E[\dot m_t^2 1\{ \dot m_t^2 \ge  n\varepsilon^2 \dot M_t \}] \dot M_t^{-1}\right).
\end{align*}
Hence under \ref{as:cond1}, we obtain 
\begin{align}
	\E[\Delta_n] \le \varepsilon + \mathbb{P}(\|\widehat \theta-\theta_0\| < C_\varepsilon). 
\end{align}
Alternatively, it follows that 
\begin{align}
	&\E[\dot m_t^2 1\{\dot m_t^2 > n\dot M_t\}] \dot M_t^{-1} +  n^{-1/2}\E[|\dot m_t|^3 1\{\dot m_t^2 \le  n\dot M_t\}] \dot M_t^{-3/2}\\
	&\qquad = \E[\dot m_t^2 1\{\dot m_t^{\delta} > n^{\delta/2}\dot M_t^{\delta/2}\}] \dot M_t^{-1} +  n^{-1/2}\E[|\dot m_t|^3 1\{\dot m_t^{1-\delta} \le  n^{(1-\delta)/2}\dot M_t^{(1-\delta)/2}\}] \dot M_t^{-3/2}\\
	&\qquad \le  2n^{-\delta/2}\E[\dot m_t^{2+\delta}] \dot M_t^{-(1+\delta/2)} \\
	&\qquad =  2n^{-\delta/2}\left(\frac{\E[\dot m_t^{2+\delta}]^{1/(2+\delta)}}{\E[\dot m_t^2]^{1/2}}\right)^{2+\delta}.
\end{align}
Hence under \ref{as:cond2}, we obtain 
\begin{align}
	\E[\Delta_n] \le \varepsilon + n^{-\delta/2}L^{2+\delta} + \mathbb{P}(\|\widehat \theta-\theta_0\| < C_\varepsilon). 
\end{align}
%It is without loss of generality to assume that $B_n^{-2} \sum_{i=1}^n\E X_i^2 1\{X_i^2> B_n^2\}  \le 1/4$ since otherwise the below hold with $C > 4$ trivially. We thus have 
%\begin{align}
%	\delta_n &\le C\left (  \right) \\
%	&= C\left ( \sum_{i=1}^n \E[X_i^2 1\{X_i^2 > B_n^2\}] B_n^{-2} +  \sum_{i=1}^n \E[|X_i|^3 1\{X_i^2 \le  \varepsilon^2 B_n^2\}] B_n^{-3} + \sum_{i=1}^n \E[|X_i|^3 1\{\varepsilon^2 B_n^2 < X_i^2 \le  B_n^2\}] B_n^{-3}\right)\\
%	&\le C\left ( \sum_{i=1}^n \E[X_i^2 1\{X_i^2 > B_n^2\}] B_n^{-2} +  \varepsilon + \sum_{i=1}^n \E[|X_i|^2 B_n 1\{\varepsilon^2 B_n^2 < X_i^2 \le  B_n^2\}] B_n^{-3}\right)\\
%	&\le C\left ( \varepsilon + \sum_{i=1}^n \E[|X_i|^2 1\{X_i^2 > \varepsilon^2 B_n^2 \}] B_n^{-2}\right)
%\end{align}
%
%An easier sufficient condition to deal with is 
%\begin{align}
%	\sum_{i=1}^n \E[X_i^2 1\{X_i^2 > B_n^2\}] B_n^{-2} \le \sum_{i=1}^n \E \left[X_i^2 \frac{|X_i|^{\delta}}{B_n^{\delta}}\right] B_n^{-2} = \sum_{i=1}^n \E|X_i|^{2+\delta} B_n^{-(2+\delta)}
%\end{align}
%and 
%\begin{align}
%	\sum_{i=1}^n \E[|X_i|^3 1\{X_i^2 \le  B_n^2\}] B_n^{-3} \le \sum_{i=1}^n \E|X_i|^{2+\delta} B_n^{-(2+\delta)}
%\end{align}
%Thus we have 
%\begin{align}
%	\delta_n \le C\sum_{i=1}^n \E|X_i|^{2+\delta} B_n^{-(2+\delta)}
%\end{align}
%We thus have two options. To get a Berry-Esseeen,
%%\begin{itemize}
%%	\item For some $\delta \in (0,1]$, we have $\E_{P_i}|X_i|^{2+\delta} < \infty$ for all distributions $\{P_i\}_{i=1}^n$.
%%\end{itemize}
%To get asymptotic control only, we need 
%\[\frac{\sum_{i=1}^n \E_i |X_i|^{2+\delta}}{(\sum_{i=1}^n \E_i |X_i|^{2})^{(2+\delta)/2}} = \left(\frac{(\sum_{i=1}^n \E_i |X_i|^{2+\delta})^{1/(2+\delta)}}{(\sum_{i=1}^n \E_i |X_i|^{2})^{1/2}}\right)^{2+\delta} \longrightarrow 0\]
%We note that under IID we have
%\[n^{-\delta/2}\left(\frac{(\E |Y|^{2+\delta})^{1/(2+\delta)}}{(\E |Y|^{2})^{1/2}}\right)^{2+\delta} \longrightarrow 0\]
%Hence, we need $L_{2+\delta}$-$L_2$ norm equivalence. 


\begin{lemma}\label{lemma:moment-bounds}
    Suppose that $X$ and $Y$ are the random variables defined on a common measurable space, satisfying $\E|X-Y|^2 \le C \E[X^2]$ with some constant $C>0$.
    Then we have the following upper bounds:
    \begin{align*}
        \mathbb{E}\left[\left|\frac{X^2}{\mathbb{E}[X^2]}-\frac{Y^2}{\mathbb{E}[Y^2]}\right|\right] \leq 4 (C+ C^{1 / 2}), 
    \end{align*}
    \begin{align*}
        \mathbb{E} & {\left[\frac{X^2}{\mathbb{E}[X^2]} 1\{X^2>t\mathbb{E}[X^2]\}\right]-\mathbb{E}\left[\frac{Y^2}{\mathbb{E}[Y^2]}  1\{Y^2>t\mathbb{E}[Y^2]\}\right] } \leq  16(C+ C^{1 / 2}), \quad \mbox{and}
    \end{align*}
    \begin{align*}
        \mathbb{E} & {\left[\left(\frac{X^2}{\mathbb{E}[X^2]}\right)^{3/2} 1\{X^2\le s\mathbb{E}[X^2]\}\right]-\mathbb{E}\left[\left(\frac{Y^2}{\mathbb{E}[Y^2]}\right)^{3/2}  1\{Y^2\le s\mathbb{E}[Y^2]\}\right] } \leq  16 s^{1/2} (C+ C^{1 / 2}).
    \end{align*}
\end{lemma}
\begin{proof}[\bfseries{Proof of Lemma~\ref{lemma:moment-bounds}}]
    Suppose $X$ and $Y$ are random variables such that $\E|X-Y|^2 \le C \E[X^2]$.
To obtain the first result, we observe that 
\begin{align*}
\mathbb{E}\left[\left|\frac{X^2}{\mathbb{E}[X^2]}-\frac{Y^2}{\mathbb{E}[Y^2]}\right|\right] 
&=\mathbb{E}\left[\left|\frac{X^2 \mathbb{E}[Y^2]-\mathbb{E}[X^2] Y^2}{\mathbb{E}[X^2] \mathbb{E}[Y^2]}\right|\right] \\
&=\mathbb{E}\left[\left|\frac{(X^2-Y^2) \mathbb{E}[Y^2]}{\mathbb{E}[X^2] \mathbb{E}[Y^2]}\right|\right]+\mathbb{E}\left[\left|\frac{Y^2(\mathbb{E}[Y^2]-\mathbb{E}[X^2])}{\mathbb{E}[X^2] \mathbb{E}[Y^2]}\right|\right] \\
& =\frac{\mathbb{E}[|X^2-Y^2|]}{\mathbb{E}[X^2]}+\frac{|\mathbb{E}[Y^2-X^2]|}{\mathbb{E}[X^2]} \\
&\leq 2 \frac{\mathbb{E}[|Y^2-X^2|]}{\mathbb{E}[X^2]} 
\end{align*}
by Jensen's inequality. Since $Y^2=(Y-X)^2+2 X(Y-X)+X^2$, we obtain
\begin{align*}
	\mathbb{E}[| Y^2-X^2|] &= \mathbb{E}[|Y-X|^2] +2\E[ X(Y-X)]\\
	&\leq  \mathbb{E}[|Y-X|^2]+2\left(\mathbb{E}[X^2]\right)^{1/2}\left(\mathbb{E}[|Y-X|^2]\right)^{1 / 2}\\
%	&\le  C \E[X^2]+2\left(\mathbb{E}[X^2]\right)^{1/2}\left(C \E[X^2]\right)^{1 / 2}\\
	&\le  C \E[X^2]+2C^{1/2}\mathbb{E}[X^2]
	\end{align*}
by Cauchy-Schwarz inequality. Hence we conclude 
\begin{align*}
	\mathbb{E}\left[\left|\frac{X^2}{\mathbb{E}[X^2]}-\frac{Y^2}{\mathbb{E}[Y^2]}\right|\right] 
\leq 2 \frac{\mathbb{E}[|Y^2-X^2|]}{\mathbb{E}[X^2]} \le 2C +4C^{1/2}.
\end{align*}
%$$
%\mathbb{E}[| Y^2-X^2|] \leq \mathbb{E}[|X-Y|^2]+2\left(\mathbb{E}[X^2]\right)^{1 / 2}\left(\mathbb{E}\left[\left|Y-X\right|^2\right]\right)^{1 / 2} \text {. }
%$$
%
%Therefore,
%$$
%\mathbb{E}\left[\left|\frac{X^2}{\mathbb{E}[X^2]}-\frac{Y^2}{\mathbb{E}[Y^2]}\right|\right] \leq 2 C+2 C^{1 / 2} .
%$$
%To deal with 
%\begin{align}
%	\mathbb{E}\left[\left|X-Y\right|^2\right] \leq 2 C \mathbb{E}\left[\left|Y\right|^2\right]+2 C \mathbb{E}\left[\left|X-Y\right|^2\right]
%\end{align}
%$$
%\mathbb{E}\left[\left|X-Y\right|^2\right] \leq 2 C \mathbb{E}\left[\left|Y\right|^2\right]+2 C \mathbb{E}\left[\left|X-Y\right|^2\right] \text {. }
%$$
%
%Hence, if $C<1 / 2$, then
%$$
%\mathbb{E}\left[\left|X-Y\right|^2\right] \leq \frac{2 C}{1-2 C} \mathbb{E}\left[\left|Y\right|^2\right] .
%$$
%
%We first provide the $\mathbb{E}\left[\left(X^2 / \mathbb{E}[X^2]\right) 1\left\{X^2 / \mathbb{E}[X^2]>t\right\}\right]$ in terms of $\mathbb{E}\left[\left(Y^2 / \mathbb{E}[Y^2]\right) 1\left\{Y^2 / \mathbb{E}[Y^2]>t\right\}\right]$. First, note that
%$$
%\begin{aligned}
%& \mathbb{E}\left[\left|\frac{X^2}{\mathbb{E}[X^2]}-\frac{Y^2}{\mathbb{E}[Y^2]}\right|\right] \\
%& =\mathbb{E}\left[\left|\frac{X^2 \mathbb{E}[Y^2]-\mathbb{E}[X^2] Y^2}{\mathbb{E}[X^2] \mathbb{E}[Y^2]}\right|\right] \\
%& =\mathbb{E}\left[\left\lfloor\frac{\left(X^2-Y^2\right) \mathbb{E}[Y^2]}{\mathbb{E}[X^2] \mathbb{E}[Y^2]}\right\rceil\right]+\mathbb{E}\left[\left\lfloor\frac{Y^2\left(\mathbb{E}[Y^2]-\mathbb{E}[X^2]\right)}{\mathbb{E}[X^2] \mathbb{E}[Y^2]}\right\rceil\right] \\
%& =\frac{\mathbb{E}\left[\left|X^2-Y^2\right|\right]}{\mathbb{E}[X^2]}+\frac{\left|\mathbb{E}\left[Y^2-X^2\right]\right|}{\mathbb{E}[X^2]} \leq 2 \frac{\mathbb{E}\left[\left|Y^2-X^2\right|\right]}{\mathbb{E}[X^2]} . \\
%&
%\end{aligned}
%$$
%
%Because $Y^2=\left(Y-X\right)^2+2 X\left(Y-X\right)+X^2$, we get
%$$
%\mathbb{E}\left[\mid Y^2-X^2 \|\right] \leq \mathbb{E}\left[\left|X-Y\right|^2\right]+2\left(\mathbb{E}[X^2]\right)^{1 / 2}\left(\mathbb{E}\left[\left|Y-X\right|^2\right]\right)^{1 / 2} \text {. }
%$$
%
%Therefore,
%$$
%\mathbb{E}\left[\left|\frac{X^2}{\mathbb{E}[X^2]}-\frac{Y^2}{\mathbb{E}[Y^2]}\right|\right] \leq 2 C+2 C^{1 / 2} .
%$$
Moving onto the second result, we first denote by $\widetilde{X}=X^2 / \mathbb{E}[X^2]$ and $\widetilde{Y}=Y^2 / \mathbb{E}[Y^2]$. It then follows that 
\begin{align*}
	& \mathbb{E}[\widetilde{X} 1\{\widetilde{X}>t\}]-\mathbb{E}[\widetilde{Y}1\{\widetilde{Y}>t\}] \\
& \qquad \leq \mathbb{E}[\widetilde{X} 1\{\widetilde{X}>t / 2\}]-\mathbb{E}[\widetilde{Y}1\{\widetilde{Y}>t\}] \\
& \qquad\leq \mathbb{E}[\widetilde{X} 1\{\widetilde{X}>t / 2, \widetilde{Y}>t\}]+\mathbb{E}[\widetilde{X} 1\{\widetilde{X}>t / 2, \widetilde{Y}\leq t\}] \\
&\qquad\qquad -\mathbb{E}[\widetilde{Y}1\{\widetilde{Y}>t,\widetilde{X}>t / 2\}]-\mathbb{E}[\widetilde{Y}1\{\widetilde{Y}>t,\widetilde{X} \leq t / 2\}] \\
& \qquad\leq \mathbb{E}[| \widetilde{X}-\widetilde{Y}|]+\mathbb{E}[\widetilde{X} 1\{\widetilde{X}>t / 2, \widetilde{Y}\leq t\}] \\
&\qquad \leq \mathbb{E}[|\widetilde{X}-\widetilde{Y}|]+\mathbb{E}[(\widetilde{X}-\widetilde{Y}) 1\{\widetilde{X}>t / 2,\widetilde{Y}\leq t\}]+\mathbb{E}[\widetilde{Y} 1\{\widetilde{X}>t / 2,\widetilde{Y}\leq t\}] \\
&\qquad \leq 2 \mathbb{E}[|\widetilde{X}-\widetilde{Y}|]+t \mathbb{E}[1\{|\widetilde{X}-\widetilde{Y}|>t / 2\}] \\
& \qquad\leq 4 \mathbb{E}[|\widetilde{X}-\widetilde{Y}|].
\end{align*}
Using the first result, the second claim is obtained.

Finally, it follows that 
\begin{align*}
	& \mathbb{E}[\widetilde{X}^{3 / 2} 1\{\widetilde{X} \leq s\}]-\mathbb{E}[\widetilde{Y}^{3 / 2} 1\{\widetilde{Y}\leq s\}] \\
& \qquad\leq \mathbb{E}[\widetilde{X}^{3 / 2} 1\{\widetilde{X} \leq s\}]-\mathbb{E}[\widetilde{Y}^{3 / 2} 1\{\widetilde{Y}\leq s / 2\}] \\
 &\qquad\leq \mathbb{E}[(\widetilde{X}^{3 / 2}-\widetilde{Y}^{3 / 2}) 1\{\widetilde{X} \leq s, \widetilde{Y}\leq s / 2\}] \\
&\qquad\qquad +\mathbb{E}[\widetilde{X}^{3 / 2} 1\{\widetilde{X} \leq s,\widetilde{Y}>s / 2\}]-\mathbb{E}[\widetilde{Y}^{3 / 2} 1\{\widetilde{X}>s,\widetilde{Y}\leq s / 2\}] \\
 &\qquad\leq \frac{3}{2} s^{1 / 2} \mathbb{E}[|\widetilde{Y}-\widetilde{X}|]+s^{3 / 2} \mathbb{P}(|\widetilde{X}-\widetilde{Y}|>s / 2) \\
& \qquad\leq 4 s^{1 / 2} \mathbb{E}[|\widetilde{Y}-\widetilde{X}|].
\end{align*}
Using the first result, the third claim is also obtained.
\end{proof}


==> main/width.tex <==

	% In terms of the rate of convergence, we provide the following lemma for the stochastic boundedness of the localized empirical process. 
% 	\begin{lemma}
% 	Under assumption 
% 		\[\mathbb{G}_n(m_\theta-m_{\theta_0}) = O_P((\|\theta-\theta_0\|^2 + r_n^2)r_n^{-2}\phi_n(r_n))\]
% 	\end{lemma}
% 	\begin{proof}
% 		We claim that 
% 		\begin{align}
% 			\mathbb{P}\left(|\mathbb{G}_n(m_\theta-m_{\theta_0})| > 2^M (\|\theta-\theta_0\|^2 + r_n^2)r_n^{-2}\phi_n(r_n)\right)
% 		\end{align}
% 		converges to zero as $M \longrightarrow \infty$. 
% 		\begin{align}
% 			&\mathbb{P}\left(|\mathbb{G}_n(m_\theta-m_{\theta_0})| > 2^M (\|\theta-\theta_0\|^2 + r_n^2)r_n^{-2}\phi_n(r_n)\right)\\
% 			& \qquad = \mathbb{P}\left(\frac{|\mathbb{G}_n(m_\theta-m_{\theta_0})|}{\|\theta-\theta_0\|^2 + r_n^2} > 2^M r_n^{-2}\phi_n(r_n)\right)\\
% 			& \qquad \le  \mathbb{P}\left(\sup_{\theta \in K}\, \frac{|\mathbb{G}_n(m_\theta-m_{\theta_0})|}{\|\theta-\theta_0\|^2 + r_n^2} > 2^M r_n^{-2}\phi_n(r_n)\right)
% 		\end{align}
% 		Let $B(\theta_0, r_n)$ be the $\|\cdot\|$-ball in $\Theta$ with radius $r_n$. Let $S_j$ be the ``shell"  
% 		\[S_j := \{\theta \in \Theta : 2^jr_n < \|\theta-\theta_0\| \le 2^{j+1}r_n\}\]
% 		Then any set $K \subseteq \Theta$ can be partitioned as 
% 		\begin{align}
% 			K = (K \cap B(\theta_0, r_n)) \, \cup \,  \bigcup_{j\ge 0}(K \cap S_j)
% 		\end{align}  
% 		Then we have 
% 		\begin{align}
% 			&\mathbb{P}\left(\sup_{\theta \in K}\, \frac{|\mathbb{G}_n(m_\theta-m_{\theta_0})|}{\|\theta-\theta_0\|^2 + r_n^2} > 2^M r_n^{-2}\phi_n(r_n)\right)\\
% 			& \qquad \le  \mathbb{P}\left(\sup_{\theta \in K \cap B(\theta_0, r_n)}\, \frac{|\mathbb{G}_n(m_\theta-m_{\theta_0})|}{\|\theta-\theta_0\|^2 + r_n^2} > 2^M r_n^{-2}\phi_n(r_n)\right) \\
% 			&\qquad\qquad + \sum_{j\ge 0} \mathbb{P}\left(\sup_{\theta \in K \cap S_j}\, \frac{|\mathbb{G}_n(m_\theta-m_{\theta_0})|}{\|\theta-\theta_0\|^2 + r_n^2} > 2^M r_n^{-2}\phi_n(r_n)\right)\\
% 			& \qquad \le  \mathbb{P}\left(\sup_{\theta \in K \cap B(\theta_0, r_n)}\, \frac{|\mathbb{G}_n(m_\theta-m_{\theta_0})|}{ r_n^2} > 2^M r_n^{-2}\phi_n(r_n)\right) \\
% 			&\qquad\qquad + \sum_{j\ge 0} \mathbb{P}\left(\sup_{\theta \in K \cap S_j}\, \frac{|\mathbb{G}_n(m_\theta-m_{\theta_0})|}{(2^{2j}+1) r_n^2} > 2^M r_n^{-2}\phi_n(r_n)\right)\\
% 			& \qquad \le  (2^M\phi_n(r_n))^{-1}\mathbb{E}\left[\sup_{\theta \in K \cap B(\theta_0, r_n)}\, |\mathbb{G}_n(m_\theta-m_{\theta_0})| \right] \\
% 			&\qquad\qquad + \sum_{j\ge 0} (2^M(2^{2j}+1)\phi_n(r_n))^{-1} \mathbb{E}\left[\sup_{\theta \in K \cap S_j}\, |\mathbb{G}_n(m_\theta-m_{\theta_0})| \right]\\
% 			& \qquad \le  (2^M\phi_n(r_n))^{-1}\phi_n(r_n) + \sum_{j\ge 0} (2^M(2^{2j}+1)\phi_n(r_n))^{-1} \phi_n(2^{j+1}r_n)\\
% 			& \qquad \le  2^{-M}+ \sum_{j\ge 0} \frac{2^{q(j+1)}\phi_n(r_n)}{2^M(2^{2j}+1)\phi_n(r_n)} \\
% 			& \qquad \le  2^{-M}\left(1+ \sum_{j\ge 0} \frac{2^{q(j+1)}}{(2^{2j}+1)} \rightx)	\\
% 			& \qquad \le  2^{-M}\left(1+ 4\sum_{j\ge 0} 2^{-(2-q)(j+1)} \right)		\\
% 			& \qquad =  2^{-M}\left(\frac{1+3\cdot 2^{-(2-q)}}{1-2^{-(2-q)}} \right)		
% \end{align}
% Last display can be made smaller than $\varepsilon$ by choosing $M$ large enough. Hence we have shown that there exists constant $C_\varepsilon$ only depending on $\varepsilon>0$ such that 
% \begin{align}
% 			\mathbb{P}\left(|\mathbb{G}_n(m_\theta-m_{\theta_0})| >C_\varepsilon (\|\theta-\theta_0\|^2 + r_n^2)r_n^{-2}\phi_n(r_n)\right) \le \varepsilon
% 		\end{align} 
% \end{proof}

% Coming back to the confidence set, for probability greater than $1-\varepsilon$, we have 
% \begin{align}
% 	&\left\{\theta \in \Theta : \|\theta-\theta_0\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0}) +   \sqrt{\frac{2\widehat \sigma^2_{\theta, \theta_0} \log(2/\alpha)}{n}} + \frac{6B_{\theta,  \theta_0}\log(2/\alpha)}{n} + \Gamma_n(\widehat\theta, \theta_0)\right\}\\
% 	&\subseteq  \left\{\theta \in \Theta : \|\theta-\theta_0\|^{1+\beta}\le C_\varepsilon (\|\theta-\theta_0\|^2 + r_n^2)  +   \sqrt{\frac{2\widehat \sigma^2_{\theta, \theta_0} \log(2/\alpha)}{n}} + \frac{6B_{\theta,  \theta_0}\log(2/\alpha)}{n} + \Gamma_n(\widehat\theta, \theta_0)\right\}
% \end{align}

% \kt{I realized that we do not need the requirement $r_n^{-2} \phi_n(r_n) \le \sqrt{n}$ for the result above. For instance, when $\phi(t) \sim t$, we have 
% \begin{align}
% 	&\|\theta-\theta_0\|^{1+\beta}\le -n^{-1/2}\mathbb{G}_n(m_\theta-m_{\theta_0})\\
% 	&\qquad \implies \|\theta-\theta_0\|^{1+\beta}\lesssim n^{-1/2}(\|\theta-\theta_0\|^2 + r_n^2) \phi(r_n)r_n^{-2}\\
% 	&\qquad \implies \|\theta-\theta_0\|^{1+\beta}\lesssim n^{-1/2}(\|\theta-\theta_0\|^2 + r_n^2) r_n^{-1} && \textrm{assuming $\phi(t) \sim t$}\\
% 	&\qquad \implies \|\theta-\theta_0\|^{1+\beta}\lesssim n^{-1/2}\|\theta-\theta_0\|&& \textrm{choosing $r_n = \|\theta-\theta_0\|$}
% \end{align}
% }
\kt{
Sanity check:
when $\phi_n(t) \sim t^q$ we have
\[\|\theta-\theta_0\|^{1+\beta} \lesssim r_n^2 \implies \|\theta-\theta_0\| \lesssim n^{-1/(2+2\beta-2q)}\]
For $\beta=1$, this corresponds to $ n^{-1/(4-2q)}$, which recovers typical nonparametric rate.
}


